Data driven value-at-risk forecasting using a SVR-GARCH-KDE hybrid

Appropriate risk management is crucial to ensure the competitiveness of financial institutions and the stability of the economy. One widely used financial risk measure is Value-at-Risk (VaR). VaR estimates based on linear and parametric models can lead to biased results or even underestimation of risk due to time varying volatility, skewness and leptokurtosis of financial return series. The paper proposes a nonlinear and nonparametric framework to forecast VaR that is motivated by overcoming the disadvantages of parametric models with a purely data driven approach. Mean and volatility are modeled via support vector regression (SVR) where the volatility model is motivated by the standard generalized autoregressive conditional heteroscedasticity (GARCH) formulation. Based on this, VaR is derived by applying kernel density estimation (KDE). This approach allows for flexible tail shapes of the profit and loss distribution, adapts for a wide class of tail events and is able to capture complex structures regarding mean and volatility. The SVR-GARCH-KDE hybrid is compared to standard, exponential and threshold GARCH models coupled with different error distributions. To examine the performance in different markets, one-day-ahead and ten-days-ahead forecasts are produced for different financial indices. Model evaluation using a likelihood ratio based test framework for interval forecasts and a test for superior predictive ability indicates that the SVR-GARCH-KDE hybrid performs competitive to benchmark models and reduces potential losses especially for ten-days-ahead forecasts significantly. Especially models that are coupled with a normal distribution are systematically outperformed.

==> Sections/AlteLiliIntro.tex <==
\section{Introduction}\label{Sec:intro}

Events as the world wide stock market crashes in 1987 and 2008 as well as the outcomes of the 2016 referendum in the UK or the presidential election in the USA came unexpected for most people. Therefore, from the perspective of financial risk management the words of Emil Gumbel, who made important contributions to the field of extreme value statistics, should be marked: \textit{"Il est impossible que l`improbable n`arrive jamais." (It is impossible for the improbable to never occur.)} \cite[p. 200]{Gumbel.1958}. Since such events happen rarely, they occur as outliers in data series. However, they can have a big impact on the solvency of single institutions and the whole economy. 
%For instance, strategical decisions that are based on models which underestimate existing market risks can result in large losses or even bankruptcy of the institution. If a system-relevant financial institution goes bankrupt, it can cause an economic crisis. Additionally, systematically overestimated market risk can prevent institutions from taking actions to generate profits. Thus, the use of appropriate models for measuring market risk results in a competitive advantage. 
\\
\noindent The importance of risk management for financial institutions and the economy drew researchers attention to the development of tools for handling risk. One of the most famous measures of uncertainty in financial markets is Value-at-Risk (VaR) which is e.g. described in detail by \cite{Alexander.2010} and \cite{Jorion.2009}. VaR is based on the quantiles of a portfolio's loss distribution. It can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable number. However, the use of VaR has been criticized. For instance, \cite{Artzner.1999} note that VaR is not subadditive and therefore no coherent risk measure. As a consequence, diversification can increase VaR. Despite this, regulatory frameworks for the banking and insurance industry as Basel III or Solvency II rely on VaR for the determining capital requirements of financial institutions. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{Kuester.2005} compare the performance of several classical statistical approaches for estimating VaR. 
%Moreover, a comprehensive overview over existing statistical methods is given. 
Four categories are suggested to describe existing methods for VaR estimation. 
These categories are historical simulation, fully parametric models, extreme value theory and quantile regression. In the empirical study VaR models belonging to the location scale class are superior over other approaches. In the domain of ML the literature for quantile estimation focuses mainly on neural networks (NN) and SVR. For instance, the derivation of a general approach without an explicit target application can be found in \cite{White.1992}. He used single hidden layer feedforward NNs to derive a way for nonparametric conditional quantile estimation and proved its consistency. However, the ML VaR literature is not as broad as in classical statistics. 
%Hence, this section also reviews literature where methods for the construction of prediction intervals (PI) were introduced that could be used in the estimation of VaR. Consequently, the reviewed literature is divided in three paragraphs: Prediction Intervals, Value-at-Risk and Data Driven Value-at-Risk.Here, the first two review the existing literature, whereas the last motivates the method proposed in this paper.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent 
\paragraph{Data Driven Value-at-Risk} 
One approach for estimating VaR is based on generalized autoregressive conditional heteroscedasticity (GARCH) models. For example, in an empirical study with more than 30 years of historical returns \cite{Kuester.2005} show that VaR forecasts which are based on standard GARCH models are relatively good compared to other methods. However, they have a linear and parametric structure. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation (MLE)  \citep{Bollerslev.1986}. This makes it necessary to make distributional assumptions. 
%However, the distribution of financial returns were empirically shown to have fat tails and being skewed \citep{Bali.2008,Harvey.2000}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{Franke.2006} estimate VaR for the German stock index (DAX) by fitting the mean and volatility of the return series with NNs. The mean is modeled autoregressively and the volatility is assumed to follow an autoregressive conditionally heteroscedastic (ARCH) process. Moreover, they include external regressors in both models. The predicted mean and variance are used with the normal distribution to derive the VaR and expected shortfall. As benchmark serves a standard GARCH model based on assuming normality of innovations. In terms of VaR exceedances their model is superior. Moreover, they note its ability to quickly adjust the volatility in case of shocks with only short impact. Another approach directly related to VaR is proposed by \cite{Dunis.2010} which use higher order NNs to forecast VaR. A hybrid model using higher order NNs for variance forecasting and RiskMetrics is shown to outperform other hybrid models empirically. They note also the relatively bad results of the unconditional POT method for quantile estimation. This is, however, not an appropriate comparison when benchmarked to conditional models as was e.g. shown by \cite{Kuester.2005}. 
%\cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test.
%Therefore, assuming e.g. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Assuming e.g. normality can lead to an underestimation of risk. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Data Driven Value-at-Risk} 
Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. 
%In contrast, s
Support vector regression (SVR) introduced by \cite{Vapnik.1995,Vapnik.1998} is a method originating in statistical learning theory and was derived based on minimizing the generalization error. SVR can be classified as a method belonging to the domain of machine learning (ML). \cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test. A multiperiod VaR model was introduced by \cite{Xu.2016}. They use an exponentially weighted support vector quantile regression. In the corresponding empirical study, their approach outperforms other methods that are based on GARCH models, filtered historical simulation and quantile regression. Evaluation was done with different measures as e.g. mean absolute error and p-values of prediction tests.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By considering the different model types presented in study of \cite{Kuester.2005}, they can be classified as quantile regression models. In the empirical study of  the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and peaks-over-threshold had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. 
Most of the proposed methods in the ML literature for estimating VaR 
%or PIs 
are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this paper. \\
%Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions.
%Additionally, k
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Kernel density estimation (KDE) is a nonparametric method to estimate the density of a random variable \citep{Hardle.2004}. 
%%%%%% Härdle %%%%%%%%%%%
Given a multi-market setting, \cite{Haerdle.2016} examine the relation between down-side risk and stock returns.
They apply a time varying and time related co-integrated vector auto-regression model with a non-parametric Kernel density estimation with a double exponential Laplace kernel. 
Furthermore,given a predefined period of time, the paper questions the impact and relevance of certain higher moments for VaR.
%Dynamics: Vector elements
%higher moments of risk
%VaR
%Stock returns 
%%%%% find source of VaR predictability power
%%%%%%%%%%%%%%%%%Distinction by SVM %%%%%%%%%%%%%%
In this paper a data driven VaR forecasting framework that is based on SVR and KDE is introduced. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions. 

%%%%%%%Chen et Al.
\cite{Chen.2012} employ a parametric approach for the estimation of VaR for four daily series of four stock market indices. Given an asymmetric Laplace distribution, volatility is modeled GRJ-GARCH. Introduced by \cite{Black.1976}, the latter measures leverage effects
%, which is not of interest for this study. 
. 
Inspired by \dots
%\cite{luetal}, %Finde BibTeX Quelle
the model is extended to a time-varying model allowing dynamic higher moments. Parameters are estimated by an adaptive Markov Chain Monte Carlo sampling scheme with the application of the Metropolis-Hastings algorithm with a mixture of Gaussian proposal distributions. 
%In difference the simulation performed the paper, this approach 
%%%%%%%%%% REASONS WHY BETTER THAN SIMULATION %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%accuracy \dots

\cite{Schaumburg.2012} combines extreme value theory (EVT) with non-parametric VaR estimation in order to estimate return distributions of four financial stock indexes. Conditional quantiles are estimated by the application of monotonized double kernel local linear regression (DKLL), followed by the implementation of of the EVT peaks over threshold method to standardized 
%nonparametric 
residuals.
The methodology is compared to a parametric conditional autoregressive VaR model. \\
Although this study also applies a non-parametric approach, besides of quantile estimation, KDE density estimation and higher moment
%mean and volatility
estimation via SVR are of residuals are taken into consideration.
%%%%%%%\cite{Kuester.2006} Garch outperforms other models



The aim is to compare the proposed approach with similar parametric GARCH-type models to see whether performance gains can be achieved. \\

\noindent The remainder of the paper is structured as follows. 
%In Section \ref{Sec:Lit_Rev} the literature where ML methods are used to forecast VaR are reviewed. Moreover, approaches that are used to establish prediction intervals but are also a possible framework for modeling VaR are presented as well. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Consequently, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. Based on this, the proposed SVR-GARCH-KDE hybrid is introduced at the end of the section. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions on how to modify the proposed framework for performance improvements are provided in the last section. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% Add text %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %Benefits of machine learning approach
 %


==> Sections/Archive/emp_study_short_2017Nov23_short.tex <==
\clearpage

\section{Empirical Study}\label{Sec:emp_study}

\subsection{General Setting}

The SVR-GARCH-KDE hybrid is tested using stock indices to evaluate the performance for different regions. We consider four indices, namely the Euro STOXX 50, S\&P 500 and Nikkei 225 which represent the Euro zone, the USA and Japan, respectively. The analysis is based on the log-returns of the adjusted index closing prices $P_t$:

\begin{equation}
r_t = \log(P_t) - \log(P_{t-1}).
\end{equation}

\noindent We forecast VaR for the quantiles $\alpha \in \{0.005, 0.01, 0.025, 0.05\}$, always considering a forecast horizon of one trading day. In empirical applications, the quality of SVR depends on the kernel and parameter values that need to be set manually. The prevailing approach to determine parameter settings is grid search \citep[e.g.,][]{Lessmann.2017}, which we also apply in this study. For the density estimation via KDE the Gaussian kernel function in combination with Silverman's rule of thumb are used to reduce computational cost. \\

\noindent The evaluation of the models is based on the work of \cite{Christoffersen.1998}. The core of the evaluation is a likelihood ratio test framework, which assess the unconditional and conditional coverage as well as the independence of VaR exceedances. Moreover, \cite{Christoffersen.1998} shows that the test statistic for conditional coverage can be derived as the sum of the test statistics of the test for unconditional coverage and independence of VaR exceedances. Hence, it is possible to test whether the performance of a VaR model in terms of correct conditional coverage is determined by its ability to achieve correct coverage or adjust for changing volatility. This is useful in situations where the model has relatively bad conditional coverage but only one of the test statistics for unconditional coverage or independence is small. As criterion for selecting a model from grid search and evaluate the performance of the SVR-GARCH-KDE hybrid with respect to benchmark models, the $p-$value of the test for conditional coverage is used. Since the null hypothesis corresponds to correct conditional coverage which is the desired property, the one with the highest $p-$value is considered to be the best. \\

\noindent We perform all analyses using the statistical software R. The data has been downloaded from Yahoo Finance using the quantmod package. For SVR, we use the package e1071, which is the R implementation of the LIBSVM library of \cite{Chang.2011}. To reduce computational time, we employ the doParallel package for parallelization of computations. The benchmark methods introduced below are implemented by using the rugarch package. 


\subsection{Benchmark Methods}

To test the SVR-GARCH-KDE hybrid, we compare its performance to the standard GARCH model and some of its variations. In particular, \cite{Franke.2011} state that two of the most important variations are the EGARCH and TGARCH model. Hence, they serve as benchmarks in the empirical comparison. The EGARCH and TGARCH models are introduced by \cite{Nelson.1991} and \cite{Zakoian.1994}, respectively. In contrast to standard GARCH models, both can account for asymmetric behavior with respect to past positive or negative returns. The two main differences between EGARCH and TGARCH models are that the former has a multiplicative and the latter an additive model structure. Moreover, TGARCH models allow for different coefficients depending on the lags whereas EGARCH models capture the asymmetric behavior for all lags with one coefficient.

 The GARCH-type models that \cite{Kuester.2005} analyze are coupled with different error distributions, i.e. the normal distribution, $t$ distribution and skewed $t$ distribution. We adopt this approach, which implies that we compare the SVR-GARCH-KDE hybrid to nine benchmarks.  

%\subsection{Popular Modifications of GARCH Models}
%
%\cite{Franke.2011} state that empirical studies found asymmetric reactions of the volatility depending on the sign of the return. In general, negative returns cause higher volatility than positive. To account for these empirical findings several variations of the standard GARCH model in (\ref{Eq:garch_original}) were proposed. Two crucial models are the exponential GARCH (EGARCH) and threshold GARCH (TGARCH) model which are presented below \cite[p. 308]{Franke.2011}.

%\subsubsection{Exponential GARCH Model}
%
%\cite{Nelson.1991} defines the EGARCH model as as follows, with $\omega_t$ and $\lambda_i$ denoting deterministic coefficients: 
%
%\begin{equation}
%\log(\sigma^2_t)  = \omega_t + \sum_{i = 1}^{\infty} \lambda_i m(z_{t-i}), \quad z_t \sim (0, 1) \ \text{i.i.d.}, \quad \lambda_1 = 1,
%\label{Eq:egarch_def}
%\end{equation}
%
%\noindent where
%
%\begin{equation}
%m(z_t) = \rho z_t + \gamma(|z_t| - \mathbb{E}[|z_t|]).
%\label{Eq:egarch_def_asyfct}
%\end{equation}
%
%\noindent Parameters $\rho$ and $\gamma$ are weights that need to be estimated. From $z_t \sim (0, 1) \ \text{i.i.d.}$ follows that $m(z_t)$ is i.i.d. with zero mean. There are some notable differences between the GARCH and EGARCH model. In equation (\ref{Eq:egarch_def}) $\sigma_t^2$ depends multiplicatively on past disturbances. This is in contrast to the standard GARCH model that depends additively on the mean model disturbances. Further, the asymmetric behavior of volatility is taken into account by $m(z_t)$ in (\ref{Eq:egarch_def}). Another difference is that there are no restrictions on the parameters in (\ref{Eq:egarch_def}) and (\ref{Eq:egarch_def_asyfct}).
%
%
%\subsubsection{Threshold GARCH Model}
%
%The TGARCH model is introduced by \cite{Zakoian.1994}. In TGARCH, asymmetries in the volatility are taken into account by modeling them as function of positive and negative disturbances. In contrast to the GARCH and EGARCH approach, \cite{Zakoian.1994} models the standard deviation rather than the variance. This is based on the work of \cite{Davidian.1987}, who find using absolute rather than squared disturbances to result in more efficient variance estimates. % \citep[p. 2]{Zakoian.1994}.
%Formally, with $u_t^+ = \max(u_t, 0)$ and $u_t^- = \min(u_t, 0)$ the TGARCH($p$,$q$) model is defined as:
%
%\begin{align}
%u_t &= \sigma_t z_t, \quad z_t \sim (0, 1) \ \text{i.i.d.},\\
%\sigma_t &= \omega + \sum_{i = 1}^{q} \delta_i^+ u_{t-i}^+ + \sum_{i = 1}^{q} \delta_i^- u_{t-i}^- + \sum_{j = 1}^{p} \theta_j \sigma_{t-i}.
%\label{Eq:tgarch_def}
%\end{align}
%
%\noindent \cite{Zakoian.1994} points out differences to the EGARCH model. First, the TGARCH model is additive whereas the EGARCH model is multiplicative due to modeling the logarithm of $\sigma^2_t$. Moreover, for EGARCH models, asymmetry is captured by the same structure for all lags since the coefficients in (\ref{Eq:egarch_def_asyfct}) are constant. In contrast, TGARCH models allow for different coefficients depending on the lag. 

\subsection{Results}
%\subsection{Analysis for $\boldsymbol{\mu_t = 0}$ and GARCH(1,1)}

\subsubsection{Model Setting and Tuning}

We assume the mean process of $r_t$ in (\ref{Eq:svr_mean_estimate}) is zero. Moreover, we assume the variance process to have one AR and one MA part. These assumptions are imposed on both the SVR-GARCH-KDE hybrid and the benchmark models. We then forecast VaR  for every index trading day from 2011-07-01 until 2016-06-30. The data is  scaled to zero mean and unit variance in the SVR step; as suggested in the documentation of the e1071 package. Model training is done in a moving window approach using 251 return observations, which corresponds to approximately one trading year. Here, a trading year is assumed to have 252 price observations. Hence, one observation less is available when returns are considered. Tuning is done using the same moving window approach for forecasting VaR from 2006-07-01 until 2011-06-30. The considered parameter values in the grid for SVR are

\begin{itemize}
	\item $C \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$
	\item $\psi \in \{0, 0.1, \dots, 0.9 \}$  where $\epsilon = Q_{u^2_{scale}}(\psi)$
	\item $\gamma \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$.
\end{itemize}    
 

\noindent Note that the second point indicates that tuning is not done over fixed values of $\epsilon$. Instead, in every step of the estimation, $\epsilon$ is determined based on the $\psi$-quantile of the squared scaled disturbances of the mean model. This corresponds to the squared scaled returns because we assume zero mean of $r_t$. The motivation behind this is the tendency of returns to form volatility clusters. Hence, a fixed $\epsilon$ can lead to good results in one volatility regime but might have a poor performance after a regime change. For instance, in the case of a financial crisis, the right tail of the distribution of past volatilities gets thicker. Hence, an $\epsilon$ that depends on the quantile of the distribution will increase such that large volatilities have automatically a higher influence on the estimated parameters from the SVR optimization. By using squared values it is ensured that only positive values are obtained for $\epsilon$. However, notice that the distribution of the scaled squared disturbances, which are used in the SVR training, is shifted to the left of the distribution of the squared scaled disturbances. Hence, it is possible that for high values of $\psi$ no observations are outside the $\epsilon$-tube such that the model cannot be estimated.     \\

\noindent The parameter settings that resulted in the best models for the SVR-GARCH-KDE hybrid during the tuning period are shown in Table \ref{Tab:tuning_case1}.  
It can be seen that especially for $\psi$ only a certain range appears among the best models. Moreover, the optimal $\psi$ tends to be higher for lower quantiles. Based on the obtained parameters, VaR forecasts are produced from 2011-07-01 until 2016-06-30. 
%For all indices and parameter settings no results were obtained for $\psi = 0.9$ due to R returning the error message "Model is empty!". This is caused by the point described in the passage above, meaning that for $\psi = 0.9$ no values are left for SVR model training.

%\vspace{-1cm}
%\input{Tables/Case_1Results_Case1_EuroStoxx50.tex}
%\clearpage

\subsubsection{Model Comparison}

\noindent The results of the simulations are presented for each quantile separately in the Tables \ref{Tab:case1_0.5}, \ref{Tab:case1_1}, \ref{Tab:case1_2.5} and \ref{Tab:case1_5} at the end of the section. To clearly identify the best performing models, every table is sorted in descending order for every index according to the p-value of the conditional coverage test. The abbreviations NORM, STD and SSTD indicate the normal, $t$ and skewed $t$ distribution, respectively. Additionally, the column headers UC, ID and CC refer to the corresponding $p$-value of the LR test for unconditional coverage, independence of violations and conditional coverage.  

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.005}$}
 For the Euro STOXX 50, the SVR-GARCH-KDE hybrid has together with the TGARCH-STD and TGARCH-SSTD model the best results according to their p-values of the LR test for conditional coverage. However, all models have low CC values in comparison to the other time series. This comes from many violations which lead to low values in the LR test for UC. Despite having the most independent violations for the Nikkei 225, there are five models being better than the SVR-GARCH-KDE hybrid according to the CC value. This is mainly caused due to overestimating the market risk; as shown by the violations. In practice, risk overestimation is more desirable than underestimation. In particular, overestimation may lead to some potential profits not being  realized, whereas risk underestimation can lead to bankruptcy in the short term. The SVR-GARCH-KDE hybrid is the second best model in terms of unconditional coverage for the S\&P 500 but tends to form violation clusters. This can be concluded from the $p$-value in the ID column. As a result, only the GARCH-NORM and EGARCH-NORM model perform worse in terms of CC. 

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.01}$}  As for $\alpha = 0.005$, the SVR-GARCH-KDE hybrid is the best model for the Euro STOXX 50 for $\alpha = 0.01$. A visualization of its performance is given in Figure~\ref{Fig:model_comparision_SP500_1}. It is compared to the EGARCH-NORM model, which ranked worst. Here, the SVR-GARCH-KDE hybrid estimates in general higher values for VaR than the EGARCH-NORM model and exhibits more variability. The results are also similar to the 0.5\% level for the S\&P 500 and Nikkei 225, meaning that the SVR-GARCH-KDE hybrid has an average performance for both series. Moreover, this is again caused by having a low unconditional coverage for the Nikkei 225 and a tendency to form violation clusters for the S\&P 500.  In addition, the models coupled with a normal distribution perform poorly for all indices for $\alpha \in \{0.005, 0.01\} $. This comes as no surprise since the distribution of asset returns is usually leptokurtic. Accordingly, models that are coupled with a skewed $t$ distribution perform best.

\begin{figure}[h]
\centering
\includegraphics[scale = 0.65]{Figures/VaR_Plots_ES1}
\caption[SVR-GARCH-KDE and EGARCH-NORM for the Euro STOXX 50 at $\alpha = 0.01$]{VaR forecast model comparison for the Euro STOXX 50 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the EGARCH-NORM model.}
\label{Fig:model_comparision_SP500_1}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.025}$} The performance of the SVR-GARCH-KDE hybrid at the 2.5\% level is not as good as for $\alpha \in \{0.005, 0.01\}$ for the Euro STOXX 50. We observe the lowest $p$-value in the test for independence of violations. Interestingly, although the TGARCH and EGARCH model account for asymmetries in volatility, the former is the best and the latter the worst variance model. A relatively high risk overestimation for the S\&P 500 and Nikkei 225 causes the SVR-GARCH-KDE hybrid to be on the sixth and ninth rank, respectively. Rank nine is the worst that the SVR-GARCH-KDE hybrid achieves across all comparisons. A visual inspection of the model's performance compared to the GARCH-SSTD model, which performed best, is given in Figure \ref{Fig:model_comparision_SP500_5}.  
\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.65]{Figures/VaR_Plots_Nik25}
	\caption[SVR-GARCH-KDE and GARCH-SSTD for the Nikkei 225 at $\alpha = 0.025$]{VaR forecast model comparison for the Nikkei 225 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the GARCH-SSTD model.}
	\label{Fig:model_comparision_SP500_5}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.05}$} The best performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is rank two for the Nikkei 225. Here, it is only beaten by the EGARCH-SSTD model. For the other indices the SVR-GARCH-KDE hybrid ranks on place five. This is caused by having relatively low $p$-values for the ID test. In terms of UC, the SVR-GARCH-KDE hybrid is the second and third best model for the S\&P 500 and Nikkei 225, respectively. In comparison to the results for $\alpha \in \{0.005, 0.01\}$, the models with a normal distribution are not the worst for $\alpha \in \{0.025, 0.05\}$. However, using the skewed $t$ distribution leads also for $\alpha \in \{0.025, 0.05\}$ to the best rankings.  \\

\noindent Summarizing the results observed across all indices and quantiles, we conclude that the SVR-GARCH-KDE hybrid displays an average performance. Unlike the benchmarks, the SVR-GARCH-KDE hybrid tends to overestimate market risk. This might come from the choice of time interval for SVR parameter tuning. In particular, the tuning period covers the financial crisis of 2008 where market risk was extremely high. However, the SVR-GARCH-KDE hybrid usually outperforms benchmark models coupled with a normal distribution. This can be seen in Table \ref{Tab:mean_ranks} where the mean ranks per index and quantile are presented for each model. Moreover, there is no setting where the models using a normal distribution perform best. This provides further evidence that using the normal distribution to measure market risk is inappropriate. However, models with a skewed $t$ distribution show in many cases the best performance. For instance, the TGARCH model coupled with the skewed $t$ distribution is always among the top three. This confirms the results of previous research related to return distribution being skewed skewed.   
%Table has been moved to appendix

\begin{table}[ht]
	\centering
	\begin{tabular}{l|c}
		\hline
		\hline
		 \textbf{Model} & \textbf{Mean Rank} \\ 
		 \hline
		\hline
		 TGARCH-SSTD & 2.1 \\ 
		 GARCH-SSTD & 2.4 \\ 
		 EGARCH-SSTD & 4.8 \\ 
		 TGARCH-STD & 4.8 \\ 
		 SVR-GARCH-KDE & 4.9 \\ 
		 GARCH-STD & 5.7 \\ 
		 TGARCH-NORM & 6.3 \\ 
		 GARCH-NORM & 6.6 \\ 
		 EGARCH-STD & 7.8 \\ 
		 EGARCH-NORM & 8.7 \\ 
		\hline
		\hline
	\end{tabular}
	\caption[Model comparison via mean ranks]{The models are presented with their mean rank. The mean rank was computed per index and quantile using the ties method \textit{min} in the \textit{frankv} function of the R package  data.table. The lower the mean rank, the better the model.}
	\label{Tab:mean_ranks}
\end{table}

%\clearpage
\newgeometry{left=6cm, right=1cm, top=3.5cm,bottom=1cm}
%\vspace*{-1cm}
\input{Tables/Results_Tunig_Results_Case_1.tex}

\input{Tables/Results_Case1_05.tex}
%\clearpage

%\vspace{-1cm}
\input{Tables/Results_Case1_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_5.tex}
%\clearpage
\restoregeometry

\clearpage

==> Sections/IntroLili.tex <==
%\section{Introduction}\label{Sec:intro}
%%%%%%%%%%%%%%%%%%%%
%Description%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\iffalse
This is a suggested introduction by Lili Matic.
\fi
%%%%%%%%%%%%%%%%%%%%%
%%Introducing words%%
%%%%%%%%%%%%%%%%%%%%%
Events as the world wide stock market crashes in 1987 and 2008 as well as the outcomes of the 2016 referendum in the UK or the presidential election in the USA came unexpected for most people. However, as these examples illustrate, unlikely events occur at times and may have far reaching consequences. Risk management is the practice to analyze the macro-environment of an organization, identify possible adverse developments, and develop suitable countermeasures. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% Out %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Therefore, from the perspective of financial risk management the words of Emil Gumbel, who made important contributions to the field of extreme value statistics, should be marked: \textit{"Il est impossible que l`improbable n`arrive jamais." (It is impossible for the improbable to never occur.)} \cite[p. 200]{Gumbel.1958}. Since such events happen rarely, they occur as outliers in data series. However, they can have a big impact on the solvency of single institutions and the whole economy. 
For instance, strategical decisions that are based on models which underestimate existing market risks can result in large losses or even bankruptcy of the institution. If a system-relevant financial institution goes bankrupt, it can cause an economic crisis. Additionally, systematically overestimated market risk can prevent institutions from taking actions to generate profits. Thus, the use of appropriate models for measuring market risk results in a competitive advantage. 
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%% Risk Management %%
%%       VAR       %%
%%%%%%%%%%%%%%%%%%%%%
For financial institutions and systemically important institutions in particular, a key risk management task is to sustain solvency under adverse economic conditions \citep[e.g.,][]{Silva.2017, Kraus.2017}. One of the most popular measures of uncertainty in financial markets is Value-at-Risk (VaR) (e.g., \cite{Alexander.2010}). VaR is based on the quantiles of a portfolio's $P\&L$ distribution andcan be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable number \citep[e.g.,][]{Chen.2012}. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% VaR critique %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Comment: Misfits to text, however component of text. Ideas welcomed !
%However, the use of VaR has been criticized. For instance, \cite{Artzner.1999} note that VaR is not subadditive and therefore no coherent risk measure. As a consequence, diversification can increase VaR. Despite this, 
Regulatory frameworks for the banking and insurance industry such as Basel III or Solvency II also rely on VaR for determining capital requirements. Compared to expected shortfall, an alternative risk measure with superior mathematical properties \citep[e.g.,][]{Kim.2016}, an advantage of VaR may be seen in the fact that its estimation is more robust due the putting less weight on tail risks and large losses which may deteriorate the quality of statistical estimation routines \citep{Sarykalin.2008}. Especially the latter property make VaR the right choice for this paper, which focuses on developing estimates of risk exposure using data-driven forecasting methods.  \\
%%%%%%%%%%%%%%%%%%%%%
%% VAR ESTIMATION %%
%%%%%%%%%%%%%%%%%%%%%
Several approaches have been proposed to estimate VaR including various parametric statistical models and data-driven machine learning algorithms such as neural networks (NN) and support vector regression (SVR). In a seminal study, \cite{Kuester.2005} review several statistical forecasting methods and compare these in a forecasting benchmark. Using more than 30 years of historical returns data, they find standard generalized autoregressive conditional heteroscedasticity (GARCH) models to forecast VaR with relatively high accuracy. \\
GARCH models are also employed by \cite{Chen.2012} to estimate VaR for four daily series of four stock market indices. More specifically, \cite{Chen.2012} they rely on an asymmetric Laplace distribution and model volatility using GJR-GARCH to introduce leverage effects. They then develop a time-varying model to allow for dynamic higher moments. These extensions allow for wider application of the model beyond forecasting. \\  

%%%%%%%%%%
%% Chen %%
%%%%%%%%%%
%\cite{Chen.2012} employ a parametric approach for the estimation of VaR for four daily series of four stock market indices. Given an asymmetric Laplace distribution, volatility is modeled GRJ-GARCH. Introduced by \cite{Black.1976}, the latter measures leverage effects
%, which is not of interest for this study. 
%Inspired by \cite{Lu.2010}, the model is extended to a time-varying model allowing dynamic higher moments. Parameters are estimated numerically. An adaptive Markov Chain Monte Carlo sampling scheme with the application of the Metropolis-Hastings algorithm with a mixture of Gaussian proposal distributions is applied. 
%\begin{center}
%   \textbf{Read comments \dots }  
%\end{center}
%%%%%%%%%%%%%%%
%%% COMMENT %%%
%%%%%%%%%%%%%%%
%In difference the simulation performed the paper, this approach 
%We employ a frequetionistical approach (data driven)
%Maximum likelihood already mentionen \dots 
%Our approach: Non-parametric, no distributional assumption
%Simulation: Numerical iterations depend on \theta_0 (higher error)
%SVR: Mean & volatility 

Unlike the parametric approach of \cite{Chen.2012}, \cite{Franke.2006} estimate VaR for the German stock index through fitting the mean and volatility of the return series using NN. More specifically, they model the mean and volatility as an autoregressive and autoregressive conditionally heteroscedastic (ARCH) process, respectively. To derive VaR and expected shortfall, the predicted mean and variance are used with the normal distribution. \cite{Franke.2006} find this approach to outperform a standard GARCH model in terms of VaR exceedances. Moreover, they note the model's ability to quickly adjust  volatility in case of shocks with only short impact. \cite{Dunis.2010} propose another NN-based approach toward forecasting VaR and conditional VaR. \\
\cite{Khan.2011} develop a VaR-model that forecast realized volatilities using a combination of a heterogeneous autoregressive (AR) model and SVR. VaR is then computed based on the normal, $t$ and skewed $t$ distribution. Applying this model to 5- and 15-minutes return data, \cite{Khan.2011} is able to confirm the suitability of the SVR component.  \cite{Stankovic.2015} provide further evidence that SVR is a useful method for VaR forecasting. \cite{Xu.2016} introduce a multiperiod VaR model using SVR in a quantile regression framework. This approach is shown it outperform GARCH models. \\
The findings of \cite{Xu.2016} seem to disagree prior results of \cite{Kuester.2005} where GARCH models have been found to predict VaR with high accuracy and more accurately than approaches based on quantile regression in particular. Implementation of the quantile regression using a data-driven SVR model might be an explanation for this result. Indeed, the linear and parametric structure of standard GARCH models might be a limiting factor. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation \citep{Bollerslev.1986}. This necessitates making distributional assumptions, which might be problematic when modeling financial returns, which are characterized by fat tails and large skew \citep{Bali.2008,Harvey.2000}. \\
An approach particularly related to the one proposed in this paper is that of \cite{Schaumburg.2012}. She combines extreme value theory (EVT) with non-parametric VaR estimation to estimate return distributions of four financial stock indexes. A parametric conditional autoregressive value at risk (CAViaR) model serves as benchmark. The benchmark and the proposed model both circumvent the estimation of the mean and variance of the $P\&L$ distribution through predicting a quantile directly. In this regard, the approach of \cite{Schaumburg.2012} can be characterized as a non-parametric CAViaR model. \\
VaR forecasts based on CAViaR frameworks have also been considered in the benchmarking study of \cite{Kuester.2005}. In fact, the authors also introduce a novel CAViaR model in the paper and test is alongside various other VaR models. However, GARCH models and models relying on the $t$ distribution or EVT in particular emerge as most suitable framework for VaR modeling. Therefore, this paper introduces a novel VaR model that bases on the GARCH framework but estimates individual components in a purely non-parametric manner. More specifically, we estimate the mean and variance of the $P\&L$ distribution distribution using using SVR and employ kernel density estimation (KDE) to model the density of the standardized residuals  \citep[e.g.,][]{Hardle.2004}. We then integrate these components to derive a VaR forecast. In summary, the idea of the proposed method is to start from  the most effective parametric modeling approach of \cite{Kuester.2005} and to develop models that estimate its components in a non-parametric manner. Although KDE is not a new  approach in VaR forecasting \citep[e.g.,][]{Haerdle.2016, Schaumburg.2012, Malec.2014}, the particular combination of data-driven VaR estimation using SVR and non-parametric density estimation, which we propose in this paper, has, to the best of our knowledge, not been considered in prior work. \\
We assess the performance of the proposed model in comparison to GARCH-type models with different error distributions also including skewed and fat-tailed distributions. Empirical experiments using data from three major financial indices, namely the Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500), suggest that the SVR-GARCH-KDE hybrid typically outperforms models that are coupled with a normal distribution and performs competitive to benchmark models that use a skewed $t$ distribution. \\

\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%       KDE       %%
%%%%%%%%%%%%%%%%%%%%%
Kernel density estimation (KDE) is a nonparametric method to estimate the density of a random variable. 

%%%% Übergang/Transfer %%%%%%%%
%%%%%%%%%CONS OF GARCH TYPE MODELS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Distributional asumptions %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%However, they 
GARCH-type models 
%have 
are limited by a linear and parametric structure.  
%%%%%%%%%%%%%%%%%%%%%
%% Data driven VAR %%
%%%%%%%%%%%%%%%%%%%%%
\paragraph{Data Driven Value-at-Risk} %Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. 
%%%%%%%%%%%%%%%%%%%%%%% Reshaped text %%%%%%%%%%%%%%%%%%%%%%
There have been attempts to bypass distributional assumptions.
\cite{Wu.2005} prososes SVR and NNs, as these methods do not rely on distributional assumptions. 
By considering the different model types presented in study of \cite{Kuester.2005}, they can be classified as quantile regression models. In the empirical study of the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and peaks-over-threshold had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. Most of the proposed methods in the ML literature for estimating VaR 
%or PIs 
are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. 
%%%%%%%%%%%%%%%%%%%%%%%  Moved  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this paper. 

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Härdle %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
In another VaR related paper, \cite{Haerdle.2016} examine the relation between down-side risk and stock returns. Given a multi-market setting,  they apply, inter alia, co-integrated vector auto-regression and the non-parametric Kernel density estimation. 
%with a double exponential Laplace kernel. 
%Furthermore,given a predefined period of time, the paper questions the impact and relevance of certain higher moments for VaR.
%Dynamics: Vector elements
%higher moments of risk
%VaR
%Stock returns 
%%%%% find source of VaR predictability power
   \begin{center}
   \textbf{Read comments \dots }  
\end{center}
%%%%%%%%%%%%%%%
%%% COMMENT %%%
%%%%%%%%%%%%%%%
%Var estimation and KDE in common
%different focus
%SVE argument
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%  IMPORTANT %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Schaumburg %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
In a non-parametric approach, \cite{Schaumburg.2012} combines extreme value theory (EVT) with non-parametric VaR estimation in order to estimate return distributions of four financial stock indexes. Conditional quantiles are estimated by the application of monotonized double kernel local linear regression (DKLL), followed by the implementation of of the EVT peaks over threshold method to standardized 
%nonparametric 
residuals.
The methodology is compared to a parametric conditional autoregressive VaR model. \\
 \begin{center}
   \textbf{Read comments \dots }  
\end{center}
%%%%%%%%%%%%%%%
%%% COMMENT %%%
%%%%%%%%%%%%%%%
%]
\iffalse
Although this study also applies a non-parametric approach, besides of quantile estimation, KDE density estimation and higher moment
%mean and volatility
estimation of residuals via are not taken into consideration.
%%%%%%%\cite{Kuester.2006} Garch outperforms other models
\\
\fi
%SVR Machine Learning benefits 

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%   Contribution    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper a data driven VaR forecasting framework that is based on SVR and KDE is introduced. In order to obtain a purely data driven location scale VaR approach, we employ a hybrid based on SVR and nonparametric density estimation. 
Its performance %will be 
is evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions. The aim is to compare the proposed approach with similar parametric GARCH-type models to see whether performance gains can be achieved.\\
%%%%%%%%%%%%%
%%%% Idea %%%
%%%%%%%%%%%%%
The uniqueness of this approach is characterized by both  employing a data driven VaR estimation and non-parametric density estimation. To the best of our knowledge, this is the work that applies this methodology for VaR estimator.\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Structure  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent The remainder of the paper is structured as follows. 
%In Section \ref{Sec:Lit_Rev} the literature where ML methods are used to forecast VaR are reviewed. Moreover, approaches that are used to establish prediction intervals but are also a possible framework for modeling VaR are presented as well. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Consequently, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. Based on this, the proposed SVR-GARCH-KDE hybrid is introduced at the end of the section. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions on how to modify the proposed framework for performance improvements are provided in the last section.

















==> Sections/New_literature.tex <==
\section{Literature Review}\label{Sec:Lit_Rev}

%%%%%%%Chen et Al.
\cite{Chen.2012} employ a parametric approach for the estimation of VaR for four daily series of four stock market indices. Given an asymmetric Laplace distribution, volatility is modeled GRJ-GARCH. Introduced by \cite{black76}, the latter measures leverage effects
%, which is not of interest for this study. 
. 
Inspired by \dots
%\cite{luetal}, %Finde BibTeX Quelle
the model is extended to a time-varying model allowing dynamic higher moments. Parameters are estimated by an adaptive Markov Chain Monte Carlo sampling scheme with the application of the Metropolis-Hastings algorithm with a mixture of Gaussian proposal distributions. 
%Non parametric approach perks (underestimation left out..)
%In difference the simulation performed the paper, this approach 
%%%%%%%%%% REASONS WHY BETTER THAN SIMULATION %%%%%%%%%%%%%%%%%

%%%%%% Härdle %%%%%%%%%%%
Given a multi-market setting, \cite{haerdleetal} examine the relation between down-side risk and stock returns.
They apply a time varying and time related co-integrated vector auto-regression model with a non-parametric Kernel density estimation with a double exponential Laplace kernel. 
Furthermore,given a period of time, the paper questions the impact and relevance of certain higher moments for VaR.
%Dynamics: Vector elements
%higher moments of risk
%VaR
%Stock returns 
%%%%% find source of VaR predictability power
%%%%%%%%%%%%%%%%%Distinction by SVM %%%%%%%%%%%%%%%%%


%%%%%%%% Schaumburg 1 %%%%%%%%%%%%
\cite{Schaumburg.2012} combines extreme value theory (EVT) with non-parametric VaR estimation in order to estimate return distributions of four financial stock indexes. Conditional quantiles are estimated by the application of monotonized double kernel local linear regression (DKLL), followed by the implementation of of the EVT peaks over threshold method to standardized 
%nonparametric 
residuals.
The methodology is compared to a parametric conditional autoregressive VaR model. \\
Although this study also applies a non-parametric approach, besides of quantile estimation, KDE density estimation and higher moment
%mean and volatility
estimation via SVR are of residuals are taken into consideration.
%%%%%%%\cite{Kuester.2006} Garch outperforms


%%%%%% Schaumburg 2 %%%%%%%%%%%%%%
%%%%%%%%%Formulieren%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
















==> Sections/abstract.tex <==
\clearpage

{\LARGE{\bf \noindent Data Driven Value-at-Risk Forecasting \\ \vspace{0.1cm} \noindent Using a SVR-GARCH-KDE Hybrid}} \vspace{0.5cm}

\vspace{0.5cm}

%{\large Master Thesis by: \\ \vspace{0.1cm} \LARGE Marius Lux (558415)}

\section*{Abstract}

Appropriate risk management is crucial to ensure the competitiveness of financial institutions and stability of the economy. One widely used financial risk measure is \mbox{Value-at-Risk (VaR)}. VaR estimations that are based on linear and parametric models which are e.g. coupled with a normal distribution can lead to risk underestimation. This is caused by the time varying volatility, skewness and leptokurtosis of financial return series. Hence, a nonlinear and nonparametric framework to forecast VaR is introduced. The mean and volatility are modeled via support vector regression~(SVR) where the volatility model is motivated by the standard generalized autoregressive conditional heteroscedasticity (GARCH) formulation. Based on this, VaR is derived by applying kernel density estimation (KDE). Additionally, the SVR-GARCH-KDE hybrid is compared to standard, exponential and threshold GARCH models that are coupled with different error distributions. To examine the performance in different markets, one-day-ahead forecasts are produced for three indices, i.e. Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500). Model evaluation is done via a likelihood ratio based test framework for interval forecasts. The SVR-GARCH-KDE hybrid has a competitive performance. In most cases it outperforms models that are coupled with a normal distribution. However, benchmark models that are using a skewed t distribution have usually a better performance. \\

% For instance, it is the best model for the Euro STOXX 50 for the 0.5\% and 1\% quantile. In contrast, only one benchmark model performs worse for the Nikkei 225 at the 2.5\% level. \\

\noindent \textbf{Keywords:} Value-at-Risk, Support Vector Regression, Kernel Density Estimation, GARCH



==> Sections/conc.tex <==
\section{Conclusion}\label{Sec:Conc}
%$\R$
%\newline
%In the empirical study of \cite{Kuester.2005} VaR models belonging to the location-scale class were superior over other approaches. However, the mean and volatility processes of the proposed location-scale models were parametric and based on distributional assumptions. Moreover, assumptions were also made for the distribution of the standardized residuals. Motivated by this, a nonparametric and nonlinear VaR forecasting framework that is based on the location-scale class was introduced in this thesis. The mean and volatility model were proposed to be modeled with SVR in an ARMA and GARCH like fashion, respectively. Additionally, the VaR forecast is obtained by estimating the distribution function of the standardized residuals via KDE. \\

In a large-scale empirical comparison \cite{Kuester.2005} find VaR models belonging to the location-scale class superior to alternative approaches. However, the location-scale models considered in their study are parametric and based on distributional assumptions. Motivated by the potential shortcomings of a parametric approach, the paper introduces a nonparametric and nonlinear VaR forecasting framework based on the location-scale class. The mean and volatility model are modeled with SVR in an ARMA and GARCH like fashion, respectively. In addition, the VaR forecast is obtained by estimating the distribution function of the standardized residuals via KDE. 

To evaluate the performance of the SVR-GARCH-KDE hybrid, VaR is forecasted for three indices: Euro STOXX 50, Nikkei 225 and S\&P 500, considering the different quantiles of $\alpha \in \{0.01, 0.025, 0.05\}$ for forecast horizons of one and ten days. GARCH, EGARCH and TGARCH models coupled with the normal, $t$- and skewed $t$-distribution serve as benchmarks and are compared to the proposed model using a LR testing framework for interval forecasts \citep{Christoffersen.1998} and the SPA test of \cite{Hansen.2005}. Grid search with the goal to maximize the $p$-value of the LR test for conditional coverage is used to set the SVR parameters. The SVR-GARCH-KDE hybrid delivers competitive results. For instance, in case of the one-day-ahead forecast horizon it is the best model for the Euro STOXX 50 for $\alpha= 0.01$ and the third best model overall. The TGARCH and GARCH model in combination with the skewed $t$-distribution show the best results. In contrast to the benchmark models, which usually underestimate risk, the SVR-GARCH-KDE hybrid tends to overestimate risk. This can lead to situations where the SVR-GARCH-KDE hybrid has an average performance regarding the $p$-value of the test for conditional coverage. However, with respect to risk management, the use of the SVR-GARCH-KDE might be still favorable over using the benchmarks since all approaches exhibit statistical uncertainty. The tendency to overestimate risk can, therefore, serve as a model risk buffer. This is supported by the results of the SPA test that evaluates the loss function which penalizes especially large VaR violations. For instance, the proposed model has the best performance for the ten-days-ahead forecast horizon. 

\color{red}
In general, the competitive results indicate that the proposed SVR-GARCH-KDE hybrid is a promising alternative. Despite fixing and not retuning the hyperparameters for five years, it is among the top three models with respect to conditional coverage and loss minimization measured by the SPA test for a forecast horizon of one as well as ten days. Additionally, it is the best model in minimizing the loss function for ten-days-ahead forecasts. This indicates the proposed SVR-GARCH-KDE hybrid is a robust VaR modeling approach that is capable of capturing complex nonlinear structures in the volatility process and has the flexibility to model a wide class of tail events. \color{black} Moreover, further improvements can be expected by refining the tuning routine. However, there exist several ways that can lead to an improved performance. First, tuning could be done for more parameters. For instance, in the KDE part of the estimation procedure, the kernel function and bandwidth estimator are set without tuning. Hence, considering different kernel functions and more flexible bandwidth estimators are potential ways to improve the performance further. Moreover, the kernel in the SVR part is also fixed and could be varied. Second, more recent information could be used in the parameter selection by re-tuning the model. Here, tuning is done for a block of five years of data. Then, based on the optimal parameters found for this data block, forecasts for five years are made and the parameters are held fixed. Thus, annual or even shorter re-tuning periods could result in parameters that are more appropriate for the existing market risk. Additionally, refining the grid can also result in better parameter choices.

In addition to modifying the tuning routine, the SVR-GARCH-KDE hybrid could be improved by changing the model specification. Overall, the TGARCH model with the skewed $t$-distribution achieves very good results. Hence, the SVR-GARCH-KDE hybrid could be modified such that it also accounts for asymmetric reactions of the volatility to past returns in a TGARCH like manner. Moreover, the proposed procedure does not ensure that the estimated variances are positive. Here, this problem is handled by replacing non-positive estimates with the last positive. However, positive variance estimates could be ensured by modeling the logarithm of the squared mean model residuals instead. 

All above mentioned adjustments are potential starting points for future research to further improve the proposed framework. However, although the suggested modifications of the tuning procedure are reasonable approaches to improve the model performance, they also increase the computational complexity. After all, this is a slight drawback of the SVR-GARCH-KDE hybrid in comparison to standard models. It is, however offset by potential performance gains. 
 








==> Sections/emp_study.tex <==
\clearpage

\section{Empirical Study}\label{Sec:emp_study}

\subsection{General Setting}

The SVR-GARCH-KDE hybrid is tested using stock indices to evaluate the performance for different regions. We consider four indices, namely the Euro STOXX 50, S\&P 500 and Nikkei 225 which represent the Euro zone, the USA and Japan, respectively. The analysis is based on the log-returns of the adjusted index closing prices $P_t$:

\begin{equation}
r_t = \log(P_t) - \log(P_{t-1}).
\end{equation}

\noindent We forecast VaR for the quantiles $\alpha \in \{0.005, 0.01, 0.025, 0.05\}$, always considering a forecast horizon of one trading day. In empirical applications, the quality of SVR depends on the kernel and parameter values that need to be set manually. The prevailing approach to determine parameter settings is grid search \citep[e.g.,][]{Lessmann.2017}, which we also apply in this study. For the density estimation via KDE the Gaussian kernel function in combination with Silverman's rule of thumb are used to reduce computational cost. \\

\noindent The evaluation of the models is based on the work of \cite{Christoffersen.1998}. The core of the evaluation is a likelihood ratio test framework, which assess the unconditional and conditional coverage as well as the independence of VaR exceedances. Moreover, \cite{Christoffersen.1998} shows that the test statistic for conditional coverage can be derived as the sum of the test statistics of the test for unconditional coverage and independence of VaR exceedances. Hence, it is possible to test whether the performance of a VaR model in terms of correct conditional coverage is determined by its ability to achieve correct coverage or adjust for changing volatility. This is useful in situations where the model has relatively bad conditional coverage but only one of the test statistics for unconditional coverage or independence is small. As criterion for selecting a model from grid search and evaluate the performance of the SVR-GARCH-KDE hybrid with respect to benchmark models, the $p-$value of the test for conditional coverage is used. Since the null hypothesis corresponds to correct conditional coverage which is the desired property, the one with the highest $p-$value is considered to be the best. \\

\noindent We perform all analyses using the statistical software R. The data has been downloaded from Yahoo Finance using the quantmod package. For SVR, we use the package e1071, which is the R implementation of the LIBSVM library of \cite{Chang.2011}. To reduce computational time, we employ the doParallel package for parallelization of computations. The benchmark methods introduced below are implemented by using the rugarch package. 


\subsection{Benchmark Methods}

To test the SVR-GARCH-KDE hybrid, we compare its performance to the standard GARCH model and some of its variations. In particular, \cite{Franke.2011} state that two of the most important variations are the EGARCH and TGARCH model. Hence, they serve as benchmarks in the empirical comparison. The GARCH-type models that \cite{Kuester.2005} analyze are coupled with different error distributions, i.e. the normal distribution, $t$ distribution and skewed $t$ distribution. We adopt this approach, which implies that we compare the SVR-GARCH-KDE hybrid to nine benchmarks.  

%\subsection{Popular Modifications of GARCH Models}
%
%\cite{Franke.2011} state that empirical studies found asymmetric reactions of the volatility depending on the sign of the return. In general, negative returns cause higher volatility than positive. To account for these empirical findings several variations of the standard GARCH model in (\ref{Eq:garch_original}) were proposed. Two crucial models are the exponential GARCH (EGARCH) and threshold GARCH (TGARCH) model which are presented below \cite[p. 308]{Franke.2011}.

\subsubsection{Exponential GARCH Model}

\cite{Nelson.1991} defines the EGARCH model as as follows, with $\omega_t$ and $\lambda_i$ denoting deterministic coefficients: 

\begin{equation}
\log(\sigma^2_t)  = \omega_t + \sum_{i = 1}^{\infty} \lambda_i m(z_{t-i}), \quad z_t \sim (0, 1) \ \text{i.i.d.}, \quad \lambda_1 = 1,
\label{Eq:egarch_def}
\end{equation}

\noindent where

\begin{equation}
m(z_t) = \rho z_t + \gamma(|z_t| - \mathbb{E}[|z_t|]).
\label{Eq:egarch_def_asyfct}
\end{equation}

\noindent Parameters $\rho$ and $\gamma$ are weights that need to be estimated. From $z_t \sim (0, 1) \ \text{i.i.d.}$ follows that $m(z_t)$ is i.i.d. with zero mean. There are some notable differences between the GARCH and EGARCH model. In equation (\ref{Eq:egarch_def}) $\sigma_t^2$ depends multiplicatively on past disturbances. This is in contrast to the standard GARCH model that depends additively on the mean model disturbances. Further, the asymmetric behavior of volatility is taken into account by $m(z_t)$ in (\ref{Eq:egarch_def}). Another difference is that there are no restrictions on the parameters in (\ref{Eq:egarch_def}) and (\ref{Eq:egarch_def_asyfct}).


\subsubsection{Threshold GARCH Model}

The TGARCH model is introduced by \cite{Zakoian.1994}. In TGARCH, asymmetries in the volatility are taken into account by modeling them as function of positive and negative disturbances. In contrast to the GARCH and EGARCH approach, \cite{Zakoian.1994} models the standard deviation rather than the variance. This is based on the work of \cite{Davidian.1987}, who find using absolute rather than squared disturbances to result in more efficient variance estimates. % \citep[p. 2]{Zakoian.1994}.
Formally, with $u_t^+ = \max(u_t, 0)$ and $u_t^- = \min(u_t, 0)$ the TGARCH($p$,$q$) model is defined as:

\begin{align}
u_t &= \sigma_t z_t, \quad z_t \sim (0, 1) \ \text{i.i.d.},\\
\sigma_t &= \omega + \sum_{i = 1}^{q} \delta_i^+ u_{t-i}^+ + \sum_{i = 1}^{q} \delta_i^- u_{t-i}^- + \sum_{j = 1}^{p} \theta_j \sigma_{t-i}.
\label{Eq:tgarch_def}
\end{align}

\noindent \cite{Zakoian.1994} points out differences to the EGARCH model. First, the TGARCH model is additive whereas the EGARCH model is multiplicative due to modeling the logarithm of $\sigma^2_t$. Moreover, for EGARCH models, asymmetry is captured by the same structure for all lags since the coefficients in (\ref{Eq:egarch_def_asyfct}) are constant. In contrast, TGARCH models allow for different coefficients depending on the lag. 

\subsection{Results}
%\subsection{Analysis for $\boldsymbol{\mu_t = 0}$ and GARCH(1,1)}

\subsubsection{Model Setting and Tuning}

We assume the mean process of $r_t$ in (\ref{Eq:svr_mean_estimate}) is zero. Moreover, we assume the variance process to have one AR and one MA part. These assumptions are imposed on both the SVR-GARCH-KDE hybrid and the benchmark models. We then forecast VaR  for every index trading day from 2011-07-01 until 2016-06-30. The data is  scaled to zero mean and unit variance in the SVR step; as suggested in the documentation of the e1071 package. Model training is done in a moving window approach using 251 return observations, which corresponds to approximately one trading year. Here, a trading year is assumed to have 252 price observations. Hence, one observation less is available when returns are considered. Tuning is done using the same moving window approach for forecasting VaR from 2006-07-01 until 2011-06-30. The considered parameter values in the grid for SVR are

\begin{itemize}
	\item $C \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$
	\item $\psi \in \{0, 0.1, \dots, 0.9 \}$  where $\epsilon = Q_{u^2_{scale}}(\psi)$
	\item $\gamma \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$.
\end{itemize}    
 

\noindent Note that the second point indicates that tuning is not done over fixed values of $\epsilon$. Instead, in every step of the estimation, $\epsilon$ is determined based on the $\psi$-quantile of the squared scaled disturbances of the mean model. This corresponds to the squared scaled returns because we assume zero mean of $r_t$. The motivation behind this is the tendency of returns to form volatility clusters. Hence, a fixed $\epsilon$ can lead to good results in one volatility regime but might have a poor performance after a regime change. For instance, in the case of a financial crisis, the right tail of the distribution of past volatilities gets thicker. Hence, an $\epsilon$ that depends on the quantile of the distribution will increase such that large volatilities have automatically a higher influence on the estimated parameters from the SVR optimization. By using squared values it is ensured that only positive values are obtained for $\epsilon$. However, notice that the distribution of the scaled squared disturbances, which are used in the SVR training, is shifted to the left of the distribution of the squared scaled disturbances. Hence, it is possible that for high values of $\psi$ no observations are outside the $\epsilon$-tube such that the model cannot be estimated.     \\

\noindent The parameter settings that resulted in the best models for the SVR-GARCH-KDE hybrid during the tuning period are shown in Table \ref{Tab:tuning_case1}.  
It can be seen that especially for $\psi$ only a certain range appears among the best models. Moreover, the optimal $\psi$ tends to be higher for lower quantiles. Based on the obtained parameters, VaR forecasts are produced from 2011-07-01 until 2016-06-30. 
%For all indices and parameter settings no results were obtained for $\psi = 0.9$ due to R returning the error message "Model is empty!". This is caused by the point described in the passage above, meaning that for $\psi = 0.9$ no values are left for SVR model training.

%\vspace{-1cm}
%\input{Tables/Case_1Results_Case1_EuroStoxx50.tex}
%\clearpage

\subsubsection{Model Comparison}

\noindent The results of the simulations are presented for each quantile separately in the Tables \ref{Tab:case1_0.5}, \ref{Tab:case1_1}, \ref{Tab:case1_2.5} and \ref{Tab:case1_5} at the end of the section. To clearly identify the best performing models, every table is sorted in descending order for every index according to the p-value of the conditional coverage test. The abbreviations NORM, STD and SSTD indicate the normal, $t$ and skewed $t$ distribution, respectively. Additionally, the column headers UC, ID and CC refer to the corresponding $p$-value of the LR test for unconditional coverage, independence of violations and conditional coverage.  

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.005}$}
 For the Euro STOXX 50, the SVR-GARCH-KDE hybrid has together with the TGARCH-STD and TGARCH-SSTD model the best results according to their p-values of the LR test for conditional coverage. However, all models have low CC values in comparison to the other time series. This comes from many violations which lead to low values in the LR test for UC. Despite having the most independent violations for the Nikkei 225, there are five models being better than the SVR-GARCH-KDE hybrid according to the CC value. This is mainly caused due to overestimating the market risk; as shown by the violations. In practice, risk overestimation is more desirable than underestimation. In particular, overestimation may lead to some potential profits not being  realized, whereas risk underestimation can lead to bankruptcy in the short term. The SVR-GARCH-KDE hybrid is the second best model in terms of unconditional coverage for the S\&P 500 but tends to form violation clusters. This can be concluded from the $p$-value in the ID column. As a result, only the GARCH-NORM and EGARCH-NORM model perform worse in terms of CC. 

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.01}$}  As for $\alpha = 0.005$, the SVR-GARCH-KDE hybrid is the best model for the Euro STOXX 50 for $\alpha = 0.01$. A visualization of its performance is given in Figure~\ref{Fig:model_comparision_SP500_1}. It is compared to the EGARCH-NORM model, which ranked worst. Here, the SVR-GARCH-KDE hybrid estimates in general higher values for VaR than the EGARCH-NORM model and exhibits more variability. The results are also similar to the 0.5\% level for the S\&P 500 and Nikkei 225, meaning that the SVR-GARCH-KDE hybrid has an average performance for both series. Moreover, this is again caused by having a low unconditional coverage for the Nikkei 225 and a tendency to form violation clusters for the S\&P 500.  In addition, the models coupled with a normal distribution perform poorly for all indices for $\alpha \in \{0.005, 0.01\} $. This comes as no surprise since the distribution of asset returns is usually leptokurtic. Accordingly, models that are coupled with a skewed $t$ distribution perform best.

\begin{figure}[h]
\centering
\includegraphics[scale = 0.65]{Figures/VaR_Plots_ES1}
\caption[SVR-GARCH-KDE and EGARCH-NORM for the Euro STOXX 50 at $\alpha = 0.01$]{VaR forecast model comparison for the Euro STOXX 50 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the EGARCH-NORM model.}
\label{Fig:model_comparision_SP500_1}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.025}$} The performance of the SVR-GARCH-KDE hybrid at the 2.5\% level is not as good as for $\alpha \in \{0.005, 0.01\}$ for the Euro STOXX 50. We observe the lowest $p$-value in the test for independence of violations. Interestingly, although the TGARCH and EGARCH model account for asymmetries in volatility, the former is the best and the latter the worst variance model. A relatively high risk overestimation for the S\&P 500 and Nikkei 225 causes the SVR-GARCH-KDE hybrid to be on the sixth and ninth rank, respectively. Rank nine is the worst that the SVR-GARCH-KDE hybrid achieves across all comparisons. A visual inspection of the model's performance compared to the GARCH-SSTD model, which performed best, is given in Figure \ref{Fig:model_comparision_SP500_5}.  
\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.65]{Figures/VaR_Plots_Nik25}
	\caption[SVR-GARCH-KDE and GARCH-SSTD for the Nikkei 225 at $\alpha = 0.025$]{VaR forecast model comparison for the Nikkei 225 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the GARCH-SSTD model.}
	\label{Fig:model_comparision_SP500_5}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.05}$} The best performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is rank two for the Nikkei 225. Here, it is only beaten by the EGARCH-SSTD model. For the other indices the SVR-GARCH-KDE hybrid ranks on place five. This is caused by having relatively low $p$-values for the ID test. In terms of UC, the SVR-GARCH-KDE hybrid is the second and third best model for the S\&P 500 and Nikkei 225, respectively. In comparison to the results for $\alpha \in \{0.005, 0.01\}$, the models with a normal distribution are not the worst for $\alpha \in \{0.025, 0.05\}$. However, using the skewed $t$ distribution leads also for $\alpha \in \{0.025, 0.05\}$ to the best rankings.  \\

\noindent Summarizing the results observed across all indices and quantiles, we conclude that the SVR-GARCH-KDE hybrid displays an average performance. Unlike the benchmarks, the SVR-GARCH-KDE hybrid tends to overestimate market risk. This might come from the choice of time interval for SVR parameter tuning. In particular, the tuning period covers the financial crisis of 2008 where market risk was extremely high. However, the SVR-GARCH-KDE hybrid usually outperforms benchmark models coupled with a normal distribution. This can be seen in Table \ref{Tab:mean_ranks} where the mean ranks per index and quantile are presented for each model. Moreover, there is no setting where the models using a normal distribution perform best. This provides further evidence that using the normal distribution to measure market risk is inappropriate. However, models with a skewed $t$ distribution show in many cases the best performance. For instance, the TGARCH model coupled with the skewed $t$ distribution is always among the top three. This confirms the results of previous research related to return distribution being skewed skewed.   
%Table has been moved to appendix

\begin{table}[ht]
	\centering
	\begin{tabular}{l|c}
		\hline
		 \textbf{Model} & \textbf{Mean Rank} \\ 
		 \hline
		\hline
		 TGARCH-SSTD & 2.1 \\ 
		 GARCH-SSTD & 2.4 \\ 
		 EGARCH-SSTD & 4.8 \\ 
		 TGARCH-STD & 4.8 \\ 
		 SVR-GARCH-KDE & 4.9 \\ 
		 GARCH-STD & 5.7 \\ 
		 TGARCH-NORM & 6.3 \\ 
		 GARCH-NORM & 6.6 \\ 
		 EGARCH-STD & 7.8 \\ 
		 EGARCH-NORM & 8.7 \\ 
		\hline
		\hline
	\end{tabular}
	\caption[Model comparison via mean ranks]{The models are presented with their mean rank. The mean rank was computed per index and quantile using the ties method \textit{min} in the \textit{frankv} function of the R package  data.table. The lower the mean rank, the better the model.}
	\label{Tab:mean_ranks}
\end{table}

%\clearpage
\newgeometry{left=6cm, right=1cm, top=3.5cm,bottom=1cm}
%\vspace*{-1cm}
\input{Tables/Results_Tunig_Results_Case_1.tex}

\input{Tables/Results_Case1_05.tex}
%\clearpage

%\vspace{-1cm}
\input{Tables/Results_Case1_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_5.tex}
%\clearpage
\restoregeometry

\clearpage

==> Sections/emp_study_short_2017Nov23.tex <==
\section{Empirical Study}\label{Sec:emp_study}

\subsection{General Setting}

The SVR-GARCH-KDE hybrid is tested using stock indices to evaluate the performance for different regions. We consider three indices, namely the Euro STOXX 50, S\&P 500 and Nikkei 225 which represent the Euro zone, the USA and Japan, respectively. The analysis is based on the log-returns of the adjusted index closing prices $P_t$:

\begin{equation}
r_t = \log(P_t) - \log(P_{t-1}).
\end{equation}

\noindent The descriptive statistics of the analyzed indices are given in Table \ref{Tab:desc_stats}.

\input{Tables/Descriptive_Statistics_Adjusted.tex}
\color{red}
We forecast VaR for the quantiles $\alpha \in \{0.01, 0.025, 0.05\}$, considering forecast horizons of one and ten trading days. Estimating VaR for a horizon of ten trading days is especially important regarding the applicability of a VaR model. Besides forecasting VaR for a confidence level of 99\%, which is equivalent to $\alpha = 0.01$ in our setting, a ten days forecast horizon is required in the regulations of the Basel Committee on Banking Supervision. 
\color{black}
In empirical applications, the quality of SVR depends on the kernel and parameter values which need to be set manually. The prevailing approach to determine parameter settings is grid search \citep[e.g.,][]{Lessmann.2017}, which we also apply in this study. For the density estimation via KDE, the Gaussian kernel function in combination with Silverman's rule of thumb are used to reduce computational cost. The Gaussian kernel function in KDE is equivalent to the standard normal distribution:

\begin{equation}
K(u) = \dfrac{1}{2\pi} e^{-\frac{u^2}{2}}.
\label{Eq:kde_gauss}
\end{equation}

\cite{Silverman.1986} showed that when (\ref{Eq:kde_gauss}) is used, robust density estimates can be obtained with the following estimator for the bandwidth $h$:

\begin{equation}
h_{rot} = 0.9 \min\{ \widehat{\sigma}_e, \widehat{\sigma}_{iqr} \} n^{-1/5}.
\label{Eq:kde_silverman}
\end{equation}

In \ref{Eq:kde_silverman} $\widehat{\sigma}_e$ denotes the empirical standard deviation and $\widehat{\sigma}_{iqr}$ is an estimate of the standard deviation that is based on the interquartile range $R$:

\begin{equation}
\widehat{\sigma}_{iqr} = \dfrac{R}{1.34}.
\label{Eq:kde_iqr_sd}
\end{equation}

The rule-of-thumb estimator $h_{rot}$ is computationally inexpensive whereas other proposed approaches to bandwidth estimation are more expensive since they are usually based on cross validation \citep{Hardle.2004}. Moreover, the importance of the kernel choice regarding the performance of KDE is limited. For instance, \cite{Hardle.2004} conclude that the kernel choice has almost no practical relevance after deriving the asymptotic mean integrated squared error for different kernel choices.

The evaluation of the models is based on \cite{Christoffersen.1998} who proposes a likelihood ratio (LR) test framework, which assesses the unconditional and conditional coverage as well as the independence of VaR exceedances. Moreover, \cite{Christoffersen.1998} shows that the test statistic for conditional coverage can be derived as the sum of the test statistics of the test for unconditional coverage and independence of VaR exceedances. Hence, it is possible to test whether the performance of a VaR model in terms of conditional coverage is determined by its ability to achieve correct unconditional coverage or adjust for changing volatility. This is useful in situations where the model has relatively bad conditional coverage but only one of the test statistics for unconditional coverage or independence is small. The hypotheses for the three tests are shown in Table \ref{Tab:hypotheses_cov} where $\alpha$ is the target quantile and $\mathcal{F}_{t-1}$ the information set available at $t-1$. $V_t$ is a series of VaR violations with $V_t = \mathbb{I}(r_t < -VaR_t^{\alpha})$ where $\mathbb{I}(x < c)$ denotes the indicator function:
	\begin{equation}
	\mathbb{I}(x < c) = \begin{cases}
	1 \text{ \ if \ } x < c \\
	0 \text{ \ if \ } x \ge c. \\
	\end{cases} 
	\end{equation}
For the test of independence of violations $V_t$ is assumed to be a binary first-order Markov chain. The corresponding transition probability matrix of $V_t$ is
	
	\begin{equation}
	\Pi_1 = \begin{bmatrix}
	1 - \pi_{01} & \pi_{01} \\
	1 - \pi_{11} & \pi_{11} 
	\end{bmatrix}
	\end{equation}
	
\noindent where 
	
	\begin{equation}
	\pi_{ij} = \mathbb{P}(V_t = j | V_{t-1} = i).
	\end{equation}
	

\begin{table}[ht]
	\centering
	\begin{tabular}{l|l|l}
		\hline
		\textbf{Test} & \boldmath{$\textbf{H}_0$} & \boldmath{$\textbf{H}_1$} \\ 
		\hline
		\hline
		Unconditional Coverage & $\mathbb{E}[V_t] = \alpha$ & $\mathbb{E}[V_t] \ne \alpha$  \\ 
		\hline
		Independence of Violations & $\pi_{01} = \pi_{11}$ & $\pi_{01} \ne \pi_{11}$ \\ 
		\hline
		Conditional Coverage & $\mathbb{E}[V_t| \mathcal{F}_{t-1}] = \alpha$ & $\mathbb{E}[V_t| \mathcal{F}_{t-1}] \ne \alpha$  \\ 

		\hline
		\hline
	\end{tabular}
	\caption{Hypotheses for evaluating the appropriateness of VaR forecasts with the testing framework introduced by \cite{Christoffersen.1998}.
	\label{Tab:hypotheses_cov}} 
\end{table}


 As criterion for selecting a model from grid search and evaluate the performance of the SVR-GARCH-KDE hybrid with respect to benchmark models, the $p$-value of the test for conditional coverage is used. Since the null hypothesis corresponds to correct conditional coverage which is the desired property, the one with the highest $p$-value is considered to be the best. 

\color{red} 
By using the framework of \cite{Christoffersen.1998} to evaluate and select models, the main focus is put on the statistical properties and VaR violations of the considered models. In order to measure the performance from the perspective of a loss function that also takes into account the magnitude of violations, the quadratic and asymmetric loss function that was introduced in one of the seminal papers for evaluating VaR models by \cite{Lopez.1998} will be used: 

\begin{equation}
L(r_t, VaR_t^{\alpha}) = \begin{cases}
1 + (r_t - VaR_t^{\alpha})^2  &\text{ \ if \ } r_t < VaR_t^{\alpha}  \\
0 &\text{ \ if \ } r_t \ge VaR_t^{\alpha}. \\
\end{cases} 
\end{equation}

\noindent The model losses will be evaluated by employing the superior predictive ability test (SPA) framework proposed by \cite{Hansen.2005}. Following the notation of \cite{Hansen.2005}, for a finite set of decision rules $[\delta_{k, t-h}, k = 0, 1, \dots, m]$ made $h$ periods in advance with respect to a random variable $\xi_t$, the relative performance corresponding to the benchmark $\delta_{0, t-h}$ is measured as

\begin{equation}
d_{k,t} = L(\xi_t, \delta_{0, t-h}) - L(\xi_t, \delta_{k, t-h}).
\end{equation}

\noindent Based on the assumption that the alternatives are superior if and only if  $\mathbb{E}[d_{k,t}] > 0$, \cite{Hansen.2005} formulates the hypothesis of interest for $ \boldsymbol{d_t} = (d_{1,t}, \dots, d_{m,t})^\top $ as

\begin{equation}
	 \text{H}_0: \mathbb{E}[\boldsymbol{d_t}] \le \boldmath{0}.
\end{equation}

\noindent A high $p$-value indicates that none of the alternatives is superior to the benchmark. For further information regarding the SPA test we refer to \cite{Hansen.2005}. As for the LR test of \cite{Christoffersen.1998}, the SPA test will be performed for every model. This is done by using every considered model once as benchmark in terms of \cite{Hansen.2005} and comparing it to all other models. Note that due to performing multiple statistical tests the $p$-values should be interpreted rather as an indication of model performance than in the context of a fixed significance level. 

\color{black}

We perform all analyses using the statistical software R. The data has been downloaded from Yahoo Finance using the quantmod package. For SVR, we use the package e1071, which is the R implementation of the LIBSVM library of \cite{Chang.2011}. To reduce computational time, we employ the doParallel package for parallelization of computations. The benchmark methods introduced below are implemented by using the rugarch package. All codes are available on \url{www.quantlet.de}. For details we refer to \cite{Borke.2018} and \cite{Borke.2017}.


\subsection{Benchmark Methods}

To test the SVR-GARCH-KDE hybrid, we compare its performance to the standard GARCH model and two of its variations. In particular, \cite{Franke.2011} state that the most important variations are the EGARCH and TGARCH model. Hence, they serve as benchmarks in the empirical comparison. The EGARCH and TGARCH models are introduced by \cite{Nelson.1991} and \cite{Zakoian.1994}, respectively. In contrast to standard GARCH models, both can account for asymmetric behavior with respect to past positive or negative returns. The two main differences between EGARCH and TGARCH models are that the former has a multiplicative and the latter an additive model structure. Moreover, TGARCH models allow for different coefficients depending on the lags whereas EGARCH models capture the asymmetric behavior for all lags with one coefficient. The GARCH-type models that \cite{Kuester.2005} analyze are coupled with different error distributions, i.e. the normal distribution, $t$-distribution and skewed $t$-distribution. We adopt this approach, which implies that we compare the SVR-GARCH-KDE hybrid to nine benchmarks.  

%\subsection{Popular Modifications of GARCH Models}
%
%\cite{Franke.2011} state that empirical studies found asymmetric reactions of the volatility depending on the sign of the return. In general, negative returns cause higher volatility than positive. To account for these empirical findings several variations of the standard GARCH model in (\ref{Eq:garch_original}) were proposed. Two crucial models are the exponential GARCH (EGARCH) and threshold GARCH (TGARCH) model which are presented below \cite[p. 308]{Franke.2011}.

%\subsubsection{Exponential GARCH Model}
%
%\cite{Nelson.1991} defines the EGARCH model as as follows, with $\omega_t$ and $\lambda_i$ denoting deterministic coefficients: 
%
%\begin{equation}
%\log(\sigma^2_t)  = \omega_t + \sum_{i = 1}^{\infty} \lambda_i m(z_{t-i}), \quad z_t \sim (0, 1) \ \text{i.i.d.}, \quad \lambda_1 = 1,
%\label{Eq:egarch_def}
%\end{equation}
%
%\noindent where
%
%\begin{equation}
%m(z_t) = \rho z_t + \gamma(|z_t| - \mathbb{E}[|z_t|]).
%\label{Eq:egarch_def_asyfct}
%\end{equation}
%
%\noindent Parameters $\rho$ and $\gamma$ are weights that need to be estimated. From $z_t \sim (0, 1) \ \text{i.i.d.}$ follows that $m(z_t)$ is i.i.d. with zero mean. There are some notable differences between the GARCH and EGARCH model. In equation (\ref{Eq:egarch_def}) $\sigma_t^2$ depends multiplicatively on past disturbances. This is in contrast to the standard GARCH model that depends additively on the mean model disturbances. Further, the asymmetric behavior of volatility is taken into account by $m(z_t)$ in (\ref{Eq:egarch_def}). Another difference is that there are no restrictions on the parameters in (\ref{Eq:egarch_def}) and (\ref{Eq:egarch_def_asyfct}).
%
%
%\subsubsection{Threshold GARCH Model}
%
%The TGARCH model is introduced by \cite{Zakoian.1994}. In TGARCH, asymmetries in the volatility are taken into account by modeling them as function of positive and negative disturbances. In contrast to the GARCH and EGARCH approach, \cite{Zakoian.1994} models the standard deviation rather than the variance. This is based on the work of \cite{Davidian.1987}, who find using absolute rather than squared disturbances to result in more efficient variance estimates. % \citep[p. 2]{Zakoian.1994}.
%Formally, with $u_t^+ = \max(u_t, 0)$ and $u_t^- = \min(u_t, 0)$ the TGARCH($p$,$q$) model is defined as:
%
%\begin{align}
%u_t &= \sigma_t z_t, \quad z_t \sim (0, 1) \ \text{i.i.d.},\\
%\sigma_t &= \omega + \sum_{i = 1}^{q} \delta_i^+ u_{t-i}^+ + \sum_{i = 1}^{q} \delta_i^- u_{t-i}^- + \sum_{j = 1}^{p} \theta_j \sigma_{t-i}.
%\label{Eq:tgarch_def}
%\end{align}
%
%\noindent \cite{Zakoian.1994} points out differences to the EGARCH model. First, the TGARCH model is additive whereas the EGARCH model is multiplicative due to modeling the logarithm of $\sigma^2_t$. Moreover, for EGARCH models, asymmetry is captured by the same structure for all lags since the coefficients in (\ref{Eq:egarch_def_asyfct}) are constant. In contrast, TGARCH models allow for different coefficients depending on the lag. 

\subsection{Results}
%\subsection{Analysis for $\boldsymbol{\mu_t = 0}$ and GARCH(1,1)}

\subsubsection{Model Setting and Tuning}

We assume the mean process of $r_t$ in (\ref{Eq:svr_mean_estimate}) is zero. Moreover, we assume the variance process to have one AR and one MA part. These assumptions are imposed on both the SVR-GARCH-KDE hybrid and the benchmark models. We then forecast VaR  for every index trading day from 2011-07-01 until 2016-06-30. The data is scaled to zero mean and unit variance in the SVR step; as suggested in the documentation of the e1071 package. 

The tuning of the hyperparameters is done in a moving window approach using 251 return observations, which corresponds to approximately one trading year. The hyperparameters are tuned for every combination of index and quantile separately. For a given set of hyperparameters the model is trained based on the returns of the last trading year to predict the next day's VaR. Then, the window is shifted by one trading day. The tuning period reaches from 2006-07-01 until 2011-06-30, where 2006-07-01 marks the date of the first VaR prediction. The considered parameter values in the grid for SVR are

\begin{itemize}
	\item $C \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$
	\item $\psi \in \{0, 0.1, \dots, 0.9 \}$  where $\epsilon = Q_{u^2_{scale}}(\psi)$
	\item $\gamma \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$.
\end{itemize}    
 
Note that the second point indicates that tuning is not done over fixed values of $\epsilon$. Instead, in every step of the estimation, $\epsilon$ is determined based on the $\psi$-quantile of the squared scaled disturbances of the mean model. This corresponds to the squared scaled returns because we assume zero mean of $r_t$. The motivation behind this is the tendency of returns to form volatility clusters. Hence, a fixed $\epsilon$ can lead to good results in one volatility regime but might have a poor performance after a regime change. For instance, in the case of a financial crisis, the right tail of the distribution of past volatilities gets thicker. Hence, an $\epsilon$ that depends on the quantile of the distribution will increase such that large volatilities have automatically a higher influence on the estimated parameters from the SVR optimization. By using squared values it is ensured that only positive values are obtained for $\epsilon$. However, notice that the distribution of the scaled squared disturbances, which are used in the SVR training, is shifted to the left of the distribution of the squared scaled disturbances. Hence, it is possible that for high values of $\psi$ no observations are outside the $\epsilon$-tube such that the model cannot be estimated.    

The parameter settings that resulted in the best models for the SVR-GARCH-KDE hybrid during the tuning period are shown in Table \ref{Tab:tuning_case1}.  
It can be seen that especially for $\psi$ only a certain range appears among the best models. Moreover, the optimal $\psi$ tends to be higher for lower quantiles. Based on the obtained parameters, VaR forecasts are produced from 2011-07-01 until 2016-06-30. 
%\vspace{-1cm}
\input{Tables/Results_Tunig_Results_Case_1_Only_1to5.tex}
%\clearpage

\subsubsection{Model Comparison}

\noindent The results are presented for each quantile separately at the end of the section. In the Tables \ref{Tab:case1_1}, \ref{Tab:case1_2.5} and \ref{Tab:case1_5} are the results for the one-day-ahead forecast. The results for the ten-days-ahead forecasts can be found in the Tables \ref{Tab:case1_10days_1}, \ref{Tab:case1_10days_2.5} and \ref{Tab:case1_10days_5}. To clearly identify the best performing models, every table is sorted in descending order for every index according to the $p$-value of the conditional coverage test. The $p$-value of the conditional coverage test is used for sorting to focus rather on statistical properties than pure losses. The abbreviations NORM, STD and SSTD indicate the normal, $t$- and skewed $t$-distribution, respectively. Additionally, the column headers UC, ID, CC and SPA refer to the corresponding $p$-value of the test for unconditional coverage, independence of violations, conditional coverage and superior predictive ability.  

%\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.005}$}
% For the Euro STOXX 50, the SVR-GARCH-KDE hybrid has together with the TGARCH-STD and TGARCH-SSTD model the best results according to their p-values of the LR test for conditional coverage. However, all models have low CC values in comparison to the other time series. This comes from many violations which lead to low values in the LR test for UC. Despite having the most independent violations for the Nikkei 225, there are five models being better than the SVR-GARCH-KDE hybrid according to the CC value. This is mainly caused due to overestimating the market risk; as shown by the violations. In practice, risk overestimation is more desirable than underestimation. In particular, overestimation may lead to some potential profits not being  realized, whereas risk underestimation can lead to bankruptcy in the short term. The SVR-GARCH-KDE hybrid is the second best model in terms of unconditional coverage for the S\&P 500 but tends to form violation clusters. This can be concluded from the $p$-value in the ID column. As a result, only the GARCH-NORM and EGARCH-NORM model perform worse in terms of CC. 

\paragraph{One-Step-Ahead Forecast Model Evaluation for $\alpha = 0.01$} The SVR-GARCH-KDE hybrid is the best model for the Euro STOXX 50 for $\alpha = 0.01$. A visualization of its performance is given in Figure~\ref{Fig:model_comparision_estoxx_1}. Here, the SVR-GARCH-KDE hybrid estimates in general higher values for VaR than the other models and exhibits more variability. For the S\&P 500 and Nikkei 225 the SVR-GARCH-KDE hybrid outperforms all models that are coupled with a normal distribution. However, all models using a skewed $t$-distribution perform better. Especially for the Nikkei 225 this is caused by having low unconditional coverage due to risk overestimation. However, since risk overestimation causes less losses the SPA test $p$-value is highest. In general, the models coupled with a normal distribution perform poorly for all indices. This comes as no surprise since the distribution of asset returns is usually leptokurtic. 


\paragraph{One-Step-Ahead Forecast Model Evaluation for $\alpha = 0.025$} The performance of the SVR-GARCH-KDE hybrid at the 2.5\% level is not as good as for $\alpha = 0.01$ for the Euro STOXX 50. We observe the lowest $p$-value in the test for independence of violations but the third best regarding the test for unconditional coverage. Interestingly, although the TGARCH and EGARCH model account for asymmetries in volatility, the former is the best and the latter the worst variance model. A relatively high risk overestimation for the S\&P 500 and Nikkei 225 causes the SVR-GARCH-KDE hybrid to be on the sixth and ninth rank, respectively. As seen for $\alpha = 0.01$ this leads, however, to high $p$-values in the SPA test due to lower losses. The performance for the S\&P 500 can be seen in Figure~\ref{Fig:model_comparision_SP500_25}.

\paragraph{One-Step-Ahead Forecast Model Evaluation for $\alpha = 0.05$} The best performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is rank two for the Nikkei 225. Here, it is only beaten by the EGARCH-SSTD model. A visualization is given in Figure~\ref{Fig:model_comparision_nikkei_5}. For the other indices the SVR-GARCH-KDE hybrid ranks on place five. This is caused by having relatively low $p$-values for the ID test. In terms of UC, the SVR-GARCH-KDE hybrid is the second and third best model for the S\&P 500 and Nikkei 225, respectively. In comparison to the results for $\alpha = 0.01$, the models with a normal distribution show a better performance for $\alpha \in \{0.025, 0.05\}$. However, using the skewed $t$-distribution leads also for $\alpha \in \{0.025, 0.05\}$ to the best rankings.  

\color{red}
\paragraph{Ten-Steps-Ahead Forecast Model Evaluation for $\alpha = 0.01$} As for the one-step-ahead forecasts, the SVR-GARCH-KDE hybrid is also the best model for the Euro STOXX 50. For the S\&P 500 and Nikkei 225 the SVR-GARCH-KDE hybrid is the second and third best model, respectively. For all indices, it is the only model not underestimating the risk. Especially the EGARCH models perform poorly. A visualization is given in Figure~\ref{Fig:model_comparision_nikkei_1_10days}. In contrast to the one-step-ahead forecasts, the models using a normal distribution are not shown but the EGARCH models due to their bad performance for ten-days-ahead forecasts. With respect to the SPA test, the SVR-GARCH-KDE hybrid causes less severe losses than any other model for all levels of the ten-steps-ahead forecast horizon.

\paragraph{Ten-Steps-Ahead Forecast Model Evaluation for $\alpha = 0.025$} Overall, the SVR-GARCH-KDE hybrid performs worse at the 2.5\% than for the 1\% level. In case of the the S\&P 500 and Nikkei 225 this is mainly driven by overestimating the risk leading to low $p$-values in the UC test. In contrast, even though the SVR-GARCH-KDE hybrid has the highest $p$-value in the UC test for the EURO STOXX 50, it is relatively low for the ID test. An exemplary visualization is given for the EURO STOXX 50 in Figure~\ref{Fig:model_comparision_eurostoxx_25_10days}.

\paragraph{Ten-Steps-Ahead Forecast Model Evaluation for $\alpha = 0.05$} The performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is mixed. While it is by far the best model for the EURO STOXX 50, it achieves only rank seven and nine for the Nikkei 225 and S\&P 500, respectively. As for $\alpha = 0.025$ this is mainly driven by risk overestimation and low $p$-values for the UC test. Similar to the one-day-ahead forecasts, the models using a normal distribution perform better for $\alpha = 0.05$ than for the other quantiles. The TGARCH-NORM model is even the best for the S\&P 500. A visualization is shown in Figure~\ref{Fig:model_comparision_sap_5_10days}. 
\color{black}

\paragraph{Evaluation Summary} Summarizing the results observed across all indices, quantiles and the two forecast horizons, we conclude that the SVR-GARCH-KDE hybrid displays a competitive performance. This can be seen in Table \ref{Tab:mean_ranks} where the mean ranks per index and quantile are presented for each model with respect to the CC and SPA test as well as the two forecast horizons. The SVR-GARCH-KDE hybrid is overall and for the CC test $p$-values the third best model for both forecast horizons. Regarding the SPA test it has rank two for the one-day-ahead forecast horizon and is the best model for the ten-days-ahead forecast horizon. Benchmark models coupled with a normal distribution are usually outperformed by the SVR-GARCH-KDE hybrid. Consequently, the SVR-GARCH-KDE hybrid has a relatively high accuracy especially compared to models with a normal distribution. The importance of this result stems from the fact that GARCH models with a normal distribution can be seen as a popular standard approach for modeling VaR or volatility and are, therefore, a natural benchmark. Additionally, excepting the case of the ten-days-ahead S\&P 500 forecast for $\alpha = 0.05$ there is no setting where the models using a normal distribution perform best. This provides further evidence that using the normal distribution to measure market risk is inappropriate. However, models with a skewed $t$-distribution show in many cases the best performance. For instance, the TGARCH model coupled with the skewed $t$-distribution is with two exceptions always among the top three in terms of the CC test. This confirms the results of previous research showing usually skewed return distributions. Unlike the benchmarks, the SVR-GARCH-KDE hybrid tends to overestimate market risk. This might come from the choice of time interval for SVR parameter tuning. In particular, the tuning period covers the financial crisis of 2008 where market risk was extremely high. However, in the context of risk management, risk underestimation is more critical than risk overestimation because it can lead to bankruptcy in the short term. For instance, assume a hypothetical situation with the goal to forecast the 5\% VaR, where the SVR-GARCH-KDE hybrid and a benchmark model have the same $p$-value regarding the independence test. Additionally, assume the $p$-value of the benchmark in the test of conditional coverage is higher because it has an unconditional coverage of 5.5\% whereas that of the SVR-GARCH-KDE hybrid is 4\%. The 1\% overestimation of the SVR-GARCH-KDE hybrid works like a buffer for model risk since all estimation techniques exhibit statistical uncertainty. Hence, the use of the SVR-GARCH-KDE hybrid may be still more appealing than the use of benchmark models that tend to underestimate risk.    
   
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Table has been moved to appendix

\begin{table}[ht]
	\centering
	\begin{tabular}{l|c|c|c|c|c|c}
		\hline
		 \textbf{Model} & \textbf{Overall} & \textbf{CC 1 Day}  & \textbf{SPA 1 Day}  & \textbf{CC 10 Days} & \textbf{SPA 10 Days}  \\ 
		 \hline
 		\hline
TGARCH-SSTD & 2.3 & 2.2 & 1.4 & 2.3 & 3.2 \\ 
GARCH-SSTD & 2.6 & 2.3 & 2.6 & 2.7 & 2.7 \\ 
SVR-GARCH-KDE & 3.2 & 4.9 & 2.2 & 4.8 & 1.0 \\ 
GARCH-STD & 5.9 & 6.1 & 6.4 & 4.9 & 6.3 \\ 
TGARCH-NORM & 6.0 & 6.0 & 7.7 & 5.1 & 5.1 \\ 
GARCH-NORM & 6.6 & 6.1 & 6.8 & 6.3 & 7.3 \\ 
TGARCH-STD & 6.7 & 5.3 & 9.0 & 5.1 & 7.4 \\ 
EGARCH-SSTD & 6.9 & 5.0 & 5.3 & 9.4 & 7.9 \\ 
EGARCH-NORM & 8.6 & 8.7 & 7.3 & 9.3 & 9.0 \\ 
EGARCH-STD & 8.6 & 8.8 & 7.2 & 9.6 & 8.8 \\ 
		 \hline
		\hline
	\end{tabular}
	\caption[Model comparison via mean ranks]{The models are presented with their mean rank. The mean rank was computed per index and quantile using the ties method \textit{max} in the \textit{frankv} function of the R package data.table. The lower the mean rank, the better the model.}
	\label{Tab:mean_ranks}
\end{table}



%\clearpage

%\vspace*{-1cm}
%\input{Tables/Results_Tunig_Results_Case_1_Only_1to5.tex}

%\newgeometry{left=6cm, right=1cm, top=3.5cm,bottom=1cm}
%\input{Tables/Results_Case1_05.tex}
%\clearpage

%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_1Day_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_1Day_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_1Day_5.tex}
%\clearpage
%\restoregeometry

% Fuer 10-Days-Ahead
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_10Day_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_10Day_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_10Day_5.tex}

%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plots
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1/EuroStoxx50_1VaR}
	\caption{VaR one-day-ahead forecast model comparison for the Euro Stoxx 50 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the models using a normal distribution.}
	\label{Fig:model_comparision_estoxx_1}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1/SaP500_25VaR}
	\caption{VaR one-day-ahead forecast model comparison for the S\&P 500 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the models using a normal distribution.}
	\label{Fig:model_comparision_SP500_25}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1/Nikkei225_5VaR}
	\caption{VaR one-day-ahead forecast model comparison for the Nikkei 225 at $\alpha = 0.05$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the models using a normal distribution.}
	\label{Fig:model_comparision_nikkei_5}	
\end{figure}

%% 10 Days %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1_10Days/Nikkei225_1VaR}
	\caption{VaR ten-days-ahead forecast model comparison for the Nikkei 225 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the EGARCH models.}
	\label{Fig:model_comparision_nikkei_1_10days}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1_10Days/EuroStoxx50_25VaR}
	\caption{VaR ten-days-ahead forecast model comparison for the Euro Stoxx 50 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the EGARCH models.}
	\label{Fig:model_comparision_eurostoxx_25_10days}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1_10Days/SaP500_5VaR}
	\caption{VaR ten-days-ahead forecast model comparison for the S\&P 500 at $\alpha = 0.05$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the EGARCH models.}
	\label{Fig:model_comparision_sap_5_10days}	
\end{figure}

\clearpage


==> Sections/garch.tex <==
\subsection{Modeling Volatility Using GARCH Models}\label{Sec:garch}
%%%%Comment out
\iffalse
%Due to the non-stationarity of financial time series it is inadequate to model the original series with ARMA models. 
Figure~\ref{vola_clust} depicts the returns of the adjusted daily closing prices of the Standard and Poors 500 (S\&P 500) from 1 July 1996 to 30 June 2016. The time series is mean stationary but not stationary because the variance of returns of financial time series were found to be conditionally heteroscedastic causing volatility clustering. Hence, this section introduces the standard approach for modeling volatility: GARCH models. The focus of the section is to present the structure of GARCH models due to its importance for the proposed SVR-GARCH-KDE hybrid.

%\begin{figure}[h!]
%	\centering
%	\includegraphics[scale = 0.7]{Figures/Price_SP500_SecGARCH}
%	\caption[Adjusted daily closing prices of the S\&P 500]{Adjusted daily closing prices of the S\&P 500 from 1 July 1996 to 30 June 2016. Data Source: Yahoo Finance.}
%	\label{mean_trend}	
%\end{figure}

%\noindent The time series exhibits a trend, i.e. it is not mean stationary. However, the return series is usually mean stationary but not stationary. The variance of returns of financial time series were found to be conditionally heteroscedastic causing volatility clustering. This effect is illustrated in Figure~\ref{vola_clust}.

\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.7]{Figures/Returns_SP500_SecGARCH}
	\caption[Log-returns of the adjusted daily closing prices of the S\&P 500]{Log-returns of the adjusted daily closing prices of the S\&P 500 from 1 July 1996 to 30 June 2016. Data Source: Yahoo Finance.}	
	\label{vola_clust}
\end{figure}

%\noindent Especially during the financial crisis in 2008, volatility was relatively high. In contrast, in the years before the crisis it was relatively low. 
%\noindent Hence, this section introduces the standard approach for modeling volatility: GARCH models. The focus of the section is to present the structure of GARCH models due to its importance for the proposed SVR-GARCH-KDE hybrid.  \\
\fi
%%%%%%%End comment out
\noindent \cite{Bollerslev.1986} introduces GARCH models by generalizing the volatility modeling approach of \cite{Engle.1982}. In deriving the GARCH regression model \cite{Bollerslev.1986} starts by assuming conditional normality of the return process $r_t$:

\begin{equation}
r_t|\mathcal{F}_{t-1} \sim N(\beta^\top x_t, \sigma_t^2).
\label{Eq:arch_cond_norm}
\end{equation}

\noindent where $x_t$ is a vector of lagged endogenous as well as exogenous variables, $\beta$ an unknown parameter vector and $\mathcal{F}_{t-1}$ the information set available at $t-1$. Rewriting (\ref{Eq:arch_cond_norm}) as linear model with conditionally heteroscedastic and normally distributed disturbances gives:

\begin{equation}
r_t = \beta^\top x_t + u_t, \qquad u_t|\mathcal{F}_{t-1} \sim N(0, \sigma_t^2).
\label{Eq:arch_mean_mdl}
\end{equation}


\noindent Then, the GARCH($p$,$q$) representation of the variance $\sigma_t^2$ is
 
\begin{equation}
\sigma_t^2 = \omega + \sum_{i = 1}^{q} \delta_i u^2_{t-i} + \sum_{j = 1}^{p} \theta_j\sigma^2_{t-j}.
\label{Eq:garch_original}
\end{equation}

\noindent \cite{Bollerslev.1986} notes that (\ref{Eq:garch_original}) has an ARMA representation. To see this let $\nu_t = u_t^2 - \sigma_t^2$ and substitute $\sigma_t^2$ in (\ref{Eq:garch_original}) with $u_t^2 - \nu_t$ to obtain

\begin{equation}
u_t^2 - \nu_t = \omega + \sum_{i = 1}^{q} \delta_i u^2_{t-i} + \sum_{j = 1}^{p} \theta_j(u_{t-j}^2 - \nu_{t-j}).
\label{Eq:garch_arma1}
\end{equation}

\noindent Rearranging (\ref{Eq:garch_arma1}) yields an ARMA representation for $u_t^2$:

\begin{align}
u_t^2  &= \omega + \sum_{i = 1}^{q} \delta_i u^2_{t-i} + \sum_{j = 1}^{p} \theta_j(u_{t-j}^2 - \nu_{t-j}) + \nu_t  \\
&=\omega + \sum_{i = 1}^{\max(p,q)} (\delta_i + \theta_i) u_{t-i}^2 - \sum_{j = 1}^{p} \theta_j \nu_{t-j} + \nu_t. 
\label{Eq:garch_arma2}
\end{align}

\noindent Based on (\ref{Eq:garch_arma2}) nonlinear and nonparametric volatility models can be introduced. This can be seen by noting that the conditional expectation of $u_t^2$ is equal to $\sigma^2$. Consequently, the variance process can be modeled solely based on the observed values without making assumptions about the distributional form of the residuals or the structure of the variance process. Hence, the volatility model in the SVR-GARCH-KDE hybrid is motivated by the ARMA representation of $\sigma^2$. 


==> Sections/intro.tex <==
\clearpage


%\section{Introduction}\label{Sec:intro}

Events as the world wide stock market crashes in 1987 and 2008 as well as the outcomes of the 2016 referendum in the UK or the presidential election in the USA came unexpected for most people. Therefore, from the perspective of financial risk management the words of Emil Gumbel, who made important contributions to the field of extreme value statistics, should be marked: \textit{"Il est impossible que l`improbable n`arrive jamais." (It is impossible for the improbable to never occur.)} \cite[p. 200]{Gumbel.1958}. Since such events happen rarely, they occur as outliers in data series. However, they can have a big impact on the solvency of single institutions and the whole economy. For instance, strategical decisions that are based on models which underestimate existing market risks can result in large losses or even bankruptcy of the institution. If a system-relevant financial institution goes bankrupt, it can cause an economic crisis. Additionally, systematically overestimated market risk can prevent institutions from taking actions to generate profits. Thus, the use of appropriate models for measuring market risk results in a competitive advantage. \\

\noindent The importance of risk management for financial institutions and the economy drew researchers attention to the development of tools for handling risk. One of the most famous measures of uncertainty in financial markets is Value-at-Risk (VaR) which is e.g. described in detail by \cite{Alexander.2010} and \cite{Jorion.2009}. VaR is based on the quantiles of a portfolio's loss distribution. It can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable number. However, the use of VaR has been criticized. For instance, \cite{Artzner.1999} note that VaR is not subadditive and therefore no coherent risk measure. As a consequence, diversification can increase VaR. Despite this, regulatory frameworks for the banking and insurance industry as Basel III or Solvency II rely on VaR for the determining capital requirements of financial institutions. \\

\noindent One approach for estimating VaR is based on generalized autoregressive conditional heteroscedasticity (GARCH) models. For example, in an empirical study with more than 30 years of historical returns \cite{Kuester.2005} show that VaR forecasts which are based on standard GARCH models are relatively good compared to other methods. However, they have a linear and parametric structure. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation (MLE)  \citep{Bollerslev.1986}. This makes it necessary to make distributional assumptions. However, the distribution of financial returns were empirically shown to have fat tails and being skewed \citep{Bali.2008,Harvey.2000}. Therefore, assuming e.g. normality can lead to an underestimation of risk. In contrast, support vector regression (SVR) introduced by \cite{Vapnik.1995,Vapnik.1998} is a method originating in statistical learning theory and was derived based on minimizing the generalization error. SVR can be classified as a method belonging to the domain of machine learning (ML). Additionally, kernel density estimation (KDE) is a nonparametric method to estimate the density of a random variable \citep{Hardle.2004}. In this paper a data driven VaR forecasting framework that is based on SVR and KDE is introduced. The aim is to compare the proposed approach with similar parametric GARCH-type models to see whether performance gains can be achieved. \\

\noindent The remainder of the paper is structured as follows. In Section \ref{Sec:Lit_Rev} the literature where ML methods are used to forecast VaR are reviewed. Moreover, approaches that are used to establish prediction intervals but are also a possible framework for modeling VaR are presented as well. In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Consequently, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. Based on this, the proposed SVR-GARCH-KDE hybrid is introduced at the end of the section. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions on how to modify the proposed framework for performance improvements are provided in the last section. 



==> Sections/introSL.tex <==
\section{Introduction}\label{Sec:intro}
Events like the 2008 financial crisis or the outcome of the 2016 referendum in the UK came unexpected for many people. Yet, as these examples illustrate, unlikely events occur at times and they might have far reaching consequences. Risk management is the practice to analyze the macro-environment of an organization, identify possible adverse developments, and design suitable countermeasures.

%%%%%%%%%%%%%%%%%%%%%
%% Risk Management %%
%%       VAR       %%
%%%%%%%%%%%%%%%%%%%%%

For financial institutions and systemically important institutions in particular, a key risk management responsibility is to sustain solvency under adverse economic conditions \citep[e.g.,][]{Silva.2017, Kraus.2017}. One of the most popular measures of uncertainty in financial markets is VaR (e.g., \cite{Alexander.2010}). VaR is based on the quantiles of a portfolio's profit and loss ($P\&L$) distribution and can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable figure \citep[e.g.,][]{Chen.2012}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% VaR critique %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Regulatory frameworks for the banking and insurance industry such as Basel III or Solvency II also rely on VaR for determining capital requirements. Compared to expected shortfall, an alternative risk measure with some superior mathematical properties \citep[e.g.,][]{Kim.2016}, an advantage of VaR may be seen in the fact that its estimation is more robust due to putting less weight on tail events and large losses, which may deteriorate the quality of statistical estimation routines \citep{Sarykalin.2008}.  %Especially the latter property makes VaR the right choice for this paper, which focuses on developing estimates of risk exposure using data-driven forecasting methods.  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% VAR ESTIMATION and related work %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parametric only

Several approaches have been proposed to estimate VaR including parametric statistical models and data-driven machine learning algorithms such as neural networks (NN) and SVR. In a seminal study, \cite{Kuester.2005} review several statistical methods and compare these in a forecasting benchmark. Using more than 30 years of historical returns data, they find standard GARCH models to forecast VaR with the highest accuracy on average.

GARCH models are also employed by \cite{Chen.2012} to estimate VaR for four daily series of stock market indices. More specifically, \cite{Chen.2012} rely on an asymmetric Laplace distribution and model volatility using a GJR-GARCH model to introduce leverage effects. They then develop a time-varying model to allow for dynamic higher moments. These extensions allow for wider application of the model beyond forecasting. 

% Models with some ML element
Unlike the parametric approach of \cite{Chen.2012}, \cite{Franke.2006} estimate VaR for the German stock index through fitting the mean and volatility of the return series using NNs. More specifically, they model the mean and volatility as an autoregressive (AR) and autoregressive conditionally heteroscedastic (ARCH) process, respectively. To derive VaR and expected shortfall, \cite{Franke.2006} use the predicted mean and variance with the normal distribution. This model outperforms a standard GARCH model in terms of VaR exceedances and proofs capable of quickly adjusting volatility in case of shocks with only short impact. \cite{Dunis.2010} also  propose a NN-based approach towards forecasting VaR and expected shortfall. 

\cite{Khan.2011} develops a VaR-model that forecasts realized volatilities using a combination of a heterogeneous AR model and SVR. VaR is then computed based on the normal, $t$- and skewed $t$-distribution. Applying this model to 5- and 15-minutes return data, \cite{Khan.2011} is able to confirm the suitability of the SVR component.  \cite{Stankovic.2015} provide further evidence that SVR is a useful method for VaR forecasting. Likewise, \cite{Xu.2016} introduce a multi-period VaR model using SVR in a quantile regression framework and show this approach to outperform GARCH models. 

% Shortcomings of (partly) parametric models
The findings of \cite{Xu.2016} seem to disagree with prior results of \cite{Kuester.2005} where GARCH models predict VaR with highest average accuracy and more accurately than quantile regression approaches in particular. Implementations of the quantile regression using a data-driven SVR model might explain the results of \cite{Xu.2016}. More specifically, the linear and parametric structure of standard GARCH models might be a limiting factor in VaR forecasting. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation \citep{Bollerslev.1986}. This necessitates distributional assumptions, which might be problematic since the distribution of financial returns is skewed and exhibits fat tails \citep{Bali.2008,Harvey.2000}. 

% Key paper of Schaumburg
Noting the possible limitation of the parametric framework, \cite{Schaumburg.2012} combines extreme value theory with nonparametric VaR estimation to forecast return distributions of four financial stock indices. A parametric conditional autoregressive value at risk (CAViaR) model serves as benchmark. The benchmark and the proposed model both circumvent the estimation of the mean and variance of the $P\&L$ distribution through predicting a quantile directly. In this regard, the approach of \cite{Schaumburg.2012} can be characterized as a nonparametric CAViaR model. 

% Soft critic of Schaumburg and contribution
VaR forecasts based on CAViaR frameworks have also been considered in the benchmarking study of \cite{Kuester.2005}. In fact, the authors also introduce a novel CAViaR model in the paper and test it alongside various other VaR models. However, GARCH models and models relying on the $t$-distribution in particular emerge as most suitable for VaR modeling.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Motivating Method (including suggestions of Kiho)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In summary, parametric GARCH models are superior to parametric quantile regression approaches for modeling VaR. To achieve better results with quantile regression approaches, it is necessary to include nonparametric parts into the model. Additionally, data driven GARCH models where the mean and variance components are modeled nonlinearly and nonparametrically lead to better results than parametric GARCH models. However, one shortcoming of the so far proposed data driven GARCH models is the use of parametric residual distributions. Particularly with regard to skewness and kurtosis, this can lead to misspecified residual distributions, resulting in wrong VaR estimates. Therefore, a novel purely nonparametric VaR model that grounds on the GARCH framework is proposed here. We apply data driven approaches to all GARCH components, i.e. mean, variance and residual distribution. Using this approach, we can overcome the possible misspecification of the residual distribution as well as the misspecifications of mean and variance. More specifically, we estimate the mean and variance of the $P\&L$ distribution using SVR and employ KDE to model the density of the standardized residuals  \citep[e.g.,][]{Hardle.2004}. We then integrate these components to derive a VaR forecast. In other words, we propose to start from the most effective parametric modeling approach of \cite{Kuester.2005} and develop models that estimate its components in a purely data-driven manner. Although KDE is not a new  approach in VaR forecasting \citep[e.g.,][]{Haerdle.2016, Schaumburg.2012, Malec.2014}, the particular combination of data-driven VaR estimation using SVR and nonparametric density estimation, which we propose in this paper, has, to the best of our knowledge, not been considered in prior work. 

% Evaluation
We assess the performance of the proposed model in comparison to GARCH-type models with different error distributions also including skewed and fat-tailed distributions. Empirical experiments using data from three major financial indices, namely the Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500), suggest that the SVR-GARCH-KDE hybrid typically outperforms models that are coupled with a normal distribution and performs competitive to other benchmark models. %For example, SVR-GARCH-KDE performs best model for the Euro STOXX 50 for the 0.5\% and 1\% quantile. In contrast, only one benchmark model performs worse for the Nikkei 225 at the 2.5\% level. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Structure  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
The remainder of the paper is organized as follows. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Specifically, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. The proposed SVR-GARCH-KDE hybrid is then developed based on these building blocks. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions for future research are provided in the last section.

















==> Sections/intro_v003.tex <==
\section{Introduction}\label{Sec:intro}
Events like the 2008 financial crisis or the outcome of the 2016 referendum in the UK came unexpected for many people. Yet, as these examples illustrate, unlikely events occur at times and they might have far reaching consequences. Risk management is the practice to analyze the macro-environment of an organization, identify possible adverse developments, and design suitable countermeasures.

%%%%%%%%%%%%%%%%%%%%%
%% Risk Management %%
%%       VAR       %%
%%%%%%%%%%%%%%%%%%%%%

For financial institutions and systemically important institutions in particular, a key risk management responsibility is to sustain solvency under adverse economic conditions \citep[e.g.,][]{Silva.2017, Kraus.2017}. One of the most popular measures of uncertainty in financial markets is VaR (e.g., \cite{Alexander.2010}). VaR is based on the quantiles of a portfolio's profit and loss ($P\&L$) distribution and can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable figure \citep[e.g.,][]{Chen.2012}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% VaR critique %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Regulatory frameworks for the banking and insurance industry such as Basel III or Solvency II also rely on VaR for determining capital requirements. Compared to expected shortfall, an alternative risk measure with some superior mathematical properties \citep[e.g.,][]{Kim.2016}, an advantage of VaR may be seen in the fact that its estimation is more robust due to putting less weight on tail events and large losses, which may deteriorate the quality of statistical estimation routines \citep{Sarykalin.2008}.  %Especially the latter property makes VaR the right choice for this paper, which focuses on developing estimates of risk exposure using data-driven forecasting methods.  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% VAR ESTIMATION and related work %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parametric only

Several approaches have been proposed to estimate VaR including parametric statistical models and data-driven machine learning algorithms such as neural networks (NN) and SVR. In a seminal study, \cite{Kuester.2005} review several statistical methods and compare these in a forecasting benchmark. Using more than 30 years of historical returns data, they find standard GARCH models to forecast VaR with the highest accuracy on average.

GARCH models are also employed by \cite{Chen.2012} to estimate VaR for four daily series of stock market indices. More specifically, \cite{Chen.2012} rely on an asymmetric Laplace distribution and model volatility using a GJR-GARCH model to introduce leverage effects. They then develop a time-varying model to allow for dynamic higher moments. These extensions allow for wider application of the model beyond forecasting. 

% Models with some ML element
Unlike the parametric approach of \cite{Chen.2012}, \cite{Franke.2006} estimate VaR for the German stock index through fitting the mean and volatility of the return series using NNs. More specifically, they model the mean and volatility as an autoregressive (AR) and autoregressive conditionally heteroscedastic (ARCH) process, respectively. To derive VaR and expected shortfall, \cite{Franke.2006} use the predicted mean and variance with the normal distribution. This model outperforms a standard GARCH model in terms of VaR exceedances and proofs capable of quickly adjusting volatility in case of shocks with only short impact. \cite{Dunis.2010} also  propose a NN-based approach towards forecasting VaR and expected shortfall. 

\cite{Khan.2011} develops a VaR-model that forecasts realized volatilities using a combination of a heterogeneous AR model and SVR. VaR is then computed based on the normal, $t$- and skewed $t$-distribution. Applying this model to 5- and 15-minutes return data, \cite{Khan.2011} is able to confirm the suitability of the SVR component.  \cite{Stankovic.2015} provide further evidence that SVR is a useful method for VaR forecasting. Likewise, \cite{Xu.2016} introduce a multi-period VaR model using SVR in a quantile regression framework and show this approach to outperform GARCH models. 

% Shortcomings of (partly) parametric models
The findings of \cite{Xu.2016} seem to disagree with prior results of \cite{Kuester.2005} where GARCH models predict VaR with highest average accuracy and more accurately than quantile regression approaches in particular. Implementations of the quantile regression using a data-driven SVR model might explain the results of \cite{Xu.2016}. More specifically, the linear and parametric structure of standard GARCH models might be a limiting factor in VaR forecasting. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation \citep{Bollerslev.1986}. This necessitates distributional assumptions, which might be problematic since the distribution of financial returns is skewed and exhibits fat tails \citep{Bali.2008,Harvey.2000}. 

% Key paper of Schaumburg
Noting the possible limitation of the parametric framework, \cite{Schaumburg.2012} combines extreme value theory with nonparametric VaR estimation to forecast return distributions of four financial stock indices. A parametric conditional autoregressive value at risk (CAViaR) model serves as benchmark. The benchmark and the proposed model both circumvent the estimation of the mean and variance of the $P\&L$ distribution through predicting a quantile directly. In this regard, the approach of \cite{Schaumburg.2012} can be characterized as a nonparametric CAViaR model. 

% Soft critic of Schaumburg and contribution
VaR forecasts based on CAViaR frameworks have also been considered in the benchmarking study of \cite{Kuester.2005}. In fact, the authors also introduce a novel CAViaR model in the paper and test it alongside various other VaR models. However, GARCH models and models relying on the $t$-distribution in particular emerge as most suitable for VaR modeling.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Motivating Method (including suggestions of Kiho)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In summary, parametric GARCH models are superior to parametric quantile regression approaches for modeling VaR. To achieve better results with quantile regression approaches, it is necessary to include nonparametric parts into the model. Additionally, data driven GARCH models where the mean and variance components are modeled nonlinearly and nonparametrically lead to better results than parametric GARCH models. However, one shortcoming of the so far proposed data driven GARCH models is the use of parametric residual distributions. Particularly with regard to skewness and kurtosis, this can lead to misspecified residual distributions, resulting in wrong VaR estimates. Therefore, a novel purely nonparametric VaR model that grounds on the GARCH framework is proposed here. We apply data driven approaches to all GARCH components, i.e. mean, variance and residual distribution. Using this approach, we can overcome the possible misspecification of the residual distribution as well as the misspecifications of mean and variance. More specifically, we estimate the mean and variance of the $P\&L$ distribution using SVR and employ KDE to model the density of the standardized residuals  \citep[e.g.,][]{Hardle.2004}. We then integrate these components to derive a VaR forecast. In other words, we propose to start from the most effective parametric modeling approach of \cite{Kuester.2005} and develop models that estimate its components in a purely data-driven manner. In contrast to other so far proposed GARCH based approaches to forecast VaR \citep[e.g.,][]{Youssef.2015, Khosravi.2013, Aloui.2010, Huang.2009, Fan.2008, Chan.2007, Hartz.2006} no assumptions about process dependence structures or the distribution of residuals are made by combining SVR and KDE in a GARCH like fashion. Training the SVR-GARCH-KDE hybrid is, therefore, mainly computationally driven. 

The use of SVR is motivated by the existence of a large body of research showing the effectiveness of SVR in forecasting financial time series \citep[e.g.,][]{Chang.2016, Devi.2015, Tay.2001}. Additionally, \cite{Sheta.2015} compare the forecasting performance of SVR, ANN and traditional linear regression for the S\&P 500. They find that SVR solves the task most successfully. \cite{Kazem.2013} also provide evidence that SVR based models outperform ANNs in the context of financial forecasting. Moreover, \cite{Chen.2009} use a SVR approach for predicting stock market volatility and use a recurrent ANN as benchmark which is outperformed. The use of nonparametric density estimation is motivated by the fact that the existence of fat tails and skewness in the distribution of financial returns can be considered as an empirically proven fact \citep[e.g.,][]{Bali.2008, Harvey.2000}. Although KDE is not a new  approach in VaR forecasting \citep[e.g.,][]{Haerdle.2016, Schaumburg.2012, Malec.2014}, the particular combination of data-driven VaR estimation using SVR and nonparametric density estimation, which we propose in this paper, has, to the best of our knowledge, not been considered in prior work. 

% Evaluation
We assess the performance of the proposed model in comparison to GARCH-type models with different error distributions also including skewed and fat-tailed distributions. Empirical experiments using data from three major financial indices, namely the Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500), suggest that the SVR-GARCH-KDE hybrid typically outperforms models that are coupled with a normal distribution and performs competitive to other benchmark models. %For example, SVR-GARCH-KDE performs best model for the Euro STOXX 50 for the 0.5\% and 1\% quantile. In contrast, only one benchmark model performs worse for the Nikkei 225 at the 2.5\% level. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Structure  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
The remainder of the paper is organized as follows. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Specifically, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. The proposed SVR-GARCH-KDE hybrid is then developed based on these building blocks. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions for future research are provided in the last section.











==> Sections/kde.tex <==
\subsection{Nonparametric Density Estimation}\label{Sec:NDE}

%The motivation for Section \ref{Sec:garch} was the existence of volatility clusters in stock returns. %Moreover, the conditional expectation was found to often exhibit a dependence on past information, e.g. the last day's return. 
 The volatility of stock returns varies over time and a similar behavior has been observed for the third and fourth moment of the return distribution. For example, \cite{Bali.2008} show that VaR forecasts can be improved by using past estimates of skewness and kurtosis. Given the evidence for the leptokurtic nature of stock returns \citep{Franke.2011}, parametric distributional models might lack the flexibility to capture such distributional characteristics, which motivates the use of nonparametric methods such as KDE  \citep[e.g.,][]{Hardle.2004}.
 
%In addition with the found evidence for the leptokurtic nature of stock returns, %parametric distribution models often lack the flexibility to appropriately capture the distributional characteristics of stock returns. 
%These considerations make the use of nonparametric methods appealingbecause they can estimate distributions more flexible than parametric approaches. %One approach is the histogram. However, it has some drawbacks, e.g. histograms are not smooth even if the underlying density fube. This and other critiques can be avoided by using KDE which has more favorable properties than the histogram.
%The nonparametric method introduced here is called kernel density estimation (KDE). The derivations are based on \cite{Hardle.2004} and \cite{Silverman.1986}. An overview for other nonparametric density estimators can be found in \cite{Silverman.1986}. This subsubsection considers only the univariate case. For the derivationp[e.g.,][] of multivariate KDE see \cite{Hardle.2004} or \cite{Silverman.1986}. 

%\subsubsection{Kernel Density Estimation}

Let $X$ be a random variable with an absolutely continuous distribution function $F$. Further, denote the corresponding density function as $f$ and let $\{x_1, \dots, x_n\}$ be a sample of i.i.d. realizations of $X$. Then, the kernel density estimator $\hat{f}_h(x)$ of $f(x)$ is defined as   

%$F$ can be estimated by the empirical distribution function $F_n$:
%
%\begin{equation}
%	F_n(x) = \frac{1}{n} \sum_{i = 1}^{n} \mathbb{I}(x_i \le x).
%	\label{kde_naive_set}
%\end{equation}
%
%\noindent Based on this, \cite{Parzen.1962} starts its derivation of the density estimator for $f(x)$ by the following approach:
%
%\begin{equation}
%\hat{f}_h(x) = \dfrac{F_n(x + h) - F_n(x - h) }{2h}.
%\label{Eq:emp_pdf}
%\end{equation}

%Then, the density $f(x)$ of $X$ can written as
%
%\begin{equation}
%f(x) = \lim_{x \to 0} \dfrac{1}{2h} P[x-h < X \le x + h].
%\label{pdf_approx}
%\end{equation}
%\newline
%\noindent Here, $h$ is a bandwidth parameter with $h>0$. \cite{Hardle.2004} write the estimator in (\ref{Eq:emp_pdf}) as
%
%\begin{equation}
%\hat{f}_h(x) = \dfrac{1}{2nh} \# \{x_i \in [x-h, x+h)\},
%\label{kde_naive_set}
%\end{equation}
%\newline
%where $\#\{\cdot\}$ denotes the cardinality of a set. Equation (\ref{kde_naive_set}) can be rewritten as
%
%\begin{align}
%\hat{f}_h(x)  &= \dfrac{1}{2hn} \sum_{i = 1}^{n} I\{x_i \in [x-h, x+h)\} \\ 
% &= \dfrac{1}{2hn} \sum_{i = 1}^{n} I\{ x-h \le x_i < x+h \} \\
% &= \dfrac{1}{hn} \sum_{i = 1}^{n} \dfrac{1}{2} I\{ -1 \le \dfrac{x_i - x}{h} < 1 \}. \label{Eq:kde_simple}
%\end{align}
%\newline
%\noindent In the initial formulation of \cite{Rosenblatt.1956} or \cite{Parzen.1962} \cite, the terms in the sum are replaced by a weight function. However, they used intervals that are open or closed, respectively. Following the approach of using a weight function $w(\cdot)$ with a closed interval as in \cite{Parzen.1962} and substituting $u = (x_i - x)/h$, (\ref{Eq:kde_simple}) can be written as 
%\begin{align}
%\hat{f}_h(x) &= \dfrac{1}{hn} \sum_{i = 1}^{n} \dfrac{1}{2} I\{|u| \le 1 \} \label{Eq:kde_uniform} \\
%&= \dfrac{1}{hn} \sum_{i = 1}^{is c). a  
%\%end{align}
%\noindent In the KDE literature $w(\cdot)$ is called the uniform kernel. By using the uniform kernel the same weight is assigned to every observation in the considered interval. However, assigning a high weight to observations that are close and a low weight to those far from $x$ preserves more information about the real density $f(x)$. Consequently, other weighting functions taking this into account were introduced. These are the so-called kernel functions. Introducing a general kernel function $K(u)$ into (\ref{Eq:kde_uniform}) results in

\begin{equation}
\hat{f}_h(x) = \dfrac{1}{hn} \sum_{i = 1}^{n} K\left(\dfrac{x_i - x}{h}\right) 
\label{Eq:kde_definition} 
\end{equation}

\noindent where $h$ is a bandwidth parameter with $h>0$ and $K$ is a so-called kernel function. %There exist different kernel functions. Table \ref{Tab:kernel_functions} is a list of kernel functions that are presented in \cite{Hardle.2004}. 
Usually, a kernel function is assumed to be a symmetric density function, i.e.  %%Therefore, the general form of the kernel density estimate is obtained as 

%\begin{equation}
%\hat{f}_h(x) = \dfrac{1}{n} \sum_{i = 1}^{n} K_h(x - x_i)
%\label{Eq:kde_general}
%\end{equation}
%
%\noindent with
%
%\begin{equation}
%K_h(\cdot) = \dfrac{1}{h} K\left(\dfrac{\cdot}{h}\right). 
%\end{equation}

%\noindent There exist different kernel functions. Table \ref{Tab:kernel_functions} is a list of kernel functions that are presented in \cite{Hardle.2004}. Usually, a kernel function is assumed to be a symmetric density function, i.e.

\begin{equation}
	\int_{-\infty}^{\infty} K(u)du = 1 \quad \text{with} \ K(u) \ge 0
	\label{Eq:kernel_function_density}
\end{equation}

\noindent and

\begin{equation}
\int_{-\infty}^{\infty} uK(u)du = 0.
\end{equation}

\noindent Conveniently, (\ref{Eq:kernel_function_density}) implies that $\hat{f}_h(x)$ is also a density. Note that $\hat{f}_h(x)$ inherits all properties of $K$ regarding continuity and differentiability.

\iffalse
\begin{table}[H]
	\begin{center}
	\begin{tabular}{c|c}
		\hline \hline
		\textbf{Kernel} & \textbf{K(u)} \\
		\hline
		Uniform & $\frac{1}{2}I(|u| \le 1)$ \\
	    \hline
		Triangel & $(1 - |u|)I(|u| \le 1)$ \\
		\hline
		Epanechnikov & $\frac{3}{4}(1 - u^2)I(|u| \le 1)$ \\
		\hline
		Quartic/Biweight & $\frac{15}{16}(1 - u^2)^2I(|u| \le 1)$ \\
		\hline
		Triweight & $\frac{35}{32}(1 - u^2)^3I(|u| \le 1)$ \\
		\hline
		Gaussian & $\frac{1}{\sqrt{2 \pi}}\exp (-\frac{u^2}{2})$ \\
		\hline
		Cosine & $\frac{\pi}{4} \cos (\frac{\pi u}{2}) I(|u| \le 1)$ \\
		\hline \hline
	\end{tabular}
	\end{center}
	\caption[Kernel functions for kernel density estimation]{The table shows possible functions that can be used in the process of estimating the density of a random variable via KDE. Source: \cite{Hardle.2004}.}
	 \label{Tab:kernel_functions}	
\end{table}
\fi

%%%%%end

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\subsubsection{Bias-Variance-Trade-Off}
%
%Choosing $h$ is a central point when using KDE. Since (\ref{Eq:kde_general}) is a biased estimator of $f(x)$, a too high $h$ will result in a high bias. Decreasing $h$ will, however, result in a higher variance. In order to indicate these dependencies, bias, variance and mean squared error (MSE) will be derived in this subsubsection. Since the derivations use Taylor expansions with Landau symbols it is assumed that $n \to \infty$, $h \to 0$ and $nh \to \infty$. Note that by $\mathcal{O}(\cdot)$ and $o(\cdot)$ it is referred to the big-O and little-o-notation.
%
%\subsubsection{Bias} \label{Sec:kde_bias_subsubsection}
%
%The bias $\mathbb{B}$ of an estimator $\hat{\beta}$ for a parameter $\beta$ is defined as 
%
%\begin{equation}
%\mathbb{B}[\hat{\beta}] = \mathbb{E}[\hat{\beta}] - \beta.
%\label{Eq:bias_def}
%\end{equation}
%
%\noindent In the case where $f(x)$ is a density and $\hat{f}_h(x)$ an estimator for $f(x)$, equation (\ref{Eq:bias_def}) becomes
%
%\begin{equation}
%\mathbb{B}[\hat{f}_h(x)] = \mathbb{E}[\hat{f}_h(x)] - f(x). 
%\end{equation}
%
%\noindent Deriving $\mathbb{E}[\hat{f}_h(x)]$ yields
%
%\begin{align}
%\mathbb{E}[\hat{f}_h(x)] &= \mathbb{E}\left[\dfrac{1}{n} \sum_{i=1}^{n} K_h(x - x_i)\right]  \\ &=  \dfrac{1}{n} \sum_{i=1}^{n} \mathbb{E}[K_h(x - x_i)] \\ 
%& =  \mathbb{E}[K_h(x - X)] \label{Eq:bias_kde_iid} \\
%& =  \int \dfrac{1}{h} K\left(\dfrac{x - z}{h}\right)f(z)dz.
%\end{align}
%
%\noindent Note that in (\ref{Eq:bias_kde_iid}) $x_i$ can be replaced by $X$ due to the i.i.d. assumption. Substituting $u = (z - x)/h$, exploiting that kernels are symmetric, i.e. $K(u) = K(-u)$, and approximating $f(z)$ around $x$ with a second-order Taylor expansion gives
%
%\begin{align}
%\mathbb{E}[\hat{f}_h(x)] &= \int \dfrac{1}{h} K\left(\dfrac{x - z}{h}\right)f(z)dz  \\
%&= \int K(u) \left(f(x) + uhf'(x) + \dfrac{u^2 h^2}{2} f''(x) + o(h^2)  \right)du\\
%&=  f(x) \underbrace{\int K(u)du}_\text{=1} + hf'(x)  \underbrace{\int K(u)udu}_\text{= 0} \\ &\phantom{{}=1} + \dfrac{h^2}{2} f''(x) \underbrace{\int K(u)u^2du}_\text{=:$\mu_2(K)$} + o(h^2) \notag \\
%&=  f(x)  + \dfrac{h^2}{2} f''(x)\mu_2(K) + o(h^2).  
%\end{align}
% 
%\noindent Consequently, the kernel density estimator is a biased estimator of $f(x)$:
%
%  \begin{equation}
%  \mathbb{B}[\hat{f}_h(x)] = \dfrac{h^2}{2} f''(x)\mu_2(K) + o(h^2).
%  \label{kde_bias}
%  \end{equation}
%  
%\noindent Equation (\ref{kde_bias}) implies that the bias vanishes as $h \to 0$. However, simply choosing a very small $h$ does not guarantee an appropriate estimate as will be shown in the next subsubsection. 
%
%\subsubsection{Variance}
%
%As in the derivation for the bias, the kernel density estimator is plugged into the variance formula and the i.i.d. assumption is exploited. 
%
%\begin{align}
%\mathbb{V}[\hat{f}_h(x)] &= \mathbb{V}\left[\dfrac{1}{n} \sum_{i=1}^{n} K_h(x - x_i)\right]  \\
%&=  \dfrac{n}{n^2 h^2} \mathbb{V}\left[K\left(\dfrac{x - X}{h}\right)\right] \\ 
%& =  \dfrac{1}{n h^2} \mathbb{E}\left[K\left(\dfrac{x - X}{h}\right)^2\right] -  \dfrac{1}{n} \mathbb{E}\left[\dfrac{1}{h} K\left(\dfrac{x - X}{h}\right)\right]^2. \label{Eq:kde_var_one}
%\end{align}
%\newline
%\noindent The result of the second term was already derived in Section \ref{Sec:kde_bias_subsubsection} because it follows from (\ref{Eq:bias_kde_iid})
%
%\begin{equation}
%\dfrac{1}{n} \mathbb{E}\left[\dfrac{1}{h} K\left(\dfrac{x - X}{h}\right)\right]^2 = \dfrac{1}{n}\left[f(x) + \mathbb{B}[\hat{f}_h(x)] \right]^2.
%\label{Eq:density_plus_bias}
%\end{equation}
%\newline
%\noindent Hence, the following steps consider the derivation of the first term in (\ref{Eq:kde_var_one}). In the first step a substitution as in the bias derivation is used. This is followed by a first order Taylor approximation of $f$ around $x$:
%
%\begin{align}
% \dfrac{1}{n h^2} \mathbb{E}\left[K\left(\dfrac{x - X}{h}\right)^2\right] &= \dfrac{1}{n} \int \dfrac{1}{h^2} K\left(\dfrac{x-z}{h}\right)^2 f(z) dz \\
%&= \dfrac{1}{n} \int \dfrac{1}{h} K\left(u \right)^2 f(x+hu) du \\
%&= \dfrac{1}{nh} \int K\left(u \right)^2\{f(x) + o(h)\} du. \label{Eq:var_taylor}
%\end{align}
%
%\noindent By noting that (\ref{Eq:density_plus_bias})  is $\mathcal{O}(n^{-1})$ and using $\int K(u)^2 du = ||K||_2^2 $ in (\ref{Eq:var_taylor}) the variance is 
%
%\begin{align}
%\mathbb{V}[\hat{f}_h(x)] &= \dfrac{1}{nh} ||K||_2^2 \{ f(x) + o(h) \} + \mathcal{O}(n^{-1}) \\
%&= \dfrac{1}{nh} ||K||_2^2 f(x) + o \left( \dfrac{1}{nh} \right).
%\label{Eq:kde_variance}
%\end{align}
%
%\noindent From (\ref{Eq:kde_variance}) can be inferred that the variance decreases with increasing $h$. Approximating $f(x)$ with large values of $h$ results in an estimator with low variability for different $x$. The variance gets also lower for higher $n$. Moreover, (\ref{Eq:kde_variance}) increases in the squared norm of the kernel $K$ as well. As \cite{Hardle.2004} indicate, due to the dependence on $||K||_2^2$ smooth and flat kernels can result in estimates with lower variance. %For instance, the uniform kernel assigns the same weight to observations in different samples from one random variable.              
%
%\subsubsection{Mean Squared Error}
%
%The derived bias in (\ref{kde_bias}) and variance in (\ref{Eq:kde_variance}) indicate the existence of a trade-off between bias and variance. For instance, choosing a small $h$ implies a small bias but a high variance. Considering the MSE is useful for balancing out this trade-off because the MSE can be written as sum of variance and squared bias:
%
%\begin{equation}
%\text{MSE}[\hat{f}_h(x)] = \mathbb{V}[\hat{f}_h(x)] + \mathbb{B}[\hat{f}_h(x)]^2.
%\label{Eq:mse_def}
%\end{equation}
%
%\noindent Plugging the results for bias and variance into (\ref{Eq:mse_def}) gives
%
%\begin{align}
%\text{MSE}[\hat{f}_h(x)] &= \dfrac{1}{nh} ||K||_2^2 f(x) + o \left( \dfrac{1}{nh} \right) + \left\{\dfrac{h^2}{2} f''(x)\mu_2(K) + o(h^2)\right\}^2\\
%&= \dfrac{1}{nh} ||K||_2^2 f(x) + \dfrac{h^4}{4} f''(x)^2\mu_2(K)^2 + o(h^4) + o \left( \dfrac{1}{nh} \right). \label{Eq:kde_mse}
%\end{align}
%\newline
%\noindent Moreover, the MSE can be used to infer consistency of an estimator. A main result in the asymptotic theory of statistics is that convergence in mean square implies convergence in probability, i.e. consistency. For $h \to 0$ and $nh \to \infty$ equation (\ref{Eq:kde_mse}) converges to zero. Therefore, the kernel density estimator is consistent. 
%\newline
%\newline
%\noindent Although the MSE is useful in proving consistency and understanding the bias-variance-trade-off in KDE, it is not advisable to derive the optimal bandwidth $h_{opt}$ with it. The MSE is a local measure of the estimation accuracy. Meaning that $h_{opt}$ would be a function of $x$. Therefore, the next subsubsection derives the mean integrated squared error (MISE) and the asymptotic MISE (AMISE) instead. In contrast to the MSE, the MISE and AMISE are global accuracy measures.  
%
%\subsubsection{Asymptotic Mean Integrated Squared Error}
%
%In order to derive $h_{opt}$ the MISE will be derived. This is done by integrating the MSE over $x$:
%
%\begin{align}
%\text{MISE}(\hat{f}_h) &= \int \text{MSE}[\hat{f_h}(x)]dx \\
%&=  \int\left\{\dfrac{1}{nh} ||K||_2^2 f(x) + \dfrac{h^4}{4} f''(x)^2\mu_2(K)^2 + o(h^4) + o \left( \dfrac{1}{nh} \right)\right\}dx \\
%&=  \dfrac{1}{nh} ||K||_2^2 \underbrace{\int f(x)dx}_\text{= 1} + \dfrac{h^4}{4}\mu_2(K)^2 \underbrace{\int f''(x)^2 dx}_\text{$||f''||^2_2$} + o(h^4) + o \left( \dfrac{1}{nh} \right) \\
%&= \dfrac{1}{nh} ||K||_2^2  + \dfrac{h^4}{4} \mu_2(K)^2 ||f''||^2_2 + o(h^4) + o \left( \dfrac{1}{nh} \right). \label{Eq:kde_mise}
%\end{align}
%
%\noindent The AMISE of the kernel density estimator is obtained by neglecting terms of higher order in (\ref{Eq:kde_mise}):
%
%\begin{equation}
%\text{AMISE}[\hat{f}_h] = \dfrac{1}{nh} ||K||_2^2  + \dfrac{h^4}{4} \mu_2(K)^2 ||f''||^2_2.
%\label{Eq:kde_amise}
%\end{equation}
%
%\noindent Based on (\ref{Eq:kde_amise}) $h_{opt}$ can be derived. This is done in the next subsubsection.

%\subsubsection{Optimal Bandwidth}
%
%After deriving the AMISE of the KDE, $h_{opt}$ can be derived by differentiating $(\ref{Eq:kde_amise})$. It will be shown that $h_{opt}$ depends on $||f''||^2_2$ which is unknown. Hence, two methods for determining $h_{opt}$ that follow different approaches are derived in this subsubsection. The first aims to minimize AMISE by referencing to a standard distribution. It is characterized by its computational simplicity. In contrast, the second approach is based on CV and minimizing a different criterion. \cite{Hardle.2004} classify the CV based bandwidth selector as one of the most popular. Other bandwidth selectors are shortly explained at the end of the subsubsection. 
%
%
%\subsubsection{Deriving the Optimal Bandwidth}
%
%The first derivative of (\ref{Eq:kde_amise}) is
%
%\begin{align}
%\frac{\partial \text{AMISE}(h)}{\partial h} &= \frac{\partial}{\partial h} \left \{ \dfrac{1}{nh} ||K||_2^2  + \dfrac{h^4}{4} \mu_2(K)^2 ||f''||^2_2 \right \} \\
%&= -\dfrac{1}{nh^{2}} ||K||_2^2  + h^3\mu_2(K)^2 ||f''||^2_2.
%\end{align}
%
%\noindent Then, the optimal bandwidth $h_{opt}$ can be derived as
%
%\begin{align}
% -\dfrac{1}{nh_{opt}^{2}} ||K||_2^2  + h_{opt}^3\mu_2(K)^2 ||f''||^2_2 &= 0 \\
%h_{opt}^3\mu_2(K)^2 ||f''||^2_2 &= \dfrac{1}{nh_{opt}^{2}} ||K||_2^2  \\
%h_{opt} &= \left(\dfrac{||K||_2^2 }{n\mu_2(K)^2 ||f''||^2_2} \right)^{1/5}. \label{Eq:kde_hopt}
%\end{align}
%\newline
%\noindent Due to the dependence of $h_{opt}$ on $||f''||^2_2$, equation (\ref{Eq:kde_hopt}) cannot be used directly to find an appropriate bandwidth. However, the result can be used to infer rule-of-thumb bandwidths by making an assumption for $f$. 
%
%\subsubsection{Bandwidth Selection by Reference Distribution} \label{Sec:kde_hopt_ref}
%
%\cite{Silverman.1986} sees referencing to a standard distribution as an easy and natural way to find $h_{opt}$. For instance, by referencing to the normal distribution it holds that
%
%\begin{align}
%%||f||_2^2 &= \sigma^{-5}\int \psi''(x)dx \\
%%&= \sigma^{-5} \dfrac{3}{8 \sqrt{\pi}}.
%||f||_2^2 = \sigma^{-5} \dfrac{3}{8 \sqrt{\pi}}. \label{Eq:f_curve_normal}
%\end{align}
%
%\noindent Then, by estimating $\sigma$ from the sample it can be plugged into (\ref{Eq:f_curve_normal}). However, this approach contradicts the nonparametric philosophy of not making distributional assumptions. \cite{Hardle.2004} justify its use because it is an explicit formula and a convenient way to compute an estimate of $h_{opt}$. Furthermore, its use is recommended in situations where the distribution of $X$ is similar to the normal distribution. \cite{Hardle.2004} state the following characteristics for similarity: unimodality, approximate symmetry and not too fat tails. If these conditions are fulfilled it is reasonable to choose the Gaussian kernel from Table~\ref{Tab:kernel_functions}. Consequently, with a Gaussian kernel the rule-of-thumb estimator $h_{rot}$ based on (\ref{Eq:kde_hopt}) becomes
%
%\begin{align}
%h_{rot} &= \left(\dfrac{||K||_2^2 }{n\mu_2(K)^2 ||f''||^2_2} \right)^{1/5} \\
%&= \left( \dfrac{4 \sigma^5}{3n} \right)^{1/5} \\
%&\approx 1.06\sigma n^{-1/5}.
%\label{Eq:hopt_kde_gauss}
%\end{align}
%
%\noindent In (\ref{Eq:hopt_kde_gauss}) $\sigma$ can be estimated by the empirical standard deviation $\widehat{\sigma}_{\text{\tiny E}}$. \cite{Silverman.1986} found that using $\widehat{\sigma}_{\text{\tiny E}}$ in (\ref{Eq:hopt_kde_gauss}) can give reasonable estimates if $f$ is multimodal. However, for fat-tailed and skewed densities it is suggested to use a more robust estimator for $\sigma$. The proposed robust estimator is based on the interquartile range (IQR) of the normal distribution. Assume that for the random variable underlying the sample holds that $X \sim N(\mu, \sigma^2)$ and let $Z \sim N(0, 1)$. Further, define $Q(0.25)_{X}$ and $Q(0.75)_{X}$ as well as $Q(0.25)_{Z}$ and $Q(0.75)_{Z}$ as the first and third quartile of $X$ and $Z$, respectively. Then, the IQR of $X$, which is denoted as $R$, can be approximated as follows:
%
%\begin{align}
%R &= Q(0.75)_{X} - Q(0.25)_{X} \\
%%&= (\mu + \sigma Q(0.75)_{X}) - (\mu + \sigma Q(0.25)_{X}) \\
%&= (\mu + \sigma Q(0.75)_{Z}) - (\mu + \sigma Q(0.25)_{Z}) \\ 
%&=  2 \sigma Q(0.75)_{Z} \\
%&\approx  1.34\sigma.  \label{Eq:interquartil_distance}
%\end{align}
%
%\noindent An implication of (\ref{Eq:interquartil_distance}) is that
%
%\begin{align}
%\widehat{\sigma}_{\text{\tiny IQR}} = \dfrac{R}{1.34}  
%\end{align}
%
%\noindent can be used as an estimator for $\sigma$. Then, the corresponding optimal bandwidth for the Gaussian kernel is obtained as
%
%\begin{align}
%\widehat{h}_{\text{\tiny IQR}}& = \dfrac{1.06}{1.34} R n^{-1/5}  \\
%&\approx 0.79Rn^{-1/5}.
%\label{Eq:hopt_iqr_1}
%\end{align} 
%
%\noindent \cite{Silverman.1986} showed in simulations that by using (\ref{Eq:hopt_kde_gauss}) as bandwidth also multimodal densities can be approximated, even though it tends to oversmooth. Moreover, it was shown that by using (\ref{Eq:hopt_iqr_1}) as bandwidth better results are obtained for skewed and fat-tailed distribution. However, the studies revealed also that (\ref{Eq:hopt_iqr_1}) yields worse results than (\ref{Eq:hopt_kde_gauss}) in situations where $f$ is multimodal. To combine the abilities of both bandwidth estimators \cite{Silverman.1986} defines the adaptive estimator $\widehat{\sigma}_A$:
%
%\begin{equation}
%\widehat{\sigma}_{\text{\tiny A}} = \min\{\widehat{\sigma}_{\text{\tiny E}}, \widehat{\sigma}_{\text{\tiny IQR}} \}.
%\end{equation}
%
%\noindent Furthermore, it is suggested to reduce the scaling factor from $1.06$ to $0.9$. Then, one obtains the following bandwidth estimator: 
%
%\begin{equation}
%\widehat{h}_{\text{\tiny A}} = 0.9\widehat{\sigma}_{\text{\tiny A}}n^{-1/5}. \label{Eq:hopt_adaptive_rot}
%\end{equation}
%
%\noindent According to \cite{Silverman.1986}, by using $\widehat{h}_{\text{\tiny A}}$ bimodal and skewed densities can be modeled appropriately. Therefore, $\widehat{h}_{\text{\tiny A}}$ is supposed to deliver reasonable results for many different densities. Consequently, in the rest of this thesis the bandwidth estimator in (\ref{Eq:hopt_adaptive_rot}) is referred to as Silverman's rule of thumb.
%
%\subsubsection{Least Squares Cross Validation} 
%
%A more flexible method than the rule-of-thumb estimator in the last subsubsection is least squares CV (LSCV). No distributional assumption about $X$ has to be made. Therefore, LSCV as a method to select $h_{opt}$ is in accordance with the nonparametric philosophy. LSCV uses the integrated squared error (ISE) as error measure:
%
%\begin{equation}
%\text{ISE}[\hat{f}_h] = \int \left(\hat{f_h}(x) - f(x) \right)^2 dx.
%\label{Eq:def_ise_kde}
%\end{equation}
%
%\noindent Then, the optimal bandwidth is found by minimizing the ISE of $\hat{f_h}$
%
%\begin{equation}
%h_\text{\tiny CV} =  \underset{h > 0}{\mathrm{argmin}} \ \text{ISE}[\hat{f}_h]. 
%\label{Eq:min_ise_kde}
%\end{equation}
%
%\noindent Rewriting (\ref{Eq:def_ise_kde}) results in 
%
%\begin{equation}
%\text{ISE}[\hat{f}_h] = \int \hat{f_h}(x)^2 dx -2\int \hat{f_h}(x)f(x)dx + \int f(x)^2 dx.
%\label{Eq:ise_kde_re}
%\end{equation}
%
%\noindent Since (\ref{Eq:min_ise_kde}) is minimized over $h$ and the last term in (\ref{Eq:ise_kde_re}) does not depend on $h$ it can be neglected. The second term of (\ref{Eq:ise_kde_re}) is the expected value of $\hat{f_h}(x)$. It can be derived based on another independent observation coming from $X$. \cite{Hardle.1991} suggests to estimate $\mathbb{E}[\hat{f_h}(X)]$ with the so-called leave-one-out estimator:
%
%\begin{equation}
%\mathbb{E}[\hat{f}_h(X)] = \dfrac{1}{n}\sum_{i = 1}^{n} \hat{f}_{h,i}(X_i)
%\label{Eq:exp_kde_cv}
%\end{equation}
%
%\noindent where
%
%\begin{equation}
%\hat{f}_{h,i}(X) = \dfrac{1}{(n-1)h} \sum_{\substack{j=1 \\ j\neq i}}^{n} K\left(\dfrac{X - X_j}{h}\right).
%\label{Eq: kde_loue}
%\end{equation}
%
%\noindent For estimating the first term of (\ref{Eq:ise_kde_re})  directly from the data, denote $K*K(X)$ as convolution of $K$ and obtain:
%
%\begin{equation}
%\int \hat{f_h^2} dx = \dfrac{1}{n^2 h} \sum_{i=1}^{n} \sum_{j=1}^{n} K*K\left( \dfrac{X_j - X_i}{h} \right).
%\label{Eq:kde_sq_conv}
%\end{equation}
% 
%\noindent Plugging (\ref{Eq:exp_kde_cv}), (\ref{Eq: kde_loue}) and (\ref{Eq:kde_sq_conv}) into (\ref{Eq:ise_kde_re}) gives the CV criterion
%
%\begin{equation}
%\text{CV}(h) = \dfrac{1}{n^2 h} \sum_{i=1}^{n} \sum_{j=1}^{n} K*K\left( \dfrac{X_j - X_i}{h} \right) - \dfrac{2}{(n-1)nh} \sum_{i = 1}^n \sum_{\substack{j=1 \\ j\neq i}}^{n} K\left(\dfrac{X_i - X_j}{h}\right).
%\end{equation}
%
%\noindent Therefore, the optimal bandwidth with respect to LSCV $h_{\text{\tiny CV}}$ is obtained as
%
%\begin{equation}
%h_{\text{\tiny CV}} =  \underset{h > 0}{\mathrm{argmin}} \ \text{CV}(h). 
%\label{Eq:min_cv_kde}
% \end{equation}
%
%\noindent With (\ref{Eq:min_cv_kde}) the bandwidth can be determined without any distributional assumption. Unlike the rule-of-thumb method in the last subsubsection, the LSCV bandwidth also adapts to the smoothness of $f(x)$. Moreover, \cite{Stone.1984} proved that if $f$ is bounded, $h_\text{\tiny CV}$ is asymptotically optimal in the sense that $\text{ISE}[h_\text{\tiny CV}]$ converges almost surely (a.s.) to $\underset{h > 0}{\min}\ \text{ISE}[h]$:
%\begin{equation}
%\dfrac{\text{ISE}[h_\text{\tiny CV}]}{\underset{h > 0}{\min} \ \text{ISE}[h]} \xrightarrow{a.s.} 1.
%\end{equation}
%\newline
%\noindent A disadvantage of the LSCV estimator is its computational complexity. \cite{Hardle.1991} notes that the number of computational steps to solve (\ref{Eq:min_cv_kde}) is of order $\mathcal{O}(mn^2)$ for $m$ denoting the number of candidate bandwidths. Thus, the number of computational steps increases quadratically in $n$.
%
%
%\subsubsection{Other Bandwidth Estimators}
%
%Another approach that \cite{Hardle.2004} refer to as one of the most popular are refined plug-in-methods. They are similar to the first presented method. However, instead of referencing to a distribution, $\|f\|_2^2$ is estimated nonparametrically as well. Despite relying on bandwidth selectors introduced in Section \ref{Sec:kde_hopt_ref} for estimating $\|f\|_2^2$, refined plug-in-methods deliver good estimates in simulations. \\
%
%\noindent Two other methods presented by \cite{Silverman.1986} are likelihood CV and the test graph method. Likelihood CV is based on computing $\log\left(\widehat{f}_h(x)\right)$ for all observations as leave-one-out estimate. Then, $h_{opt}$ corresponds to the value that maximizes the CV based likelihood criterion. However, likelihood CV is sensitive to outliers and results in inconsistent estimates for most standard densities. Thus, it is suggested to use LSCV to reduce the range for $h$ before likelihood CV is applied. The test graph method is constructed such that estimates are uniformly close to the true density. In doing so, $h_{opt}$ minimizes the maximum estimation error. However, due to the involved subjectivity it is suggested to use the test graph method as check for other estimators and not as single selection method. \\
%
%\noindent Another possible choice is the biased CV estimator proposed by \cite{Hall.1991}. It converges asymptotically with a rate of $\sqrt{n}$ to $h_{opt}$. However, studies showed its inferiority to other methods for small samples. Consequently, for most bandwidth selectors exist advantages and disadvantages and none of them has advantages only. As a result, \cite{Hardle.2004} draws the conclusion that there is no best method. Hence, estimates based on different methods should be compared to select the best one. %The final solution depends, therefore, still on a certain degree of subjectivity. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Choosing the Kernel Function}

%\subsubsection{The Asymptotically Optimal Kernel Function}
%
%Kernel functions can be compared based on their asymptotic approximation quality  by decomposing the AMISE. First, rewrite the optimal bandwidth that was derived by differentiating the AMISE in (\ref{Eq:kde_hopt}):
%
%\begin{align}
%h_{opt}^K &= \left(\dfrac{||K||_2^2 }{n\mu_2(K)^2 ||f''||^2_2} \right)^{1/5} \\
%&=  \underbrace{\left(\dfrac{||K||_2^2 }{\mu_2(K)^2} \right)^{1/5}}_\text{$=:\upsilon_K$} \underbrace{\left(\dfrac{1}{n||f''||^2_2} \right)^{1/5}}_\text{$=:\gamma_{f,n}$} \\
%&= \upsilon_K \gamma_{f,n}. \label{Eq:kde_hopt_re}
%\end{align}
%
%\noindent The first part of (\ref{Eq:kde_hopt_re}), $\upsilon_K$, depends on $K$ whereas the second part, $\gamma_{f,n}$, is independent of $K$. In the next step (\ref{Eq:kde_hopt_re}) is plugged into (\ref{Eq:kde_amise}) in order to decompose the AMISE into one part depending on $K$ and one not depending on $K$. This yields 
%
%\begin{align}
%\text{AMISE}[\hat{f}_{h_{opt}^K}] &= \dfrac{1}{nh_{opt}^K} ||K||_2^2  + \dfrac{(h_{opt}^K)^4}{4} \mu_2(K)^2 ||f''||^2_2 \\
%&= \dfrac{1}{n\upsilon_k \gamma_{f,n}} ||K||_2^2  + \dfrac{(\upsilon_k \gamma_{f,n})^4}{4} \mu_2(K)^2 ||f''||^2_2 \\
%&= \dfrac{1}{n\gamma_{f,n}} \dfrac{||K||_2^2  }{\upsilon_k}+ \dfrac{ \gamma_{f,n}^4}{4} ||f''||^2_2 \upsilon_k^4\mu_2(K)^2. \label{Eq:kde_amise_decom_p1}
%\end{align} 
%
%\noindent With 
%
%\begin{equation}
%\upsilon_K = \left(\dfrac{||K||_2^2 }{\mu_2(K)^2} \right)^{1/5}
%\end{equation}
%
%\noindent equation (\ref{Eq:kde_amise_decom_p1}) becomes 
%
%\begin{align}
%\text{AMISE}[\hat{f}_{h_{opt}^K}] &= \dfrac{1}{n\gamma_{f,n}} ||K||_2^{8/5}\mu_2(K)^{2/5}  + \dfrac{ \gamma_{f,n}^4}{4} ||f''||^2_2 ||K||_2^{8/5}\mu_2(K)^{2/5}  \\
%&= \left( \dfrac{1}{n\gamma_{f,n}} + \dfrac{\gamma_{f,n}^4}{4} ||f''||^2_2 \right) \underbrace{\left(||K||_2^8 \mu_2(K)^2 \right)^{\frac{1}{5}}}_\text{$=:T(K)$} \\
%&= \left( \dfrac{1}{n\gamma_{f,n}} + \dfrac{\gamma_{f,n}^4}{4} ||f''||^2_2 \right) T(K). \label{Eq:kde_amise_decom_p2}
%\end{align}
%
%\noindent $T(K)$ denotes the AMISE part depending on $K$ in (\ref{Eq:kde_amise_decom_p2}). Hence, the optimal kernel can be found by minimizing $T(K)$. The Epanechnikov kernel $K_{Epa}$ is derived by \cite{Epanechnikov.1969}. It can be shown that $K_{Epa}$ minimizes $T(K)$ if only nonnegative kernels with compact support are considered. The efficiency of different kernel functions is presented in Table \ref{Tab:kernel_efficency}. Moreover, the relative deviation of these kernels to $K_{Epa}$ is presented. \citet[p. 61]{Hardle.2004} suggest that from a practical point of view \textit{"the choice of the kernel function is almost irrelevant for the efficiency of the estimate"}. This conclusion is based on the small relative deviations of the other kernel functions from $T(K_{Epa})$. However, it can be argued that even though the deviations are small, $K_{Epa}$ is the most efficient kernel function and should therefore be favored over the others.
%
%\begin{table}[H]
%	\begin{center}
%		\begin{tabular}{c|c|c}
%			\hline \hline
%			\textbf{Kernel} & $\mathbf{T(K)}$ &  $\mathbf{T(K)/T(K_{Epa})}$ \\
%			\hline
%			Uniform & 0.3701  & 1.0602 \\ 
%			\hline
%			Triangel & 0.3531  & 1.0114  \\ 
%			\hline
%			Epanechnikov & 0.3491 & 1.0000  \\ 
%			\hline
%			Quartic/Biweight & 0.3507  & 1.0049 \\ 
%			\hline
%			Triweight & 0.3699 & 1.0595  \\
%			\hline
%			Gaussian & 0.3633 & 1.0408 \\
%			\hline
%			Cosine & 0.3494 & 1.0004  \\
%			\hline \hline
%		\end{tabular}
%	\end{center}
%	\caption[Kernel efficiency in kernel density estimation]{Efficiency of different kernel functions compared to the most efficient kernel, i.e. the Epanechnikov kernel. Source: \cite{Hardle.2004}.}
%	\label{Tab:kernel_efficency}	
%\end{table}

%\subsubsection{Asymptotic Normality of a Kernel Density Estimate}
%
%\cite{Parzen.1962} proved that the kernel density estimator is asymptotically normally distributed. By assuming $nh \to \infty$ and $h^2 \sqrt{nh} \to 0$ as in \cite{Pagan.1999} one obtains
%
%\begin{equation}
%\sqrt{hn} \left( \hat{f_h}(x) - f(x) \right) \xrightarrow{d}  N \left(0, f(x) ||K||_2^2 \right). 
%\end{equation}
%
%\noindent Let $\alpha \in [0,1]$ and $z_{\alpha} = \Phi^{-1}(\alpha)$ where $\Phi$ denotes the cumulative distribution function of the standard normal distribution. Then, the confidence interval ($CI^{\alpha}$) capturing $\alpha$100\% around $f(x)$ is 
%
%\begin{align}
%\left[f(x) -  z_{1 - \frac{\alpha}{2}} \left(\dfrac{||K||_2^2 f(x)}{nh}\right)^{1/2}, \ f(x) +  z_{1 - \frac{\alpha}{2}} \left(\dfrac{||K||_2^2 f(x)}{nh}\right)^{1/2} \right].
%\end{align}
%
%\noindent Since $f(x)$ is unknown, it is replaced by the KDE $\hat{f_h}(x)$
%
%\begin{align}
%\left[\hat{f_h}(x) -  z_{1 - \frac{\alpha}{2}} \left(\dfrac{||K||_2^2  \hat{f_h}(x)}{nh}\right)^{1/2}, \ \hat{f_h}(x) +  z_{1 - \frac{\alpha}{2}}  \left(\dfrac{||K||_2^2 \hat{f_h}(x)}{nh}\right)^{1/2} \right].
%\label{Eq:kde_conf_int}
%\end{align}
%
%\noindent CIs provide an uncertainty measure for $f(x)$. However, if the use of KDE is motivated by finding an appropriate parametric approximation for the observed data, an uncertainty measure for $f$ as a whole should be used. Confidence bands are the appropriate statistical tool in such situations. However, this goes beyond this work and it is instead referred to \cite{Hardle.2004} where an approach for determining confidence bands is presented. 

%\subsubsection{KDE Based Quantile Estimator}

The KDE based quantile estimator to forecast VaR can be derived as follows. First, the  estimator for $F(x)$ that is based on KDE needs to be derived. Denote $\widehat{F}_h(x)$ as the KDE based estimate of $F(x)$. Then, $\widehat{F}_h(x)$ can be derived as follows:

\begin{align}
\widehat{F}_h(x) &= \int_{-\infty}^{x} \hat{f}_h(z)dz \\
&= \int_{-\infty}^{x} \dfrac{1}{nh} \sum_{i = 1}^{n} K\left(\dfrac{z - x_i}{h}\right)dz \\
&= \dfrac{1}{nh} \sum_{i = 1}^{n} \int_{-\infty}^{x}  K\left(\dfrac{z - x_i}{h}\right)dz.
\end{align} 

\noindent Since the given kernel function $K$ is a density, let $\Gamma$ denote the corresponding CDF. Moreover, using the substitution $u = (z - x_i)/h$ one obtains

\begin{align}
\widehat{F}_h(x) &= \dfrac{1}{n} \sum_{i = 1}^{n} \int_{-\infty}^{\frac{x - x_i}{h}}  K\left(u\right)du \\ 
 &= \dfrac{1}{n} \sum_{i = 1}^{n} \Gamma \left( \dfrac{x - x_i}{h} \right).
 \label{Eq:kde_cdf_est}
\end{align} 

\noindent Thus, $\widehat{F}_h(x)$ is the mean of the CDF corresponding to $K$ evaluated at $(x-x_i)/h$ for $i = 1, \dots, n$. Then, for $\alpha  \in (0,1)$ the KDE based quantile function $\widehat{Q}_h$ is obtained as

\begin{equation}
	\widehat{Q}_h(\alpha) = \widehat{F}_h^{-1}(x).
\end{equation}

%\noindent However, it is not possible to obtain a closed form solution for every kernel function. For instance, in case the Gaussian kernel function is used, $\Gamma$ cannot be stated explicitly. Therefore, for the Gaussian kernel function, $\widehat{Q}_h(\alpha)$ is computed by numerically solving  
%
%\begin{equation}
%\widehat{Q}_h(\alpha) = \underset{x \in \mathbb{R}}{\mathrm{argmin}} \left| \dfrac{1}{n} \sum_{i = 1}^{n} \Phi \left( \dfrac{x - x_i}{h} \right) - \alpha \right|
%\label{Eq:kde_quantile_numerical}
%\end{equation}
%
%\noindent where $\Phi$ denotes the CDF of the standard normal distribution. Here, solving (\ref{Eq:kde_quantile_numerical}) corresponds to finding its root. Note, that this can be done with a reasonable speed because there exists an R function to compute $\Phi(u)$. 


==> Sections/lit_review.tex <==
\section{Literature Review}\label{Sec:Lit_Rev}

\cite{Kuester.2005} compare the performance of several classical statistical approaches for estimating VaR. Moreover, a comprehensive overview over existing statistical methods is given. Four categories are suggested to describe existing methods for VaR estimation. These categories are historical simulation, fully parametric models, extreme value theory and quantile regression. In the empirical study VaR models belonging to the location scale class are superior over other approaches. In the domain of ML the literature for quantile estimation focuses mainly on neural networks (NN) and SVR. For instance, the derivation of a general approach without an explicit target application can be found in \cite{White.1992}. He used single hidden layer feedforward NNs to derive a way for nonparametric conditional quantile estimation and proved its consistency. However, the ML VaR literature is not as broad as in classical statistics. 
Hence, this section also reviews literature where methods for the construction of prediction intervals (PI) were introduced that could be used in the estimation of VaR. Consequently, the reviewed literature is divided in three paragraphs: Prediction Intervals, Value-at-Risk and Data Driven Value-at-Risk. Here, the first two review the existing literature, whereas the last motivates the method proposed in this paper. 

\paragraph{Prediction Intervals} General approaches are developed by \cite{Hwang.1997} who derive asymptotically valid PIs and \cite{Veaux.1998} who propose a method to estimate PIs for NNs with nonlinear regression. \cite{LinWeng.2004} use SVR to generate out-of-sample residuals via cross validation (CV) and fit those to a Laplace or normal distribution for generating PIs. The results are compared to Bayesian SVR and historical simulation. Despite the mixed results they stress the competitiveness of their method especially due to its simplicity. Pointwise and simultaneous confidence intervals as well as PIs with bias correction for least-squares-SVR are derived by \cite{Brabanter.2011}.  %based on Sidak corrections and upcrossing allowing for heteroscedasticiy and modifying it because of its convervativity% - > 
%However, in comparison to bootstrapping, their method is not superior in simulations. \cite{Khosravi.2013} introduce a framework for constructing PIs of electricity prices. They employ a resampling scheme based on a moving bootstrap approach for data blocks rather than single observations to account for possible correlations. Then, NNs are trained on the bootstrapped data sets to forecast the mean of the time series as center of the prediction interval. The variance is estimated based on a GARCH model but not in the framework of MLE. Instead, they use a cost function directly related to the PI quality that can be minimized with gradient-free algorithms. The resulting mean and variance are then used in a normal distribution to get the PIs. They find that their method has a computational advantage over traditional methods. Moreover, the PIs of their approach are more informative. \cite{Lins.2015} propose a method for confidence intervals and PIs by combining bootstrapping and SVR to bagged SVR in the context of component degradation prediction in the offshore oil industry. They show that their method works in the proposed application.

\paragraph{Value-at-Risk} \cite{Franke.2006} estimate VaR for the German stock index (DAX) by fitting the mean and volatility of the return series with NNs. The mean is modeled autoregressively and the volatility is assumed to follow an autoregressive conditionally heteroscedastic (ARCH) process. Moreover, they include external regressors in both models. The predicted mean and variance are used with the normal distribution to derive the VaR and expected shortfall. As benchmark serves a standard GARCH model based on assuming normality of innovations. In terms of VaR exceedances their model is superior. Moreover, they note its ability to quickly adjust the volatility in case of shocks with only short impact. Another approach directly related to VaR is proposed by \cite{Dunis.2010} which use higher order NNs to forecast VaR. A hybrid model using higher order NNs for variance forecasting and RiskMetrics is shown to outperform other hybrid models empirically. They note also the relatively bad results of the unconditional POT method for quantile estimation. This is, however, not an appropriate comparison when benchmarked to conditional models as was e.g. shown by \cite{Kuester.2005}. \cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test. 
%A multiperiod VaR model was introduced by \cite{Xu.2016}. They use an exponentially weighted support vector quantile regression. In the corresponding empirical study, their approach outperforms other methods that are based on GARCH models, filtered historical simulation and quantile regression. Evaluation was done with different measures as e.g. mean absolute error and p-values of prediction tests.

\paragraph{Data Driven Value-at-Risk} Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. By considering the different model types presented in study of \cite{Kuester.2005}, they can be classified as quantile regression models. In the empirical study of  the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and peaks-over-threshold had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. Most of the proposed methods in the ML literature for estimating VaR or PIs are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this paper. Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions.



==> Sections/methods.tex <==
\section{Methodology} \label{Sec:meths}

\input{Sections/value_at_risk.tex}
\input{Sections/garch.tex}
\input{Sections/kde.tex}
\input{Sections/svrSL.tex}
\input{Sections/svrgarchkde.tex}



==> Sections/svr.tex <==
%\section{Support Vector Regression}\label{Sec:SVR}

%This section introduces regression based on support vector machines (SVM). Initially, the SVM algorithm was derived for classification. However, in this thesis the methodological focus lies on regression with SVMs. Hence, the SVM algorithm for classification is not covered. Instead, it is referred to \cite{Burges.1998} where a comprehensive and exemplified introduction of SVMs for classification is given. Generally, SVMs are embedded in the framework of statistical learning theory. Consequently, its fundamentals will be introduced in the following section that is based on \cite{Vapnik.1995,Vapnik.1998}. The second part of this section is concerned with SVR. 

%\subsection{Fundamentals of Statistical Learning Theory}
%\label{Sec:SVR_SLT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{The General Model}
%
%In \cite{Vapnik.1995} the framework for learning from data consists of three parts: a generator (G), supervisor (S) and learning machine (LM). G generates random input vectors $x \in \mathbb{R}^p$ that are i.i.d. with an unknown distribution function $F(x)$. Outputs $y$ which correspond to the input vectors $x$ are returned by S according to an unknown and fixed conditional distribution function $F(y|x)$. Although S is unknown, its existence is assumed. Additionally, S is also assumed to not change. Hence, the so-called training set with i.i.d. observations is obtained from G and S:
%\begin{equation}
%\{(y_i, x_i) | i = 1, \dots, n; \ n \in \mathbb{N}\}.
%\end{equation}  
%\noindent Then, the LM is concerned with finding a function to approximate the output of S based on the training set. Formally, for a parameter set $\Theta$, the LM learns the dependence between $x$ and $y$ by implementing a set of functions $g(x, \theta)$ with $\theta \in \Theta$. Consequently, the problem of how to determine $\theta \in \Theta$ for obtaining the best approximation of the supervisor's response needs to be solved. Solving this problem is the so-called learning process which can be described as follows: \textit{"The learning process is a process of choosing an appropriate function from a given set of functions."} \cite[p. 21]{Vapnik.1998}.
%
%%For a parameter set $\Theta$, the dependence between $x$ and $y$ is learned by a LM that implements a set of functions $g(x, \theta)$ with $\theta \in \Theta$. The function $g$ is determined by an i.i.d. training set $\{(y_i, x_i) | i = 1, \dots, l \in \mathbb{N}\}$ with the joint distribution $F(x,y) = F(x)F(y|x)$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Minimizing the Risk Functional}
%
%The LM is used to approximate the values $y$ returned by S. However, to find an appropriate approximation it is necessary to measure the discrepancy between $y$ and $g(x, \theta)$. In the terminology of \cite{Vapnik.1995, Vapnik.1998} this discrepancy is called loss. Hence, the so-called loss function $L(y, g(x, \theta))$ is introduced. Based on this, the risk functional $\mathcal{R}(\theta)$ which measures the expected loss and, therefore, the approximation's quality is defined as 
%
%\begin{equation}
%\mathcal{R}(\theta) = \int L(y, g(x, \theta)) dF(x,y).
%\label{Eq:risk_fct}
%\end{equation}
%
%\noindent Consequently, the optimal parameter $\theta_0 \in \Theta$ minimizes (\ref{Eq:risk_fct}):
%\begin{equation}
%\theta_{0} = \underset{\theta \in  \Theta}{\mathrm{argmin}} \ \mathcal{R}(\theta).
%\end{equation} 
%
%%Let $G = \{g(z) | z \in Z \subset \mathbb{R}^n \}$ be the set of admissible functions and $R(g(z))$ the function to measure the quality of the approximation. By constructing $R(g(z))$ so that its minimum corresponds the approximation with the highest quality, the optimal approximation $g(z)^* \in G$ is
%%\begin{equation}
%%g(x, \theta_{opt}) = \underset{g(x, \theta) \in \ G}{\mathrm{argmin}} \ R(g(x, \theta)).
%%\end{equation} 
%%
%%\noindent \cite{Vapnik.1995} defines $R(g(z))$ as the mathematical expectation: 
%%
%%\begin{equation}
%%R(\theta) = \int L(y, g(x, \theta)) dF((x,y)).
%%\label{risk_fct}
%%\end{equation}
%%
%%$R(\theta)$ is the so-called risk functional which is minimized by the function $g(x, \theta)$ that fits the training data best.
%
%\noindent Now, the problem arises of how to minimize (\ref{Eq:risk_fct}) with unknown $F(x,y)$. The only available information is contained in the training set. Thus, an approach based on the empirical data needs to be derived.
%%Direct minimization requires to find $g(x, \theta)$ whereas minimization with empirical data requires to state a construction criterion to choose the function. This follows from the unknownness of $F(x,y)$ whereby (\ref{Eq:risk_fct}) cannot be used as a selection criterion.   
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Empirical Risk Minimization Inductive Principle}
%     
%Since the joint distribution $F(x, y)$ is unknown, minimizing the risk functional in practice cannot be done analytically but relies on empirical data. For introducing a corresponding inductive principle, \cite{Vapnik.1995,Vapnik.1998} considers the general case of an i.i.d. sample $\{z_1, \dots, z_n\}$ coming from a random variable $Z$ with unknown probability measure $F(z)$. Further, a set of functions $P(z, \theta)$, $\theta \in \Theta$, is considered such that (\ref{Eq:risk_fct}) can be generalized to
%
%\begin{equation}
%\mathcal{R}(\theta) = \int P(z, \theta) dF(z).
%\label{Eq:risk_fct_general}
%\end{equation}
%  
%\noindent In terms of (\ref{Eq:risk_fct}), $P(z, \theta)$ represents the loss function and $z$ some values $(y,x)$. Then, instead of minimizing $\mathcal{R}(\theta)$ the corresponding explicitly defined empirical risk functional can be minimized: 
%
%\begin{equation}
%\mathcal{R}_{emp}(\theta) = \frac{1}{n}\sum_{i = 1}^{n} P(z_i, \theta).
%\end{equation}
%
%\noindent In addition to defining the empirical risk functional, denote $\theta_0$ and $\theta_{train}$ as the parameter vectors minimizing $\mathcal{R}(\theta)$ and $\mathcal{R}_{emp}(\theta)$, respectively. Then, minimizing $\mathcal{R}_{emp}(\theta)$ corresponds to approximating $P(z, \theta_0)$ with $P(z, \theta_{train})$. In summary, the core of the Empirical Risk Minimization (ERM) inductive principle is replacing $\mathcal{R}(\theta)$ with $\mathcal{R}_{emp}(\theta)$ and approximating $P(z, \theta_0)$ with $P(z, \theta_{train})$. \\
%
%\noindent The ERM principle is a central point in statistical learning theory because appropriate conditions must be found in order to approximate $P(z, \theta_0)$ closely. Moreover, \cite{Vapnik.1998} shows that classical methods as least squares regression and maximum likelihood based density estimation are covered by the ERM inductive principle. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Structural Risk Minimization Inductive Principle}
%
%The goal of the ERM inductive principle is to minimize the empirical risk. However, this is done without considering the complexity of the function that fits the training set best. Large sample sizes ensure that the ERM inductive principle is appropriate for minimizing risk. This is due to the fact that the empirical risk will be close to the actual risk. Hence, low empirical risk will be observed if the actual risk is low as well. However, in case of a small sample size overfitting might occur, i.e. the empirical risk is low even though the actual risk is not. Complex functions are able to perfectly fit the training data. However, while the empirical risk is minimized, their generalization ability can be bad in out-of-sample predictions. The Structural Risk Minimization (SRM) inductive principle is a way to overcome the above mentioned problems. The core of the SRM inductive principle is an error bound on the actual risk. This bound depends on the empirical risk and the complexity of the function.   \\ 
%
%
%%\cite{Vapnik.1995,Vapnik.1998} concludes this from a bound he derived for the actual risk functional (\ref{Eq:risk_fct}). This bound is the sum of the empirical risk and a confidence interval which depends on the so-called capacity of a function. \\
%
%\noindent For deriving the SRM inductive principle it is necessary to show how the complexity of a function can be measured. In doing so, the terminology of \cite{Vapnik.1995,Vapnik.1998} is used where capacity is used as synonym for complexity. Capacity in the considered bound is measured as Vapnik-Chervonenkis (VC) dimension $h$. Intuitively, in case of a classification problem, the VC dimension measures how many vectors can be classified correctly. For instance, \cite{Vapnik.1995} demonstrates that for a set of linear indicator functions with $p$ attributes the VC dimension is $h = p + 1$. The intuition behind this result is that at most $p + 1$ data points can be classified correctly. Figure~\ref{vc_dim_example} depicts the case of three random vectors coming from $\mathbb{R}^2$. Here, $p = 2$ and the VC dimension is consequently $h = 3$. Hence, all possible label assignments ($2^3 = 8$) of the three vectors can be perfectly classified. However, this does not hold for four vectors as is indicated in Figure~\ref{Fig:vc_dim_example}. Assume the labels of $z_2$ and $z_4$ are equal and different from $z_1$ and $z_3$. Then, there is no line that can separate $z_2$ and $z_4$ from $z_1$ and $z_3$. Thus, no perfect classification is possible using linear decision functions. \\
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale = 0.39]{Figures/vc_dim_burges}
%	\caption[VC dimension for three points in $\mathbb{R}^2$]{Shattering three points in $\mathbb{R}^2$ in case of linear indicator functions. The color of the point indicates the class. A perfect classifier can be found for all eight possible label assignments. Source: \cite{Burges.1998}.}
%	\label{vc_dim_example}
%\end{figure}
%  \begin{figure}[H]
% 	\centering
% 	\includegraphics[scale = 0.39]{Figures/vc_dim_vapnik}
% 	\caption[VC dimension for four points in $\mathbb{R}^2$]{Separating four points in $\mathbb{R}^2$ is not possible for all possible labels with linear decision functions. Source: \cite{Vapnik.1995}.}
% 	\label{Fig:vc_dim_example}
% \end{figure}
% 
%% \clearpage
% 
% \noindent To formally introduce the VC dimension consider the following definitions for indicator and real functions taken from \citet[p. 76-77]{Vapnik.1995}. 
%
%% In contrast, small sample sizes correspond usually to a small $l/h$. Consequently, low empirical risk does not necessarily imply low actual risk. Such cases can be accommodated by indtroducing the  \textit{Structural Risk Minimization} (SRM) inductive principle. The SRM inductive principle accounts in minimizing the risk functional for the empirical risk and the confidence interval. 
%%
%%Define S as a set of functions that consists of nested subsets of functions $S_k = \{P(z, \theta \in \Theta_k)\}$ with $S_1 \subset S_2 \subset \dots \subset S_n \dots$. The structure of $S$ is an \textit{admissible structure} if it has the properties stated in \cite[p.~90-91]{Vapnik.1995}. The ERM inductive principle was characterized by choosing the function $P(z, \theta_{train}$) which minimizes the empirical risk. In contrast, the SRM inductive principle takes the training error and complexity of $P(z, \theta_{train}$) into account. This is done by choosing the function from the subset $S_n$ where the empirical risk and error bound on the actual risk is minimized. 
%%
%%The error bounds were derived by CORTES AND VAPNIK and depend on the empirical risk and a confidence interval $\Psi$. $\Psi$ grows monotonically with the complexity $h_k$ of $S_k$. VAPNIK introduced the term \textit{capacity} to describe the complexity of a function. The so-called Vapnik-Chervonenkis (VC) dimension $h$ is a measure for the capacity of a function class. In \cite{Vapnik.1995}, the VC dimension for a set indicator and real functions is defined as follows.  
%\newtheorem{mydef}{Definition}
%\begin{mydef}
%	\textbf{The VC dimension of a set of indicator functions} 
%	
%	The VC dimension of a set of indicator functions $P(z, \theta)$, $\theta \in \Theta$, is the maximum number $h$ of vectors $z_1, \dots, z_n$ that can be separated into two classes in all $2^h$ possible ways using functions of the set (i.e., the maximum number of vectors that can be shattered by the set of functions). If for any $n$ there exists a set of $n$ vectors which can be shattered by the set $P(z, \theta)$, $\theta \in \Theta$, then the VC dimension is equal to infinity.
%
%\end{mydef}
%
%\begin{mydef}
%		
%	\textbf{The VC dimension of a set of real functions}
%	
%	Let $A \le P(z, \theta) \le B$, $\theta \in \Theta$, be a set of real functions bounded by constants $A$ and $B$ ($A$ can be $-\infty$ and $B$ can be $\infty$). Let us consider along with the set of real functions $P(z, \theta)$, $\theta \in \Theta$, the set of indicators
%	
%	\begin{equation}
%	\mathscr{I}(z, \theta, \beta) = \mathbb{I}(P(z,\theta)- \beta), \ \theta \in \Theta, \ \beta \in (A,B),
%	\end{equation}
%	
%	\noindent where $\mathbb{I}(z)$ is the step function
%	
%	\begin{equation}
%	\mathbb{I}(z) = \begin{cases}
%	0 \text{ \ if \ } z < 0 \\
%	1 \text{ \ if \ } z \ge 0. \\
%	\end{cases}
%	\end{equation}
%		
%	\noindent The VC dimension of a set of real functions $P(z,\theta)$, $\theta \in \Theta$, is defined to be the VC dimension of the set of corresponding indicators with parameters $\theta \in \Theta$ and $\beta \in (A,B)$.
%	
%\end{mydef}
%
%\noindent One should note that the VC dimension of a set of functions is not equal to the number of free parameters in the functions. \citet[p. 65]{Vapnik.1995} states that \textit{"constructive distribution-independent bounds"} can be obtained by using the VC dimension $h$ as a capacity measure for a set of functions. \\
%
%\noindent To obtain bounds for the actual risk let $S = \{P(z, \theta)| \ \theta \in \Theta\}$ be a set of functions with a structure such that $S$ consists of nested subsets of functions $S_m = \{P(z, \theta| \ \theta \in \Theta_m)\}$. \citet[p.~90-91]{Vapnik.1995} states conditions under which $S$ has an admissible structure. Consequently, in the following is assumed that $S$ fulfills these conditions. Then, a learning machine's generalization ability can be controlled by the corresponding risk bounds. In general, the bound on the actual risk for functions in $S_m$ is with probability $(1-\eta)$
%
%\begin{equation}
%\mathcal{R}(\theta_{train}^m) \le \mathcal{R}_{emp}(\theta_{train}^m) + B_m E_m(n) \left(1 + \sqrt{1 + \dfrac{4 \mathcal{R}_{emp}(\theta_{train}^m)}{B_m E_m(n)}} \right)
%\label{Eq:guaranteed_risk}
%\end{equation}
%
%\noindent with 
%
%\begin{equation}
%E_m(n) = \dfrac{4 h_m \left( \log \dfrac{2n}{h_m} + 1\right) - \log \dfrac{\eta}{4}}{n},
%\end{equation}
%
%\noindent where $h_m$ is the VC dimension, $B_m $ the upper bound for the functions in $S_m$ with $B_m \ge 0 $ and 
%\begin{equation}
%\sup \dfrac{ \sqrt[v]{ \mathbb{E}[P^v(z,\theta)] } }{ \mathbb{E}[P(z,\theta)] }  \le \tau_m < \infty.
%\end{equation}
%
%\noindent  Moreover, $h_m$, $B_m$ and $\tau_m$ are non-decreasing series:
%\begin{align}
%&h_1 \le h_2 \le \dots \le h_m \le \dots \label{Eq:kappa_nond} \\
%&B_1 \le B_2 \le \dots \le B_m \le \dots \\
%&\tau_1 \le \tau_2 \le \dots \le \tau_m \le \dots .
%\end{align}
%
%\noindent The ERM inductive principle was characterized by choosing the function $P(z, \theta_{train}$) which minimizes the empirical risk. In contrast, the SRM inductive principle takes the training error and complexity of $P(z, \theta_{train})$ into account. This is done by choosing the set of functions $S_m$ that minimizes the bound of the actual risk on the right hand side of (\ref{Eq:guaranteed_risk}). The term that is added to the empirical risk in (\ref{Eq:guaranteed_risk}) is called confidence interval. The confidence interval measures the complexity of a set of functions relative to the number of training instances. Figure~\ref{Fig:srm_fig} demonstrates the motivation behind the SRM inductive principle. In balancing out the trade-off between function capacity and empirical risk minimization, an appropriate nested subset of functions $S^*$ in $S$ is obtained to control possible over- and underfitting. Moreover, one can see that the capacity gets lower the deeper a set $S_m$ is nested in $S$. This follows from (\ref{Eq:kappa_nond}). Consequently, $S_1$ contains the functions with the lowest capacity.    
%\begin{figure}[H]
%	\centering
%	\includegraphics[scale = 0.5]{Figures/SRM_Figure}
%	\caption[Illustration of the SRM inductive principle]{Illustration of the SRM inductive principle. The sum of empirical risk and confidence interval is equal to the bound on the actual risk. The SRM inductive principle aims at finding a compromise between empirical risk minimization and function capacity for a given training set. Source: \cite{Vapnik.1995}.}
%	\label{Fig:srm_fig}
%\end{figure}
%
%%\subsubsection{Minimizing the Guaranteed Risk}
%
%%\noindent Thus, constructing a learning machine on the basis of the SRM inductive principle requires minimizing the guaranteed risk. The second term of the right hand side of (\ref{Eq:guaranteed_risk}) can be rewritten as a function $\Psi$ depending on the ratio $l/h_k$. So, rewriting (\ref{Eq:guaranteed_risk}) results in 
%%
%%\begin{equation}
%%R(\theta_{train}^k) \le R_{emp}(\theta_{train}^k) + \Psi (\dfrac{l}{h_k}).
%%\label{guaranteed_risk_simple}
%%\end{equation}
%
%%\noindent Based on (\ref{guaranteed_risk_simple}) \cite{Vapnik.1995} suggests two ways for minimizing the guaranteed risk: 
%
%%\begin{enumerate}
%%
%%\item Fix $\Psi (l/h_k)$ by choosing an appropriate $S_k$ and minimize $R_{emp}(\theta_{train}^k)$.
%%
%%\item Fix $R_{emp}(\theta_{train}^k)$ and minimize $\Psi (l/h_k)$.
%%
%%\end{enumerate}
%%
%%\noindent Neural Networks are an example for the first and Support Vector machines for the second approach. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Classification with Support Vector Machines} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Support Vector Regression}
SVR can be understood as a learning method to solve nonlinear regression tasks  \cite[e.g.,][]{Smola.2004}. It shares some similarities with a three-layer feed-forward neural network and is able to approximate arbitrarily complex functions (i.e., universal approximator) \citep{Chen.2009}. 
%\cite{Chen.2009} describe SVMs as feedforward NNs with one input, single hidden and output layer where the regression function is obtained via quadratic programming. In the hidden layer, the information of the input layer is mapped into a high-dimensional space to capture nonlinearities. As a consequence, SVMs can learn any nonlinear relationship if the dimension of the hidden space is high enough. The algorithm for doing regression with SVMs is introduced in this section. If not indicated otherwise, the derivations are based on the work of \cite{Smola.2004}. 
To describe the SVR model, 
%\subsubsection{Support Vector Regression and Dual Optimization}

let $\{(y_i, x_i)| i = 1,\dots, n; \ n\in \mathbb{N}\}$ with $x_i \in \mathbb{R}^p$ and $y_i \in \mathbb{R}$ denote the training data set. Suppose $f$ is a linear function such that 

\begin{equation}
f(x) = \omega^T x + b
\label{Eq:svr_lin_base_mdl}
\end{equation}

\noindent where  $\omega \in \mathbb{R}^p$ and $b \in \mathbb{R}$. Then, SVR aims to find an approximation of $f$ that deviates at most by $\epsilon$ from the observed target $y$ while being as flat as possible (i.e., in the sense that weights in $\omega$ are small). This translates into the following convex optimization problem:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 \\
& \text{subject to} & & \begin{cases}
y_i - \omega^T x_i - b \le \epsilon  \\
\omega^T x_i + b - y_i \le \epsilon.
\end{cases} 
\end{aligned}
\label{svm_mean_eq}
\end{equation}
\newline

In view that (\ref{svm_mean_eq}) might lack a feasible solution, \cite{Vapnik.1995} introduces an $\epsilon$-insensitive loss function: 

\begin{equation}
L_{\epsilon}(y - f(x))  = \begin{cases}
0 \qquad \qquad \qquad  \text{if} \ |y - f(x)| \le \epsilon \\
|y - f(x)| - \epsilon \ \ \text{otherwise}.
\end{cases}
\label{Eq:svr_alt_loss_fct}
\end{equation}

\noindent To measure empirical loss (and thus model fit) using (\ref{Eq:svr_alt_loss_fct}) \cite{Vapnik.1995} reformulates (\ref{svm_mean_eq}) using slack variables $\zeta$ and $\zeta^{*}$ that capture losses above and below the $\epsilon$-tube around $f(x)$, respectively. Figure~\ref{loss_fct} depicts this approach. Only points outside the gray shaded $\epsilon$-tube contribute linearly to the loss function. \\ 

%\cite{Vapnik.1995} integrated this type of loss function by using slack variables $\zeta_i$ and $\zeta^{*}_{i}$ in the optimization problem.
%
%To account for possibly infeasible constrains, SVR is defined with respect to a so-called $\epsilon$-insensitive loss function. \cite{Vapnik.1995} integrated this type of loss function by using slack variables $\zeta_i$ and $\zeta^{*}_{i}$ in the optimization problem. Based on this, the $\epsilon$-insensitive loss function $|\zeta|_\epsilon $ can be defined as

%\begin{equation}
%|\zeta|_\epsilon =: \begin{cases} 
%0 \text{  if   } |\zeta| \le \epsilon  \\
%|\zeta| - \epsilon \text{    otherwise}
%\end{cases}
%\label{Eq:slack_loss}
%\end{equation}


%\noindent It can be interpreted as tolerance measure for absolute errors that are greater than $\epsilon$. Based on this, \cite{Vapnik.1995} integrated slack variables $\zeta_i$ and $\zeta^{*}_{i}$ in the optimization problem.

\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.4]{Figures/svm_loss_fct_correct}
	\caption[The $\epsilon$-insensitive loss function]{The $\epsilon$-insensitive loss function of the SVR algorithm. Slack variable $\zeta$ captures the loss above the $\epsilon$-tube. Points within the grey shaded area have no impact on the loss. In contrast, all other observations contribute linearly to the loss. Source: \cite{Smola.2004}.}
	\label{loss_fct}
\end{figure}


Integrating the slack variables $\zeta$ and $\zeta^*$ into (\ref{svm_mean_eq}), the task to estimate a SVR model is equivalent to solving:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 + C\sum_{i = 1}^{n}(\zeta_i + \zeta^{*}_i) \\
& \text{subject to} & &  \begin{cases}
y_i - \omega^T x_i - b \le \epsilon + \zeta_i \\
\omega^T x_i + b - y_i \le \epsilon + \zeta_i^{*} \\
\zeta_i, \zeta_i^{*} \ge 0.
\end{cases} 
\end{aligned}
\label{svr_opt_fct}
\end{equation}
\newline

where $C > 0$ is a regularization parameter to balance between model fit and complexity \citep[e.g.,][]{Hastie.2009}. Larger (smaller) values of $C$ put more (less) weight on maximizing model fit during SVR learning. 
 
To capture nonlinear relationships between covariates and the response variable, SVR maps the input data into a higher dimensional feature space. The linear regression is then constructed in the transformed space, which corresponds to a nonlinear regression in the input space. The transformation is feasible from a computational point of view because SVR calculates the mapping implicitly using a kernel function 
$k(x_i^T x)=\Theta(x^T) \Theta(x)$. To implement this approach, it is common practice to estimate a SVR model through solving the dual of (\ref{svr_opt_fct}), which is given as \citep[e.g.,][]{Smola.2004}:

\begin{equation}
\begin{aligned}
& \text{maximize} 
	-\dfrac{1}{2} \sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)x_i^T x_j 
	-\epsilon\sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n}y_i(\rho_i - \rho_i^*)
 \\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
	\rho_i, \rho_i^* \in [0, C].
	\end{cases}
\end{aligned}
\label{dual_lin_opt}
\end{equation}
\newline

The dual program (\ref{dual_lin_opt}) includes the input data only in the form of scalar products $x_i^T x_j$. Replacing the scalar product by means of a kernel function is thus straightforward and does not affect the solver. In this work, we employ the Gaussian radial basis function (RBF) kernel (\ref{rbf_kernel}) because it includes other kernels as special cases, posses numerical advantages compared to alternatives, and often performs well in practical applications \citep{Keerthi.2003}.  

\begin{equation}
\begin{aligned}
k(x_i^T x)= \exp \left(\dfrac{\| x - x_i \|}{2 \gamma^2} \right)
\end{aligned}
\label{rbf_kernel}
\end{equation}
\newline



%######### SL####################################################################

among covariats and between 
It is common practice to estimate a SVR model through solving the dual of (\ref{svr_opt_fct}). In addition to computational advantages, an important feature of the dual is that the input data appears only in the form of scalar products $x_i^T x_j$. Replacing the scalar product with kernel function, which calculates the scalar product in a nonlinearly transformed feature space of higher dimension directly in the input space, enables SVR to account for nonlinear relationships. 


That is, forming the Langrangian (\ref{svr_opt_fct}) of An important  \citep[e.g.,][]{Smola.2004}. 
 
\iffalse

\noindent Solving (\ref{svr_opt_fct}) is usually easier by using its dual formulation. % which is moreover the central point in the estimation of nonlinear functions by SVR.
 This can be done by setting up the corresponding Lagrange function. The reason behind this is that it can be shown that the Lagrange function has a saddle point at the solution of an optimization problem with inequalities as constraints.
Let $ \rho $, $ \rho^* $, $ \eta $ and $ \eta^*$ be Lagrange multipliers which are consequently non-negative. Then, for SVR the corresponding Lagrange function is

\begin{equation}
\begin{aligned}
L(\omega, C, \zeta, \zeta^*, \rho, \rho^*, \eta, \eta^*) = & \frac{1}{2}\|\omega\|^2 + C\sum_{i=1}^{n}(\zeta_i + \zeta_i^*) \\
& - \sum_{i=1}^{n}(\eta_i\zeta_i + \eta_i^*\zeta_i^*) \\
& - \sum_{i=1}^{n}\rho_i(\epsilon + \zeta_i - y_i + \omega^Tx_i + b) \\
& - \sum_{i=1}^{n}\rho_i^*(\epsilon + \zeta_i^* + y_i - \omega^Tx_i - b).
\end{aligned}
\label{Eq:lagrange_lin_svr}
\end{equation}
\newline
\noindent The solution of the optimization problem (\ref{svr_opt_fct}) is at the saddle point of (\ref{Eq:lagrange_lin_svr}). Hence, for the partial derivatives of (\ref{Eq:lagrange_lin_svr}) with respect to $\omega$, $b$, $\zeta_i$ and $\zeta_i^*$ holds the following:

\begin{align}
\frac{\partial L(\cdot)}{\partial b} &= \sum_{i = 1}^{n} (\rho_i^* - \rho_i) = 0
\label{sp_c1} \\
\frac{\partial L(\cdot)}{\partial \omega} &= \omega - \sum_{i = 1}^{n} (\rho_i - \rho_i^*)x_i = 0
\label{sp_c2} \\
\frac{\partial L(\cdot)}{\partial \zeta_i} &= C - \rho_i - \eta_i = 0
\label{sp_c3} \\
\frac{\partial L(\cdot)}{\partial \zeta_i^*} &= C - \rho_i^* - \eta_i^* = 0.
\label{sp_c4} 
\end{align}

\fi

\noindent By solving (\ref{svr_opt_fct})
%substituting (\ref{sp_c1}), (\ref{sp_c2}), (\ref{sp_c3}) and (\ref{sp_c4}) into (\ref{Eq:lagrange_lin_svr}) 
one obtains 

\begin{equation}
\begin{aligned}
& \text{maximize}  
-\frac{1}{2}\sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)x_i^T x_j -\epsilon \sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n} y_i (\rho_i - \rho_i^*) 
\\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
\rho_i, \rho_i^* \in [0, C].
\end{cases}
\end{aligned}
\label{dual_lin_opt}
\end{equation}


%\begin{equation}
%\begin{aligned}
%& \text{maximize} && \begin{cases}
%-\frac{1}{2}\sum_{i,j = 1}^{j}(\rho_j - \rho_j^*)x_i' x_j \\
%-\epsilon \sum_{i = 1}^{l}(\rho_i + \rho_i^*) + \sum_{i = 1}^{l} y_i (\rho_i - \rho_i^*) 
%\end{cases} \\
%& \text{subject to} && \begin{cases} \sum_{1}^{l} (\rho_i - \rho_i^*) = 0\\
%\rho_i, \rho_i^* \in [0, C]
%\end{cases}
%\end{aligned}
%\label{dual_lin_opt}
%\end{equation}

\noindent Due to the dual formulation of the optimization problem one can 
%rearrange (\ref{sp_c2}) to 
%%%%Multiple steps skipped
get a representation of the weight vector $\omega$:

\begin{equation}
\omega = \sum_{i = 1}^{n} (\rho_i - \rho_i^*)x_i.
\label{Eq:weight_lin_svr}
\end{equation}
\newline
Thus, $\omega$ is a linear combination of the observations $x_i$. So, the theoretical starting point in (\ref{Eq:svr_lin_base_mdl}) can be rewritten as the so called SV expansion:
\begin{equation}
f(x) = \sum_{i = 1}^{n}(\rho_i - \rho_i^*)x_i^T x + b.  
\label{sv_exp_lin}
\end{equation}
\newline
For those $x_i$ where $f(x_i)$ is within the $\epsilon$-tube it holds that  $\rho_i = \rho_i^* = 0$. Hence, $f(x)$ is determined by the observations outside the $\epsilon$-tube. These $x_i$ are the so-called SVs. Consequently, the complexity of $f(x)$ depends on the number of SVs rather than the dimension of the input space.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Deriving the Constant Term}
%
%After $\rho_i$ and $\rho_i^*$ are obtained, $b$ can be derived from the Karush-Kuhn-Tucker (KKT) conditions. Their central statement is that the product of constraints and dual variables is zero at the solution. Therefore, the KKT conditions corresponding to (\ref{dual_lin_opt}) are:
%
%\begin{equation}
%\begin{aligned}
%\rho_i(\epsilon + \zeta_i - y_i + \omega' x_i + b) & = 0 \\
%\rho_i^*(\epsilon + \zeta_i^* + y_i - \omega' x_i - b) & = 0 \\
%(C - \rho_i)\zeta_i & = 0 \\
%(C - \rho_i^*)\zeta_i^* & = 0.
%\end{aligned}
%\label{kkt}
%\end{equation}
%From (\ref{kkt}) follows that  
%\begin{equation}
%\begin{aligned}
%\epsilon - y_i + \omega'x_i+ b & \ge 0 \text{\quad and \quad} \zeta_i = 0  & \text{if \quad} \rho_i < C \\
%\epsilon - y_i + \omega'x_i + b & \le 0                                     & \text{if \quad} \rho_i > 0.
%\end{aligned}
%\label{kkt_conc}
%\end{equation}
%
%\noindent By doing the same derivation for $\rho^*$ as for $\rho$ in (\ref{kkt_conc}) the following bounds on $b$ can be obtained:  
%% 
%%\begin{equation}
%%\begin{aligned}
%%\max_i & \{-\epsilon + y_i -\omega'x_i | \rho_i < C \text{ or } \rho_i^* > 0 \} \le b  \\ \min_i & \{-\epsilon + y_i - \omega'x_i | \rho_i > 0 \text{ or } \rho_i^* < C\} \ge b.
%%\end{aligned}
%%\label{ineq_b}
%%\end{equation}
%
%\begin{align}
%b_\text{lower} := \max_i & \{-\epsilon + y_i -\omega'x_i | \rho_i < C \text{ or } \rho_i^* > 0 \} \le b  \\ b_\text{upper} := \min_i & \{-\epsilon + y_i - \omega'x_i | \rho_i > 0 \text{ or } \rho_i^* < C\} \ge b.
%\end{align}
%
%
%\noindent Since $\rho_i$ and $\rho_i^*$ cannot be simultaneously nonzero the bounds are tight if $\rho_i\in(0, C)$ or $\rho_i^*\in(0, C)$ such that $b = b_\text{lower} = b_\text{upper}$. However, due to the constraints of (\ref{dual_lin_opt}) there can be training instances where $\rho_i$ or $\rho_i^*$ is equal to $C$. However, according to \cite{Chen.2009}, such situations can be hardly found in reality.  
%
%   
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Capturing Nonlinearity with Kernels}

%One approach to capture potential nonlinearities of the training data is to map the space of the training data $X$ into a feature space $F$, i.e. $\Theta: X \rightarrow F$. 
One approach to capture potential nonlinearities is to use a mapping $\Theta$ to map the training data space into some feature space. In practice, this can be done by preprocessing the training data to obtain polynomial features. Depending on the dimension of the training data space and order of the polynomials, the number of features can increase rapidly. More formally, for $p$ being the dimension of the training data space and $d$ being the degree to which polynomial features for all attributes of the training data are computed, the number of features will be determined by the binomial coefficient $\binom{d + p - 1}{d}$. The exponential increase of the feature space size is visualized in Figure~\ref{feat_size}. Hence, \cite{Smola.2004} consider this approach to be not feasible. \\
%%%out
\iffalse
\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.6]{Figures/size_feat_space}
	\caption[Feature space dimension for polynomial mappings]{Number of features in dependence of the dimension of the input space, i.e. training data space, and the degree of the polynomial mappings. Source: Own illustration.}
	\label{feat_size}
\end{figure}
\fi

\noindent A more feasible approach is obtained by noting that the solution of (\ref{dual_lin_opt}) depends on the input variables in form of dot products, i.e. $x^T x$. Hence, the input vectors can be mapped into a higher dimensional space by considering different dot products. As a consequence, it is not necessary to know $\Theta$ explicitly but sufficient to know the result of $\Theta(x^T) \Theta(x)$. Thus, by introducing the so-called kernel function $k(x^T, x) = \Theta(x^T)\Theta(x)$, (\ref{dual_lin_opt}) can be reformulated as follows:

\begin{equation}
\begin{aligned}
& \text{maximize} 
	-\dfrac{1}{2} \sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)k(x_i^T, x_j) 
	-\epsilon\sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n}y_i(\rho_i - \rho_i^*)
 \\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
	\rho_i, \rho_i^* \in [0, C].
	\end{cases}
\end{aligned}
\label{dual_nonlin_opt}
\end{equation}
\newline
\noindent Due to reformulating (\ref{dual_lin_opt}), the representation of the weight vector in (\ref{Eq:weight_lin_svr}) and  the SV expansion in (\ref{sv_exp_lin}) become 

\begin{equation}
\begin{aligned}
\omega & = \sum_{i = 1}^{n} (\rho_i - \rho_i^*)\Theta(x_i)  \\
f(x)& = \sum_{i = 1}^{n}(\rho_i - \rho_i^*)k(x_i^T, x) + b. 
\end{aligned}
\label{sv_exp_nonlin}
\end{equation}
\newline
The formulas in (\ref{sv_exp_nonlin}) depict two differences between the linear and nonlinear case. First, the restated optimization problem does not result in the flattest function of the input space but feature space. Moreover, since only the result of $k(x_i^T x)$ is needed in the computation of $f(x)$, $\omega$ is no longer given explicitly. \\

\noindent The use of kernel functions in SVR makes it necessary to establish conditions that ensure their results correspond to the dot product in a feature space. These conditions are the so-called Mercer's conditions which can be found in \cite{Smola.2004}. Three examples of kernel functions that are given by \cite{Smola.2004} are: 

\begin{align*}
%\text{Linear:}& \qquad x_i^T x  \\
\text{Polynomial:}& \quad (x_i^T x + c)^p \qquad &\text{with}& \ c \ge 0 \ \text{and} \ p \in \mathbb{N} \\
\text{Radial Basis Function:}& \quad \exp \left(\dfrac{\| x - x_i \|}{2 \gamma^2} \right)\qquad &\text{with}& \ \gamma > 0 \\
\text{Hyperbolic Tangent:}& \quad \text{tanh}(c +  h x_i^T x ) \qquad &\text{with}& \ c \in \mathbb{R}  \ \text{and} \ h \ge 0. \\
%\text{B-Spline:}& \quad B_{2n+1} ( \|x_i^T - x\|)  \qquad &\text{with}& \ B_k(z) = \otimes_{i = 1}^{k} \mathbb{I}(z \in [-0.5, 0.5]).
\end{align*}
\noindent %Here, $\otimes$ is the convolution operator.
 A special case of the polynomial kernel is the linear case which was used to introduce SVR. It is obtained for $c = 0$ and $p = 1$. Moreover, the hyperbolic tangent kernel is not an admissible kernel in the sense that it fulfills Mercer's conditions. However, it was shown to perform well in practice. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{SVR in Terms of Risk Minimization} \label{Sec:svr_ito_risk}
%
%SVR is rooted in statistical learning theory. However, the derivation was not based on the framework of the SRM inductive principle. The connection can be shown by reformulating the optimization problem in terms of a risk functional. In doing so, similarities of SVR and other function approximation methods can be seen. For instance, with respect to other methods for function approximation \cite{Smola.2004} show how SVR can be related to MLE. Consider the following empirical risk functional which is formulated in terms of the $\epsilon$-insensitive loss function in equation (\ref{Eq:svr_alt_loss_fct}):
%
%\begin{equation}
%\mathcal{R}_{emp}(f) = \frac{1}{n} \sum_{i = 1}^{n} L_{\epsilon}(y_i - f(x_i)).
%\label{Eq:svr_emp_risk}
%\end{equation}

%\noindent In the next step, a term to control the capacity of $f$ needs to be introduced. In (\ref{svr_opt_fct}) this was done by including $\| \omega \|^2$ in the minimization problem. Hence, the objective function to be minimized in SVR can be stated as the following regularized risk functional: 
%
%\begin{equation}
%\mathcal{R}_{reg}(f) = \frac{1}{n} \sum_{i = 1}^{n} L_{\epsilon}(y_i - f(x_i)) + \frac{\lambda}{2} \| \omega \|^2.
%\label{Eq:svr_alternative_min_fct}
%\end{equation}
%
%\noindent The parameter $\lambda > 0$ is a so-called regularization constant. Then, minimizing (\ref{Eq:svr_alternative_min_fct}) with $\lambda = 1/(C n)$ results in the same parameter estimates as solving the minimization problem in (\ref{svr_opt_fct}). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Modifications of the SV Regression Scheme}
%
%Many modifications of the SVR approach have been suggested. \cite{Smola.2004} mention two popular examples, i.e. SVR using linear programming and an approach that automatically adjusts the $\epsilon$-tube. 
%\paragraph{SVR and Linear Programming} 
%
%\noindent In the linear programming approach the regularization term in (\ref{Eq:svr_alternative_min_fct}) is replaced. This results in the following regularized risk functional
%
%\begin{equation}
%\mathcal{R}_{reg}(f) = \mathcal{R}_{emp}(f) + \lambda \sum_{i= 1}^{n} |\rho_i|
%\label{risk_svr_linear_programm}
%\end{equation}
%
%\noindent where $\rho_i$ relates to the corresponding SV expansion of (\ref{risk_svr_linear_programm}): 
%
%\begin{equation}
%f(x) = \sum_{i = 1}^{n} \rho_i k(x_i, x) + b.
%\end{equation}
%
%
% \noindent In case of an $\epsilon$-insensitive loss function (\ref{risk_svr_linear_programm}) results in a linear programming problem. Hence, it leads also to a computational advantage. However, other loss functions will not necessarily have the same advantage. \cite{Smola.2004} show that using the dualization method to minimize (\ref{risk_svr_linear_programm}) does not decrease the computational effort. The direct minimization of (\ref{risk_svr_linear_programm}) with linear optimizers is, therefore, the appropriate approach here.
%
%\paragraph{SVR with Automatized Tube Adjustment}
%
%In standard SVR, the loss function is an $\epsilon$-insensitive loss function where $\epsilon$ needs to be set manually. Thus, additionally to balancing out the trade-off between capacity and empirical risk, regression with the SV method requires to choose an adequate loss function as well. An automated adjustment of $\epsilon$ can be achieved by adding it to the risk function in (\ref{Eq:svr_alternative_min_fct}). This leads to the following risk functional that is to be minimized:
%
%\begin{equation}
%\mathcal{R}_\gamma(f) = \mathcal{R}_{emp}(f) + \dfrac{\lambda}{2}\|\omega\|^2 + \gamma \epsilon.
%\label{risk_svr_nu_reg}
%\end{equation}
%\newline
%By setting the restriction $\gamma > 0$, $\epsilon$ will be minimized. Using (\ref{risk_svr_nu_reg}) as an objective function leads asymptotically to a predetermined number of SVs. Based on (\ref{risk_svr_nu_reg}), the constrained optimization problem becomes
%
%\begin{equation}
%\begin{aligned}
%& \text{minimize} & & \frac{1}{2} \|\omega\|^2 + C\left(\sum_{i = 1}^{n}(\zeta_i + \zeta^{*}_i) + n \gamma \epsilon \right)  \\
%& \text{subject to} & &  \begin{cases}
%y_i - \omega' x_i - b \le \epsilon + \zeta_i \\
%\omega'x_i + b - y_i \le \epsilon + \zeta_i^{*} \\
%\zeta_i, \zeta_i^{*} \ge 0.
%\end{cases} 
%\end{aligned}
%\label{nu_svr_opt_fct}
%\end{equation}
%\newline
%\noindent Here, the relationship between $C$, $n$ and $\lambda$ stated in Section \ref{Sec:svr_ito_risk} was used to state a optimization problem similar to (\ref{dual_nonlin_opt}). Assuming the same loss function as in (\ref{svr_opt_fct}), the dual formulation of (\ref{nu_svr_opt_fct}) is 
%
%\begin{equation}
%\begin{aligned}
%& \text{maximize} && 
%-\frac{1}{2}\sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)k(x_i,x_j) 
%+ \sum_{i = 1}^{n} y_i (\rho_i - \rho_i^*) 
% \\
%& \text{subject to} && \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
%\sum_{i = 1}^{n} (\rho_i - \rho_i^*) \le C \gamma n\\
%\rho_i, \rho_i^* \in [0, C].
%\end{cases}
%\end{aligned}
%\label{dual_nu_svr_opt}
%\end{equation}
%\newline
%\noindent \cite{Smola.2004} point out that (\ref{dual_nu_svr_opt}) is similar to the dual formulation of the standard SVR in (\ref{dual_lin_opt}) and (\ref{dual_nonlin_opt}). Equation (\ref{dual_nu_svr_opt}) has one more constraint but the objective function is homogeneous and, therefore, simpler. Moreover, they show how an optimal $\gamma$ can be determined.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{The SV Algorithm at a Glance}
%
%In the last sections the SV algorithm for doing regression was derived. Figure~\ref{svm_algo} summarizes how the SV algorithm creates a regression machine from input data. At first, a mapping $\Theta$ is applied to the data contained in the test vector and the SVs. After mapping both into the feature space, dot products are computed which is equal to evaluating a kernel $k$. As given by (\ref{sv_exp_nonlin}), the last step is to multiply the evaluated kernels with weights $\nu_i = (\rho_i - \rho_i^*)$ and add $b$.  \\
%
%\begin{figure}[h!]
%\centering
%\includegraphics[scale = 0.4]{Figures/svm_algo_correct}
%\caption[The SVR architecture]{A visualization of a SV based regression machine. Source: \cite{Smola.2004}.}
%\label{svm_algo}
%\end{figure}
%
%\noindent \cite{Smola.2004} note that regression with NNs is similar to the SV approach. However, they differ with respect to the input data. Due to the $\epsilon$-insensitive loss function, only a subset of the training data is used in the SV algorithm. In contrast, NNs use different loss functions that do not exclude observations. Hence, the function that is estimated by the SV algorithm does not depend on the observations that are not SVs. Despite this redundancy, it is not advisable to exclude these observations to reduce the memory needed to store it. For instance, \cite{Smola.2004} note that this can cause difficulties when handling high-dimensional or noisy data. 
%
%
%
% 
%
%



==> Sections/svrSL.tex <==
\subsection{Support Vector Regression} \label{Sec:meths_svr}
SVR can be understood as a learning method to solve nonlinear regression tasks  \cite[e.g.,][]{Smola.2004}. It shares some similarities with a three-layer feed-forward NN and is able to approximate arbitrarily complex functions \citep{Chen.2009}. However, NNs are based on minimizing the so-called empirical risk and tend to find only locally optimal solutions. In contrast, SVR minimizes the so-called structural risk to achieve better generalization and solves a convex optimization problem leading to a globally optimal solution.
To describe the SVR model, let $\{(y_i, x_i)| i = 1,\dots, n; \ n\in \mathbb{N}\}$ with $x_i \in \mathbb{R}^p$ and $y_i \in \mathbb{R}$ denote the training data set. Suppose $f$ is a linear function such that 

\begin{equation}
f(x) = \omega^\top x + b
\label{Eq:svr_lin_base_mdl}
\end{equation}

\noindent where  $\omega \in \mathbb{R}^p$ and $b \in \mathbb{R}$. Then, SVR aims to find an approximation of $f$ that deviates at most by $\epsilon$ from the observed target $y$ while being as flat as possible (i.e., in the sense that weights in $\omega$ are small). This translates into the following convex optimization problem:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 \\
& \text{subject to} & & \begin{cases}
y_i - \omega^\top x_i - b \le \epsilon  \\
\omega^\top x_i + b - y_i \le \epsilon.
\end{cases} 
\end{aligned}
\label{svm_mean_eq}
\end{equation}
\newline
In view that (\ref{svm_mean_eq}) might lack a feasible solution, \cite{Vapnik.1995} introduces an $\epsilon$-insensitive loss function: 

\begin{equation}
L_{\epsilon}\left\{y - f(x)\right\}  = \begin{cases}
0 \qquad \qquad \qquad  \text{if} \ |y - f(x)| \le \epsilon \\
|y - f(x)| - \epsilon \ \ \text{otherwise}.
\end{cases}
\label{Eq:svr_alt_loss_fct}
\end{equation}

To measure empirical loss (and thus model fit) using (\ref{Eq:svr_alt_loss_fct}) \cite{Vapnik.1995} reformulates (\ref{svm_mean_eq}) using slack variables $\zeta$ and $\zeta^{*}$ that capture losses above and below the $\epsilon$-tube around $f(x)$, respectively. Figure~\ref{loss_fct} depicts this approach. Only points outside the gray shaded $\epsilon$-tube contribute linearly to the loss function. \\ 

\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.4]{Figures/svm_loss_fct_correct}
	\caption[The $\epsilon$-insensitive loss function]{The $\epsilon$-insensitive loss function of the SVR algorithm. Slack variable $\zeta$ captures the loss above the $\epsilon$-tube. Points within the grey shaded area have no impact on the loss. In contrast, all other observations contribute linearly to the loss. Source: \cite{Smola.2004}.}
	\label{loss_fct}
\end{figure}


Integrating the slack variables $\zeta$ and $\zeta^*$ into (\ref{svm_mean_eq}), the task to estimate a SVR model is equivalent to solving:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 + C\sum_{i = 1}^{n}(\zeta_i + \zeta^{*}_i) \\
& \text{subject to} & &  \begin{cases}
y_i - \omega^\top x_i - b \le \epsilon + \zeta_i \\
\omega^\top x_i + b - y_i \le \epsilon + \zeta_i^{*} \\
\zeta_i, \zeta_i^{*} \ge 0,
\end{cases} 
\end{aligned}
\label{svr_opt_fct}
\end{equation}
where $C > 0$ is a regularization parameter to balance between model fit and complexity \citep[e.g.,][]{Hastie.2009}. Larger (smaller) values of $C$ put more (less) weight on maximizing model fit during SVR learning. 
 
To capture nonlinear relationships between covariates and the response variable, SVR maps the input data into a higher dimensional feature space. The linear regression is then constructed in the transformed space, which corresponds to a nonlinear regression in the input space. The transformation is feasible from a computational point of view because SVR calculates the mapping by implicitly using a kernel function 
$k(x_i^\top x)=\phi^\top(x_i) \phi(x)$. To implement this approach, it is common practice to estimate a SVR model through solving the dual of (\ref{svr_opt_fct}), which is given as \citep[e.g.,][]{Smola.2004}:

\begin{equation}
\begin{aligned}
& \text{maximize} 
	-\dfrac{1}{2} \sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)x_i^\top x_j 
	-\epsilon\sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n}y_i(\rho_i - \rho_i^*)
 \\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
	\rho_i, \rho_i^* \in [0, C].
	\end{cases}
\end{aligned}
\label{dual_lin_opt}
\end{equation}
\newline
The dual program (\ref{dual_lin_opt}) includes the input data only in the form of scalar products $x_i^\top x_j$. Replacing the scalar product by means of a kernel function is thus straightforward and does not affect the solver. In this work, we employ the Gaussian radial basis function (RBF) kernel (\ref{rbf_kernel}) which is defined as
\begin{equation}
\begin{aligned}
k(x_i^\top x)= \exp \left(-\dfrac{\| x - x_i \|^2}{2 \gamma^2} \right)
\end{aligned}
\label{rbf_kernel}
\end{equation}
where the meta-parameter $\gamma>0$ governs the width of the Gaussian function and needs to be set by the modeler. The RBF kernel is used because it includes other kernels as special cases, possesses numerical advantages compared to alternatives, and often performs well in practical applications. Moreover, the RBF kernel can capture nonlinear relations. Other kernels that are usually presented as potential choices are e.g. the linear, polynomial or sigmoid kernel \citep[e.g.,][]{Smola.2004,Hastie.2009}. \cite{Keerthi.2003} show that the linear kernel is a special case of the RBF kernel. Moreover, the polynomial kernel has more parameters than the RBF kernel that make the tuning process more costly. Another advantage of the RBF over the polynomial kernel is that the polynomial kernel can converge to infinity which can cause numerical instability. In contrast, the domain of the RBF kernel is always between 0 and 1. Moreover, \cite{Lin.2003} show that the sigmoid kernel behaves similar to the RBF kernel for certain parameters.

In order to construct the regression function (\ref{Eq:svr_lin_base_mdl}), the weight vector $\omega$ is represented as a linear combination of observations in the training set:

\begin{equation}
\omega = \sum_{i = 1}^{n} (\rho_i - \rho_i^*)x_i.
\label{Eq:weight_lin_svr}
\end{equation}
\newline

More specifically, for observations $x_i$ where $f(x_i)$ is within the $\epsilon$-tube holds that  $\rho_i = \rho_i^* = 0$. Consequently, $f(x)$ depends only on the observations outside the $\epsilon$-tube. These $x_i$ are called support vectors. Accordingly, (\ref{Eq:weight_lin_svr}) is also called the support vector expansion of $\omega$. Rewriting the regression function in terms of the support vector expansion gives the SVR forecasting model:

\begin{equation}
f(x) = \sum_{i = 1}^{n}(\rho_i - \rho_i^*)x_i^\top x + b.  
\label{sv_exp_lin}
\end{equation}
\newline

\noindent In the nonlinear case, the scalar product in (\ref{sv_exp_lin}) is once again replaced by a kernel function.

==> Sections/svrgarchkde.tex <==
\subsection{SVR-GARCH-KDE Hybrid}\label{Sec:SVRGARCHKDE}
In the following section, we introduce a nonlinear GARCH hybrid to forecast VaR based on a combination of SVR and KDE. Subsequently, we elaborate on the estimation of the corresponding forecasting model. 
%\subsubsection{Derivation of the SVR-GARCH-KDE Hybrid}

%In the following a nonparametric and nonlinear GARCH hybrid to forecast VaR based on a combination of SVR and KDE is introduced. In equation (\ref{Eq:garch_arma2}) it was shown that GARCH processes can be given an ARMA representation. 

%Recall the formulation for a return series $r_t$ where the mean equation is described by an AR(1) process and the variance equation by a GARCH(1,1) process:
%
%%\begin{align}
%%r_t &= c + \alpha r_{t-1} + \epsilon_t, \qquad \epsilon_t \sim N(0, \sigma_t^2) \\
%%\sigma_t^2 &= \omega + \beta \sigma_{t-1}^2 + \delta \epsilon_{t-1}^2. \label{Eq:GARCH_11}
%%\end{align}
%%
%%\noindent Since the conditional expectation of $\epsilon_t^2$ is $\sigma_t^2$, the conditional variance in GARCH models can be modeled via an ARMA process \citep{Chen.2009}. \cite{Poo.2003} derived the ARMA representation for the general GARCH($p$,$q$) case. For the GARCH(1,1) model in (\ref{Eq:GARCH_11}) let $\nu_t = \epsilon^2_t - \sigma^2_t$ and replace $\sigma^2_t$ with $\epsilon_t^2 - \nu_t$ to obtain 
%%
%%\begin{equation}
%%\epsilon_t^2 - \nu_t = \omega + \beta (\epsilon_{t-1}^2 - \nu_{t-1}) + \delta \epsilon_{t-1}^2.
%%\label{garch_re1}
%%\end{equation}
%%
%%\noindent Rewriting (\ref{garch_re1}) in the form of an ARMA(1,1) process for $\epsilon_t^2$ results in 
%%
%%\begin{equation}
%%	u_t^2  = \omega + \sum_{i = 1}^{\max(p,q)} (\beta_i + \delta_i) u_{t-i}^2 - \sum_{j = 1}^{q} \beta_j \nu_{t-j} + \nu_t , \quad \nu_t \sim WN(0,u_t)
%%%\epsilon_t^2  = \omega + (\beta + \delta) \epsilon_{t-1}^2 - \beta \nu_{t-1} + \nu_t.
%%\label{garch_re2}
%%\end{equation}

We assume the distribution of the return series $r_t$ to belong to the location-scale class, such that:

\begin{equation}
r_t = \mu_t + u_t = \mu_t + \sigma_t z_t, \qquad z_t \sim (0,1) \ \text{i.i.d.}
\label{Eq:hybrid_locs}
\end{equation}

%\noindent \cite{Engle.1982} and \cite{Bollerslev.1986} assumed a parametric mean model with linear structure. Based on this, they derived ARCH and GARCH processes that are also linear and parametric. In addition, the proposed estimation procedures rely on MLE and therefore distributional assumptions. To overcome the restrictions of a linear parametric structure with distributional assumptions, a nonparametric and nonlinear GARCH hybrid to forecast VaR based on a combination of SVR and KDE is introduced. \\  

\noindent Consider an ARMA structure for the mean model where the only assumption  about the error distribution is a zero mean and a finite variance. In addition, recall equation (\ref{Eq:garch_arma2}), which shows that GARCH processes can also be given an ARMA representation. This leads to the following mean and variance model:
\begin{align}
r_t &= c + \sum_{i = 1}^{s} \alpha_i r_{t-i} + \sum_{j = 1}^{d} \kappa_j u_{t-j} + u_t, \quad u_t \sim (0, \sigma_t^2) \\
u_t^2 &=\omega + \sum_{i = 1}^{\max(p,q)} (\delta_i + \beta_i) u_{t-i}^2 - \sum_{j = 1}^{p} \beta_j \nu_{t-j} + \nu_t.
\end{align}


\noindent Let $e = \max(p,q)$, $\mathbf{r}_{t,s} = (r_{t-1}, r_{t-2}, \dots, r_{t-s})$, $\mathbf{u}_{t,k} = (u_{t-1}, u_{t-2}, \dots, u_{t-k})$ and 
$\boldsymbol{\nu}_{t,p} = (\nu_{t-1}, \nu_{t-2}, \dots, \nu_{t-p})$. Then,  following \cite{Chen.2009}, we introduce the nonlinear and nonparametric functions $h$ and $g$ such that the conditional mean and variance models of $r_t$ are

\begin{align}
r_t &= h(\mathbf{r_{t,s}}, \mathbf{u_{t,d}}) + u_t \qquad u_t \sim (0, \sigma_t^2) \label{Eq:garch_mean_no_dis}\\
u_t^2 &= g(\mathbf{u_{t,e}}, \boldsymbol{\nu_{t,p}}) +  \nu_{t} \qquad \nu_t \sim WN(0,a_t^2)\label{Eq:garch_var_no_dis}
\end{align}

%\noindent 
%Section \ref{Sec:NDE} was motivated by research showing time varying structures for stock return distribution regarding the first four moments. In order to obtain more flexibility in the estimation of VaR $\epsilon_t$ is replaced with $\epsilon_t^* \sim (0,  \sigma_t^2)$ such that no distributional assumption about the error term are made. Assuming zero mean and finite variance . This results in 
%\begin{align}
%r_t &= f(r_{t-1}) + \epsilon_t^* \qquad \epsilon_t^* \sim (0, \sigma_t^2)  \label{Eq:garch_mean_no_dis}\\
%\epsilon_t^{*2} &= g(\epsilon_{t-1}^{*2}, \nu_{t-1}^*) +  \nu_{t}^* \qquad \nu_t^* \sim WN(0,u_t). \label{Eq:garch_var_no_dis}
%\end{align}

\noindent where $ WN(0,a_t^2)$ denotes white noise with expectation zero and variance $a_t^2$. We propose to estimate $h(\cdot)$ and $g(\cdot)$ using SVR. The estimates for $\mu_t$ and $\sigma_t$ in (\ref{Eq:hybrid_locs}) are then obtained as:

\begin{align}
\widehat{\mu}_t &= h(\mathbf{r_{t,s}}, \mathbf{u_{t,d}}) \label{Eq:svr_mean_estimate} \\
\widehat{\sigma}_t &= \sqrt{g(\mathbf{u_{t,e}}, \boldsymbol{\nu_{t,p}})}.
\end{align}

\noindent By defining the estimated residuals as $\widehat{u}_t = r_t - \widehat{\mu}_t$, estimates of $z_t$ are obtained as
\begin{equation}
\widehat{z}_t = \dfrac{\widehat{u}_t}{\widehat{\sigma}_t}.
\label{Eq:standardizes_residuals}
\end{equation}


% However, $\widehat{z}_t$ has not necessarily have zero mean and unit variance. Hence, the quantile estimation will be done using scaled standardized residuals $\widehat{z}_t^*$:
%%
%\begin{equation}
%\widehat{z}_t^* = \dfrac{\widehat{z}_t - \overline{\widehat{z}_t}}{\sqrt{\frac{1}{n-1}\sum_{i = 1}^{T}  (\widehat{z}_t - \overline{\widehat{z}_t})^2  }}
%\end{equation}
%
%\noindent where $\overline{\widehat{z}_t}$ denotes the empirical mean of $\widehat{z}_t$.  
\noindent Then, for $\widehat{Q}_{\widehat{z}}(\alpha)$ being the estimated quantile function of $z$, the VaR estimate for $r_t$ is:

\begin{equation}
\widehat{VaR}_t^\alpha = - \left\{ h(\mathbf{r_{t,s}}, \mathbf{u_{t,d}}) +\sqrt{g(\mathbf{u_{t,e}}, \boldsymbol{\nu_{t,p}})} \widehat{Q}_{\widehat{z}}(\alpha) \right\}.
\label{Eq:nonlin_var}
\end{equation}

\noindent whereby we estimate $\widehat{Q}_{\widehat{z}}(\alpha)$ using KDE.
%\noindent Then, in the SVR-GARCH-KDE hybrid approach, the estimation of $f(\cdot)$ and $g(\cdot)$ is done via SVR and $Q_{\widehat{z}_t}(\alpha)$ is obtained through KDE.
%\subsubsection{Estimating the SVR-GARCH-KDE Hybrid}

We now present a procedure to estimate VaR as in (\ref{Eq:nonlin_var}) and describe it in the context of producing one-day-ahead VaR forecasts. A step-by-step overview is given in Algorithm \ref{Algo:svr-garch-kde_algo}. Let $\{r_t\}_{t = 1}^T$ be the training set consisting of the daily returns from a portfolio where $r_T$ is the most recent observation. In the first step, we model the mean process (\ref{Eq:garch_mean_no_dis}). To do this, we estimate an AR($s$) model using SVR to obtain the estimated returns $\{\widehat{r}_t\}_{t = 1+s}^T$. The set of estimated residuals $\{\widehat{u}_t\}_{t = 1 + s}^T$ is derived as $\widehat{u}_t = r_t - \widehat{r}_t$. Then, a moving average (MA) part can be introduced to the model such that $r_t$ can be modeled as an ARMA($s$,$d$) process by running SVR and including $\widehat{u}_t$. The sets of estimated returns and residuals from the ARMA($s$,$d$) model are denoted as $\{\widehat{r}_t^*\}_{t = 1 + s + d}^T$ and $\{\widehat{u}_t^*\}_{t = 1 + s + d}^T$ , respectively.

 We also estimate the variance process in a two step approach and start by fitting the squared mean model residuals $\{\widehat{u}_t^{*2}\}_{t = 1 + s +d}^T$ in the way of an AR($e$) process with SVR. Based on this, fitted variances $\{\widehat{\sigma}_t^2\}_{t = 1 + s+d +e}^T$ are obtained. Then, an ARMA model for (\ref{Eq:garch_var_no_dis}) is obtained in the same way as for the mean process by using the estimated model residuals $\{\widehat{\nu}_t\}_{t = 1 + s + d + e}^T$ where $\widehat{\nu}_t = \widehat{u}_t^{*2} - \widehat{\sigma}_t^2$. Consequently, the final set of fitted variances is denoted as $\{\widehat{\sigma}_t^{*2}\}_{t = 1 + s +d+e+p}^T$. No assumptions are made about the starting values of the residuals. Hence, the final estimation of (\ref{Eq:garch_var_no_dis}) is done using data for $T-s-d-e-p$ time points. Since SVR is applied without introducing further restrictions, it is not ensured that $\widehat{\sigma}_t^2$ and $\widehat{\sigma}_t^{*2}$ are positive. Therefore, if the SVR estimate is $\widehat{\sigma}_t^{\left(*\right)2} \le 0$, it will be replaced by the last positive estimated variance. In case the first fitted variance is negative, it will be replaced by the first squared residual from the final mean model. 

The set of estimated standardized residuals $\{\widehat{z}_t\}_{t = 1 + s +d+e+p}^T$ can be computed by applying (\ref{Eq:standardizes_residuals}). However, $\widehat{z}_t$ does not necessarily have zero mean and unit variance. Hence, we perform the quantile estimation using scaled standardized residuals $\widehat{z}_t^*$:

\begin{equation}
\widehat{z}_t^* = \dfrac{\widehat{z}_t - \overline{\widehat{z}_t}}{\sqrt{\frac{1}{T-1}\sum_{i = 1}^{T}  (\widehat{z}_t - \overline{\widehat{z}_t})^2  }}
\end{equation}

\noindent where $\overline{\widehat{z}_t}$ denotes the empirical mean of $\widehat{z}_t$. The forecasted mean $\widehat{\mu}_{T+1}$ and standard deviation $\widehat{\sigma}_{T+1}$ are obtained from the mean and variance model. Finally, we use KDE to estimate the $\alpha$-quantile of $\{\widehat{z}^*_t\}_{t = 1 + s + d+e+p}^T$. Then, the one-day-ahead VaR forecast is: 

%-----------------------------------------------------------------\\
% is estimated by SVR such that the estimates $\widehat{r}_t$ and $\widehat{\epsilon}_t^* = r_t - \widehat{r}_t$ are obtained for $r_t$ and $\epsilon_t^*$, respectively. The variance process is estimated by a two step procedure. Since $\nu_{t-1}^*$ is not available the estimation of (\ref{Eq:garch_var_no_dis}) starts by fitting the series $\{\widehat{\epsilon}_t^*: t = 2, \dots, T\}$ in the way of an AR(1) process with SVR. Then, an ARMA model for (\ref{Eq:garch_var_no_dis}) is obtained by using the estimated model residuals $\{\widehat{\nu}_t^*: t = 3, \dots, T\}$. Note that no assumptions are made about the starting values of the residuals. Hence, the final estimation of (\ref{Eq:garch_var_no_dis}) is done by using data for $T-3$ time points. Denote ${\{\widehat{\sigma}_t^2: t = 3, \dots, T\}}$ as set of estimated variances. Since the SVR is done without introducing further restrictions it is not ensured that $\widehat{\sigma}_t^2 > 0$. Therefore, if the SVR estimate is $\widehat{\sigma}_t^2 \le 0$, it will be replaced by $\widehat{\sigma}_{t-1}^2$. In order to obtain the set of estimated standardized residuals $\widehat{z}_t$ divide $\widehat{\epsilon}_t$ by $\widehat{\sigma}_t$. Theoretically holds that $z_t \sim (0, 1)$. This is not ensured in practical applications. To ensure that (\ref{Eq:nonlin_var}) holds $\widehat{z}_t$ will be standardized to zero mean and unit variance. The one-day ahead VaR forecast is then obtained by

\begin{equation}
\widehat{VaR}_{T+1}^\alpha = -[ \widehat{\mu}_{T+1} + \widehat{\sigma}_{T+1} \widehat{Q}_{\widehat{z}^*} (\alpha)].
\label{Eq:var_est_svrkde}
\end{equation}

An important aspect to note is that SVR and KDE depend on hyperparameters which cannot be derived analytically but must be found computationally. Therefore, the above described estimation procedure describes the estimation process only for one fixed set of hyperparameters. The hyperparameters for SVR given a RBF kernel is used are $\epsilon$, $\gamma$ and $C$. Additionally, if the SVR kernel is not set beforehand, it can be seen as hyperparameter itself. In the context of KDE the bandwidth $h$ and the KDE specific kernel function $K$ are hyperparameters. Since the goal is to train an efficient model on a purely data driven basis it is advisable to derive the hyperparameters computationally. However, for some hyperparameters exist theoretical results that support fixing them beforehand. As stated in Section \ref{Sec:meths_svr} the RBF kernel is a reasonable choice in SVR. Moreover, for KDE the kernel choice has only a low practical relevance and there exist rule-of-thumb estimators for $h$ when a Gaussian kernel  is used which are computationally inexpensive \citep{Hardle.2004, Silverman.1986}. Hence, the most relevant aspect in hyperparameter tuning of the SVR-GARCH-KDE hybrid are $\epsilon$, $\gamma$ and $C$ for the SVR with a RBF kernel. It is important to note that the overall goal is to forecast VaR. Hence, the hyperparameters should be set with respect to the measure that is used to evaluate quantile forecasts. There exist different approaches as grid search, random search or more advanced optimization strategies that can be used to automate the process of hyperparameter optimization.

%
%\noindent where $F_{\widehat{z_t}}^{-1}$ is obtained based on the nonparametric density estimation with KDE for $\widehat{z_t}$. 

%\renewcommand{\thealgorithm}{}
%\begin{algorithm*}
%	\caption{SV-GRACH-KDE Algorithm for forecasting VaR}
%	\begin{algorithmic}[1]
%	\State Estimate an AR(1) model for $\{r_t: t = 1, \dots, T\}$ using SVR
%	\State Compute the model residuals from Step 1 $\{\widehat{\epsilon}_t: t = 1, \dots, T\}$
%	\State Estimate an AR(1) model for $\{\widehat{\epsilon}_t^2: t = 1, \dots, T\}$ using SVR
%	\State Compute the model residuals from Step 3 $\{\widehat{\nu}_t: t = 2, \dots, T\}$
%	\State Reestimate the model in Step 3 as ARMA(1,1) by introducing $\{\widehat{\nu}_t: t = 2, \dots, T\}$
%	\State Obtain the set of estimated variances $\{\widehat{\sigma}_t^2: t = 3, \dots, T\}$ from Step 5
%	\State Compute the standardized residuals $z_t = \widehat{\epsilon}_t / \widehat{\sigma}_t$ for $t = 3, \dots, T$
%	\State Normalize $\widehat{z}_t$ to zero mean and unit variance
%	\State Estimate the $\alpha$-quantile $F_{\widehat{z_t}}^{-1}(\alpha)$ with KDE
%	\State Obtain $\widehat{r}_{T+1}$ and $\widehat{\sigma}_{T+1}$ by using the models from Step 1 and 5
%	\State Compute the VaR forecast as $VaR_{T+1}^\alpha = \widehat{r}_{T+1} + \widehat{\sigma}_{T+1} F_{\widehat{z_t}}^{-1} (\alpha)$
%	\end{algorithmic}
%\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%Moved to appendix%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Choose whether to move algorithm to appendix
%\iffalse
\begin{algorithm}
	\caption{SVR-GRACH-KDE Estimation Algorithm for Forecasting VaR}
	\label{Algo:svr-garch-kde_algo}
	\begin{algorithmic}[1]
		
		\State AR($s$) model for $\{r_t\}_{t=1}^T$ using SVR
		\vspace{0.1cm}
		\State Get errors from Step 1 $\{\widehat{u}\}_{t=1+s}^T$
		\vspace{0.1cm}
		\State ARMA($s$,$d$) model for $\{r_t\}_{t=1+s}^T$ with results from Step 2 using SVR
		\vspace{0.1cm}
		\State Get errors from Step 3 $\{\widehat{u}^*\}_{t=1+s+d}^T$
		\vspace{0.1cm}
		\State AR($e$) model for $\{\widehat{u}_t^{*2}\}_{t=1+s+d}^T$ using SVR
		\vspace{0.1cm}
		\State Get errors from Step 5 $\{\widehat{\nu}_t\}_{t=1+s+d+e}^T$
		\vspace{0.1cm}
		\State ARMA($e$,$p$) model for $\{\widehat{u}_t^{*2}\}_{t=1+s+d+e}^T$  with results from Step 6 using SVR
		\vspace{0.1cm}
		\State Obtain volatility estimates $\{\widehat{\sigma}^*\}_{t=1+s+d+e+p}^T$ from Step 7
		\vspace{0.1cm}
		\State Get standardized residuals $\widehat{z}_t = \widehat{u}_t^* / \widehat{\sigma}_t$ for $t = 1+s+d+e+p, \dots, T$
		\vspace{0.1cm}
		\State Scale $\{\widehat{z_t}\}_{t=1+s+d+e+p}^T$ to zero mean and unit variance and obtain $\{\widehat{z}_t^*\}_{t=1+s+d+e+p}^T$
		\vspace{0.1cm}
		\State Estimate the $\alpha$-quantile $\widehat{Q}_{\widehat{z}^*}(\alpha)$ with KDE
		\vspace{0.1cm}
		\State Obtain $\widehat{r}_{T+1}$ and $\widehat{\sigma}_{T+1}$ by using the models from Step 3 and 7
		\vspace{0.1cm}
		\State VaR forecast: $\widehat{VaR}_{T+1}^\alpha = -[ \widehat{\mu}_{T+1} + \widehat{\sigma}_{T+1} \widehat{Q}_{\widehat{z}^*} (\alpha)]$
		
		
	\end{algorithmic}
\end{algorithm}
%\fi

After defining the SVR-GARCH-KDE hybrid the question arises how model complexity, predictive power and the computational time for making VaR forecasts are related. Regarding the time to compute predictions the KDE part is fixed beforehand. This is can be seen in Equation \ref{Eq:kde_definition} and Algorithm \ref{Algo:svr-garch-kde_algo}. In order to compute an estimate the sum needs to be evaluated making the computational complexity $O(n)$ where $n$ is number of observations. Regarding the SVR-GARCH-KDE hybrid the computational complexity of the KDE part is reduced depending on the order of the autoregressive and moving-average part of the mean and variance process to $O(n-s-d-e-p)$. With respect to SVR the complexity of making a prediction is $O(n_{SV} d)$, where $d$ is the dimension of the feature space and $n_{SV}$ the number of SVs. For the proposed application of forecasting the mean and variance of a financial time series the number of features is usually low. Therefore, the computational time for generating predictions is mainly driven by the sample size and negligible in this application.
	
Regarding the predictive performance, the regression function of the mean and variance process is determined by the SVs which implies that the higher the number of SVs, the higher the complexity. Using a SVR decision function with a high number of SVs can, therefore, lead to a mediocre out-of-sample performance. However, it is not possible to make an ex ante exact statement since the Vapnik-Chervonenkis dimension of the RBF kernel is infinite \citep{Burges.1998}. %Hence, the generalization error which is the bound for the actual risk is also infinite. 
Moreover, the goal of the SVR-GARCH-KDE hybrid is to forecast quantiles. Evaluating the performance ex ante does, therefore, depend on the measure that is used to evaluate forecasted quantiles rather than the statistical properties of KDE and potential error bounds of SVR. In Section \ref{Sec:emp_study} the framework of \cite{Christoffersen.1998} will be applied. For achieving a good performance it is necessary to tune the parameters of the SVR and KDE part appropriately with respect to the target measure. Consequently, in this study the focus is put on the out-of-sample performance to optimize the quality of predictions and the hyperparameter tuning is done with a separate training set.


==> Sections/titlepage.tex <==
\begin{center}

	
	\LARGE \text{Humboldt-Universit{\"a}t zu Berlin} 
	
\vspace{0.5cm}

	\begin{figure}[h]
		\centering
		\includegraphics{Figures/hulogo}
	\end{figure}

\vspace{-0.5cm}

    {\LARGE{\bf Data Driven Value-at-Risk Forecasting \\ \vspace{0.1cm} Using a SVR-GARCH-KDE Hybrid}} \vspace{0.5cm}

\vspace{0.5cm}
   
    {\large Master Thesis by: \\ \vspace{0.1cm} \LARGE Marius Lux (558415)}
               
    \vspace{0.2cm}

\large

\begin{align*}
\text{First Supervisor:}& \text{ Prof. Dr. Stefan Lessmann} \\
\text{Second Supervisor:}& \text{ Prof. Dr. Wolfgang K. H{\"a}rdle} \\
\end{align*}
\vspace{-1.5cm}
	
	\normalsize  School of Business and Economics \\
	Chair of Information Systems \\ Ladislaus von Bortkiewicz Chair of Statistics

 \vspace{0.8cm}
 
 \large
In partial fulfillment of the requirements \\ for the degree \\ {\bf Master of Science in Statistics} 

 \vspace{.8cm}
 
 \large Berlin, March 30, 2017

\end{center}


==> Sections/value_at_risk.tex <==
%\section{Value-at-Risk}\label{Sec:var}
%$\R$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Defining Value at Risk
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Defining Value-at-Risk}

%\cite{Jorion.2009} defines VaR as \textit{"the worst loss over a target horizon that will not be exceeded with a given level of confidence"}. Therefore, two parameters are essential for measuring VaR. First, the confidence level $ 1 - \alpha$ which corresponds to the probability that no loss larger than the VaR occurs in a given time horizon. Here, $\alpha$ is referred to as significance level. The second parameter is the time horizon $d$ which is usually measured in trading days. For instance, assume an investor who has a portfolio with a total value of $100.000\$$. He wants to know the next day's VaR for a confidence level of $95\%$. Further assume the next day's return is higher than $-2.5\%$ with a probability of $95\%$. Then, the portfolio's VaR for a confidence level of $95\%$ and time horizon of one trading day is $100.000\$ \cdot 0.025 = 2.500\$$. \newline

%\noindent In general, VaR can be derived from the portfolio's loss distribution. However, since today's portfolio value is usually known, it suffices to model the return distribution. Hence, by following \cite{Kuester.2005} for a formal description of VaR, let the portfolio returns be a random variable $X \in \mathbb{R}$ with cumulative distribution function $F$. Then, the VaR in $d$ trading days for a confidence level $1-\alpha$ is defined as

In general, VaR can be derived from the portfolio's $P\&L$ distribution. However, since today's portfolio value is usually known, it suffices to model the return distribution. For a formal description of VaR, let the portfolio returns $r_t$ in period $t$ have the cumulative distribution function (CDF) $F_t$. Then, the VaR in $d$ trading days for a confidence level $1-\alpha$ is defined as

\begin{equation}
VaR_{t+d}^\alpha = -F^{-1}_{t+d}(\alpha) = -\inf\{ x \in \mathbb{R}: F_{t+d}(x) \geq \alpha \} \quad \text{with} \quad \alpha \in (0,1) .
\end{equation}

\noindent In the rest of the paper, VaR refers to the negative $\alpha$-quantile of the next period's portfolio return distribution. %This is illustrated in Figure~\ref{var_illu}. 

%\noindent Hence, VaR is the negative $\alpha$-quantile of the next period's portfolio return distribution which is equivalent in saying that VaR indicates the next period's loss that will not be exceeded with a probability of 100(1-$\alpha$)$\%$. Figure~\ref{var_illu} illustrates the VaR concept. Estimating VaR requires the estimation of the loss distribution. However, the next period's loss is derived by multiplying today's portfolio value with the relative change of the portfolio in $h$ trading days. Today's portfolio value is usually known. Therefore, by assuming the portfolio value is known it suffices to estimate next period's distribution of relative portfolio changes. Then, VaR is derived by multiplying  today's portfolio value with the negative $\alpha$-quantile of the next period's portfolio return distribution. Therefore, in the rest of this thesis the use of the term VaR refers to the $\alpha$ quantile of the a portfolios return distribution.

%\begin{figure}[h]
%	\centering
%	\includegraphics{Figures/var-quantile-tails_TEST}
%	\caption{Illustration of VaR for a hypothetical portfolio return density function. Source: \cite{Alexander.2010}}
%	\label{var_illu}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% APPROACHES FOR ESTIMATING VAR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Approaches for Estimating VaR}
%
%The VaR forecasting model proposed in this thesis combines nonlinear function approximation via SVR and nonparametric density estimation by KDE. Since this work aims to compare machine learning methods as SVR in risk management, the proposed method will be compared to similar traditional statistical methods. However, already existing approaches to quantile regression in machine learning are described as well. So, the following two sections review methods to estimate quantiles that were proposed in the context of traditional statistics and machine learning, respectively. 

%\subsubsection{Approaches Related Related to Traditional Statistics}
\subsection{Estimating VaR Using Location-Scale Models} \label{Sec:var_est_approaches}

%\cite{Kuester.2005} compare the performance of several approaches for estimating VaR. Moreover, a comprehensive overview over existing statistical methods is given. Four categories are suggested to describe existing methods for VaR estimation. These categories are historical simulation, fully parametric models, extreme value theory and quantile regression. In this section, the above mentioned modeling approaches are introduced by closely following \cite{Kuester.2005}. 
%
%\paragraph{Historical Simulation} \cite{Kuester.2005} use the term historical simulation to refer to methods using empirical quantiles of historical return data. However, this approach has some drawbacks. First, returns are typically not independent and identically distributed (i.i.d.). Historical simulation does not account for this. Moreover, VaR predictions are bounded by the observed minimum of the return data. As a consequence, in moving window approaches the entering or dropping out of large extreme returns from the data set can cause jumps in VaR. Hence, modifications were proposed. For instance, the return data can be pre-filtered with location-scale models described in the next paragraph. Based on this, i.i.d. disturbances of the return series can be obtained. Then, the i.i.d. disturbances can be bootstrapped to overcome the shortcomings. \\

%\paragraph{Fully Parametric Models}

The proposed VaR modeling framework is based on the location-scale approach. Models of this class estimate the entire distribution of asset returns and derive VaR as a quantile of that distribution \citep[e.g.,][]{Kuester.2005}. Such approaches assume the return process is described as

\begin{equation}
	r_t = \mu_t + u_t = \mu_t + \sigma_t z_t, \qquad z_t \sim (0,1) \ \text{i.i.d.}
	\label{Eq:location_scale_model}
\end{equation}

In (\ref{Eq:location_scale_model}), $\mu_t$ is the location and $\sigma_t > 0$ the scale parameter. Given $r_t$ belongs to the location-scale family and $F_z$ is the CDF of $z$, we can compute VaR as
 
\begin{equation}
	VaR_{t}^{\alpha} = -\left\{\mu_t + \sigma_tF^{-1}_{z}(\alpha)\right\}.
	\label{Eq:location_scale_var}
\end{equation}

\noindent Autoregressive moving average (ARMA) processes and GARCH-type models are commonly used to estimate $\mu_t$ and $\sigma_t$ in (\ref{Eq:location_scale_model}).

%\newline
%\noindent Standard dynamic feedback models estimate the distribution of a stochastic process as discrete mixture of normal distributions. Moreover, volatility can be modeled using a GARCH model. Let $u_t$ be generated by a conditionally heteroscedastic mixture of normal distributions. Further, let $w \in (0,1)^n$, $\mu \in \mathbb{R}^n$ and $\sigma_t \in \mathbb{R}_{>0}$. Then, 
%\begin{equation}
%u_t|\mathcal{F}_{t-1} \sim MN(w, \mu, \sigma_t^2) ,
%\end{equation}
%where MN denotes a mixture of normal distributions with density function 
%\begin{equation}
%f_{MN}(x, w, \mu, \sigma_t^2) = \sum_{i = 1}^{n} w_i \varphi (x, \mu_i, \sigma_{it}^2).
%\end{equation}
%Here, $\varphi$ is the probability density function of the normal distribution with $\sum_{i = 1}^{n} w_i = 1$ and $\mathcal{F}_{t-1}$ being the information set available at $t-1$. \cite{Kuester.2005} note that also mixtures of other distributions can be used. For instance, in their study they use the generalized exponential distribution and refer to literature where the t distribution was considered. 

%Assuming an unconditional model in equivalent in setting $\mu_t = \mu$ and $\sigma_t = \sigma$. Conditionally homoscedastic models incorporate the possibility of a time-varying conditional mean. Autoregressive moving average (ARMA) processes are a possible modeling approach. However, return series of financial time series are subject to volatility clustering. Hence, applying conditionally heteroscedastic models with a time-varying location and scale parameter are the most promising ones for VaR predictions.

%\paragraph{Extreme Value Theory} Procedures for modeling the tails rather than the entire distribution are developed in extreme value theory. There are two main approaches: block maxima (BM) and peaks over threshold (POT) models. \\
%
%\noindent To introduce the BM model let $M_n = \max\{X_1, \dots, X_n\}$ with $X_t$, $t = 1, \dots, n$, being i.i.d. random variables. For $c_n > 0$, $d_n \in \mathbb{R}$ and $G$ being a non-degenerate distribution, it holds that 
%\begin{equation}
%	\dfrac{M_n - d_n}{c_n} \xrightarrow{d} G \qquad \text{for} \ n \rightarrow \infty,
%\end{equation}
%where $G$ is the generalized extreme value distribution. Hence, sample maxima have only one class of limiting distributions. Based on this, VaR can be derived. \\
%
%\noindent POT models estimate the excess distribution $F_{\tau}$ of a random variable $X$ based on values exceeding a threshold $\tau$. Formally, $F_{\tau}$ is defined as   
%\begin{equation}
%	F_{\tau}(x) = \mathbb{P}(X - \tau \le x | X > \tau), \qquad x \ge 0.
%	\label{Eq:pot_excess_dist}
%\end{equation}
%Under this setting, the limiting distribution of scaled excesses is the generalized Pareto distribution. 
%
%
%\paragraph{Quantile Regression} 
%The aforementioned methods are based on modeling either the entire distribution or its tail. In contrast, quantile regression aims at estimating the quantile directly without considering other parts of the distribution. Hence, the $\alpha$-quantile of a random variable is modeled directly in dependence of explanatory variables $x_t \in \mathbb{R}^p$:   
%\begin{equation}
%		VaR_t^{\alpha} = -h_{\alpha}(x_t, \beta_{\alpha}).
%\end{equation}
%Note that the function $h(\cdot, \cdot)$ and parameter vector $\beta$ are depending directly on $\alpha$.
%
%%\cite{Abberger.1997} Kernel based forecast compared to GARCH. Did not compare results based on tests for the appropriateness of distribution. However, he compared the difference and found asymmetries by comparing the first and third quartile forecast showing asymetries in the data that can not be captured by normal distribution. -> Massive deviation. 

%\subsubsection{Approaches Related to Machine Learning}
%\subsection{Related Literature}
%
%In the domain of ML the literature for quantile estimation focuses mainly on neural networks (NN) and SVR. For instance, the derivation of a general approach without an explicit target application can be found in \cite{White.1992}. He used single hidden layer feedforward NNs to derive a way for nonparametric conditional quantile estimation and proved its consistency. However, the ML VaR literature is not as broad as in classical statistics. 
%Hence, this section also reviews literature where methods for the construction of prediction intervals (PI) were introduced that could be used in the estimation of VaR. Consequently, the reviewed literature is divided in three paragraphs: Prediction Intervals, Value-at-Risk and Data Driven Value-at-Risk. Here, the first two review the existing literature, whereas the last motivates the method proposed in this thesis. 
%
%%Hence, the literature is reviewed explicitly and the section is divided in three paragraphs: prediction intervals (PI), VaR and Data Driven VaR. Whereas the first two review the existing literature, the last motivates the method proposed in this thesis. 
%
%\paragraph{Prediction Intervals} General approaches are developed by \cite{Hwang.1997} who derive asymptotically valid PIs and \cite{Veaux.1998} who propose a method to estimate PIs for NNs with nonlinear regression. \cite{LinWeng.2004} use SVR to generate out-of-sample residuals via cross validation (CV) and fit those to a Laplace or normal distribution for generating PIs. The results are compared to Bayesian SVR and historical simulation. Despite the mixed results they stress the competitiveness of their method especially due to its simplicity. Pointwise and simultaneous confidence intervals as well as PIs with bias correction for least-squares-SVR are derived by \cite{Brabanter.2011}.  %based on Sidak corrections and upcrossing allowing for heteroscedasticiy and modifying it because of its convervativity% - > 
%However, in comparison to bootstrapping, their method is not superior in simulations. \cite{Khosravi.2013} introduce a framework for constructing PIs of electricity prices. They employ a resampling scheme based on a moving bootstrap approach for data blocks rather than single observations to account for possible correlations. Then, NNs are trained on the bootstrapped data sets to forecast the mean of the time series as center of the prediction interval. The variance is estimated based on a GARCH model but not in the framework of MLE. Instead, they use a cost function directly related to the PI quality that can be minimized with gradient-free algorithms. The resulting mean and variance are then used in a normal distribution to get the PIs. They find that their method has a computational advantage over traditional methods. Moreover, the PIs of their approach are more informative. \cite{Lins.2015} propose a method for confidence intervals and PIs by combining bootstrapping and SVR to bagged SVR in the context of component degradation prediction in the offshore oil industry. They show that their method works in the proposed application.
%
%\paragraph{Value-at-Risk} \cite{Franke.2006} estimate VaR for the German stock index (DAX) by fitting the mean and volatility of the return series with NNs. The mean is modeled autoregressively and the volatility is assumed to follow an autoregressive conditionally heteroscedastic (ARCH) process. Moreover, they include external regressors in both models. The predicted mean and variance are used with the normal distribution to derive the VaR and expected shortfall. As benchmark serves a standard GARCH model based on assuming normality of innovations. In terms of VaR exceedances their model is superior. Moreover, they note its ability to quickly adjust the volatility in case of shocks with only short impact. Another approach directly related to VaR is proposed by \cite{Dunis.2010} which use higher order NNs to forecast VaR. A hybrid model using higher order NNs for variance forecasting and RiskMetrics is shown to outperform other hybrid models empirically. They note also the relatively bad results of the unconditional POT method for quantile estimation. This is, however, not an appropriate comparison when benchmarked to conditional models as was e.g. shown by \cite{Kuester.2005}. \cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test. A multiperiod VaR model was introduced by \cite{Xu.2016}. They use an exponentially weighted support vector quantile regression. In the corresponding empirical study, their approach outperforms other methods that are based on GARCH models, filtered historical simulation and quantile regression. Evaluation was done with different measures as e.g. mean absolute error and p-values of prediction tests.
%  
%\paragraph{Data Driven Value-at-Risk} Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. By considering the model types in Section \ref{Sec:var_est_approaches}, they can be classified as quantile regression models. In the empirical study of  the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and POT had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. Most of the proposed methods in the ML literature for estimating VaR or PIs are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this thesis. Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions.
%

    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% EVALUATING VAR MODELS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%\subsection{Evaluating VaR-Models}
%
%\cite{Christoffersen.1998} proposes a framework for assessing interval forecasts and uses it for evaluating VaR models. This approach is also applied here. Let ${V_t = \mathbb{I}(r_t < -VaR_t^{\alpha})}$, with $t = 1, \dots, n$, be a series of VaR violations where $\mathbb{I}(x < c)$ denotes the indicator function:
%%Let $\{V_t\}_{t=1}^n$ be a series of VaR violations with $V_t = \mathbb{I}(r_t < -VaR_t^{\alpha})$ where $\mathbb{I}(x < c)$ denotes the indicator function: 
%\begin{equation}
%\mathbb{I}(x < c) = \begin{cases}
%1 \text{ \ if \ } x < c \\
%0 \text{ \ if \ } x \ge c. \\
%\end{cases} 
%\end{equation}
%
%\noindent Moreover, let $\mathcal{F}_{t-1}$ be the information set available at time ${t-1}$. Then, according to \cite{Christoffersen.1998} a VaR forecast model is efficient if
%
%\begin{equation}
%\mathbb{E}[V_t | \mathcal{F}_{t-1}] = \alpha.
%\label{Eq:chris_mdl_eff}
%\end{equation}
%
%\noindent \cite{Kuester.2005} note that (\ref{Eq:chris_mdl_eff}) implies that $V_t$ is uncorrelated with any function of a variable contained in $\mathcal{F}_{t-1}$. Additionally, under (\ref{Eq:chris_mdl_eff}) VaR models exhibit conditionally and unconditionally the correct number of violations. Consequently, they are optimal because no further improvement is possible. Moreover, \cite{Christoffersen.1998} proves that for $\{V_1, V_2, \dots, V_{t-1} \} \subseteq \mathcal{F}_{t-1}$ the following holds:
%
%\begin{equation}
%V_t | \mathcal{F}_{t-1} \sim Bern(\alpha) \quad \text{i.i.d.},
%\label{Eq:eval_cc_bern}
%\end{equation}
%
%\noindent which is considered as correct conditional coverage. Here, $Bern$ denotes the Bernoulli distribution. Based on this, \cite{Christoffersen.1998} derives a testing framework by combining three likelihood ratio (LR) tests to evaluate the correct unconditional coverage, independence of violations and correct conditional coverage of interval forecasts. The use of this approach is appealing because it allows to evaluate VaR models from different perspectives. 
%
%\subsubsection{Test for Correct Unconditional Coverage}
%
%The test for correct unconditional coverage is used to examine whether the relative number of VaR violations is appropriate for the chosen $\alpha$. By the law of iterated expectations it can be shown that (\ref{Eq:chris_mdl_eff}) implies correct unconditional coverage, i.e.
%
%\begin{equation}
%\mathbb{E}[V_t] = \alpha.
%\end{equation}
%
%\noindent To test for the correct number of violations, the following hypotheses are stated:
%
%\begin{equation}
%\text{H}_0: \mathbb{E}[V_t] = \alpha \qquad \text{vs.} \qquad \text{H}_1: \mathbb{E}[V_t] \ne \alpha.
%\end{equation}
%
%\noindent Since $V_t$ has a Bernoulli distribution under $\text{H}_0$, the corresponding likelihood is with $n$ denoting the sample size and $n_1$ being the number of VaR violations
%
%\begin{equation}
%	L(\alpha; V_1, V_2, \dots, V_{n}) = (1 - \alpha)^{n - n_1} \alpha^{n_1}. 
%	\label{Eq:ll_uc_h0}
%\end{equation} 
%
%\noindent The maximum likelihood estimate of $\alpha$ based on (\ref{Eq:ll_uc_h0}) is obtained as
%
%\begin{equation}
%\hat{\alpha} = \dfrac{n_1}{n}.
%\end{equation}
%
%\noindent Denote the log-likelihood function as $\mathcal{L}(\cdot) = \log L(\cdot)$. Then, by plugging $\hat{\alpha}$ into (\ref{Eq:ll_uc_h0}), the following result can be used to perform a LR test for correct unconditional coverage: 
%\begin{equation}
%\text{LR}_{\tiny\text{UC}} = 2\left[\mathcal{L}(\hat{\alpha}; V_1, V_2, \dots, V_n) - \mathcal{L}(\alpha; V_1, V_2, \dots, V_n) \right] \stackrel{\text{asy}}{\sim}  \mathcal{X}^2_1.
%\label{Eq:lr_uc}
%\end{equation} 
%
%\noindent Here, $\mathcal{X}^2_1$ denotes the $\mathcal{X}^2$ distribution with one degree of freedom. In (\ref{Eq:lr_uc}) only the number of violations is considered. However, it is not tested for the existence of violation clusters, i.e. dependence of the violations. As a consequence, a model can have optimal unconditional coverage even though it does not appropriately adjust for changed market risk. Testing for unconditional coverage is, therefore, not sufficient for appropriately evaluating the model. For instance, if the market risk increases and more violations occur, the model should adjust accordingly by forecasting higher VaR values. By taking this into account, \cite{Christoffersen.1998} introduces also a test for the independence of violations which is presented below. 
%
%%\noindent Here, $\hat{\alpha}$ is the maximum likelihood estimate of $\alpha$ which in case of a Bernoulli distribution is 
%
%%\begin{equation}
%%\hat{\alpha} = \dfrac{n_1}{n_0 + n_1}
%%\end{equation}
%%
%%\noindent where the denominator corresponds to the total number of observations and the numerator to number of exceedances. 
%
%\subsubsection{Test for Independence of Violations}
%
%%In the next step, \cite{Christoffersen.1998} introduces a framework for testing the independence of interval forecasts. \cite{Kuester.2005} notes that taking the independence of VaR forecasts into account is important for avoiding violation clusters. Testing for unconditional coverage is, therefore, not sufficient for appropriately evaluating the model.
%To test for independence of VaR violations assume $V_t$ is a binary first-order Markov chain. Define the transition probability matrix of $V_t$ as
% 
% \begin{equation}
% \Pi_1 = \begin{bmatrix}
% 1 - \pi_{01} & \pi_{01} \\
% 1 - \pi_{11} & \pi_{11} 
% \end{bmatrix}
% \end{equation}
% 
% \noindent where 
% 
% \begin{equation}
% \pi_{ij} = \mathbb{P}(V_t = j | V_{t-1} = i).
% \end{equation}
% 
% \noindent \cite{Christoffersen.1998} states the approximate likelihood function of $V_t$ as 
%
%\begin{equation}
%L(\Pi_1; V_1, \dots, V_n) = (1 - \pi_{01})^{n_{00}} \pi_{01}^{n_{01}} (1 - \pi_{11})^{n_{10}} \pi_{11}^{n_{11}}.
%\label{Eq:ll_indep}
%\end{equation}
%
%\noindent Here, $n_{ij}$ denotes the number of observations where state $i$ was followed by state $j$:
%
%\begin{equation}
%n_{ij} = \sum_{t = 2}^{n} \mathbb{I}(V_t = i| V_{t-1} = j).
%\end{equation}
%
%\noindent An estimate for $\Pi_1$ is obtained by conditioning (\ref{Eq:ll_indep}) on $V_1$ everywhere and maximizing the corresponding log-likelihood function. Then, the resulting maximum likelihood estimates are 
%
%\begin{equation}
%\hat{\pi}_{01} = \dfrac{n_{01}}{n_{00} + n_{01}} \qquad \text{and} \qquad \hat{\pi}_{11} = \dfrac{n_{11}}{n_{10} + n_{11}}.
%\label{Eq:ml_indep_tprob}
%\end{equation}
%
%\noindent Under the null hypothesis that the observed violations $V_t$ are independent, the transition probabilities $\pi_{01}$ and $\pi_{11}$ are equal such that the transition probability matrix becomes 
%
%\begin{equation}
%\Pi_2 = \begin{bmatrix}
%1 - \pi_{0} & \pi_{0} \\
%1 - \pi_{0} & \pi_{0} 
%\end{bmatrix}
%\end{equation}
%
%\noindent where $\pi_0 = \pi_{01} = \pi_{11}$. \noindent Hence, the hypotheses corresponding to the test of independent violations can be stated as follows: 
%
%\begin{equation}
%\text{H}_0: \pi_{01} = \pi_{11} \qquad \text{vs.} \qquad \text{H}_1: \pi_{01} \ne \pi_{11}.
%\end{equation}
%
%\noindent Consequently, the likelihood function corresponding to $\text{H}_0$ is  
%
%\begin{equation}
%L(\Pi_2; V_1, V_2, \dots, V_n) = (1 - \pi_{0})^{n_{00} + n_{10}} \pi_{0}^{n_{01} + n_{11}}
%\label{Eq:ll_indep_null}
%\end{equation}
%
%\noindent with the maximum likelihood estimate 
%
%\begin{equation}
%\hat{\pi}_{0} = \dfrac{n_{01} + n_{11}}{n_{00} + n_{10} + n_{01} + n_{11}}. %=  \dfrac{T_{01} + T_{11}}{T - 1}.
%\end{equation}
%
%
%\noindent \cite{HOEL.1954} derives the LR test statistic as a goodness of fit measure for Markov chains with unknown transition probabilities. Based on this work, \cite{Christoffersen.1998} concludes that the LR test statistic for independence has asymptotically a $\mathcal{X}^2$ distribution with one degree of freedom:
%
%\begin{equation}
%\text{LR}_{\text{ID}} = 2\left[\mathcal{L}\left(\widehat{\Pi}_1; V_1, V_2, \dots, V_n\right) - \mathcal{L}\left(\widehat{\Pi}_2; V_1, V_2, \dots, V_n \right) \right] \stackrel{\text{asy}}{\sim}  \mathcal{X}^2_1.
%\label{Eq:lr_ind}
%\end{equation} 
%
%\noindent Equation (\ref{Eq:lr_ind}) does not depend on the true coverage. Hence, it is limited to testing for independence. However, \cite{Christoffersen.1998} stresses the test's usefulness for assessing the dynamics of interval forecasts which is possible even though the true error distribution is unknown. \\
%
%\noindent \cite{Christoffersen.2004} notes that especially for low $\alpha$ or small samples it is likely that $n_{11} = 0$. Consequently, also $\hat{\pi}_{11}$ and (\ref{Eq:ll_indep}) will be zero. Since $\log(0)$ is not defined, (\ref{Eq:lr_ind}) cannot be computed. To overcome this limitation, \cite{Christoffersen.2004} suggests to use the following modification of (\ref{Eq:ll_indep}) if $n_{11} = 0$: 
%
% \begin{equation}
% L(\Pi_1; V_1, V_2, \dots, V_n) = (1 - \pi_{01})^{n_{00}} \pi_{01}^{n_{01}}.
% \label{Eq:modification_ll_ind}
% \end{equation}
%
%\noindent This modification is used in the empirical study in Section \ref{Sec:emp_study}.
%
%
%\subsubsection{Test for Correct Conditional Coverage}
%
%Ideally, a model for forecasting VaR combines the ability to capture temporarily changing market risk regimes and has correct coverage. Although (\ref{Eq:lr_ind}) accounts for the former, it does not for the latter. However, both abilities can be assessed by introducing a test for correct conditional coverage. By combining (\ref{Eq:lr_uc}) and (\ref{Eq:lr_ind}), \cite{Christoffersen.1998} derives the following likelihood ratio test statistic for correct conditional coverage:
%
%\begin{equation}
%\text{LR}_{\text{CC}} = 2\left[ \mathcal{L}(\hat{\Pi}_1; V_1, V_2, \dots, V_n) - \mathcal{L}(\alpha; V_1, V_2, \dots, V_n) \right] \stackrel{\text{asy}}{\sim}  \mathcal{X}^2_2.
%\label{Eq:LR_cc}
%\end{equation}
%
%\noindent Note that (\ref{Eq:LR_cc}) is asymptotically $\mathcal{X}^2$ distributed with two degrees of freedom. Moreover, \cite{Christoffersen.1998} points out that from conditioning on $V_1$ in (\ref{Eq:lr_uc}) it follows that $\hat{\alpha} = \hat{\pi}_0$. Then, by neglecting $V_1$, $\text{LR}_{\text{CC}}$ can be rewritten as
%
%\begin{equation}
%\text{LR}_{\text{CC}} = \text{LR}_{\text{UC}} + \text{LR}_{\text{ID}}.
%\label{Eq:LR_cc_re}
%\end{equation}
%
%\noindent Rewriting (\ref{Eq:LR_cc}) as (\ref{Eq:LR_cc_re}) makes it possible to evaluate whether the performance of a VaR model in terms of correct conditional coverage is determined by its ability to achieve correct coverage or adjust for changing volatility. This is useful in situations where $\text{LR}_{\text{CC}}$ is relatively small but only one of the test statistics, i.e. $\text{LR}_{\text{UC}}$ or $\text{LR}_{\text{ID}}$, is small. Then, it is easier to appropriately adjust the model.
%
%%\subsection{Other Risk Measures}
%


==> Tables/Case_1/Archiv/Results_Case1_10Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:13:17 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 1 & 1.03 & 90.58 & 30.09 & 29.88 & 13.8 \\ 
  SVR-KDE & S\&P500 & 1 & 0.95 & 86.85 & 25.94 & 25.59 & 58.2 \\ 
  GARCH-SSTD & S\&P500 & 1 & 1.19 & 50.57 & 3.91 & 3.14 & 9.2 \\ 
  TGARCH-STD & S\&P500 & 1 & 1.99 & 0.19 & 25.26 & 0.21 & 0.8 \\ 
  GARCH-STD & S\&P500 & 1 & 1.99 & 0.19 & 25.26 & 0.21 & 3.8 \\ 
  TGARCH-NORM & S\&P500 & 1 & 2.31 & 0.01 & 39.72 & 0.01 & 3 \\ 
  GARCH-NORM & S\&P500 & 1 & 2.54 & 0 & 51.83 & 0 & 2.6 \\ 
  EGARCH-STD & S\&P500 & 1 & 2.78 & 0 & 64.14 & 0 & 0 \\ 
  EGARCH-SSTD & S\&P500 & 1 & 2.7 & 0 & 4.5 & 0 & 0.6 \\ 
  EGARCH-NORM & S\&P500 & 1 & 3.26 & 0 & 14.87 & 0 & 0.6 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1 & 1.45 & 13.59 & 52.97 & 17.42 & 2.6 \\ 
  GARCH-SSTD & Nikkei225 & 1 & 1.45 & 13.59 & 52.97 & 17.42 & 2.8 \\ 
  SVR-KDE & Nikkei225 & 1 & 0.32 & 0.51 & 87.23 & 1.97 & 0 \\ 
  GARCH-STD & Nikkei225 & 1 & 1.85 & 0.7 & 19.57 & 0.51 & 1.2 \\ 
  TGARCH-STD & Nikkei225 & 1 & 1.93 & 0.34 & 22.56 & 0.31 & 2 \\ 
  GARCH-NORM & Nikkei225 & 1 & 2.01 & 0.16 & 25.77 & 0.18 & 2.2 \\ 
  TGARCH-NORM & Nikkei225 & 1 & 2.09 & 0.07 & 5.45 & 0.02 & 2.2 \\ 
  EGARCH-STD & Nikkei225 & 1 & 3.95 & 0 & 75.92 & 0 & 0.2 \\ 
  EGARCH-SSTD & Nikkei225 & 1 & 2.5 & 0 & 48.53 & 0 & 0.8 \\ 
  EGARCH-NORM & Nikkei225 & 1 & 2.58 & 0 & 15.65 & 0 & 1.4 \\ 
   \hline
\hline
SVR-KDE & EuroStoxx50 & 1 & 0.97 & 90.41 & 62.85 & 88.31 & 0 \\ 
  GARCH-SSTD & EuroStoxx50 & 1 & 2.01 & 0.16 & 25.77 & 0.18 & 9.6 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1 & 2.33 & 0.01 & 40.43 & 0.01 & 6.2 \\ 
  TGARCH-STD & EuroStoxx50 & 1 & 2.58 & 0 & 15.65 & 0 & 6.8 \\ 
  TGARCH-NORM & EuroStoxx50 & 1 & 2.66 & 0 & 18.07 & 0 & 5.8 \\ 
  GARCH-STD & EuroStoxx50 & 1 & 2.33 & 0.01 & 9.64 & 0 & 7.4 \\ 
  GARCH-NORM & EuroStoxx50 & 1 & 2.58 & 0 & 15.65 & 0 & 1.4 \\ 
  EGARCH-STD & EuroStoxx50 & 1 & 4.03 & 0 & 17.32 & 0 & 1.4 \\ 
  EGARCH-SSTD & EuroStoxx50 & 1 & 3.7 & 0 & 2.49 & 0 & 1.2 \\ 
  EGARCH-NORM & EuroStoxx50 & 1 & 3.3 & 0 & 44.47 & 0 & 0.6 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> Tables/Case_1/Archiv/Results_Case1_10Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:13:17 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 2.5 & 2.62 & 78.12 & 55.96 & 53.84 & 10.8 \\ 
  GARCH-SSTD & S\&P500 & 2.5 & 2.78 & 52.88 & 22.94 & 18.81 & 3.6 \\ 
  GARCH-STD & S\&P500 & 2.5 & 3.18 & 13.82 & 39.68 & 13.22 & 3.6 \\ 
  TGARCH-STD & S\&P500 & 2.5 & 3.42 & 4.8 & 51.32 & 7.27 & 0.8 \\ 
  GARCH-NORM & S\&P500 & 2.5 & 3.58 & 2.14 & 59.33 & 4.2 & 1 \\ 
  SVR-KDE & S\&P500 & 2.5 & 1.75 & 7.15 & 16.45 & 3.24 & 55.8 \\ 
  TGARCH-NORM & S\&P500 & 2.5 & 3.58 & 2.14 & 25.03 & 1.77 & 0.8 \\ 
  EGARCH-STD & S\&P500 & 2.5 & 4.37 & 0.01 & 30.25 & 0.02 & 0.2 \\ 
  EGARCH-SSTD & S\&P500 & 2.5 & 4.77 & 0 & 22.74 & 0 & 0 \\ 
  EGARCH-NORM & S\&P500 & 2.5 & 4.61 & 0 & 17.75 & 0 & 0 \\ 
   \hline
\hline
GARCH-STD & Nikkei225 & 2.5 & 2.74 & 59.74 & 60.95 & 53.02 & 0.6 \\ 
  GARCH-SSTD & Nikkei225 & 2.5 & 2.25 & 57.31 & 36.53 & 31.17 & 8.6 \\ 
  GARCH-NORM & Nikkei225 & 2.5 & 3.3 & 8.45 & 86.53 & 19.54 & 0 \\ 
  TGARCH-SSTD & Nikkei225 & 2.5 & 2.74 & 59.74 & 20.72 & 18.02 & 0 \\ 
  TGARCH-STD & Nikkei225 & 2.5 & 3.06 & 22.21 & 33.3 & 15.8 & 0 \\ 
  TGARCH-NORM & Nikkei225 & 2.5 & 3.46 & 3.99 & 52.4 & 6.35 & 0 \\ 
  EGARCH-SSTD & Nikkei225 & 2.5 & 4.03 & 0.15 & 43.03 & 0.28 & 0.2 \\ 
  EGARCH-NORM & Nikkei225 & 2.5 & 4.11 & 0.09 & 46.87 & 0.19 & 0 \\ 
  SVR-KDE & Nikkei225 & 2.5 & 1.29 & 0.26 & 5.17 & 0.06 & 7 \\ 
  EGARCH-STD & Nikkei225 & 2.5 & 5.31 & 0 & 96.4 & 0 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.5 & 3.22 & 11.91 & 40.62 & 12.06 & 49.2 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.5 & 3.3 & 8.45 & 44.47 & 10.04 & 49.8 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.5 & 3.38 & 5.87 & 48.4 & 8.11 & 8.2 \\ 
  GARCH-STD & EuroStoxx50 & 2.5 & 3.46 & 3.99 & 52.4 & 6.35 & 9.4 \\ 
  SVR-KDE & EuroStoxx50 & 2.5 & 3.06 & 22.21 & 9.73 & 4.61 & 61 \\ 
  TGARCH-STD & EuroStoxx50 & 2.5 & 3.46 & 3.99 & 20.23 & 2.45 & 12.2 \\ 
  GARCH-NORM & EuroStoxx50 & 2.5 & 3.78 & 0.7 & 68.4 & 1.8 & 0.2 \\ 
  EGARCH-STD & EuroStoxx50 & 2.5 & 5.88 & 0 & 43.78 & 0 & 0.4 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.5 & 4.91 & 0 & 3.67 & 0 & 0.4 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.5 & 4.83 & 0 & 23.77 & 0 & 0 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> Tables/Case_1/Archiv/Results_Case1_10Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:13:17 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
TGARCH-NORM & S\&P500 & 5 & 5.09 & 88.72 & 34.98 & 34.63 & 1.2 \\ 
  TGARCH-STD & S\&P500 & 5 & 5.01 & 98.97 & 31.66 & 31.66 & 0 \\ 
  GARCH-SSTD & S\&P500 & 5 & 4.29 & 23.85 & 57.38 & 28.64 & 1.8 \\ 
  GARCH-STD & S\&P500 & 5 & 5.17 & 78.7 & 17.88 & 17.24 & 0.2 \\ 
  TGARCH-SSTD & S\&P500 & 5 & 4.21 & 18.86 & 24.22 & 10.2 & 5 \\ 
  GARCH-NORM & S\&P500 & 5 & 5.48 & 43.69 & 4.89 & 3.62 & 0.2 \\ 
  EGARCH-NORM & S\&P500 & 5 & 6.52 & 1.8 & 29.69 & 1.81 & 0 \\ 
  EGARCH-STD & S\&P500 & 5 & 6.6 & 1.3 & 32.87 & 1.5 & 0 \\ 
  SVR-KDE & S\&P500 & 5 & 3.34 & 0.41 & 17.11 & 0.28 & 5 \\ 
  EGARCH-SSTD & S\&P500 & 5 & 7.23 & 0.06 & 62.62 & 0.18 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 5 & 5.23 & 70.78 & 94.63 & 88.21 & 16 \\ 
  GARCH-SSTD & Nikkei225 & 5 & 4.99 & 98.96 & 87.41 & 87.4 & 20.4 \\ 
  TGARCH-STD & Nikkei225 & 5 & 5.31 & 61.51 & 72.91 & 64.25 & 8.8 \\ 
  TGARCH-NORM & Nikkei225 & 5 & 5.31 & 61.51 & 72.91 & 64.25 & 7 \\ 
  GARCH-NORM & Nikkei225 & 5 & 5.72 & 25.68 & 99.95 & 52.55 & 6.8 \\ 
  GARCH-STD & Nikkei225 & 5 & 5.72 & 25.68 & 89.19 & 46.89 & 6.4 \\ 
  SVR-KDE & Nikkei225 & 5 & 3.95 & 7.7 & 75.92 & 15.9 & 46.4 \\ 
  EGARCH-SSTD & Nikkei225 & 5 & 6.36 & 3.44 & 90.35 & 9.65 & 0.2 \\ 
  EGARCH-NORM & Nikkei225 & 5 & 6.12 & 7.99 & 31.6 & 6.82 & 2.2 \\ 
  EGARCH-STD & Nikkei225 & 5 & 7.97 & 0 & 91.62 & 0 & 0 \\ 
   \hline
\hline
SVR-KDE & EuroStoxx50 & 5 & 5.07 & 90.69 & 61.34 & 60.92 & 4 \\ 
  TGARCH-NORM & EuroStoxx50 & 5 & 6.12 & 7.99 & 6.55 & 1.41 & 3.8 \\ 
  TGARCH-SSTD & EuroStoxx50 & 5 & 6.12 & 7.99 & 2.43 & 0.53 & 3.6 \\ 
  TGARCH-STD & EuroStoxx50 & 5 & 6.36 & 3.44 & 4.28 & 0.46 & 0.4 \\ 
  GARCH-NORM & EuroStoxx50 & 5 & 6.36 & 3.44 & 4.28 & 0.46 & 1 \\ 
  GARCH-SSTD & EuroStoxx50 & 5 & 6.52 & 1.85 & 6.06 & 0.38 & 1.8 \\ 
  GARCH-STD & EuroStoxx50 & 5 & 6.76 & 0.67 & 9.76 & 0.25 & 0.4 \\ 
  EGARCH-STD & EuroStoxx50 & 5 & 9.1 & 0 & 1.03 & 0 & 0.2 \\ 
  EGARCH-SSTD & EuroStoxx50 & 5 & 7.41 & 0.03 & 0.13 & 0 & 0.2 \\ 
  EGARCH-NORM & EuroStoxx50 & 5 & 7.17 & 0.1 & 0.18 & 0 & 0.8 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> Tables/Case_1/Archiv/Results_Case1_1Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:10:35 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
EGARCH-SSTD & S\&P500 & 1 & 1.11 & 69.27 & 57.46 & 79.01 & 6.2 \\ 
  TGARCH-SSTD & S\&P500 & 1 & 0.72 & 28.52 & 71.87 & 52.94 & 64.4 \\ 
  GARCH-SSTD & S\&P500 & 1 & 1.27 & 35.24 & 43.34 & 28.13 & 23.6 \\ 
  TGARCH-STD & S\&P500 & 1 & 1.43 & 14.91 & 46.97 & 27.2 & 0.8 \\ 
  SVR-KDE & S\&P500 & 1 & 0.79 & 44.83 & 18.28 & 13.71 & 28.8 \\ 
  GARCH-STD & S\&P500 & 1 & 1.67 & 2.95 & 65.77 & 6.15 & 14.4 \\ 
  EGARCH-STD & S\&P500 & 1 & 1.75 & 1.58 & 37.62 & 3.67 & 7.2 \\ 
  TGARCH-NORM & S\&P500 & 1 & 2.15 & 0.04 & 27.64 & 0.1 & 3.6 \\ 
  EGARCH-NORM & S\&P500 & 1 & 2.23 & 0.02 & 25.88 & 0.04 & 2 \\ 
  GARCH-NORM & S\&P500 & 1 & 2.38 & 0 & 94.85 & 0.01 & 0.8 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1 & 1.21 & 47.61 & 54.48 & 64.58 & 5 \\ 
  GARCH-SSTD & Nikkei225 & 1 & 1.21 & 47.61 & 54.48 & 64.58 & 4.2 \\ 
  EGARCH-SSTD & Nikkei225 & 1 & 1.37 & 21.61 & 49.21 & 36.76 & 6.8 \\ 
  GARCH-STD & Nikkei225 & 1 & 1.69 & 2.6 & 66.33 & 5.56 & 2.6 \\ 
  TGARCH-STD & Nikkei225 & 1 & 1.77 & 1.37 & 37.3 & 3.23 & 0.8 \\ 
  SVR-KDE & Nikkei225 & 1 & 0.24 & 0.13 & 90.41 & 0.55 & 0 \\ 
  EGARCH-STD & Nikkei225 & 1 & 2.09 & 0.07 & 29.17 & 0.19 & 1.4 \\ 
  GARCH-NORM & Nikkei225 & 1 & 2.17 & 0.03 & 88.16 & 0.14 & 0.8 \\ 
  TGARCH-NORM & Nikkei225 & 1 & 2.33 & 0.01 & 93.19 & 0.03 & 0.2 \\ 
  EGARCH-NORM & Nikkei225 & 1 & 2.42 & 0 & 95.21 & 0.01 & 0.2 \\ 
   \hline
\hline
SVR-KDE & EuroStoxx50 & 1 & 1.53 & 8.17 & 44.23 & 16.36 & 67 \\ 
  GARCH-SSTD & EuroStoxx50 & 1 & 1.69 & 2.6 & 39.54 & 5.84 & 74.6 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1 & 1.69 & 2.6 & 66.33 & 5.56 & 44.2 \\ 
  TGARCH-STD & EuroStoxx50 & 1 & 1.77 & 1.37 & 70.53 & 3.39 & 1.2 \\ 
  GARCH-STD & EuroStoxx50 & 1 & 1.85 & 0.7 & 35.15 & 1.7 & 1.2 \\ 
  TGARCH-NORM & EuroStoxx50 & 1 & 2.09 & 0.07 & 85.17 & 0.28 & 0.8 \\ 
  GARCH-NORM & EuroStoxx50 & 1 & 2.17 & 0.03 & 27.33 & 0.08 & 5.2 \\ 
  EGARCH-STD & EuroStoxx50 & 1 & 2.33 & 0.01 & 93.19 & 0.03 & 12.4 \\ 
  EGARCH-SSTD & EuroStoxx50 & 1 & 2.42 & 0 & 95.21 & 0.01 & 2.8 \\ 
  EGARCH-NORM & EuroStoxx50 & 1 & 2.5 & 0 & 96.87 & 0 & 3.8 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> Tables/Case_1/Archiv/Results_Case1_1Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:10:35 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 2.5 & 2.62 & 78.12 & 98.97 & 95.22 & 30.6 \\ 
  EGARCH-SSTD & S\&P500 & 2.5 & 3.02 & 25.18 & 98.94 & 51.31 & 0.6 \\ 
  TGARCH-SSTD & S\&P500 & 2.5 & 2.38 & 79.19 & 22.6 & 46.4 & 61.8 \\ 
  GARCH-STD & S\&P500 & 2.5 & 3.5 & 3.24 & 93.45 & 9.47 & 2.8 \\ 
  GARCH-NORM & S\&P500 & 2.5 & 3.82 & 0.55 & 99.2 & 2.1 & 1 \\ 
  SVR-KDE & S\&P500 & 2.5 & 1.43 & 0.83 & 52.45 & 1.62 & 34.2 \\ 
  TGARCH-STD & S\&P500 & 2.5 & 3.9 & 0.33 & 75.52 & 1.02 & 0.2 \\ 
  TGARCH-NORM & S\&P500 & 2.5 & 4.05 & 0.12 & 69.37 & 0.36 & 0.4 \\ 
  EGARCH-STD & S\&P500 & 2.5 & 4.37 & 0.01 & 96.11 & 0.06 & 0 \\ 
  EGARCH-NORM & S\&P500 & 2.5 & 4.53 & 0 & 92.48 & 0.02 & 0.2 \\ 
   \hline
\hline
GARCH-SSTD & Nikkei225 & 2.5 & 2.9 & 38.01 & 99.9 & 67.96 & 44.2 \\ 
  TGARCH-SSTD & Nikkei225 & 2.5 & 2.42 & 84.78 & 22.29 & 46.72 & 69.6 \\ 
  TGARCH-STD & Nikkei225 & 2.5 & 3.14 & 16.44 & 97.67 & 37.15 & 2 \\ 
  TGARCH-NORM & Nikkei225 & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 & 0.4 \\ 
  EGARCH-NORM & Nikkei225 & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 & 0.6 \\ 
  GARCH-NORM & Nikkei225 & 2.5 & 3.38 & 5.87 & 92.85 & 15.55 & 0.2 \\ 
  GARCH-STD & Nikkei225 & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 & 0 \\ 
  EGARCH-SSTD & Nikkei225 & 2.5 & 3.06 & 22.21 & 12.14 & 14.3 & 17.4 \\ 
  SVR-KDE & Nikkei225 & 2.5 & 1.69 & 5.26 & 14.27 & 2.18 & 59 \\ 
  EGARCH-STD & Nikkei225 & 2.5 & 3.86 & 0.43 & 99.42 & 1.68 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.5 & 2.98 & 29.36 & 72.9 & 42 & 71.8 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.5 & 3.22 & 11.91 & 83.46 & 24.78 & 0.2 \\ 
  TGARCH-STD & EuroStoxx50 & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 & 0 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.5 & 3.46 & 3.99 & 91.84 & 11.13 & 73.4 \\ 
  SVR-KDE & EuroStoxx50 & 2.5 & 3.14 & 16.44 & 11.43 & 4.35 & 34.2 \\ 
  GARCH-STD & EuroStoxx50 & 2.5 & 3.7 & 1.11 & 97.42 & 3.88 & 3.4 \\ 
  GARCH-NORM & EuroStoxx50 & 2.5 & 3.95 & 0.26 & 75.92 & 0.81 & 6 \\ 
  EGARCH-STD & EuroStoxx50 & 2.5 & 4.27 & 0.03 & 88.73 & 0.12 & 0.6 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.5 & 4.51 & 0 & 95.5 & 0.02 & 1.6 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.5 & 4.59 & 0 & 97.11 & 0.01 & 1 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> Tables/Case_1/Archiv/Results_Case1_1Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:10:35 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 5 & 5.01 & 98.97 & 89.07 & 89.06 & 62.8 \\ 
  GARCH-NORM & S\&P500 & 5 & 5.72 & 24.94 & 99.79 & 51.4 & 0.2 \\ 
  TGARCH-SSTD & S\&P500 & 5 & 5.41 & 51.47 & 60.38 & 48.83 & 62.6 \\ 
  GARCH-STD & S\&P500 & 5 & 5.8 & 20.21 & 99.23 & 43.99 & 2.8 \\ 
  SVR-KDE & S\&P500 & 5 & 4.37 & 29.68 & 30.25 & 17.55 & 26.4 \\ 
  EGARCH-SSTD & S\&P500 & 5 & 6.44 & 2.47 & 83.92 & 6.73 & 0.4 \\ 
  TGARCH-NORM & S\&P500 & 5 & 6.6 & 1.3 & 77.88 & 3.56 & 0.4 \\ 
  EGARCH-NORM & S\&P500 & 5 & 6.76 & 0.65 & 94.35 & 2.33 & 0.8 \\ 
  TGARCH-STD & S\&P500 & 5 & 6.76 & 0.65 & 71.36 & 1.77 & 0 \\ 
  EGARCH-STD & S\&P500 & 5 & 7 & 0.21 & 87.46 & 0.78 & 0.6 \\ 
   \hline
\hline
EGARCH-SSTD & Nikkei225 & 5 & 5.23 & 70.78 & 97.26 & 90.66 & 13 \\ 
  SVR-KDE & Nikkei225 & 5 & 4.59 & 50.1 & 97.11 & 77.43 & 35.2 \\ 
  TGARCH-SSTD & Nikkei225 & 5 & 4.67 & 58.95 & 89.41 & 77.3 & 72.8 \\ 
  GARCH-SSTD & Nikkei225 & 5 & 5.07 & 90.69 & 75.29 & 74.78 & 34 \\ 
  TGARCH-NORM & Nikkei225 & 5 & 5.23 & 70.78 & 68.85 & 64.18 & 0 \\ 
  TGARCH-STD & Nikkei225 & 5 & 5.56 & 37.71 & 89.62 & 60.67 & 0 \\ 
  GARCH-NORM & Nikkei225 & 5 & 5.88 & 16.68 & 78.41 & 30.16 & 4 \\ 
  EGARCH-NORM & Nikkei225 & 5 & 5.72 & 25.68 & 49.18 & 25.85 & 0 \\ 
  GARCH-STD & Nikkei225 & 5 & 6.04 & 10.34 & 71.98 & 19.11 & 0 \\ 
  EGARCH-STD & Nikkei225 & 5 & 6.04 & 10.34 & 71.98 & 19.11 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 5 & 5.15 & 80.55 & 65.27 & 63.32 & 70.6 \\ 
  GARCH-SSTD & EuroStoxx50 & 5 & 5.96 & 13.21 & 95.83 & 30.84 & 56.8 \\ 
  GARCH-NORM & EuroStoxx50 & 5 & 5.96 & 13.21 & 95.83 & 30.84 & 47.2 \\ 
  TGARCH-NORM & EuroStoxx50 & 5 & 6.04 & 10.34 & 78.1 & 20.73 & 2.2 \\ 
  SVR-KDE & EuroStoxx50 & 5 & 5.48 & 44.9 & 26.86 & 20.17 & 29.6 \\ 
  EGARCH-SSTD & EuroStoxx50 & 5 & 6.12 & 7.99 & 68.65 & 14.82 & 1.2 \\ 
  TGARCH-STD & EuroStoxx50 & 5 & 6.2 & 6.11 & 59.29 & 10.26 & 0 \\ 
  EGARCH-NORM & EuroStoxx50 & 5 & 6.52 & 1.85 & 99.1 & 6.18 & 1.6 \\ 
  GARCH-STD & EuroStoxx50 & 5 & 6.6 & 1.33 & 96.58 & 4.52 & 3.8 \\ 
  EGARCH-STD & EuroStoxx50 & 5 & 6.84 & 0.46 & 69.51 & 1.27 & 0.8 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> Tables/Case_1/Archive2/Results_Case1_10Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:36:26 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 1.03 & 11.78 & 90.58 & 30.09 & 29.88 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.95 & 94.01 & 86.85 & 25.94 & 25.59 \\ 
  GARCH-SSTD & S\&P500 & 1.19 & 10.38 & 50.57 & 3.91 & 3.14 \\ 
  TGARCH-STD & S\&P500 & 1.99 & 1.80 & 0.19 & 25.26 & 0.21 \\ 
  GARCH-STD & S\&P500 & 1.99 & 2.99 & 0.19 & 25.26 & 0.21 \\ 
  TGARCH-NORM & S\&P500 & 2.31 & 3.59 & 0.01 & 39.72 & 0.01 \\ 
  GARCH-NORM & S\&P500 & 2.54 & 3.39 & 0.00 & 51.83 & 0.00 \\ 
  EGARCH-STD & S\&P500 & 2.78 & 0.00 & 0.00 & 64.14 & 0.00 \\ 
  EGARCH-SSTD & S\&P500 & 2.70 & 0.80 & 0.00 & 4.50 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 3.26 & 0.60 & 0.00 & 14.87 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.45 & 3.19 & 13.59 & 52.97 & 17.42 \\ 
  GARCH-SSTD & Nikkei225 & 1.45 & 2.40 & 13.59 & 52.97 & 17.42 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.32 & 57.29 & 0.51 & 87.23 & 1.97 \\ 
  GARCH-STD & Nikkei225 & 1.85 & 0.80 & 0.70 & 19.57 & 0.51 \\ 
  TGARCH-STD & Nikkei225 & 1.93 & 1.80 & 0.34 & 22.56 & 0.31 \\ 
  GARCH-NORM & Nikkei225 & 2.01 & 1.80 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-NORM & Nikkei225 & 2.09 & 2.20 & 0.07 & 5.45 & 0.02 \\ 
  EGARCH-STD & Nikkei225 & 3.95 & 0.20 & 0.00 & 75.92 & 0.00 \\ 
  EGARCH-SSTD & Nikkei225 & 2.50 & 1.20 & 0.00 & 48.53 & 0.00 \\ 
  EGARCH-NORM & Nikkei225 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 0.97 & 64.07 & 90.41 & 62.85 & 88.31 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.01 & 8.78 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-SSTD & EuroStoxx50 & 2.33 & 5.99 & 0.01 & 40.43 & 0.01 \\ 
  TGARCH-STD & EuroStoxx50 & 2.58 & 4.99 & 0.00 & 15.65 & 0.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.66 & 4.79 & 0.00 & 18.07 & 0.00 \\ 
  GARCH-STD & EuroStoxx50 & 2.33 & 5.79 & 0.01 & 9.64 & 0.00 \\ 
  GARCH-NORM & EuroStoxx50 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
  EGARCH-STD & EuroStoxx50 & 4.03 & 1.40 & 0.00 & 17.32 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 3.70 & 1.80 & 0.00 & 2.49 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 3.30 & 0.20 & 0.00 & 44.47 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 10 days ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_1}
\end{table}


==> Tables/Case_1/Archive2/Results_Case1_10Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:36:26 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 2.62 & 13.57 & 78.12 & 55.96 & 53.84 \\ 
  GARCH-SSTD & S\&P500 & 2.78 & 6.99 & 52.88 & 22.94 & 18.81 \\ 
  GARCH-STD & S\&P500 & 3.18 & 3.39 & 13.82 & 39.68 & 13.22 \\ 
  TGARCH-STD & S\&P500 & 3.42 & 0.20 & 4.80 & 51.32 & 7.27 \\ 
  GARCH-NORM & S\&P500 & 3.58 & 2.79 & 2.14 & 59.33 & 4.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.75 & 95.21 & 7.15 & 16.45 & 3.24 \\ 
  TGARCH-NORM & S\&P500 & 3.58 & 0.40 & 2.14 & 25.03 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 30.25 & 0.02 \\ 
  EGARCH-SSTD & S\&P500 & 4.77 & 0.20 & 0.00 & 22.74 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 4.61 & 0.20 & 0.00 & 17.75 & 0.00 \\ 
   \hline
\hline
GARCH-STD & Nikkei225 & 2.74 & 0.20 & 59.74 & 60.95 & 53.02 \\ 
  GARCH-SSTD & Nikkei225 & 2.25 & 8.58 & 57.31 & 36.53 & 31.17 \\ 
  GARCH-NORM & Nikkei225 & 3.30 & 0.00 & 8.45 & 86.53 & 19.54 \\ 
  TGARCH-SSTD & Nikkei225 & 2.74 & 0.00 & 59.74 & 20.72 & 18.02 \\ 
  TGARCH-STD & Nikkei225 & 3.06 & 0.00 & 22.21 & 33.30 & 15.80 \\ 
  TGARCH-NORM & Nikkei225 & 3.46 & 0.00 & 3.99 & 52.40 & 6.35 \\ 
  EGARCH-SSTD & Nikkei225 & 4.03 & 0.40 & 0.15 & 43.03 & 0.28 \\ 
  EGARCH-NORM & Nikkei225 & 4.11 & 0.00 & 0.09 & 46.87 & 0.19 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.29 & 48.10 & 0.26 & 5.17 & 0.06 \\ 
  EGARCH-STD & Nikkei225 & 5.31 & 0.20 & 0.00 & 96.40 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 3.22 & 50.30 & 11.91 & 40.62 & 12.06 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.30 & 50.10 & 8.45 & 44.47 & 10.04 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.38 & 9.38 & 5.87 & 48.40 & 8.11 \\ 
  GARCH-STD & EuroStoxx50 & 3.46 & 8.78 & 3.99 & 52.40 & 6.35 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.06 & 85.03 & 22.21 & 9.73 & 4.61 \\ 
  TGARCH-STD & EuroStoxx50 & 3.46 & 13.77 & 3.99 & 20.23 & 2.45 \\ 
  GARCH-NORM & EuroStoxx50 & 3.78 & 0.20 & 0.70 & 68.40 & 1.80 \\ 
  EGARCH-STD & EuroStoxx50 & 5.88 & 0.40 & 0.00 & 43.78 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.91 & 0.20 & 0.00 & 3.67 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.83 & 0.00 & 0.00 & 23.77 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 10 days ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_2.5}
\end{table}


==> Tables/Case_1/Archive2/Results_Case1_10Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:36:26 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-NORM & S\&P500 & 5.09 & 1.20 & 88.72 & 34.98 & 34.63 \\ 
  TGARCH-STD & S\&P500 & 5.01 & 0.00 & 98.97 & 31.66 & 31.66 \\ 
  GARCH-SSTD & S\&P500 & 4.29 & 2.20 & 23.85 & 57.38 & 28.64 \\ 
  GARCH-STD & S\&P500 & 5.17 & 0.00 & 78.70 & 17.88 & 17.24 \\ 
  TGARCH-SSTD & S\&P500 & 4.21 & 4.39 & 18.86 & 24.22 & 10.20 \\ 
  GARCH-NORM & S\&P500 & 5.48 & 0.00 & 43.69 & 4.89 & 3.62 \\ 
  EGARCH-NORM & S\&P500 & 6.52 & 0.00 & 1.80 & 29.69 & 1.81 \\ 
  EGARCH-STD & S\&P500 & 6.60 & 0.00 & 1.30 & 32.87 & 1.50 \\ 
  SVR-GARCH-KDE & S\&P500 & 3.34 & 56.89 & 0.41 & 17.11 & 0.28 \\ 
  EGARCH-SSTD & S\&P500 & 7.23 & 0.00 & 0.06 & 62.62 & 0.18 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 5.23 & 10.18 & 70.78 & 94.63 & 88.21 \\ 
  GARCH-SSTD & Nikkei225 & 4.99 & 21.16 & 98.96 & 87.41 & 87.40 \\ 
  TGARCH-STD & Nikkei225 & 5.31 & 8.18 & 61.51 & 72.91 & 64.25 \\ 
  TGARCH-NORM & Nikkei225 & 5.31 & 12.18 & 61.51 & 72.91 & 64.25 \\ 
  GARCH-NORM & Nikkei225 & 5.72 & 5.99 & 25.68 & 99.95 & 52.55 \\ 
  GARCH-STD & Nikkei225 & 5.72 & 8.18 & 25.68 & 89.19 & 46.89 \\ 
  SVR-GARCH-KDE & Nikkei225 & 3.95 & 88.82 & 7.70 & 75.92 & 15.90 \\ 
  EGARCH-SSTD & Nikkei225 & 6.36 & 0.60 & 3.44 & 90.35 & 9.65 \\ 
  EGARCH-NORM & Nikkei225 & 6.12 & 3.59 & 7.99 & 31.60 & 6.82 \\ 
  EGARCH-STD & Nikkei225 & 7.97 & 0.00 & 0.00 & 91.62 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 5.07 & 50.10 & 90.69 & 61.34 & 60.92 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.12 & 2.59 & 7.99 & 6.55 & 1.41 \\ 
  TGARCH-SSTD & EuroStoxx50 & 6.12 & 4.99 & 7.99 & 2.43 & 0.53 \\ 
  TGARCH-STD & EuroStoxx50 & 6.36 & 0.00 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-NORM & EuroStoxx50 & 6.36 & 2.20 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-SSTD & EuroStoxx50 & 6.52 & 2.99 & 1.85 & 6.06 & 0.38 \\ 
  GARCH-STD & EuroStoxx50 & 6.76 & 0.40 & 0.67 & 9.76 & 0.25 \\ 
  EGARCH-STD & EuroStoxx50 & 9.10 & 0.20 & 0.00 & 1.03 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 7.41 & 0.20 & 0.03 & 0.13 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 7.17 & 0.60 & 0.10 & 0.18 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 10 days ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_5}
\end{table}


==> Tables/Case_1/Archive2/Results_Case1_1Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:34:41 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
EGARCH-SSTD & S\&P500 & 1.11 & 4.99 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & S\&P500 & 0.72 & 92.22 & 28.52 & 71.87 & 52.94 \\ 
  GARCH-SSTD & S\&P500 & 1.27 & 20.76 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & S\&P500 & 1.43 & 0.20 & 14.91 & 46.97 & 27.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.79 & 29.34 & 44.83 & 18.28 & 13.71 \\ 
  GARCH-STD & S\&P500 & 1.67 & 16.17 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & S\&P500 & 1.75 & 5.79 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & S\&P500 & 2.15 & 3.39 & 0.04 & 27.64 & 0.10 \\ 
  EGARCH-NORM & S\&P500 & 2.23 & 2.40 & 0.02 & 25.88 & 0.04 \\ 
  GARCH-NORM & S\&P500 & 2.38 & 0.20 & 0.00 & 94.85 & 0.01 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.21 & 4.99 & 47.61 & 54.48 & 64.58 \\ 
  GARCH-SSTD & Nikkei225 & 1.21 & 2.79 & 47.61 & 54.48 & 64.58 \\ 
  EGARCH-SSTD & Nikkei225 & 1.37 & 4.19 & 21.61 & 49.21 & 36.76 \\ 
  GARCH-STD & Nikkei225 & 1.69 & 1.80 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & Nikkei225 & 1.77 & 1.00 & 1.37 & 37.30 & 3.23 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.24 & 59.48 & 0.13 & 90.41 & 0.55 \\ 
  EGARCH-STD & Nikkei225 & 2.09 & 0.80 & 0.07 & 29.17 & 0.19 \\ 
  GARCH-NORM & Nikkei225 & 2.17 & 0.40 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & Nikkei225 & 2.33 & 0.20 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & Nikkei225 & 2.42 & 0.20 & 0.00 & 95.21 & 0.01 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 1.53 & 76.25 & 8.17 & 44.23 & 16.36 \\ 
  GARCH-SSTD & EuroStoxx50 & 1.69 & 72.85 & 2.60 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1.69 & 43.51 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & EuroStoxx50 & 1.77 & 1.60 & 1.37 & 70.53 & 3.39 \\ 
  GARCH-STD & EuroStoxx50 & 1.85 & 1.80 & 0.70 & 35.15 & 1.70 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.09 & 0.20 & 0.07 & 85.17 & 0.28 \\ 
  GARCH-NORM & EuroStoxx50 & 2.17 & 6.19 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & EuroStoxx50 & 2.33 & 9.38 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.42 & 4.79 & 0.00 & 95.21 & 0.01 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.50 & 3.19 & 0.00 & 96.87 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 1 day ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> Tables/Case_1/Archive2/Results_Case1_1Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:34:41 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 2.62 & 34.33 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & S\&P500 & 3.02 & 1.40 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & S\&P500 & 2.38 & 80.44 & 79.19 & 22.60 & 46.40 \\ 
  GARCH-STD & S\&P500 & 3.50 & 0.80 & 3.24 & 93.45 & 9.47 \\ 
  GARCH-NORM & S\&P500 & 3.82 & 1.20 & 0.55 & 99.20 & 2.10 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.43 & 34.53 & 0.83 & 52.45 & 1.62 \\ 
  TGARCH-STD & S\&P500 & 3.90 & 0.00 & 0.33 & 75.52 & 1.02 \\ 
  TGARCH-NORM & S\&P500 & 4.05 & 1.60 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & S\&P500 & 4.53 & 0.20 & 0.00 & 92.48 & 0.02 \\ 
   \hline
\hline
GARCH-SSTD & Nikkei225 & 2.90 & 43.91 & 38.01 & 99.90 & 67.96 \\ 
  TGARCH-SSTD & Nikkei225 & 2.42 & 71.66 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & Nikkei225 & 3.14 & 0.40 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & Nikkei225 & 3.22 & 1.60 & 11.91 & 96.33 & 28.60 \\ 
  EGARCH-NORM & Nikkei225 & 3.22 & 0.40 & 11.91 & 96.33 & 28.60 \\ 
  GARCH-NORM & Nikkei225 & 3.38 & 0.00 & 5.87 & 92.85 & 15.55 \\ 
  GARCH-STD & Nikkei225 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & Nikkei225 & 3.06 & 13.97 & 22.21 & 12.14 & 14.30 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.69 & 73.65 & 5.26 & 14.27 & 2.18 \\ 
  EGARCH-STD & Nikkei225 & 3.86 & 0.20 & 0.43 & 99.42 & 1.68 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.98 & 79.84 & 29.36 & 72.90 & 42.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.22 & 0.00 & 11.91 & 83.46 & 24.78 \\ 
  TGARCH-STD & EuroStoxx50 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.46 & 68.86 & 3.99 & 91.84 & 11.13 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.14 & 29.74 & 16.44 & 11.43 & 4.35 \\ 
  GARCH-STD & EuroStoxx50 & 3.70 & 5.19 & 1.11 & 97.42 & 3.88 \\ 
  GARCH-NORM & EuroStoxx50 & 3.95 & 5.59 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & EuroStoxx50 & 4.27 & 1.20 & 0.03 & 88.73 & 0.12 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.51 & 1.40 & 0.00 & 95.50 & 0.02 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.59 & 1.60 & 0.00 & 97.11 & 0.01 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 1 day ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> Tables/Case_1/Archive2/Results_Case1_1Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:34:41 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 5.01 & 57.49 & 98.97 & 89.07 & 89.06 \\ 
  GARCH-NORM & S\&P500 & 5.72 & 0.00 & 24.94 & 99.79 & 51.40 \\ 
  TGARCH-SSTD & S\&P500 & 5.41 & 87.82 & 51.47 & 60.38 & 48.83 \\ 
  GARCH-STD & S\&P500 & 5.80 & 2.20 & 20.21 & 99.23 & 43.99 \\ 
  SVR-GARCH-KDE & S\&P500 & 4.37 & 24.95 & 29.68 & 30.25 & 17.55 \\ 
  EGARCH-SSTD & S\&P500 & 6.44 & 1.20 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & S\&P500 & 6.60 & 0.40 & 1.30 & 77.88 & 3.56 \\ 
  EGARCH-NORM & S\&P500 & 6.76 & 1.00 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & S\&P500 & 6.76 & 0.00 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 7.00 & 0.80 & 0.21 & 87.46 & 0.78 \\ 
   \hline
\hline
EGARCH-SSTD & Nikkei225 & 5.23 & 15.17 & 70.78 & 97.26 & 90.66 \\ 
  SVR-GARCH-KDE & Nikkei225 & 4.59 & 27.74 & 50.10 & 97.11 & 77.43 \\ 
  TGARCH-SSTD & Nikkei225 & 4.67 & 94.81 & 58.95 & 89.41 & 77.30 \\ 
  GARCH-SSTD & Nikkei225 & 5.07 & 34.93 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & Nikkei225 & 5.23 & 0.20 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & Nikkei225 & 5.56 & 0.20 & 37.71 & 89.62 & 60.67 \\ 
  GARCH-NORM & Nikkei225 & 5.88 & 4.99 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & Nikkei225 & 5.72 & 0.60 & 25.68 & 49.18 & 25.85 \\ 
  GARCH-STD & Nikkei225 & 6.04 & 0.00 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & Nikkei225 & 6.04 & 0.60 & 10.34 & 71.98 & 19.11 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 5.15 & 89.62 & 80.55 & 65.27 & 63.32 \\ 
  GARCH-SSTD & EuroStoxx50 & 5.96 & 57.29 & 13.21 & 95.83 & 30.84 \\ 
  GARCH-NORM & EuroStoxx50 & 5.96 & 48.90 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.04 & 2.59 & 10.34 & 78.10 & 20.73 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 5.48 & 33.53 & 44.90 & 26.86 & 20.17 \\ 
  EGARCH-SSTD & EuroStoxx50 & 6.12 & 1.40 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & EuroStoxx50 & 6.20 & 0.00 & 6.11 & 59.29 & 10.26 \\ 
  EGARCH-NORM & EuroStoxx50 & 6.52 & 1.80 & 1.85 & 99.10 & 6.18 \\ 
  GARCH-STD & EuroStoxx50 & 6.60 & 3.99 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & EuroStoxx50 & 6.84 & 0.80 & 0.46 & 69.51 & 1.27 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 1 day ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> Tables/Case_1/Results_Case1_10Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:07:04 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 1.03 & 11.78 & 90.58 & 30.09 & 29.88 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.95 & 94.01 & 86.85 & 25.94 & 25.59 \\ 
  GARCH-SSTD & S\&P500 & 1.19 & 10.38 & 50.57 & 3.91 & 3.14 \\ 
  TGARCH-STD & S\&P500 & 1.99 & 1.80 & 0.19 & 25.26 & 0.21 \\ 
  GARCH-STD & S\&P500 & 1.99 & 2.99 & 0.19 & 25.26 & 0.21 \\ 
  TGARCH-NORM & S\&P500 & 2.31 & 3.59 & 0.01 & 39.72 & 0.01 \\ 
  GARCH-NORM & S\&P500 & 2.54 & 3.39 & 0.00 & 51.83 & 0.00 \\ 
  EGARCH-STD & S\&P500 & 2.78 & 0.00 & 0.00 & 64.14 & 0.00 \\ 
  EGARCH-SSTD & S\&P500 & 2.70 & 0.80 & 0.00 & 4.50 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 3.26 & 0.60 & 0.00 & 14.87 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.45 & 3.19 & 13.59 & 52.97 & 17.42 \\ 
  GARCH-SSTD & Nikkei225 & 1.45 & 2.40 & 13.59 & 52.97 & 17.42 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.32 & 57.29 & 0.51 & 87.23 & 1.97 \\ 
  GARCH-STD & Nikkei225 & 1.85 & 0.80 & 0.70 & 19.57 & 0.51 \\ 
  TGARCH-STD & Nikkei225 & 1.93 & 1.80 & 0.34 & 22.56 & 0.31 \\ 
  GARCH-NORM & Nikkei225 & 2.01 & 1.80 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-NORM & Nikkei225 & 2.09 & 2.20 & 0.07 & 5.45 & 0.02 \\ 
  EGARCH-STD & Nikkei225 & 3.95 & 0.20 & 0.00 & 75.92 & 0.00 \\ 
  EGARCH-SSTD & Nikkei225 & 2.50 & 1.20 & 0.00 & 48.53 & 0.00 \\ 
  EGARCH-NORM & Nikkei225 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 0.97 & 64.07 & 90.41 & 62.85 & 88.31 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.01 & 8.78 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-SSTD & EuroStoxx50 & 2.33 & 5.99 & 0.01 & 40.43 & 0.01 \\ 
  TGARCH-STD & EuroStoxx50 & 2.58 & 4.99 & 0.00 & 15.65 & 0.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.66 & 4.79 & 0.00 & 18.07 & 0.00 \\ 
  GARCH-STD & EuroStoxx50 & 2.33 & 5.79 & 0.01 & 9.64 & 0.00 \\ 
  GARCH-NORM & EuroStoxx50 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
  EGARCH-STD & EuroStoxx50 & 4.03 & 1.40 & 0.00 & 17.32 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 3.70 & 1.80 & 0.00 & 2.49 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 3.30 & 0.20 & 0.00 & 44.47 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for ten-days-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_1}
\end{table}


==> Tables/Case_1/Results_Case1_10Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:07:04 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 2.62 & 13.57 & 78.12 & 55.96 & 53.84 \\ 
  GARCH-SSTD & S\&P500 & 2.78 & 6.99 & 52.88 & 22.94 & 18.81 \\ 
  GARCH-STD & S\&P500 & 3.18 & 3.39 & 13.82 & 39.68 & 13.22 \\ 
  TGARCH-STD & S\&P500 & 3.42 & 0.20 & 4.80 & 51.32 & 7.27 \\ 
  GARCH-NORM & S\&P500 & 3.58 & 2.79 & 2.14 & 59.33 & 4.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.75 & 95.21 & 7.15 & 16.45 & 3.24 \\ 
  TGARCH-NORM & S\&P500 & 3.58 & 0.40 & 2.14 & 25.03 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 30.25 & 0.02 \\ 
  EGARCH-SSTD & S\&P500 & 4.77 & 0.20 & 0.00 & 22.74 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 4.61 & 0.20 & 0.00 & 17.75 & 0.00 \\ 
   \hline
\hline
GARCH-STD & Nikkei225 & 2.74 & 0.20 & 59.74 & 60.95 & 53.02 \\ 
  GARCH-SSTD & Nikkei225 & 2.25 & 8.58 & 57.31 & 36.53 & 31.17 \\ 
  GARCH-NORM & Nikkei225 & 3.30 & 0.00 & 8.45 & 86.53 & 19.54 \\ 
  TGARCH-SSTD & Nikkei225 & 2.74 & 0.00 & 59.74 & 20.72 & 18.02 \\ 
  TGARCH-STD & Nikkei225 & 3.06 & 0.00 & 22.21 & 33.30 & 15.80 \\ 
  TGARCH-NORM & Nikkei225 & 3.46 & 0.00 & 3.99 & 52.40 & 6.35 \\ 
  EGARCH-SSTD & Nikkei225 & 4.03 & 0.40 & 0.15 & 43.03 & 0.28 \\ 
  EGARCH-NORM & Nikkei225 & 4.11 & 0.00 & 0.09 & 46.87 & 0.19 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.29 & 48.10 & 0.26 & 5.17 & 0.06 \\ 
  EGARCH-STD & Nikkei225 & 5.31 & 0.20 & 0.00 & 96.40 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 3.22 & 50.30 & 11.91 & 40.62 & 12.06 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.30 & 50.10 & 8.45 & 44.47 & 10.04 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.38 & 9.38 & 5.87 & 48.40 & 8.11 \\ 
  GARCH-STD & EuroStoxx50 & 3.46 & 8.78 & 3.99 & 52.40 & 6.35 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.06 & 85.03 & 22.21 & 9.73 & 4.61 \\ 
  TGARCH-STD & EuroStoxx50 & 3.46 & 13.77 & 3.99 & 20.23 & 2.45 \\ 
  GARCH-NORM & EuroStoxx50 & 3.78 & 0.20 & 0.70 & 68.40 & 1.80 \\ 
  EGARCH-STD & EuroStoxx50 & 5.88 & 0.40 & 0.00 & 43.78 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.91 & 0.20 & 0.00 & 3.67 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.83 & 0.00 & 0.00 & 23.77 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for ten-days-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_2.5}
\end{table}


==> Tables/Case_1/Results_Case1_10Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:07:04 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-NORM & S\&P500 & 5.09 & 1.20 & 88.72 & 34.98 & 34.63 \\ 
  TGARCH-STD & S\&P500 & 5.01 & 0.00 & 98.97 & 31.66 & 31.66 \\ 
  GARCH-SSTD & S\&P500 & 4.29 & 2.20 & 23.85 & 57.38 & 28.64 \\ 
  GARCH-STD & S\&P500 & 5.17 & 0.00 & 78.70 & 17.88 & 17.24 \\ 
  TGARCH-SSTD & S\&P500 & 4.21 & 4.39 & 18.86 & 24.22 & 10.20 \\ 
  GARCH-NORM & S\&P500 & 5.48 & 0.00 & 43.69 & 4.89 & 3.62 \\ 
  EGARCH-NORM & S\&P500 & 6.52 & 0.00 & 1.80 & 29.69 & 1.81 \\ 
  EGARCH-STD & S\&P500 & 6.60 & 0.00 & 1.30 & 32.87 & 1.50 \\ 
  SVR-GARCH-KDE & S\&P500 & 3.34 & 56.89 & 0.41 & 17.11 & 0.28 \\ 
  EGARCH-SSTD & S\&P500 & 7.23 & 0.00 & 0.06 & 62.62 & 0.18 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 5.23 & 10.18 & 70.78 & 94.63 & 88.21 \\ 
  GARCH-SSTD & Nikkei225 & 4.99 & 21.16 & 98.96 & 87.41 & 87.40 \\ 
  TGARCH-STD & Nikkei225 & 5.31 & 8.18 & 61.51 & 72.91 & 64.25 \\ 
  TGARCH-NORM & Nikkei225 & 5.31 & 12.18 & 61.51 & 72.91 & 64.25 \\ 
  GARCH-NORM & Nikkei225 & 5.72 & 5.99 & 25.68 & 99.95 & 52.55 \\ 
  GARCH-STD & Nikkei225 & 5.72 & 8.18 & 25.68 & 89.19 & 46.89 \\ 
  SVR-GARCH-KDE & Nikkei225 & 3.95 & 88.82 & 7.70 & 75.92 & 15.90 \\ 
  EGARCH-SSTD & Nikkei225 & 6.36 & 0.60 & 3.44 & 90.35 & 9.65 \\ 
  EGARCH-NORM & Nikkei225 & 6.12 & 3.59 & 7.99 & 31.60 & 6.82 \\ 
  EGARCH-STD & Nikkei225 & 7.97 & 0.00 & 0.00 & 91.62 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 5.07 & 50.10 & 90.69 & 61.34 & 60.92 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.12 & 2.59 & 7.99 & 6.55 & 1.41 \\ 
  TGARCH-SSTD & EuroStoxx50 & 6.12 & 4.99 & 7.99 & 2.43 & 0.53 \\ 
  TGARCH-STD & EuroStoxx50 & 6.36 & 0.00 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-NORM & EuroStoxx50 & 6.36 & 2.20 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-SSTD & EuroStoxx50 & 6.52 & 2.99 & 1.85 & 6.06 & 0.38 \\ 
  GARCH-STD & EuroStoxx50 & 6.76 & 0.40 & 0.67 & 9.76 & 0.25 \\ 
  EGARCH-STD & EuroStoxx50 & 9.10 & 0.20 & 0.00 & 1.03 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 7.41 & 0.20 & 0.03 & 0.13 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 7.17 & 0.60 & 0.10 & 0.18 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for ten-days-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_5}
\end{table}


==> Tables/Case_1/Results_Case1_1Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:04:49 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
EGARCH-SSTD & S\&P500 & 1.11 & 4.99 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & S\&P500 & 0.72 & 92.22 & 28.52 & 71.87 & 52.94 \\ 
  GARCH-SSTD & S\&P500 & 1.27 & 20.76 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & S\&P500 & 1.43 & 0.20 & 14.91 & 46.97 & 27.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.79 & 29.34 & 44.83 & 18.28 & 13.71 \\ 
  GARCH-STD & S\&P500 & 1.67 & 16.17 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & S\&P500 & 1.75 & 5.79 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & S\&P500 & 2.15 & 3.39 & 0.04 & 27.64 & 0.10 \\ 
  EGARCH-NORM & S\&P500 & 2.23 & 2.40 & 0.02 & 25.88 & 0.04 \\ 
  GARCH-NORM & S\&P500 & 2.38 & 0.20 & 0.00 & 94.85 & 0.01 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.21 & 4.99 & 47.61 & 54.48 & 64.58 \\ 
  GARCH-SSTD & Nikkei225 & 1.21 & 2.79 & 47.61 & 54.48 & 64.58 \\ 
  EGARCH-SSTD & Nikkei225 & 1.37 & 4.19 & 21.61 & 49.21 & 36.76 \\ 
  GARCH-STD & Nikkei225 & 1.69 & 1.80 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & Nikkei225 & 1.77 & 1.00 & 1.37 & 37.30 & 3.23 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.24 & 59.48 & 0.13 & 90.41 & 0.55 \\ 
  EGARCH-STD & Nikkei225 & 2.09 & 0.80 & 0.07 & 29.17 & 0.19 \\ 
  GARCH-NORM & Nikkei225 & 2.17 & 0.40 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & Nikkei225 & 2.33 & 0.20 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & Nikkei225 & 2.42 & 0.20 & 0.00 & 95.21 & 0.01 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 1.53 & 76.25 & 8.17 & 44.23 & 16.36 \\ 
  GARCH-SSTD & EuroStoxx50 & 1.69 & 72.85 & 2.60 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1.69 & 43.51 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & EuroStoxx50 & 1.77 & 1.60 & 1.37 & 70.53 & 3.39 \\ 
  GARCH-STD & EuroStoxx50 & 1.85 & 1.80 & 0.70 & 35.15 & 1.70 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.09 & 0.20 & 0.07 & 85.17 & 0.28 \\ 
  GARCH-NORM & EuroStoxx50 & 2.17 & 6.19 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & EuroStoxx50 & 2.33 & 9.38 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.42 & 4.79 & 0.00 & 95.21 & 0.01 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.50 & 3.19 & 0.00 & 96.87 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for one-day-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> Tables/Case_1/Results_Case1_1Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:04:49 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 2.62 & 34.33 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & S\&P500 & 3.02 & 1.40 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & S\&P500 & 2.38 & 80.44 & 79.19 & 22.60 & 46.40 \\ 
  GARCH-STD & S\&P500 & 3.50 & 0.80 & 3.24 & 93.45 & 9.47 \\ 
  GARCH-NORM & S\&P500 & 3.82 & 1.20 & 0.55 & 99.20 & 2.10 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.43 & 34.53 & 0.83 & 52.45 & 1.62 \\ 
  TGARCH-STD & S\&P500 & 3.90 & 0.00 & 0.33 & 75.52 & 1.02 \\ 
  TGARCH-NORM & S\&P500 & 4.05 & 1.60 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & S\&P500 & 4.53 & 0.20 & 0.00 & 92.48 & 0.02 \\ 
   \hline
\hline
GARCH-SSTD & Nikkei225 & 2.90 & 43.91 & 38.01 & 99.90 & 67.96 \\ 
  TGARCH-SSTD & Nikkei225 & 2.42 & 71.66 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & Nikkei225 & 3.14 & 0.40 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & Nikkei225 & 3.22 & 1.60 & 11.91 & 96.33 & 28.60 \\ 
  EGARCH-NORM & Nikkei225 & 3.22 & 0.40 & 11.91 & 96.33 & 28.60 \\ 
  GARCH-NORM & Nikkei225 & 3.38 & 0.00 & 5.87 & 92.85 & 15.55 \\ 
  GARCH-STD & Nikkei225 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & Nikkei225 & 3.06 & 13.97 & 22.21 & 12.14 & 14.30 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.69 & 73.65 & 5.26 & 14.27 & 2.18 \\ 
  EGARCH-STD & Nikkei225 & 3.86 & 0.20 & 0.43 & 99.42 & 1.68 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.98 & 79.84 & 29.36 & 72.90 & 42.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.22 & 0.00 & 11.91 & 83.46 & 24.78 \\ 
  TGARCH-STD & EuroStoxx50 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.46 & 68.86 & 3.99 & 91.84 & 11.13 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.14 & 29.74 & 16.44 & 11.43 & 4.35 \\ 
  GARCH-STD & EuroStoxx50 & 3.70 & 5.19 & 1.11 & 97.42 & 3.88 \\ 
  GARCH-NORM & EuroStoxx50 & 3.95 & 5.59 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & EuroStoxx50 & 4.27 & 1.20 & 0.03 & 88.73 & 0.12 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.51 & 1.40 & 0.00 & 95.50 & 0.02 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.59 & 1.60 & 0.00 & 97.11 & 0.01 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for one-day-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> Tables/Case_1/Results_Case1_1Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:04:49 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 5.01 & 57.49 & 98.97 & 89.07 & 89.06 \\ 
  GARCH-NORM & S\&P500 & 5.72 & 0.00 & 24.94 & 99.79 & 51.40 \\ 
  TGARCH-SSTD & S\&P500 & 5.41 & 87.82 & 51.47 & 60.38 & 48.83 \\ 
  GARCH-STD & S\&P500 & 5.80 & 2.20 & 20.21 & 99.23 & 43.99 \\ 
  SVR-GARCH-KDE & S\&P500 & 4.37 & 24.95 & 29.68 & 30.25 & 17.55 \\ 
  EGARCH-SSTD & S\&P500 & 6.44 & 1.20 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & S\&P500 & 6.60 & 0.40 & 1.30 & 77.88 & 3.56 \\ 
  EGARCH-NORM & S\&P500 & 6.76 & 1.00 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & S\&P500 & 6.76 & 0.00 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 7.00 & 0.80 & 0.21 & 87.46 & 0.78 \\ 
   \hline
\hline
EGARCH-SSTD & Nikkei225 & 5.23 & 15.17 & 70.78 & 97.26 & 90.66 \\ 
  SVR-GARCH-KDE & Nikkei225 & 4.59 & 27.74 & 50.10 & 97.11 & 77.43 \\ 
  TGARCH-SSTD & Nikkei225 & 4.67 & 94.81 & 58.95 & 89.41 & 77.30 \\ 
  GARCH-SSTD & Nikkei225 & 5.07 & 34.93 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & Nikkei225 & 5.23 & 0.20 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & Nikkei225 & 5.56 & 0.20 & 37.71 & 89.62 & 60.67 \\ 
  GARCH-NORM & Nikkei225 & 5.88 & 4.99 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & Nikkei225 & 5.72 & 0.60 & 25.68 & 49.18 & 25.85 \\ 
  GARCH-STD & Nikkei225 & 6.04 & 0.00 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & Nikkei225 & 6.04 & 0.60 & 10.34 & 71.98 & 19.11 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 5.15 & 89.62 & 80.55 & 65.27 & 63.32 \\ 
  GARCH-SSTD & EuroStoxx50 & 5.96 & 57.29 & 13.21 & 95.83 & 30.84 \\ 
  GARCH-NORM & EuroStoxx50 & 5.96 & 48.90 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.04 & 2.59 & 10.34 & 78.10 & 20.73 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 5.48 & 33.53 & 44.90 & 26.86 & 20.17 \\ 
  EGARCH-SSTD & EuroStoxx50 & 6.12 & 1.40 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & EuroStoxx50 & 6.20 & 0.00 & 6.11 & 59.29 & 10.26 \\ 
  EGARCH-NORM & EuroStoxx50 & 6.52 & 1.80 & 1.85 & 99.10 & 6.18 \\ 
  GARCH-STD & EuroStoxx50 & 6.60 & 3.99 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & EuroStoxx50 & 6.84 & 0.80 & 0.46 & 69.51 & 1.27 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for one-day-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> Tables/Case_1Results_Case1_EuroStoxx50.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Jan 28 15:27:23 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 0.79 & 17.22 & 18.28 & 7.2 \\ 
  TGARCH-STD & 0.5 & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  TGARCH-SSTD & 0.5 & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  SGARCH-STD & 0.5 & 1.21 & 0.28 & 54.48 & 0.95 \\ 
  EGARCH-STD & 0.5 & 1.29 & 0.1 & 43.8 & 0.2 \\ 
  SGARCH-SSTD & 0.5 & 1.37 & 0.04 & 49.21 & 0.13 \\ 
  TGARCH-NORM & 0.5 & 1.45 & 0.01 & 46.68 & 0.05 \\ 
  SGARCH-NORM & 0.5 & 1.53 & 0 & 44.23 & 0.01 \\ 
  EGARCH-SSTD & 0.5 & 1.61 & 0 & 61.98 & 0 \\ 
  EGARCH-NORM & 0.5 & 1.93 & 0 & 78.34 & 0 \\ 
   \hline
\hline
SGARCH-SSTD & 1 & 1.69 & 2.6 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & 1 & 1.69 & 2.6 & 66.33 & 5.56 \\ 
  TGARCH-STD & 1 & 1.77 & 1.37 & 70.53 & 3.39 \\ 
  SGARCH-STD & 1 & 1.85 & 0.7 & 35.15 & 1.7 \\ 
  SVM-KDE & 1 & 1.91 & 0.4 & 77.78 & 1.24 \\ 
  TGARCH-NORM & 1 & 2.09 & 0.07 & 85.17 & 0.28 \\ 
  SGARCH-NORM & 1 & 2.17 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & 1 & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & 1 & 2.42 & 0 & 95.21 & 0.01 \\ 
  EGARCH-NORM & 1 & 2.5 & 0 & 96.87 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & 2.5 & 2.98 & 29.36 & 72.9 & 42 \\ 
  TGARCH-NORM & 2.5 & 3.22 & 11.91 & 83.46 & 24.78 \\ 
  SVM-KDE & 2.5 & 3.1 & 18.85 & 36.01 & 15.17 \\ 
  TGARCH-STD & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  SGARCH-SSTD & 2.5 & 3.46 & 3.99 & 91.84 & 11.13 \\ 
  SGARCH-STD & 2.5 & 3.7 & 1.11 & 97.42 & 3.88 \\ 
  SGARCH-NORM & 2.5 & 3.95 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & 2.5 & 4.35 & 0.02 & 91.29 & 0.07 \\ 
  EGARCH-SSTD & 2.5 & 4.51 & 0 & 95.5 & 0.02 \\ 
  EGARCH-NORM & 2.5 & 4.59 & 0 & 97.11 & 0.01 \\ 
   \hline
\hline
TGARCH-SSTD & 5 & 5.15 & 80.55 & 65.27 & 63.32 \\ 
  SGARCH-SSTD & 5 & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  SGARCH-NORM & 5 & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & 5 & 6.04 & 10.34 & 78.1 & 20.73 \\ 
  EGARCH-SSTD & 5 & 6.12 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & 5 & 6.2 & 6.11 & 59.29 & 10.26 \\ 
  SVM-KDE & 5 & 4.69 & 61.03 & 7.46 & 6.56 \\ 
  EGARCH-NORM & 5 & 6.52 & 1.85 & 99.1 & 6.18 \\ 
  SGARCH-STD & 5 & 6.6 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & 5 & 6.84 & 0.46 & 69.51 & 1.27 \\ 
  \end{tabular}
\caption{Results for the VaR forecasts from 1 July 2011 to 30 June 2016 for EuroStoxx50.} 
\end{table}


==> Tables/Case_1Results_Case1_Nikkei225.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Jan 28 15:27:23 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
SGARCH-SSTD & 0.5 & 0.48 & 93.23 & 80.93 & 96.78 \\ 
  EGARCH-SSTD & 0.5 & 0.56 & 75.55 & 77.82 & 91.56 \\ 
  TGARCH-SSTD & 0.5 & 0.64 & 49.07 & 74.74 & 74.87 \\ 
  SVM-KDE & 0.5 & 0.24 & 15.09 & 90.41 & 35.39 \\ 
  TGARCH-STD & 0.5 & 0.81 & 16.15 & 68.7 & 34.6 \\ 
  SGARCH-STD & 0.5 & 0.81 & 16.15 & 68.7 & 34.6 \\ 
  EGARCH-STD & 0.5 & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  SGARCH-NORM & 0.5 & 1.45 & 0.01 & 52.97 & 0.03 \\ 
  TGARCH-NORM & 0.5 & 1.61 & 0 & 41.84 & 0 \\ 
  EGARCH-NORM & 0.5 & 1.61 & 0 & 41.84 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & 1 & 1.21 & 47.61 & 54.48 & 64.58 \\ 
  SGARCH-SSTD & 1 & 1.21 & 47.61 & 54.48 & 64.58 \\ 
  SVM-KDE & 1 & 0.64 & 17.76 & 74.74 & 38.26 \\ 
  EGARCH-SSTD & 1 & 1.37 & 21.61 & 49.21 & 36.76 \\ 
  SGARCH-STD & 1 & 1.69 & 2.6 & 66.33 & 5.56 \\ 
  TGARCH-STD & 1 & 1.77 & 1.37 & 37.3 & 3.23 \\ 
  EGARCH-STD & 1 & 2.09 & 0.07 & 29.17 & 0.19 \\ 
  SGARCH-NORM & 1 & 2.17 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & 1 & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & 1 & 2.42 & 0 & 95.21 & 0.01 \\ 
   \hline
\hline
SGARCH-SSTD & 2.5 & 2.9 & 38.01 & 99.9 & 67.96 \\ 
  TGARCH-SSTD & 2.5 & 2.42 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & 2.5 & 3.14 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 \\ 
  EGARCH-NORM & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 \\ 
  SGARCH-NORM & 2.5 & 3.38 & 5.87 & 92.85 & 15.55 \\ 
  SGARCH-STD & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & 2.5 & 3.06 & 22.21 & 12.14 & 14.3 \\ 
  SVM-KDE & 2.5 & 2.42 & 84.78 & 11.43 & 11.23 \\ 
  EGARCH-STD & 2.5 & 3.86 & 0.43 & 99.42 & 1.68 \\ 
   \hline
\hline
EGARCH-SSTD & 5 & 5.23 & 70.78 & 97.26 & 90.66 \\ 
  SVM-KDE & 5 & 5.23 & 70.78 & 94.63 & 88.21 \\ 
  TGARCH-SSTD & 5 & 4.67 & 58.95 & 89.41 & 77.3 \\ 
  SGARCH-SSTD & 5 & 5.07 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & 5 & 5.23 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & 5 & 5.56 & 37.71 & 89.62 & 60.67 \\ 
  SGARCH-NORM & 5 & 5.88 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & 5 & 5.72 & 25.68 & 49.18 & 25.85 \\ 
  SGARCH-STD & 5 & 6.04 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & 5 & 6.04 & 10.34 & 71.98 & 19.11 \\ 
  \end{tabular}
\caption{Results for the VaR forecasts from 1 July 2011 to 30 June 2016 for Nikkei225.} 
\end{table}


==> Tables/Case_1Results_Case1_SP500.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Jan 28 15:27:23 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
EGARCH-SSTD & 0.5 & 0.4 & 59.27 & 84.17 & 84.96 \\ 
  SVM-KDE & 0.5 & 0.63 & 53.09 & 75.03 & 78.11 \\ 
  TGARCH-SSTD & 0.5 & 0.32 & 32.65 & 87.31 & 61.01 \\ 
  SGARCH-SSTD & 0.5 & 0.72 & 30.91 & 71.87 & 55.87 \\ 
  TGARCH-STD & 0.5 & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  EGARCH-STD & 0.5 & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  TGARCH-NORM & 0.5 & 1.11 & 0.8 & 57.46 & 2.54 \\ 
  SGARCH-STD & 0.5 & 1.11 & 0.8 & 57.46 & 2.54 \\ 
  SGARCH-NORM & 0.5 & 1.67 & 0 & 65.77 & 0 \\ 
  EGARCH-NORM & 0.5 & 1.67 & 0 & 39.84 & 0 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.02 & 93.73 & 60.44 & 87.17 \\ 
  EGARCH-SSTD & 1 & 1.11 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & 1 & 0.72 & 28.52 & 71.87 & 52.94 \\ 
  SGARCH-SSTD & 1 & 1.27 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & 1 & 1.43 & 14.91 & 46.97 & 27.2 \\ 
  SGARCH-STD & 1 & 1.67 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & 1 & 1.75 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & 1 & 2.15 & 0.04 & 27.64 & 0.1 \\ 
  EGARCH-NORM & 1 & 2.23 & 0.02 & 25.88 & 0.04 \\ 
  SGARCH-NORM & 1 & 2.38 & 0 & 94.85 & 0.01 \\ 
   \hline
\hline
SGARCH-SSTD & 2.5 & 2.62 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & 2.5 & 3.02 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & 2.5 & 2.38 & 79.19 & 22.6 & 46.4 \\ 
  SGARCH-STD & 2.5 & 3.5 & 3.24 & 93.45 & 9.47 \\ 
  SGARCH-NORM & 2.5 & 3.82 & 0.55 & 99.2 & 2.1 \\ 
  TGARCH-STD & 2.5 & 3.9 & 0.33 & 75.52 & 1.02 \\ 
  SVM-KDE & 2.5 & 1.57 & 2.31 & 11.5 & 0.87 \\ 
  TGARCH-NORM & 2.5 & 4.05 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & 2.5 & 4.37 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & 2.5 & 4.53 & 0 & 92.48 & 0.02 \\ 
   \hline
\hline
SGARCH-SSTD & 5 & 5.01 & 98.97 & 89.07 & 89.06 \\ 
  SGARCH-NORM & 5 & 5.72 & 24.94 & 99.79 & 51.4 \\ 
  TGARCH-SSTD & 5 & 5.41 & 51.47 & 60.38 & 48.83 \\ 
  SGARCH-STD & 5 & 5.8 & 20.21 & 99.23 & 43.99 \\ 
  EGARCH-SSTD & 5 & 6.44 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & 5 & 6.6 & 1.3 & 77.88 & 3.56 \\ 
  EGARCH-NORM & 5 & 6.76 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & 5 & 6.76 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & 5 & 7 & 0.21 & 87.46 & 0.78 \\ 
  SVM-KDE & 5 & 4.72 & 64.02 & 0 & 0 \\ 
  \end{tabular}
\caption{Results for the VaR forecasts from 1 July 2011 to 30 June 2016 for Standard and Poors 500.} 
\end{table}


==> Tables/Descriptive_Statistics.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Feb 03 16:35:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
  \hline
  \hline
\textbf{Index} & \textbf{1st Quartile} & \textbf{Mean} & \textbf{Median} & \textbf{3rd Quartile} & \textbf{Variance} & \textbf{Skewness} & \textbf{Kurtosis} \\ 
  \hline
EuroStoxx50 & -0.74 & -0.01 & 0.01 & 0.78 & 2.39 & -0.06 & 5.15 \\ 
  S\&P500 & -0.46 & 0.02 & 0.07 & 0.59 & 1.74 & -0.33 & 9.94 \\ 
  Nikkei225 & -0.76 & 0.00 & 0.05 & 0.88 & 2.68 & -0.51 & 7.49 \\ 
   \hline
    \hline
\end{tabular}
\caption{Descriptive statistics for the log-returns of the analyzed
                      indices in the period from July 1, 2006 to June 30, 2016. Note that the log-returns were multiplied by 100
                      before computing the descriptive statistics.} 
\label{Tab:desc_stats}
\end{table}


==> Tables/Descriptive_Statistics_Adjusted.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Feb 03 16:35:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
  \hline
\textbf{Index} & \textbf{1st Quartile} & \textbf{Mean} & \textbf{Median} & \textbf{3rd Quartile} & \textbf{Variance} & \textbf{Skewness} & \textbf{Kurtosis} \\ 
  \hline
EuroStoxx50 & -0.74 & -0.01 & 0.01 & 0.78 & 2.39 & -0.06 & 5.15 \\ 
  S\&P500 & -0.46 & 0.02 & 0.07 & 0.59 & 1.74 & -0.33 & 9.94 \\ 
  Nikkei225 & -0.76 & 0.00 & 0.05 & 0.88 & 2.68 & -0.51 & 7.49 \\ 
   \hline
    \hline
\end{tabular}
\caption{Descriptive statistics for the log-returns of the analyzed
                      indices in the period from July 1, 2006 to June 30, 2016. Note that the log-returns were multiplied by 100
                      before computing the descriptive statistics.} 
\label{Tab:desc_stats}
\end{table}


==> Tables/Results_Case1_05.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
  \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
EGARCH-SSTD & S\&P500 %%& 0.5 
& 0.40 & 59.27 & 84.17 & 84.96 \\ 
  TGARCH-SSTD & S\&P500 %& 0.5 
  & 0.32 & 32.65 & 87.31 & 61.01 \\ 
  GARCH-SSTD & S\&P500 %& 0.5 
  & 0.72 & 30.91 & 71.87 & 55.87 \\ 
  TGARCH-STD & S\&P500 %& 0.5 
  & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  EGARCH-STD & S\&P500 %& 0.5 
  & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  TGARCH-NORM & S\&P500 %& 0.5 
  & 1.11 & 0.80 & 57.46 & 2.54 \\ 
  GARCH-STD & S\&P500 %& 0.5 
  & 1.11 & 0.80 & 57.46 & 2.54 \\ 
  SVR-GARCH-KDE & S\&P500 %& 0.5 
  & 0.32 & 32.65 & 2.61 & 1.61 \\ 
  GARCH-NORM & S\&P500 %& 0.5 
  & 1.67 & 0.00 & 65.77 & 0.00 \\ 
  EGARCH-NORM & S\&P500 %& 0.5 
  & 1.67 & 0.00 & 39.84 & 0.00 \\ 
   \hline
GARCH-SSTD & Nikkei225 %& 0.5 
& 0.48 & 93.23 & 80.93 & 96.78 \\ 
  EGARCH-SSTD & Nikkei225 %& 0.5 %
  & 0.56 & 75.55 & 77.82 & 91.56 \\ 
  TGARCH-SSTD & Nikkei225 %& 0.5 
  & 0.64 & 49.07 & 74.74 & 74.87 \\ 
  TGARCH-STD & Nikkei225 %& 0.5 
  & 0.81 & 16.15 & 68.70 & 34.60 \\ 
  GARCH-STD & Nikkei225 %& 0.5 
  & 0.81 & 16.15 & 68.70 & 34.60 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 0.5 
  & 0.08 & 0.92 & 96.80 & 3.35 \\ 
  EGARCH-STD & Nikkei225 %& 0.5 
  & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  GARCH-NORM & Nikkei225 %& 0.5 
  & 1.45 & 0.01 & 52.97 & 0.03 \\ 
  TGARCH-NORM & Nikkei225 %& 0.5 
  & 1.61 & 0.00 & 41.84 & 0.00 \\ 
  EGARCH-NORM & Nikkei225 %& 0.5 
  & 1.61 & 0.00 & 41.84 & 0.00 \\ 
   \hline
TGARCH-STD & EuroStoxx50 %& 0.5 
& 1.13 & 0.72 & 57.21 & 2.29 \\ 
  TGARCH-SSTD & EuroStoxx50 %& 0.5 
  & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  SVR-GARCH-KDE & EuroStoxx50 %& 0.5 
  & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  GARCH-STD & EuroStoxx50 %& 0.5 
  & 1.21 & 0.28 & 54.48 & 0.95 \\ 
  EGARCH-STD & EuroStoxx50 %& 0.5 
  & 1.29 & 0.10 & 43.80 & 0.20 \\ 
  GARCH-SSTD & EuroStoxx50 %& 0.5 
  & 1.37 & 0.04 & 49.21 & 0.13 \\ 
  TGARCH-NORM & EuroStoxx50 %& 0.5 
  & 1.45 & 0.01 & 46.68 & 0.05 \\ 
  GARCH-NORM & EuroStoxx50 %& 0.5 
  & 1.53 & 0.00 & 44.23 & 0.01 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 0.5 
  & 1.61 & 0.00 & 61.98 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 %& 0.5 
  & 1.93 & 0.00 & 78.34 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.005$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.005$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_0.5}
\end{table}


==> Tables/Results_Case1_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
    \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
EGARCH-SSTD & S\&P500 %& 1 
& 1.11 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & S\&P500 %& 1 
  & 0.72 & 28.52 & 71.87 & 52.94 \\ 
  GARCH-SSTD & S\&P500 %& 1 
  & 1.27 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & S\&P500 %& 1 
  & 1.43 & 14.91 & 46.97 & 27.20 \\ 
  SVR-GARCH-KDE & S\&P500 %& 1 
  & 0.79 & 44.83 & 18.28 & 13.71 \\ 
  GARCH-STD & S\&P500 %& 1 
  & 1.67 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & S\&P500 %& 1 
  & 1.75 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & S\&P500 %& 1 
  & 2.15 & 0.04 & 27.64 & 0.10 \\ 
  EGARCH-NORM & S\&P500 %& 1 
  & 2.23 & 0.02 & 25.88 & 0.04 \\ 
  GARCH-NORM & S\&P500 %& 1
  & 2.38 & 0.00 & 94.85 & 0.01 \\ 
   \hline
TGARCH-SSTD & Nikkei225 %& 1 
& 1.21 & 47.61 & 54.48 & 64.58 \\ 
  GARCH-SSTD & Nikkei225 %& 1 
  & 1.21 & 47.61 & 54.48 & 64.58 \\ 
  EGARCH-SSTD & Nikkei225 %& 1 
  & 1.37 & 21.61 & 49.21 & 36.76 \\ 
  GARCH-STD & Nikkei225 %& 1 
  & 1.69 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & Nikkei225 %& 1 
  & 1.77 & 1.37 & 37.30 & 3.23 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 1 
  & 0.24 & 0.13 & 90.41 & 0.55 \\ 
  EGARCH-STD & Nikkei225 %& 1 
  & 2.09 & 0.07 & 29.17 & 0.19 \\ 
  GARCH-NORM & Nikkei225 %& 1 
  & 2.17 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & Nikkei225 %& 1 
  & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & Nikkei225 %& 1 
  & 2.42 & 0.00 & 95.21 & 0.01 \\ 
   \hline
SVR-GARCH-KDE & EuroStoxx50 %& 1 
& 1.53 & 8.17 & 44.23 & 16.36 \\ 
  GARCH-SSTD & EuroStoxx50 %& 1 
  & 1.69 & 2.60 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & EuroStoxx50 %& 1 
  & 1.69 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & EuroStoxx50 %& 1 
  & 1.77 & 1.37 & 70.53 & 3.39 \\ 
  GARCH-STD & EuroStoxx50 %& 1 
  & 1.85 & 0.70 & 35.15 & 1.70 \\ 
  TGARCH-NORM & EuroStoxx50 %& 1 
  & 2.09 & 0.07 & 85.17 & 0.28 \\ 
  GARCH-NORM & EuroStoxx50 %& 1 
  & 2.17 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & EuroStoxx50 %& 1 
  & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 1 
  & 2.42 & 0.00 & 95.21 & 0.01 \\ 
  EGARCH-NORM & EuroStoxx50 %& 1 
  & 2.50 & 0.00 & 96.87 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.01$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> Tables/Results_Case1_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
    \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
GARCH-SSTD & S\&P500 %& 2.5 
& 2.62 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & S\&P500 %& 2.5 
  & 3.02 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & S\&P500 %& 2.5 
  & 2.38 & 79.19 & 22.60 & 46.40 \\ 
  GARCH-STD & S\&P500 %& 2.5 
  & 3.50 & 3.24 & 93.45 & 9.47 \\ 
  GARCH-NORM & S\&P500 %& 2.5 
  & 3.82 & 0.55 & 99.2 & 2.10 \\ 
  SVR-GARCH-KDE & S\&P500 %& 2.5 
  & 1.43 & 0.83 & 52.45 & 1.62 \\ 
  TGARCH-STD & S\&P500 %& 2.5 
  & 3.90 & 0.33 & 75.52 & 1.02 \\ 
  TGARCH-NORM & S\&P500 %& 2.5 
  & 4.05 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & S\&P500 %& 2.5 
  & 4.37 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & S\&P500 %& 2.5 
  & 4.53 & 0.00 & 92.48 & 0.02 \\ 
   \hline
GARCH-SSTD & Nikkei225 %& 2.5 
& 2.90 & 38.01 & 99.90 & 67.96 \\ 
  TGARCH-SSTD & Nikkei225 %& 2.5 
  & 2.42 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & Nikkei225 %& 2.5 
  & 3.14 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & Nikkei225 %& 2.5 
  & 3.22 & 11.91 & 96.33 & 28.60 \\ 
  EGARCH-NORM & Nikkei225 %& 2.5 
  & 3.22 & 11.91 & 96.33 & 28.60 \\ 
  GARCH-NORM & Nikkei225 %& 2.5 
  & 3.38 & 5.87 & 92.85 & 15.55 \\ 
  GARCH-STD & Nikkei225 %& 2.5 
  & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & Nikkei225 %& 2.5 
  & 3.06 & 22.21 & 12.14 & 14.30 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 2.5 
  & 1.69 & 5.26 & 14.27 & 2.18 \\ 
  EGARCH-STD & Nikkei225 %& 2.5 
  & 3.86 & 0.43 & 99.42 & 1.68 \\ 
   \hline
TGARCH-SSTD & EuroStoxx50 %& 2.5 
& 2.98 & 29.36 & 72.9 & 42.00 \\ 
  TGARCH-NORM & EuroStoxx50 %& 2.5 
  & 3.22 & 11.91 & 83.46 & 24.78 \\ 
  TGARCH-STD & EuroStoxx50 %& 2.5 
  & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  GARCH-SSTD & EuroStoxx50 %& 2.5 
  & 3.46 & 3.99 & 91.84 & 11.13 \\ 
  SVR-GARCH-KDE & EuroStoxx50 %& 2.5 
  & 3.14 & 16.44 & 11.43 & 4.35 \\ 
  GARCH-STD & EuroStoxx50 %& 2.5 
  & 3.70 & 1.11 & 97.42 & 3.88 \\ 
  GARCH-NORM & EuroStoxx50 %& 2.5 
  & 3.95 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & EuroStoxx50 %& 2.5 
  & 4.35 & 0.02 & 91.29 & 0.07 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 2.5 
  & 4.51 & 0.00 & 95.50 & 0.02 \\ 
  EGARCH-NORM & EuroStoxx50 %& 2.5 
  & 4.59 & 0.00 & 97.11 & 0.01 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.025$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> Tables/Results_Case1_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
    \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
GARCH-SSTD & S\&P500 %%& 5
& 5.01 & 98.97 & 89.07 & 89.06 \\ 
  GARCH-NORM & S\&P500 %%& 5 
  & 5.72 & 24.94 & 99.79 & 51.40 \\ 
  TGARCH-SSTD & S\&P500 %& 5 
  & 5.41 & 51.47 & 60.38 & 48.83 \\ 
  GARCH-STD & S\&P500 %& 5 
  & 5.80 & 20.21 & 99.23 & 43.99 \\ 
  SVR-GARCH-KDE & S\&P500 %& 5 
  & 4.37 & 29.68 & 30.25 & 17.55 \\ 
  EGARCH-SSTD & S\&P500 %& 5 
  & 6.44 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & S\&P500 %& 5 
  & 6.60 & 1.30 & 77.88 & 3.56 \\ 
  EGARCH-NORM & S\&P500 %& 5 
  & 6.76 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & S\&P500 %& 5 
  & 6.76 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & S\&P500 %& 5 
  & 7.00 & 0.21 & 87.46 & 0.78 \\ 
   \hline
EGARCH-SSTD & Nikkei225 %& 5 
& 5.23 & 70.78 & 97.26 & 90.66 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 5 
  & 4.59 & 50.1 & 97.11 & 77.43 \\ 
  TGARCH-SSTD & Nikkei225 %& 5 
  & 4.67 & 58.95 & 89.41 & 77.30 \\ 
  GARCH-SSTD & Nikkei225 %& 5 
  & 5.07 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & Nikkei225 %& 5 
  & 5.23 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & Nikkei225 %& 5 
  & 5.56 & 37.71 & 89.62 & 60.67 \\ 
  GARCH-NORM & Nikkei225 %& 5 
  & 5.88 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & Nikkei225 %& 5 
  & 5.72 & 25.68 & 49.18 & 25.85 \\ 
  GARCH-STD & Nikkei225 %& 5 
  & 6.04 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & Nikkei225 %& 5 
  & 6.04 & 10.34 & 71.98 & 19.11 \\ 
   \hline
TGARCH-SSTD & EuroStoxx50 %& 5 
& 5.15 & 80.55 & 65.27 & 63.32 \\ 
  GARCH-SSTD & EuroStoxx50 %& 5 
  & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  GARCH-NORM & EuroStoxx50 %& 5 
  & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & EuroStoxx50 %& 5 
  & 6.04 & 10.34 & 78.10 & 20.73 \\ 
  SVR-GARCH-KDE & EuroStoxx50 %& 5 
  & 5.48 & 44.90 & 26.86 & 20.17 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 5 
  & 6.12 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & EuroStoxx50 %& 5 
  & 6.20 & 6.11 & 59.29 & 10.26 \\ 
  EGARCH-NORM & EuroStoxx50 %& 5 
  & 6.52 & 1.85 & 99.10 & 6.18 \\ 
  GARCH-STD & EuroStoxx50 %& 5 
  & 6.60 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & EuroStoxx50 %& 5 
  & 6.84 & 0.46 & 69.51 & 1.27 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.05$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> Tables/Results_EuroStoxx50.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Jan 16 13:55:04 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Exceedances} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{DUR} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 1.63 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 0.5 & 1.37 & 0 & 0 & 0 & 7.23 \\ 
  SGARCH-STD & 0.5 & 0.81 & 0.38 & NaN & NaN & 99.78 \\ 
  SGARCH-SSTD & 0.5 & 0.58 & 45.56 & NaN & NaN & 69.13 \\ 
  EGARCH-NORM & 0.5 & 1.61 & 0 & NaN & NaN & 53.96 \\ 
  EGARCH-STD & 0.5 & 0.97 & 0 & NaN & NaN & 83.03 \\ 
  EGARCH-SSTD & 0.5 & 0.71 & 4.22 & NaN & NaN & 45.85 \\ 
  TGARCH-NORM & 0.5 & 1.33 & 0 & 0 & 0 & 94.27 \\ 
  TGARCH-SSTD & 0.5 & 0.6 & 34.95 & NaN & NaN & 44.76 \\ 
  TGARCH-STD & 0.5 & 0.83 & 0.22 & NaN & NaN & 83.67 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.63 & 0 & 0 & 0.02 & 0 \\ 
  SGARCH-NORM & 1 & 2.42 & 0 & 0 & 0 & 32.76 \\ 
  SGARCH-STD & 1 & 1.55 & 0.03 & 0 & 0.05 & 53.39 \\ 
  SGARCH-SSTD & 1 & 1.31 & 3.44 & 0.22 & 2.02 & 44.87 \\ 
  EGARCH-NORM & 1 & 2.34 & 0 & 0 & 0 & 34.95 \\ 
  EGARCH-STD & 1 & 1.81 & 0 & 0 & 0 & 81.29 \\ 
  EGARCH-SSTD & 1 & 1.15 & 29.01 & 30.34 & 53.1 & 99.68 \\ 
  TGARCH-NORM & 1 & 2.14 & 0 & 0 & 0 & 99.92 \\ 
  TGARCH-SSTD & 1 & 0.99 & 96.04 & 81.53 & 81.63 & 58.64 \\ 
  TGARCH-STD & 1 & 1.65 & 0 & 0 & 0.01 & 27.39 \\ 
   \hline
\hline
SVM-KDE & 5 & 7.41 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 5 & 6.42 & 0 & 0 & 0 & 69.12 \\ 
  SGARCH-STD & 5 & 6.87 & 0 & 0 & 0 & 89.23 \\ 
  SGARCH-SSTD & 5 & 6.22 & 0.01 & 0 & 0.04 & 91.02 \\ 
  EGARCH-NORM & 5 & 6.38 & 0 & 0 & 0.01 & 31.65 \\ 
  EGARCH-STD & 5 & 6.75 & 0 & 0 & 0 & 43.89 \\ 
  EGARCH-SSTD & 5 & 5.66 & 3.51 & 1.05 & 9.65 & 35.1 \\ 
  TGARCH-NORM & 5 & 6.02 & 0.13 & 0 & 0.56 & 4.63 \\ 
  TGARCH-SSTD & 5 & 5.44 & 15.58 & 12.92 & 35.37 & 1.49 \\ 
  TGARCH-STD & 5 & 6.4 & 0 & 0 & 0.01 & 9.18 \\ 
   \hline
\hline
\end{tabular}
\caption{Results for the VaR forecasts from 1 July 1996 to 30 June 2016 for EuroStoxx50.} 
\end{table}


==> Tables/Results_Nikkei225.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Jan 16 13:55:04 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Exceedances} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{DUR} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 0.65 & 14.73 & 0.76 & 2.17 & 0 \\ 
  SGARCH-NORM & 0.5 & 1.36 & 0 & 0 & 0 & 82.6 \\ 
  SGARCH-STD & 0.5 & 0.91 & 0.02 & 0 & 0.08 & 21.74 \\ 
  SGARCH-SSTD & 0.5 & 0.79 & 0.73 & 0.05 & 1.69 & 81.34 \\ 
  EGARCH-NORM & 0.5 & 1.69 & 0 & 0 & 0 & 63.65 \\ 
  EGARCH-STD & 0.5 & 1.16 & 0 & 0 & 0 & 95.1 \\ 
  EGARCH-SSTD & 0.5 & 0.83 & 0.25 & NaN & NaN & 27.85 \\ 
  TGARCH-NORM & 0.5 & 1.44 & 0 & 0 & 0 & 89.71 \\ 
  TGARCH-SSTD & 0.5 & 0.73 & 3.05 & NaN & NaN & 41.02 \\ 
  TGARCH-STD & 0.5 & 0.97 & 0 & 0 & 0.01 & 84.41 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.56 & 0.02 & 0 & 0.09 & 0 \\ 
  SGARCH-NORM & 1 & 2.17 & 0 & 0 & 0 & 74.4 \\ 
  SGARCH-STD & 1 & 1.71 & 0 & 0 & 0 & 87.93 \\ 
  SGARCH-SSTD & 1 & 1.28 & 5.42 & 2.42 & 15.42 & 58.2 \\ 
  EGARCH-NORM & 1 & 2.38 & 0 & 0 & 0 & 65.63 \\ 
  EGARCH-STD & 1 & 2.03 & 0 & 0 & 0 & 59.8 \\ 
  EGARCH-SSTD & 1 & 1.6 & 0.01 & 0 & 0.04 & 78.46 \\ 
  TGARCH-NORM & 1 & 2.13 & 0 & 0 & 0 & 90.38 \\ 
  TGARCH-SSTD & 1 & 1.38 & 1.03 & 0.09 & 2.4 & 67.74 \\ 
  TGARCH-STD & 1 & 1.83 & 0 & 0 & 0 & 82.89 \\ 
   \hline
\hline
SVM-KDE & 5 & 6.78 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 5 & 6.72 & 0 & 0 & 0 & 61.05 \\ 
  SGARCH-STD & 5 & 7.15 & 0 & 0 & 0 & 44.01 \\ 
  SGARCH-SSTD & 5 & 6.38 & 0 & 0 & 0.01 & 58.28 \\ 
  EGARCH-NORM & 5 & 6.78 & 0 & 0 & 0 & 13.24 \\ 
  EGARCH-STD & 5 & 6.97 & 0 & 0 & 0 & 5.84 \\ 
  EGARCH-SSTD & 5 & 6.01 & 0.14 & 0 & 0.42 & 3.15 \\ 
  TGARCH-NORM & 5 & 6.34 & 0 & 0 & 0.01 & 0.86 \\ 
  TGARCH-SSTD & 5 & 5.81 & 0.96 & 0.12 & 3.35 & 5.09 \\ 
  TGARCH-STD & 5 & 6.58 & 0 & 0 & 0 & 1.75 \\ 
   \hline
\hline
\end{tabular}
\caption{Results for the VaR forecasts from 1 July 1996 to 30 June 2016 for Nikkei225.} 
\end{table}


==> Tables/Results_SP500.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Jan 16 13:55:04 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Exceedances} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{DUR} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 0.79 & 0.75 & 0.05 & 1.72 & 0 \\ 
  SGARCH-NORM & 0.5 & 1.24 & 0 & 0 & 0 & 55.51 \\ 
  SGARCH-STD & 0.5 & 0.73 & 3.1 & 0.53 & 5.38 & 87.95 \\ 
  SGARCH-SSTD & 0.5 & 0.49 & 93.48 & 28.46 & 28.56 & 29.03 \\ 
  EGARCH-NORM & 0.5 & 1.42 & 0 & 0 & 0 & 82.72 \\ 
  EGARCH-STD & 0.5 & 0.96 & 0 & 0 & 0.01 & 35.98 \\ 
  EGARCH-SSTD & 0.5 & 0.75 & 1.97 & 0.25 & 3.78 & 48.1 \\ 
  TGARCH-NORM & 0.5 & 1.36 & 0 & 0 & 0 & 95.12 \\ 
  TGARCH-SSTD & 0.5 & 0.63 & 20.78 & 8.98 & 19.85 & 17.05 \\ 
  TGARCH-STD & 0.5 & 0.91 & 0.02 & 0 & 0.09 & 22.12 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.53 & 0.04 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 1 & 1.99 & 0 & 0 & 0 & 85.6 \\ 
  SGARCH-STD & 1 & 1.44 & 0.33 & 0.02 & 1.35 & 66.78 \\ 
  SGARCH-SSTD & 1 & 1.1 & 47.24 & 53.87 & 69.73 & 48.11 \\ 
  EGARCH-NORM & 1 & 1.99 & 0 & 0 & 0 & 82.16 \\ 
  EGARCH-STD & 1 & 1.63 & 0 & 0 & 0.01 & 66.5 \\ 
  EGARCH-SSTD & 1 & 1.24 & 9.79 & 6.27 & 24.69 & 70.94 \\ 
  TGARCH-NORM & 1 & 1.85 & 0 & 0 & 0 & 72.47 \\ 
  TGARCH-SSTD & 1 & 1.16 & 26.08 & 11.98 & 22.54 & 77.17 \\ 
  TGARCH-STD & 1 & 1.48 & 0.15 & 0 & 0.47 & 90.61 \\ 
   \hline
\hline
SVM-KDE & 5 & 7.44 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 5 & 6.85 & 0 & 0 & 0 & 67.87 \\ 
  SGARCH-STD & 5 & 7.1 & 0 & 0 & 0 & 62.76 \\ 
  SGARCH-SSTD & 5 & 6.34 & 0 & 0 & 0.01 & 69.2 \\ 
  EGARCH-NORM & 5 & 6.89 & 0 & 0 & 0 & 8.24 \\ 
  EGARCH-STD & 5 & 7.02 & 0 & 0 & 0 & 12.46 \\ 
  EGARCH-SSTD & 5 & 6.2 & 0.02 & 0 & 0.07 & 26.53 \\ 
  TGARCH-NORM & 5 & 6.63 & 0 & 0 & 0 & 2.07 \\ 
  TGARCH-SSTD & 5 & 6.06 & 0.08 & 0 & 0.17 & 4.96 \\ 
  TGARCH-STD & 5 & 6.93 & 0 & 0 & 0 & 2.31 \\ 
   \hline
\hline
\end{tabular}
\caption{Results for the VaR forecasts from 1 July 1996 to 30 June 2016 for Standard and Poors 500.} 
\end{table}


==> Tables/Results_Tunig_Results_Case_1.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sat Jan 28 13:51:46 2017
%\begin{sidewaystable}

\begin{table}[h!t]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
  \hline
  \hline
\textbf{C} & $\boldsymbol{\psi}$ & $\boldsymbol{\gamma}$ & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
0.1 & 0.6 & 0.001 & EuroStoxx50 & 0.5 & 0.47 & 88.82 & 81.14 & 96.24 \\ 
  100 & 0.7 & 0.01 & EuroStoxx50 & 1 & 1.02 & 93.28 & 60.41 & 87.11 \\ 
  0.1 & 0.6 & 0.001 & EuroStoxx50 & 2.5 & 2.52 & 96.42 & 97.76 & 97.66 \\ 
  10000 & 0.6 & 10 & EuroStoxx50 & 5 & 4.96 & 94.86 & 99.71 & 99.50 \\ 
  \hline
1 & 0.7 & 0.001 & S\&P500 & 0.5 & 0.48 & 90.54 & 81.06 & 96.48 \\ 
  10 & 0.7 & 0.1 & S\&P500 & 1 & 0.95 & 86.62 & 63.08 & 87.84 \\ 
  10 & 0.7 & 0.01 & S\&P500 & 2.5 & 2.46 & 93.15 & 96.55 & 96.2 \\ 
  10 & 0.6 & 0.001 & S\&P500 & 5 & 5 & 99.48 & 99.57 & 99.57 \\ 
  \hline
10 & 0.8 & 0.01 & Nikkei225 & 0.5 & 0.41 & 63.92 & 83.95 & 87.77 \\ 
  100 & 0.8 & 0.01 & Nikkei225 & 1 & 0.82 & 50.63 & 68.48 & 73.85 \\ 
  100 & 0.7 & 0.01 & Nikkei225 & 2.5 & 2.7 & 66.43 & 57.80 & 52.61 \\ 
  100 & 0.7 & 0.10 & Nikkei225 & 5 & 4.49 & 40.84 & 94.38 & 67.06 \\ 
   \hline
\hline
\end{tabular}
\caption[Grid search results for SVR parameter tuning]{The best models in the tuning period according to the p-value of the test for conditional coverage.
                      UC, ID and CC indicate the p-value of the corresponding LR test. All values in the columns Quantile, Violations,
                      UC, ID and CC are given in percent.} 
\label{Tab:tuning_case1}
\end{table}
%\end{sidewaystable}

==> Tables/Results_Tunig_Results_Case_1_Only_1to5.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sat Jan 28 13:51:46 2017
%\begin{sidewaystable}

\begin{table}[h!t]
\centering
\begin{tabular}{c|c|c|c|c|c|r|r|r}
  \hline
  \hline
\textbf{C} & $\boldsymbol{\psi}$ & $\boldsymbol{\gamma}$ & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
  10 & 0.7 & 0.1 & S\&P500 & 1.0 & 0.95 & 86.62 & 63.08 & 87.84 \\ 
  10 & 0.7 & 0.01 & S\&P500 & 2.5 & 2.46 & 93.15 & 96.55 & 96.20 \\ 
  10 & 0.6 & 0.001 & S\&P500 & 5.0 & 5.00 & 99.48 & 99.57 & 99.57 \\ 
  \hline
  100 & 0.8 & 0.01 & Nikkei225 & 1.0 & 0.82 & 50.63 & 68.48 & 73.85 \\ 
  100 & 0.7 & 0.01 & Nikkei225 & 2.5 & 2.70 & 66.43 & 57.80 & 52.61 \\ 
  100 & 0.7 & 0.10 & Nikkei225 & 5.0 & 4.49 & 40.84 & 94.38 & 67.06 \\ 
      \hline
	100 & 0.7 & 0.01 & EuroStoxx50 & 1.0 & 1.02 & 93.28 & 60.41 & 87.11 \\ 
  0.1 & 0.6 & 0.001 & EuroStoxx50 & 2.5 & 2.52 & 96.42 & 97.76 & 97.66 \\ 
  10000 & 0.6 & 10 & EuroStoxx50 & 5.0 & 4.96 & 94.86 & 99.71 & 99.50 \\ 
   \hline
\hline
\end{tabular}
\caption[Grid search results for SVR parameter tuning]{The best models in the tuning period according to the p-value of the test for conditional coverage.
                      UC, ID and CC indicate the p-value of the corresponding LR test. All values in the columns Quantile, Violations,
                      UC, ID and CC are given in percent.} 
\label{Tab:tuning_case1}
\end{table}
%\end{sidewaystable}

==> source code Version for upload/Sections/AlteLiliIntro.tex <==
\section{Introduction}\label{Sec:intro}

Events as the world wide stock market crashes in 1987 and 2008 as well as the outcomes of the 2016 referendum in the UK or the presidential election in the USA came unexpected for most people. Therefore, from the perspective of financial risk management the words of Emil Gumbel, who made important contributions to the field of extreme value statistics, should be marked: \textit{"Il est impossible que l`improbable n`arrive jamais." (It is impossible for the improbable to never occur.)} \cite[p. 200]{Gumbel.1958}. Since such events happen rarely, they occur as outliers in data series. However, they can have a big impact on the solvency of single institutions and the whole economy. 
%For instance, strategical decisions that are based on models which underestimate existing market risks can result in large losses or even bankruptcy of the institution. If a system-relevant financial institution goes bankrupt, it can cause an economic crisis. Additionally, systematically overestimated market risk can prevent institutions from taking actions to generate profits. Thus, the use of appropriate models for measuring market risk results in a competitive advantage. 
\\
\noindent The importance of risk management for financial institutions and the economy drew researchers attention to the development of tools for handling risk. One of the most famous measures of uncertainty in financial markets is Value-at-Risk (VaR) which is e.g. described in detail by \cite{Alexander.2010} and \cite{Jorion.2009}. VaR is based on the quantiles of a portfolio's loss distribution. It can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable number. However, the use of VaR has been criticized. For instance, \cite{Artzner.1999} note that VaR is not subadditive and therefore no coherent risk measure. As a consequence, diversification can increase VaR. Despite this, regulatory frameworks for the banking and insurance industry as Basel III or Solvency II rely on VaR for the determining capital requirements of financial institutions. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{Kuester.2005} compare the performance of several classical statistical approaches for estimating VaR. 
%Moreover, a comprehensive overview over existing statistical methods is given. 
Four categories are suggested to describe existing methods for VaR estimation. 
These categories are historical simulation, fully parametric models, extreme value theory and quantile regression. In the empirical study VaR models belonging to the location scale class are superior over other approaches. In the domain of ML the literature for quantile estimation focuses mainly on neural networks (NN) and SVR. For instance, the derivation of a general approach without an explicit target application can be found in \cite{White.1992}. He used single hidden layer feedforward NNs to derive a way for nonparametric conditional quantile estimation and proved its consistency. However, the ML VaR literature is not as broad as in classical statistics. 
%Hence, this section also reviews literature where methods for the construction of prediction intervals (PI) were introduced that could be used in the estimation of VaR. Consequently, the reviewed literature is divided in three paragraphs: Prediction Intervals, Value-at-Risk and Data Driven Value-at-Risk.Here, the first two review the existing literature, whereas the last motivates the method proposed in this paper.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent 
\paragraph{Data Driven Value-at-Risk} 
One approach for estimating VaR is based on generalized autoregressive conditional heteroscedasticity (GARCH) models. For example, in an empirical study with more than 30 years of historical returns \cite{Kuester.2005} show that VaR forecasts which are based on standard GARCH models are relatively good compared to other methods. However, they have a linear and parametric structure. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation (MLE)  \citep{Bollerslev.1986}. This makes it necessary to make distributional assumptions. 
%However, the distribution of financial returns were empirically shown to have fat tails and being skewed \citep{Bali.2008,Harvey.2000}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{Franke.2006} estimate VaR for the German stock index (DAX) by fitting the mean and volatility of the return series with NNs. The mean is modeled autoregressively and the volatility is assumed to follow an autoregressive conditionally heteroscedastic (ARCH) process. Moreover, they include external regressors in both models. The predicted mean and variance are used with the normal distribution to derive the VaR and expected shortfall. As benchmark serves a standard GARCH model based on assuming normality of innovations. In terms of VaR exceedances their model is superior. Moreover, they note its ability to quickly adjust the volatility in case of shocks with only short impact. Another approach directly related to VaR is proposed by \cite{Dunis.2010} which use higher order NNs to forecast VaR. A hybrid model using higher order NNs for variance forecasting and RiskMetrics is shown to outperform other hybrid models empirically. They note also the relatively bad results of the unconditional POT method for quantile estimation. This is, however, not an appropriate comparison when benchmarked to conditional models as was e.g. shown by \cite{Kuester.2005}. 
%\cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test.
%Therefore, assuming e.g. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Assuming e.g. normality can lead to an underestimation of risk. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Data Driven Value-at-Risk} 
Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. 
%In contrast, s
Support vector regression (SVR) introduced by \cite{Vapnik.1995,Vapnik.1998} is a method originating in statistical learning theory and was derived based on minimizing the generalization error. SVR can be classified as a method belonging to the domain of machine learning (ML). \cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test. A multiperiod VaR model was introduced by \cite{Xu.2016}. They use an exponentially weighted support vector quantile regression. In the corresponding empirical study, their approach outperforms other methods that are based on GARCH models, filtered historical simulation and quantile regression. Evaluation was done with different measures as e.g. mean absolute error and p-values of prediction tests.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By considering the different model types presented in study of \cite{Kuester.2005}, they can be classified as quantile regression models. In the empirical study of  the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and peaks-over-threshold had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. 
Most of the proposed methods in the ML literature for estimating VaR 
%or PIs 
are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this paper. \\
%Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions.
%Additionally, k
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Kernel density estimation (KDE) is a nonparametric method to estimate the density of a random variable \citep{Hardle.2004}. 
%%%%%% Härdle %%%%%%%%%%%
Given a multi-market setting, \cite{Haerdle.2016} examine the relation between down-side risk and stock returns.
They apply a time varying and time related co-integrated vector auto-regression model with a non-parametric Kernel density estimation with a double exponential Laplace kernel. 
Furthermore,given a predefined period of time, the paper questions the impact and relevance of certain higher moments for VaR.
%Dynamics: Vector elements
%higher moments of risk
%VaR
%Stock returns 
%%%%% find source of VaR predictability power
%%%%%%%%%%%%%%%%%Distinction by SVM %%%%%%%%%%%%%%
In this paper a data driven VaR forecasting framework that is based on SVR and KDE is introduced. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Literature added%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions. 

%%%%%%%Chen et Al.
\cite{Chen.2012} employ a parametric approach for the estimation of VaR for four daily series of four stock market indices. Given an asymmetric Laplace distribution, volatility is modeled GRJ-GARCH. Introduced by \cite{Black.1976}, the latter measures leverage effects
%, which is not of interest for this study. 
. 
Inspired by \dots
%\cite{luetal}, %Finde BibTeX Quelle
the model is extended to a time-varying model allowing dynamic higher moments. Parameters are estimated by an adaptive Markov Chain Monte Carlo sampling scheme with the application of the Metropolis-Hastings algorithm with a mixture of Gaussian proposal distributions. 
%In difference the simulation performed the paper, this approach 
%%%%%%%%%% REASONS WHY BETTER THAN SIMULATION %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%accuracy \dots

\cite{Schaumburg.2012} combines extreme value theory (EVT) with non-parametric VaR estimation in order to estimate return distributions of four financial stock indexes. Conditional quantiles are estimated by the application of monotonized double kernel local linear regression (DKLL), followed by the implementation of of the EVT peaks over threshold method to standardized 
%nonparametric 
residuals.
The methodology is compared to a parametric conditional autoregressive VaR model. \\
Although this study also applies a non-parametric approach, besides of quantile estimation, KDE density estimation and higher moment
%mean and volatility
estimation via SVR are of residuals are taken into consideration.
%%%%%%%\cite{Kuester.2006} Garch outperforms other models



The aim is to compare the proposed approach with similar parametric GARCH-type models to see whether performance gains can be achieved. \\

\noindent The remainder of the paper is structured as follows. 
%In Section \ref{Sec:Lit_Rev} the literature where ML methods are used to forecast VaR are reviewed. Moreover, approaches that are used to establish prediction intervals but are also a possible framework for modeling VaR are presented as well. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Consequently, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. Based on this, the proposed SVR-GARCH-KDE hybrid is introduced at the end of the section. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions on how to modify the proposed framework for performance improvements are provided in the last section. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% Add text %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %Benefits of machine learning approach
 %


==> source code Version for upload/Sections/Archive/emp_study_short_2017Nov23_short.tex <==
\clearpage

\section{Empirical Study}\label{Sec:emp_study}

\subsection{General Setting}

The SVR-GARCH-KDE hybrid is tested using stock indices to evaluate the performance for different regions. We consider four indices, namely the Euro STOXX 50, S\&P 500 and Nikkei 225 which represent the Euro zone, the USA and Japan, respectively. The analysis is based on the log-returns of the adjusted index closing prices $P_t$:

\begin{equation}
r_t = \log(P_t) - \log(P_{t-1}).
\end{equation}

\noindent We forecast VaR for the quantiles $\alpha \in \{0.005, 0.01, 0.025, 0.05\}$, always considering a forecast horizon of one trading day. In empirical applications, the quality of SVR depends on the kernel and parameter values that need to be set manually. The prevailing approach to determine parameter settings is grid search \citep[e.g.,][]{Lessmann.2017}, which we also apply in this study. For the density estimation via KDE the Gaussian kernel function in combination with Silverman's rule of thumb are used to reduce computational cost. \\

\noindent The evaluation of the models is based on the work of \cite{Christoffersen.1998}. The core of the evaluation is a likelihood ratio test framework, which assess the unconditional and conditional coverage as well as the independence of VaR exceedances. Moreover, \cite{Christoffersen.1998} shows that the test statistic for conditional coverage can be derived as the sum of the test statistics of the test for unconditional coverage and independence of VaR exceedances. Hence, it is possible to test whether the performance of a VaR model in terms of correct conditional coverage is determined by its ability to achieve correct coverage or adjust for changing volatility. This is useful in situations where the model has relatively bad conditional coverage but only one of the test statistics for unconditional coverage or independence is small. As criterion for selecting a model from grid search and evaluate the performance of the SVR-GARCH-KDE hybrid with respect to benchmark models, the $p-$value of the test for conditional coverage is used. Since the null hypothesis corresponds to correct conditional coverage which is the desired property, the one with the highest $p-$value is considered to be the best. \\

\noindent We perform all analyses using the statistical software R. The data has been downloaded from Yahoo Finance using the quantmod package. For SVR, we use the package e1071, which is the R implementation of the LIBSVM library of \cite{Chang.2011}. To reduce computational time, we employ the doParallel package for parallelization of computations. The benchmark methods introduced below are implemented by using the rugarch package. 


\subsection{Benchmark Methods}

To test the SVR-GARCH-KDE hybrid, we compare its performance to the standard GARCH model and some of its variations. In particular, \cite{Franke.2011} state that two of the most important variations are the EGARCH and TGARCH model. Hence, they serve as benchmarks in the empirical comparison. The EGARCH and TGARCH models are introduced by \cite{Nelson.1991} and \cite{Zakoian.1994}, respectively. In contrast to standard GARCH models, both can account for asymmetric behavior with respect to past positive or negative returns. The two main differences between EGARCH and TGARCH models are that the former has a multiplicative and the latter an additive model structure. Moreover, TGARCH models allow for different coefficients depending on the lags whereas EGARCH models capture the asymmetric behavior for all lags with one coefficient.

 The GARCH-type models that \cite{Kuester.2005} analyze are coupled with different error distributions, i.e. the normal distribution, $t$ distribution and skewed $t$ distribution. We adopt this approach, which implies that we compare the SVR-GARCH-KDE hybrid to nine benchmarks.  

%\subsection{Popular Modifications of GARCH Models}
%
%\cite{Franke.2011} state that empirical studies found asymmetric reactions of the volatility depending on the sign of the return. In general, negative returns cause higher volatility than positive. To account for these empirical findings several variations of the standard GARCH model in (\ref{Eq:garch_original}) were proposed. Two crucial models are the exponential GARCH (EGARCH) and threshold GARCH (TGARCH) model which are presented below \cite[p. 308]{Franke.2011}.

%\subsubsection{Exponential GARCH Model}
%
%\cite{Nelson.1991} defines the EGARCH model as as follows, with $\omega_t$ and $\lambda_i$ denoting deterministic coefficients: 
%
%\begin{equation}
%\log(\sigma^2_t)  = \omega_t + \sum_{i = 1}^{\infty} \lambda_i m(z_{t-i}), \quad z_t \sim (0, 1) \ \text{i.i.d.}, \quad \lambda_1 = 1,
%\label{Eq:egarch_def}
%\end{equation}
%
%\noindent where
%
%\begin{equation}
%m(z_t) = \rho z_t + \gamma(|z_t| - \mathbb{E}[|z_t|]).
%\label{Eq:egarch_def_asyfct}
%\end{equation}
%
%\noindent Parameters $\rho$ and $\gamma$ are weights that need to be estimated. From $z_t \sim (0, 1) \ \text{i.i.d.}$ follows that $m(z_t)$ is i.i.d. with zero mean. There are some notable differences between the GARCH and EGARCH model. In equation (\ref{Eq:egarch_def}) $\sigma_t^2$ depends multiplicatively on past disturbances. This is in contrast to the standard GARCH model that depends additively on the mean model disturbances. Further, the asymmetric behavior of volatility is taken into account by $m(z_t)$ in (\ref{Eq:egarch_def}). Another difference is that there are no restrictions on the parameters in (\ref{Eq:egarch_def}) and (\ref{Eq:egarch_def_asyfct}).
%
%
%\subsubsection{Threshold GARCH Model}
%
%The TGARCH model is introduced by \cite{Zakoian.1994}. In TGARCH, asymmetries in the volatility are taken into account by modeling them as function of positive and negative disturbances. In contrast to the GARCH and EGARCH approach, \cite{Zakoian.1994} models the standard deviation rather than the variance. This is based on the work of \cite{Davidian.1987}, who find using absolute rather than squared disturbances to result in more efficient variance estimates. % \citep[p. 2]{Zakoian.1994}.
%Formally, with $u_t^+ = \max(u_t, 0)$ and $u_t^- = \min(u_t, 0)$ the TGARCH($p$,$q$) model is defined as:
%
%\begin{align}
%u_t &= \sigma_t z_t, \quad z_t \sim (0, 1) \ \text{i.i.d.},\\
%\sigma_t &= \omega + \sum_{i = 1}^{q} \delta_i^+ u_{t-i}^+ + \sum_{i = 1}^{q} \delta_i^- u_{t-i}^- + \sum_{j = 1}^{p} \theta_j \sigma_{t-i}.
%\label{Eq:tgarch_def}
%\end{align}
%
%\noindent \cite{Zakoian.1994} points out differences to the EGARCH model. First, the TGARCH model is additive whereas the EGARCH model is multiplicative due to modeling the logarithm of $\sigma^2_t$. Moreover, for EGARCH models, asymmetry is captured by the same structure for all lags since the coefficients in (\ref{Eq:egarch_def_asyfct}) are constant. In contrast, TGARCH models allow for different coefficients depending on the lag. 

\subsection{Results}
%\subsection{Analysis for $\boldsymbol{\mu_t = 0}$ and GARCH(1,1)}

\subsubsection{Model Setting and Tuning}

We assume the mean process of $r_t$ in (\ref{Eq:svr_mean_estimate}) is zero. Moreover, we assume the variance process to have one AR and one MA part. These assumptions are imposed on both the SVR-GARCH-KDE hybrid and the benchmark models. We then forecast VaR  for every index trading day from 2011-07-01 until 2016-06-30. The data is  scaled to zero mean and unit variance in the SVR step; as suggested in the documentation of the e1071 package. Model training is done in a moving window approach using 251 return observations, which corresponds to approximately one trading year. Here, a trading year is assumed to have 252 price observations. Hence, one observation less is available when returns are considered. Tuning is done using the same moving window approach for forecasting VaR from 2006-07-01 until 2011-06-30. The considered parameter values in the grid for SVR are

\begin{itemize}
	\item $C \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$
	\item $\psi \in \{0, 0.1, \dots, 0.9 \}$  where $\epsilon = Q_{u^2_{scale}}(\psi)$
	\item $\gamma \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$.
\end{itemize}    
 

\noindent Note that the second point indicates that tuning is not done over fixed values of $\epsilon$. Instead, in every step of the estimation, $\epsilon$ is determined based on the $\psi$-quantile of the squared scaled disturbances of the mean model. This corresponds to the squared scaled returns because we assume zero mean of $r_t$. The motivation behind this is the tendency of returns to form volatility clusters. Hence, a fixed $\epsilon$ can lead to good results in one volatility regime but might have a poor performance after a regime change. For instance, in the case of a financial crisis, the right tail of the distribution of past volatilities gets thicker. Hence, an $\epsilon$ that depends on the quantile of the distribution will increase such that large volatilities have automatically a higher influence on the estimated parameters from the SVR optimization. By using squared values it is ensured that only positive values are obtained for $\epsilon$. However, notice that the distribution of the scaled squared disturbances, which are used in the SVR training, is shifted to the left of the distribution of the squared scaled disturbances. Hence, it is possible that for high values of $\psi$ no observations are outside the $\epsilon$-tube such that the model cannot be estimated.     \\

\noindent The parameter settings that resulted in the best models for the SVR-GARCH-KDE hybrid during the tuning period are shown in Table \ref{Tab:tuning_case1}.  
It can be seen that especially for $\psi$ only a certain range appears among the best models. Moreover, the optimal $\psi$ tends to be higher for lower quantiles. Based on the obtained parameters, VaR forecasts are produced from 2011-07-01 until 2016-06-30. 
%For all indices and parameter settings no results were obtained for $\psi = 0.9$ due to R returning the error message "Model is empty!". This is caused by the point described in the passage above, meaning that for $\psi = 0.9$ no values are left for SVR model training.

%\vspace{-1cm}
%\input{Tables/Case_1Results_Case1_EuroStoxx50.tex}
%\clearpage

\subsubsection{Model Comparison}

\noindent The results of the simulations are presented for each quantile separately in the Tables \ref{Tab:case1_0.5}, \ref{Tab:case1_1}, \ref{Tab:case1_2.5} and \ref{Tab:case1_5} at the end of the section. To clearly identify the best performing models, every table is sorted in descending order for every index according to the p-value of the conditional coverage test. The abbreviations NORM, STD and SSTD indicate the normal, $t$ and skewed $t$ distribution, respectively. Additionally, the column headers UC, ID and CC refer to the corresponding $p$-value of the LR test for unconditional coverage, independence of violations and conditional coverage.  

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.005}$}
 For the Euro STOXX 50, the SVR-GARCH-KDE hybrid has together with the TGARCH-STD and TGARCH-SSTD model the best results according to their p-values of the LR test for conditional coverage. However, all models have low CC values in comparison to the other time series. This comes from many violations which lead to low values in the LR test for UC. Despite having the most independent violations for the Nikkei 225, there are five models being better than the SVR-GARCH-KDE hybrid according to the CC value. This is mainly caused due to overestimating the market risk; as shown by the violations. In practice, risk overestimation is more desirable than underestimation. In particular, overestimation may lead to some potential profits not being  realized, whereas risk underestimation can lead to bankruptcy in the short term. The SVR-GARCH-KDE hybrid is the second best model in terms of unconditional coverage for the S\&P 500 but tends to form violation clusters. This can be concluded from the $p$-value in the ID column. As a result, only the GARCH-NORM and EGARCH-NORM model perform worse in terms of CC. 

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.01}$}  As for $\alpha = 0.005$, the SVR-GARCH-KDE hybrid is the best model for the Euro STOXX 50 for $\alpha = 0.01$. A visualization of its performance is given in Figure~\ref{Fig:model_comparision_SP500_1}. It is compared to the EGARCH-NORM model, which ranked worst. Here, the SVR-GARCH-KDE hybrid estimates in general higher values for VaR than the EGARCH-NORM model and exhibits more variability. The results are also similar to the 0.5\% level for the S\&P 500 and Nikkei 225, meaning that the SVR-GARCH-KDE hybrid has an average performance for both series. Moreover, this is again caused by having a low unconditional coverage for the Nikkei 225 and a tendency to form violation clusters for the S\&P 500.  In addition, the models coupled with a normal distribution perform poorly for all indices for $\alpha \in \{0.005, 0.01\} $. This comes as no surprise since the distribution of asset returns is usually leptokurtic. Accordingly, models that are coupled with a skewed $t$ distribution perform best.

\begin{figure}[h]
\centering
\includegraphics[scale = 0.65]{Figures/VaR_Plots_ES1}
\caption[SVR-GARCH-KDE and EGARCH-NORM for the Euro STOXX 50 at $\alpha = 0.01$]{VaR forecast model comparison for the Euro STOXX 50 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the EGARCH-NORM model.}
\label{Fig:model_comparision_SP500_1}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.025}$} The performance of the SVR-GARCH-KDE hybrid at the 2.5\% level is not as good as for $\alpha \in \{0.005, 0.01\}$ for the Euro STOXX 50. We observe the lowest $p$-value in the test for independence of violations. Interestingly, although the TGARCH and EGARCH model account for asymmetries in volatility, the former is the best and the latter the worst variance model. A relatively high risk overestimation for the S\&P 500 and Nikkei 225 causes the SVR-GARCH-KDE hybrid to be on the sixth and ninth rank, respectively. Rank nine is the worst that the SVR-GARCH-KDE hybrid achieves across all comparisons. A visual inspection of the model's performance compared to the GARCH-SSTD model, which performed best, is given in Figure \ref{Fig:model_comparision_SP500_5}.  
\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.65]{Figures/VaR_Plots_Nik25}
	\caption[SVR-GARCH-KDE and GARCH-SSTD for the Nikkei 225 at $\alpha = 0.025$]{VaR forecast model comparison for the Nikkei 225 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the GARCH-SSTD model.}
	\label{Fig:model_comparision_SP500_5}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.05}$} The best performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is rank two for the Nikkei 225. Here, it is only beaten by the EGARCH-SSTD model. For the other indices the SVR-GARCH-KDE hybrid ranks on place five. This is caused by having relatively low $p$-values for the ID test. In terms of UC, the SVR-GARCH-KDE hybrid is the second and third best model for the S\&P 500 and Nikkei 225, respectively. In comparison to the results for $\alpha \in \{0.005, 0.01\}$, the models with a normal distribution are not the worst for $\alpha \in \{0.025, 0.05\}$. However, using the skewed $t$ distribution leads also for $\alpha \in \{0.025, 0.05\}$ to the best rankings.  \\

\noindent Summarizing the results observed across all indices and quantiles, we conclude that the SVR-GARCH-KDE hybrid displays an average performance. Unlike the benchmarks, the SVR-GARCH-KDE hybrid tends to overestimate market risk. This might come from the choice of time interval for SVR parameter tuning. In particular, the tuning period covers the financial crisis of 2008 where market risk was extremely high. However, the SVR-GARCH-KDE hybrid usually outperforms benchmark models coupled with a normal distribution. This can be seen in Table \ref{Tab:mean_ranks} where the mean ranks per index and quantile are presented for each model. Moreover, there is no setting where the models using a normal distribution perform best. This provides further evidence that using the normal distribution to measure market risk is inappropriate. However, models with a skewed $t$ distribution show in many cases the best performance. For instance, the TGARCH model coupled with the skewed $t$ distribution is always among the top three. This confirms the results of previous research related to return distribution being skewed skewed.   
%Table has been moved to appendix

\begin{table}[ht]
	\centering
	\begin{tabular}{l|c}
		\hline
		\hline
		 \textbf{Model} & \textbf{Mean Rank} \\ 
		 \hline
		\hline
		 TGARCH-SSTD & 2.1 \\ 
		 GARCH-SSTD & 2.4 \\ 
		 EGARCH-SSTD & 4.8 \\ 
		 TGARCH-STD & 4.8 \\ 
		 SVR-GARCH-KDE & 4.9 \\ 
		 GARCH-STD & 5.7 \\ 
		 TGARCH-NORM & 6.3 \\ 
		 GARCH-NORM & 6.6 \\ 
		 EGARCH-STD & 7.8 \\ 
		 EGARCH-NORM & 8.7 \\ 
		\hline
		\hline
	\end{tabular}
	\caption[Model comparison via mean ranks]{The models are presented with their mean rank. The mean rank was computed per index and quantile using the ties method \textit{min} in the \textit{frankv} function of the R package  data.table. The lower the mean rank, the better the model.}
	\label{Tab:mean_ranks}
\end{table}

%\clearpage
\newgeometry{left=6cm, right=1cm, top=3.5cm,bottom=1cm}
%\vspace*{-1cm}
\input{Tables/Results_Tunig_Results_Case_1.tex}

\input{Tables/Results_Case1_05.tex}
%\clearpage

%\vspace{-1cm}
\input{Tables/Results_Case1_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_5.tex}
%\clearpage
\restoregeometry

\clearpage

==> source code Version for upload/Sections/IntroLili.tex <==
%\section{Introduction}\label{Sec:intro}
%%%%%%%%%%%%%%%%%%%%
%Description%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\iffalse
This is a suggested introduction by Lili Matic.
\fi
%%%%%%%%%%%%%%%%%%%%%
%%Introducing words%%
%%%%%%%%%%%%%%%%%%%%%
Events as the world wide stock market crashes in 1987 and 2008 as well as the outcomes of the 2016 referendum in the UK or the presidential election in the USA came unexpected for most people. However, as these examples illustrate, unlikely events occur at times and may have far reaching consequences. Risk management is the practice to analyze the macro-environment of an organization, identify possible adverse developments, and develop suitable countermeasures. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% Out %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Therefore, from the perspective of financial risk management the words of Emil Gumbel, who made important contributions to the field of extreme value statistics, should be marked: \textit{"Il est impossible que l`improbable n`arrive jamais." (It is impossible for the improbable to never occur.)} \cite[p. 200]{Gumbel.1958}. Since such events happen rarely, they occur as outliers in data series. However, they can have a big impact on the solvency of single institutions and the whole economy. 
For instance, strategical decisions that are based on models which underestimate existing market risks can result in large losses or even bankruptcy of the institution. If a system-relevant financial institution goes bankrupt, it can cause an economic crisis. Additionally, systematically overestimated market risk can prevent institutions from taking actions to generate profits. Thus, the use of appropriate models for measuring market risk results in a competitive advantage. 
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%% Risk Management %%
%%       VAR       %%
%%%%%%%%%%%%%%%%%%%%%
For financial institutions and systemically important institutions in particular, a key risk management task is to sustain solvency under adverse economic conditions \citep[e.g.,][]{Silva.2017, Kraus.2017}. One of the most popular measures of uncertainty in financial markets is Value-at-Risk (VaR) (e.g., \cite{Alexander.2010}). VaR is based on the quantiles of a portfolio's $P\&L$ distribution andcan be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable number \citep[e.g.,][]{Chen.2012}. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% VaR critique %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Comment: Misfits to text, however component of text. Ideas welcomed !
%However, the use of VaR has been criticized. For instance, \cite{Artzner.1999} note that VaR is not subadditive and therefore no coherent risk measure. As a consequence, diversification can increase VaR. Despite this, 
Regulatory frameworks for the banking and insurance industry such as Basel III or Solvency II also rely on VaR for determining capital requirements. Compared to expected shortfall, an alternative risk measure with superior mathematical properties \citep[e.g.,][]{Kim.2016}, an advantage of VaR may be seen in the fact that its estimation is more robust due the putting less weight on tail risks and large losses which may deteriorate the quality of statistical estimation routines \citep{Sarykalin.2008}. Especially the latter property make VaR the right choice for this paper, which focuses on developing estimates of risk exposure using data-driven forecasting methods.  \\
%%%%%%%%%%%%%%%%%%%%%
%% VAR ESTIMATION %%
%%%%%%%%%%%%%%%%%%%%%
Several approaches have been proposed to estimate VaR including various parametric statistical models and data-driven machine learning algorithms such as neural networks (NN) and support vector regression (SVR). In a seminal study, \cite{Kuester.2005} review several statistical forecasting methods and compare these in a forecasting benchmark. Using more than 30 years of historical returns data, they find standard generalized autoregressive conditional heteroscedasticity (GARCH) models to forecast VaR with relatively high accuracy. \\
GARCH models are also employed by \cite{Chen.2012} to estimate VaR for four daily series of four stock market indices. More specifically, \cite{Chen.2012} they rely on an asymmetric Laplace distribution and model volatility using GJR-GARCH to introduce leverage effects. They then develop a time-varying model to allow for dynamic higher moments. These extensions allow for wider application of the model beyond forecasting. \\  

%%%%%%%%%%
%% Chen %%
%%%%%%%%%%
%\cite{Chen.2012} employ a parametric approach for the estimation of VaR for four daily series of four stock market indices. Given an asymmetric Laplace distribution, volatility is modeled GRJ-GARCH. Introduced by \cite{Black.1976}, the latter measures leverage effects
%, which is not of interest for this study. 
%Inspired by \cite{Lu.2010}, the model is extended to a time-varying model allowing dynamic higher moments. Parameters are estimated numerically. An adaptive Markov Chain Monte Carlo sampling scheme with the application of the Metropolis-Hastings algorithm with a mixture of Gaussian proposal distributions is applied. 
%\begin{center}
%   \textbf{Read comments \dots }  
%\end{center}
%%%%%%%%%%%%%%%
%%% COMMENT %%%
%%%%%%%%%%%%%%%
%In difference the simulation performed the paper, this approach 
%We employ a frequetionistical approach (data driven)
%Maximum likelihood already mentionen \dots 
%Our approach: Non-parametric, no distributional assumption
%Simulation: Numerical iterations depend on \theta_0 (higher error)
%SVR: Mean & volatility 

Unlike the parametric approach of \cite{Chen.2012}, \cite{Franke.2006} estimate VaR for the German stock index through fitting the mean and volatility of the return series using NN. More specifically, they model the mean and volatility as an autoregressive and autoregressive conditionally heteroscedastic (ARCH) process, respectively. To derive VaR and expected shortfall, the predicted mean and variance are used with the normal distribution. \cite{Franke.2006} find this approach to outperform a standard GARCH model in terms of VaR exceedances. Moreover, they note the model's ability to quickly adjust  volatility in case of shocks with only short impact. \cite{Dunis.2010} propose another NN-based approach toward forecasting VaR and conditional VaR. \\
\cite{Khan.2011} develop a VaR-model that forecast realized volatilities using a combination of a heterogeneous autoregressive (AR) model and SVR. VaR is then computed based on the normal, $t$ and skewed $t$ distribution. Applying this model to 5- and 15-minutes return data, \cite{Khan.2011} is able to confirm the suitability of the SVR component.  \cite{Stankovic.2015} provide further evidence that SVR is a useful method for VaR forecasting. \cite{Xu.2016} introduce a multiperiod VaR model using SVR in a quantile regression framework. This approach is shown it outperform GARCH models. \\
The findings of \cite{Xu.2016} seem to disagree prior results of \cite{Kuester.2005} where GARCH models have been found to predict VaR with high accuracy and more accurately than approaches based on quantile regression in particular. Implementation of the quantile regression using a data-driven SVR model might be an explanation for this result. Indeed, the linear and parametric structure of standard GARCH models might be a limiting factor. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation \citep{Bollerslev.1986}. This necessitates making distributional assumptions, which might be problematic when modeling financial returns, which are characterized by fat tails and large skew \citep{Bali.2008,Harvey.2000}. \\
An approach particularly related to the one proposed in this paper is that of \cite{Schaumburg.2012}. She combines extreme value theory (EVT) with non-parametric VaR estimation to estimate return distributions of four financial stock indexes. A parametric conditional autoregressive value at risk (CAViaR) model serves as benchmark. The benchmark and the proposed model both circumvent the estimation of the mean and variance of the $P\&L$ distribution through predicting a quantile directly. In this regard, the approach of \cite{Schaumburg.2012} can be characterized as a non-parametric CAViaR model. \\
VaR forecasts based on CAViaR frameworks have also been considered in the benchmarking study of \cite{Kuester.2005}. In fact, the authors also introduce a novel CAViaR model in the paper and test is alongside various other VaR models. However, GARCH models and models relying on the $t$ distribution or EVT in particular emerge as most suitable framework for VaR modeling. Therefore, this paper introduces a novel VaR model that bases on the GARCH framework but estimates individual components in a purely non-parametric manner. More specifically, we estimate the mean and variance of the $P\&L$ distribution distribution using using SVR and employ kernel density estimation (KDE) to model the density of the standardized residuals  \citep[e.g.,][]{Hardle.2004}. We then integrate these components to derive a VaR forecast. In summary, the idea of the proposed method is to start from  the most effective parametric modeling approach of \cite{Kuester.2005} and to develop models that estimate its components in a non-parametric manner. Although KDE is not a new  approach in VaR forecasting \citep[e.g.,][]{Haerdle.2016, Schaumburg.2012, Malec.2014}, the particular combination of data-driven VaR estimation using SVR and non-parametric density estimation, which we propose in this paper, has, to the best of our knowledge, not been considered in prior work. \\
We assess the performance of the proposed model in comparison to GARCH-type models with different error distributions also including skewed and fat-tailed distributions. Empirical experiments using data from three major financial indices, namely the Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500), suggest that the SVR-GARCH-KDE hybrid typically outperforms models that are coupled with a normal distribution and performs competitive to benchmark models that use a skewed $t$ distribution. \\

\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%       KDE       %%
%%%%%%%%%%%%%%%%%%%%%
Kernel density estimation (KDE) is a nonparametric method to estimate the density of a random variable. 

%%%% Übergang/Transfer %%%%%%%%
%%%%%%%%%CONS OF GARCH TYPE MODELS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Distributional asumptions %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%However, they 
GARCH-type models 
%have 
are limited by a linear and parametric structure.  
%%%%%%%%%%%%%%%%%%%%%
%% Data driven VAR %%
%%%%%%%%%%%%%%%%%%%%%
\paragraph{Data Driven Value-at-Risk} %Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. 
%%%%%%%%%%%%%%%%%%%%%%% Reshaped text %%%%%%%%%%%%%%%%%%%%%%
There have been attempts to bypass distributional assumptions.
\cite{Wu.2005} prososes SVR and NNs, as these methods do not rely on distributional assumptions. 
By considering the different model types presented in study of \cite{Kuester.2005}, they can be classified as quantile regression models. In the empirical study of the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and peaks-over-threshold had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. Most of the proposed methods in the ML literature for estimating VaR 
%or PIs 
are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. 
%%%%%%%%%%%%%%%%%%%%%%%  Moved  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this paper. 

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Härdle %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
In another VaR related paper, \cite{Haerdle.2016} examine the relation between down-side risk and stock returns. Given a multi-market setting,  they apply, inter alia, co-integrated vector auto-regression and the non-parametric Kernel density estimation. 
%with a double exponential Laplace kernel. 
%Furthermore,given a predefined period of time, the paper questions the impact and relevance of certain higher moments for VaR.
%Dynamics: Vector elements
%higher moments of risk
%VaR
%Stock returns 
%%%%% find source of VaR predictability power
   \begin{center}
   \textbf{Read comments \dots }  
\end{center}
%%%%%%%%%%%%%%%
%%% COMMENT %%%
%%%%%%%%%%%%%%%
%Var estimation and KDE in common
%different focus
%SVE argument
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%  IMPORTANT %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Schaumburg %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
In a non-parametric approach, \cite{Schaumburg.2012} combines extreme value theory (EVT) with non-parametric VaR estimation in order to estimate return distributions of four financial stock indexes. Conditional quantiles are estimated by the application of monotonized double kernel local linear regression (DKLL), followed by the implementation of of the EVT peaks over threshold method to standardized 
%nonparametric 
residuals.
The methodology is compared to a parametric conditional autoregressive VaR model. \\
 \begin{center}
   \textbf{Read comments \dots }  
\end{center}
%%%%%%%%%%%%%%%
%%% COMMENT %%%
%%%%%%%%%%%%%%%
%]
\iffalse
Although this study also applies a non-parametric approach, besides of quantile estimation, KDE density estimation and higher moment
%mean and volatility
estimation of residuals via are not taken into consideration.
%%%%%%%\cite{Kuester.2006} Garch outperforms other models
\\
\fi
%SVR Machine Learning benefits 

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%   Contribution    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper a data driven VaR forecasting framework that is based on SVR and KDE is introduced. In order to obtain a purely data driven location scale VaR approach, we employ a hybrid based on SVR and nonparametric density estimation. 
Its performance %will be 
is evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions. The aim is to compare the proposed approach with similar parametric GARCH-type models to see whether performance gains can be achieved.\\
%%%%%%%%%%%%%
%%%% Idea %%%
%%%%%%%%%%%%%
The uniqueness of this approach is characterized by both  employing a data driven VaR estimation and non-parametric density estimation. To the best of our knowledge, this is the work that applies this methodology for VaR estimator.\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Structure  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent The remainder of the paper is structured as follows. 
%In Section \ref{Sec:Lit_Rev} the literature where ML methods are used to forecast VaR are reviewed. Moreover, approaches that are used to establish prediction intervals but are also a possible framework for modeling VaR are presented as well. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Consequently, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. Based on this, the proposed SVR-GARCH-KDE hybrid is introduced at the end of the section. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions on how to modify the proposed framework for performance improvements are provided in the last section.

















==> source code Version for upload/Sections/New_literature.tex <==
\section{Literature Review}\label{Sec:Lit_Rev}

%%%%%%%Chen et Al.
\cite{Chen.2012} employ a parametric approach for the estimation of VaR for four daily series of four stock market indices. Given an asymmetric Laplace distribution, volatility is modeled GRJ-GARCH. Introduced by \cite{black76}, the latter measures leverage effects
%, which is not of interest for this study. 
. 
Inspired by \dots
%\cite{luetal}, %Finde BibTeX Quelle
the model is extended to a time-varying model allowing dynamic higher moments. Parameters are estimated by an adaptive Markov Chain Monte Carlo sampling scheme with the application of the Metropolis-Hastings algorithm with a mixture of Gaussian proposal distributions. 
%Non parametric approach perks (underestimation left out..)
%In difference the simulation performed the paper, this approach 
%%%%%%%%%% REASONS WHY BETTER THAN SIMULATION %%%%%%%%%%%%%%%%%

%%%%%% Härdle %%%%%%%%%%%
Given a multi-market setting, \cite{haerdleetal} examine the relation between down-side risk and stock returns.
They apply a time varying and time related co-integrated vector auto-regression model with a non-parametric Kernel density estimation with a double exponential Laplace kernel. 
Furthermore,given a period of time, the paper questions the impact and relevance of certain higher moments for VaR.
%Dynamics: Vector elements
%higher moments of risk
%VaR
%Stock returns 
%%%%% find source of VaR predictability power
%%%%%%%%%%%%%%%%%Distinction by SVM %%%%%%%%%%%%%%%%%


%%%%%%%% Schaumburg 1 %%%%%%%%%%%%
\cite{Schaumburg.2012} combines extreme value theory (EVT) with non-parametric VaR estimation in order to estimate return distributions of four financial stock indexes. Conditional quantiles are estimated by the application of monotonized double kernel local linear regression (DKLL), followed by the implementation of of the EVT peaks over threshold method to standardized 
%nonparametric 
residuals.
The methodology is compared to a parametric conditional autoregressive VaR model. \\
Although this study also applies a non-parametric approach, besides of quantile estimation, KDE density estimation and higher moment
%mean and volatility
estimation via SVR are of residuals are taken into consideration.
%%%%%%%\cite{Kuester.2006} Garch outperforms


%%%%%% Schaumburg 2 %%%%%%%%%%%%%%
%%%%%%%%%Formulieren%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
















==> source code Version for upload/Sections/abstract.tex <==
\clearpage

{\LARGE{\bf \noindent Data Driven Value-at-Risk Forecasting \\ \vspace{0.1cm} \noindent Using a SVR-GARCH-KDE Hybrid}} \vspace{0.5cm}

\vspace{0.5cm}

%{\large Master Thesis by: \\ \vspace{0.1cm} \LARGE Marius Lux (558415)}

\section*{Abstract}

Appropriate risk management is crucial to ensure the competitiveness of financial institutions and stability of the economy. One widely used financial risk measure is \mbox{Value-at-Risk (VaR)}. VaR estimations that are based on linear and parametric models which are e.g. coupled with a normal distribution can lead to risk underestimation. This is caused by the time varying volatility, skewness and leptokurtosis of financial return series. Hence, a nonlinear and nonparametric framework to forecast VaR is introduced. The mean and volatility are modeled via support vector regression~(SVR) where the volatility model is motivated by the standard generalized autoregressive conditional heteroscedasticity (GARCH) formulation. Based on this, VaR is derived by applying kernel density estimation (KDE). Additionally, the SVR-GARCH-KDE hybrid is compared to standard, exponential and threshold GARCH models that are coupled with different error distributions. To examine the performance in different markets, one-day-ahead forecasts are produced for three indices, i.e. Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500). Model evaluation is done via a likelihood ratio based test framework for interval forecasts. The SVR-GARCH-KDE hybrid has a competitive performance. In most cases it outperforms models that are coupled with a normal distribution. However, benchmark models that are using a skewed t distribution have usually a better performance. \\

% For instance, it is the best model for the Euro STOXX 50 for the 0.5\% and 1\% quantile. In contrast, only one benchmark model performs worse for the Nikkei 225 at the 2.5\% level. \\

\noindent \textbf{Keywords:} Value-at-Risk, Support Vector Regression, Kernel Density Estimation, GARCH



==> source code Version for upload/Sections/conc.tex <==
\section{Conclusion}\label{Sec:Conc}
%$\R$
%\newline
%In the empirical study of \cite{Kuester.2005} VaR models belonging to the location-scale class were superior over other approaches. However, the mean and volatility processes of the proposed location-scale models were parametric and based on distributional assumptions. Moreover, assumptions were also made for the distribution of the standardized residuals. Motivated by this, a nonparametric and nonlinear VaR forecasting framework that is based on the location-scale class was introduced in this thesis. The mean and volatility model were proposed to be modeled with SVR in an ARMA and GARCH like fashion, respectively. Additionally, the VaR forecast is obtained by estimating the distribution function of the standardized residuals via KDE. \\

In a large-scale empirical comparison \cite{Kuester.2005} find VaR models belonging to the location-scale class superior to alternative approaches. However, the location-scale models considered in their study are parametric and based on distributional assumptions. Motivated by the potential shortcomings of a parametric approach, the paper introduces a nonparametric and nonlinear VaR forecasting framework based on the location-scale class. The mean and volatility model are modeled with SVR in an ARMA and GARCH like fashion, respectively. In addition, the VaR forecast is obtained by estimating the distribution function of the standardized residuals via KDE. 

To evaluate the performance of the SVR-GARCH-KDE hybrid, VaR is forecasted for three indices: Euro STOXX 50, Nikkei 225 and S\&P 500, considering the different quantiles of $\alpha \in \{0.01, 0.025, 0.05\}$ for forecast horizons of one and ten days. GARCH, EGARCH and TGARCH models coupled with the normal, $t$- and skewed $t$-distribution serve as benchmarks and are compared to the proposed model using a LR testing framework for interval forecasts \citep{Christoffersen.1998} and the SPA test of \cite{Hansen.2005}. Grid search with the goal to maximize the $p$-value of the LR test for conditional coverage is used to set the SVR parameters. The SVR-GARCH-KDE hybrid delivers competitive results. For instance, in case of the one-day-ahead forecast horizon it is the best model for the Euro STOXX 50 for $\alpha= 0.01$ and the third best model overall. The TGARCH and GARCH model in combination with the skewed $t$-distribution show the best results. In contrast to the benchmark models, which usually underestimate risk, the SVR-GARCH-KDE hybrid tends to overestimate risk. This can lead to situations where the SVR-GARCH-KDE hybrid has an average performance regarding the $p$-value of the test for conditional coverage. However, with respect to risk management, the use of the SVR-GARCH-KDE might be still favorable over using the benchmarks since all approaches exhibit statistical uncertainty. The tendency to overestimate risk can, therefore, serve as a model risk buffer. This is supported by the results of the SPA test that evaluates the loss function which penalizes especially large VaR violations. For instance, the proposed model has the best performance for the ten-days-ahead forecast horizon. 

\color{red}
In general, the competitive results indicate that the proposed SVR-GARCH-KDE hybrid is a promising alternative. Despite fixing and not retuning the hyperparameters for five years, it is among the top three models with respect to conditional coverage and loss minimization measured by the SPA test for a forecast horizon of one as well as ten days. Additionally, it is the best model in minimizing the loss function for ten-days-ahead forecasts. This indicates the proposed SVR-GARCH-KDE hybrid is a robust VaR modeling approach that is capable of capturing complex nonlinear structures in the volatility process and has the flexibility to model a wide class of tail events. \color{black} Moreover, further improvements can be expected by refining the tuning routine. However, there exist several ways that can lead to an improved performance. First, tuning could be done for more parameters. For instance, in the KDE part of the estimation procedure, the kernel function and bandwidth estimator are set without tuning. Hence, considering different kernel functions and more flexible bandwidth estimators are potential ways to improve the performance further. Moreover, the kernel in the SVR part is also fixed and could be varied. Second, more recent information could be used in the parameter selection by re-tuning the model. Here, tuning is done for a block of five years of data. Then, based on the optimal parameters found for this data block, forecasts for five years are made and the parameters are held fixed. Thus, annual or even shorter re-tuning periods could result in parameters that are more appropriate for the existing market risk. Additionally, refining the grid can also result in better parameter choices.

In addition to modifying the tuning routine, the SVR-GARCH-KDE hybrid could be improved by changing the model specification. Overall, the TGARCH model with the skewed $t$-distribution achieves very good results. Hence, the SVR-GARCH-KDE hybrid could be modified such that it also accounts for asymmetric reactions of the volatility to past returns in a TGARCH like manner. Moreover, the proposed procedure does not ensure that the estimated variances are positive. Here, this problem is handled by replacing non-positive estimates with the last positive. However, positive variance estimates could be ensured by modeling the logarithm of the squared mean model residuals instead. 

All above mentioned adjustments are potential starting points for future research to further improve the proposed framework. However, although the suggested modifications of the tuning procedure are reasonable approaches to improve the model performance, they also increase the computational complexity. After all, this is a slight drawback of the SVR-GARCH-KDE hybrid in comparison to standard models. It is, however offset by potential performance gains. 
 








==> source code Version for upload/Sections/emp_study.tex <==
\clearpage

\section{Empirical Study}\label{Sec:emp_study}

\subsection{General Setting}

The SVR-GARCH-KDE hybrid is tested using stock indices to evaluate the performance for different regions. We consider four indices, namely the Euro STOXX 50, S\&P 500 and Nikkei 225 which represent the Euro zone, the USA and Japan, respectively. The analysis is based on the log-returns of the adjusted index closing prices $P_t$:

\begin{equation}
r_t = \log(P_t) - \log(P_{t-1}).
\end{equation}

\noindent We forecast VaR for the quantiles $\alpha \in \{0.005, 0.01, 0.025, 0.05\}$, always considering a forecast horizon of one trading day. In empirical applications, the quality of SVR depends on the kernel and parameter values that need to be set manually. The prevailing approach to determine parameter settings is grid search \citep[e.g.,][]{Lessmann.2017}, which we also apply in this study. For the density estimation via KDE the Gaussian kernel function in combination with Silverman's rule of thumb are used to reduce computational cost. \\

\noindent The evaluation of the models is based on the work of \cite{Christoffersen.1998}. The core of the evaluation is a likelihood ratio test framework, which assess the unconditional and conditional coverage as well as the independence of VaR exceedances. Moreover, \cite{Christoffersen.1998} shows that the test statistic for conditional coverage can be derived as the sum of the test statistics of the test for unconditional coverage and independence of VaR exceedances. Hence, it is possible to test whether the performance of a VaR model in terms of correct conditional coverage is determined by its ability to achieve correct coverage or adjust for changing volatility. This is useful in situations where the model has relatively bad conditional coverage but only one of the test statistics for unconditional coverage or independence is small. As criterion for selecting a model from grid search and evaluate the performance of the SVR-GARCH-KDE hybrid with respect to benchmark models, the $p-$value of the test for conditional coverage is used. Since the null hypothesis corresponds to correct conditional coverage which is the desired property, the one with the highest $p-$value is considered to be the best. \\

\noindent We perform all analyses using the statistical software R. The data has been downloaded from Yahoo Finance using the quantmod package. For SVR, we use the package e1071, which is the R implementation of the LIBSVM library of \cite{Chang.2011}. To reduce computational time, we employ the doParallel package for parallelization of computations. The benchmark methods introduced below are implemented by using the rugarch package. 


\subsection{Benchmark Methods}

To test the SVR-GARCH-KDE hybrid, we compare its performance to the standard GARCH model and some of its variations. In particular, \cite{Franke.2011} state that two of the most important variations are the EGARCH and TGARCH model. Hence, they serve as benchmarks in the empirical comparison. The GARCH-type models that \cite{Kuester.2005} analyze are coupled with different error distributions, i.e. the normal distribution, $t$ distribution and skewed $t$ distribution. We adopt this approach, which implies that we compare the SVR-GARCH-KDE hybrid to nine benchmarks.  

%\subsection{Popular Modifications of GARCH Models}
%
%\cite{Franke.2011} state that empirical studies found asymmetric reactions of the volatility depending on the sign of the return. In general, negative returns cause higher volatility than positive. To account for these empirical findings several variations of the standard GARCH model in (\ref{Eq:garch_original}) were proposed. Two crucial models are the exponential GARCH (EGARCH) and threshold GARCH (TGARCH) model which are presented below \cite[p. 308]{Franke.2011}.

\subsubsection{Exponential GARCH Model}

\cite{Nelson.1991} defines the EGARCH model as as follows, with $\omega_t$ and $\lambda_i$ denoting deterministic coefficients: 

\begin{equation}
\log(\sigma^2_t)  = \omega_t + \sum_{i = 1}^{\infty} \lambda_i m(z_{t-i}), \quad z_t \sim (0, 1) \ \text{i.i.d.}, \quad \lambda_1 = 1,
\label{Eq:egarch_def}
\end{equation}

\noindent where

\begin{equation}
m(z_t) = \rho z_t + \gamma(|z_t| - \mathbb{E}[|z_t|]).
\label{Eq:egarch_def_asyfct}
\end{equation}

\noindent Parameters $\rho$ and $\gamma$ are weights that need to be estimated. From $z_t \sim (0, 1) \ \text{i.i.d.}$ follows that $m(z_t)$ is i.i.d. with zero mean. There are some notable differences between the GARCH and EGARCH model. In equation (\ref{Eq:egarch_def}) $\sigma_t^2$ depends multiplicatively on past disturbances. This is in contrast to the standard GARCH model that depends additively on the mean model disturbances. Further, the asymmetric behavior of volatility is taken into account by $m(z_t)$ in (\ref{Eq:egarch_def}). Another difference is that there are no restrictions on the parameters in (\ref{Eq:egarch_def}) and (\ref{Eq:egarch_def_asyfct}).


\subsubsection{Threshold GARCH Model}

The TGARCH model is introduced by \cite{Zakoian.1994}. In TGARCH, asymmetries in the volatility are taken into account by modeling them as function of positive and negative disturbances. In contrast to the GARCH and EGARCH approach, \cite{Zakoian.1994} models the standard deviation rather than the variance. This is based on the work of \cite{Davidian.1987}, who find using absolute rather than squared disturbances to result in more efficient variance estimates. % \citep[p. 2]{Zakoian.1994}.
Formally, with $u_t^+ = \max(u_t, 0)$ and $u_t^- = \min(u_t, 0)$ the TGARCH($p$,$q$) model is defined as:

\begin{align}
u_t &= \sigma_t z_t, \quad z_t \sim (0, 1) \ \text{i.i.d.},\\
\sigma_t &= \omega + \sum_{i = 1}^{q} \delta_i^+ u_{t-i}^+ + \sum_{i = 1}^{q} \delta_i^- u_{t-i}^- + \sum_{j = 1}^{p} \theta_j \sigma_{t-i}.
\label{Eq:tgarch_def}
\end{align}

\noindent \cite{Zakoian.1994} points out differences to the EGARCH model. First, the TGARCH model is additive whereas the EGARCH model is multiplicative due to modeling the logarithm of $\sigma^2_t$. Moreover, for EGARCH models, asymmetry is captured by the same structure for all lags since the coefficients in (\ref{Eq:egarch_def_asyfct}) are constant. In contrast, TGARCH models allow for different coefficients depending on the lag. 

\subsection{Results}
%\subsection{Analysis for $\boldsymbol{\mu_t = 0}$ and GARCH(1,1)}

\subsubsection{Model Setting and Tuning}

We assume the mean process of $r_t$ in (\ref{Eq:svr_mean_estimate}) is zero. Moreover, we assume the variance process to have one AR and one MA part. These assumptions are imposed on both the SVR-GARCH-KDE hybrid and the benchmark models. We then forecast VaR  for every index trading day from 2011-07-01 until 2016-06-30. The data is  scaled to zero mean and unit variance in the SVR step; as suggested in the documentation of the e1071 package. Model training is done in a moving window approach using 251 return observations, which corresponds to approximately one trading year. Here, a trading year is assumed to have 252 price observations. Hence, one observation less is available when returns are considered. Tuning is done using the same moving window approach for forecasting VaR from 2006-07-01 until 2011-06-30. The considered parameter values in the grid for SVR are

\begin{itemize}
	\item $C \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$
	\item $\psi \in \{0, 0.1, \dots, 0.9 \}$  where $\epsilon = Q_{u^2_{scale}}(\psi)$
	\item $\gamma \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$.
\end{itemize}    
 

\noindent Note that the second point indicates that tuning is not done over fixed values of $\epsilon$. Instead, in every step of the estimation, $\epsilon$ is determined based on the $\psi$-quantile of the squared scaled disturbances of the mean model. This corresponds to the squared scaled returns because we assume zero mean of $r_t$. The motivation behind this is the tendency of returns to form volatility clusters. Hence, a fixed $\epsilon$ can lead to good results in one volatility regime but might have a poor performance after a regime change. For instance, in the case of a financial crisis, the right tail of the distribution of past volatilities gets thicker. Hence, an $\epsilon$ that depends on the quantile of the distribution will increase such that large volatilities have automatically a higher influence on the estimated parameters from the SVR optimization. By using squared values it is ensured that only positive values are obtained for $\epsilon$. However, notice that the distribution of the scaled squared disturbances, which are used in the SVR training, is shifted to the left of the distribution of the squared scaled disturbances. Hence, it is possible that for high values of $\psi$ no observations are outside the $\epsilon$-tube such that the model cannot be estimated.     \\

\noindent The parameter settings that resulted in the best models for the SVR-GARCH-KDE hybrid during the tuning period are shown in Table \ref{Tab:tuning_case1}.  
It can be seen that especially for $\psi$ only a certain range appears among the best models. Moreover, the optimal $\psi$ tends to be higher for lower quantiles. Based on the obtained parameters, VaR forecasts are produced from 2011-07-01 until 2016-06-30. 
%For all indices and parameter settings no results were obtained for $\psi = 0.9$ due to R returning the error message "Model is empty!". This is caused by the point described in the passage above, meaning that for $\psi = 0.9$ no values are left for SVR model training.

%\vspace{-1cm}
%\input{Tables/Case_1Results_Case1_EuroStoxx50.tex}
%\clearpage

\subsubsection{Model Comparison}

\noindent The results of the simulations are presented for each quantile separately in the Tables \ref{Tab:case1_0.5}, \ref{Tab:case1_1}, \ref{Tab:case1_2.5} and \ref{Tab:case1_5} at the end of the section. To clearly identify the best performing models, every table is sorted in descending order for every index according to the p-value of the conditional coverage test. The abbreviations NORM, STD and SSTD indicate the normal, $t$ and skewed $t$ distribution, respectively. Additionally, the column headers UC, ID and CC refer to the corresponding $p$-value of the LR test for unconditional coverage, independence of violations and conditional coverage.  

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.005}$}
 For the Euro STOXX 50, the SVR-GARCH-KDE hybrid has together with the TGARCH-STD and TGARCH-SSTD model the best results according to their p-values of the LR test for conditional coverage. However, all models have low CC values in comparison to the other time series. This comes from many violations which lead to low values in the LR test for UC. Despite having the most independent violations for the Nikkei 225, there are five models being better than the SVR-GARCH-KDE hybrid according to the CC value. This is mainly caused due to overestimating the market risk; as shown by the violations. In practice, risk overestimation is more desirable than underestimation. In particular, overestimation may lead to some potential profits not being  realized, whereas risk underestimation can lead to bankruptcy in the short term. The SVR-GARCH-KDE hybrid is the second best model in terms of unconditional coverage for the S\&P 500 but tends to form violation clusters. This can be concluded from the $p$-value in the ID column. As a result, only the GARCH-NORM and EGARCH-NORM model perform worse in terms of CC. 

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.01}$}  As for $\alpha = 0.005$, the SVR-GARCH-KDE hybrid is the best model for the Euro STOXX 50 for $\alpha = 0.01$. A visualization of its performance is given in Figure~\ref{Fig:model_comparision_SP500_1}. It is compared to the EGARCH-NORM model, which ranked worst. Here, the SVR-GARCH-KDE hybrid estimates in general higher values for VaR than the EGARCH-NORM model and exhibits more variability. The results are also similar to the 0.5\% level for the S\&P 500 and Nikkei 225, meaning that the SVR-GARCH-KDE hybrid has an average performance for both series. Moreover, this is again caused by having a low unconditional coverage for the Nikkei 225 and a tendency to form violation clusters for the S\&P 500.  In addition, the models coupled with a normal distribution perform poorly for all indices for $\alpha \in \{0.005, 0.01\} $. This comes as no surprise since the distribution of asset returns is usually leptokurtic. Accordingly, models that are coupled with a skewed $t$ distribution perform best.

\begin{figure}[h]
\centering
\includegraphics[scale = 0.65]{Figures/VaR_Plots_ES1}
\caption[SVR-GARCH-KDE and EGARCH-NORM for the Euro STOXX 50 at $\alpha = 0.01$]{VaR forecast model comparison for the Euro STOXX 50 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the EGARCH-NORM model.}
\label{Fig:model_comparision_SP500_1}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.025}$} The performance of the SVR-GARCH-KDE hybrid at the 2.5\% level is not as good as for $\alpha \in \{0.005, 0.01\}$ for the Euro STOXX 50. We observe the lowest $p$-value in the test for independence of violations. Interestingly, although the TGARCH and EGARCH model account for asymmetries in volatility, the former is the best and the latter the worst variance model. A relatively high risk overestimation for the S\&P 500 and Nikkei 225 causes the SVR-GARCH-KDE hybrid to be on the sixth and ninth rank, respectively. Rank nine is the worst that the SVR-GARCH-KDE hybrid achieves across all comparisons. A visual inspection of the model's performance compared to the GARCH-SSTD model, which performed best, is given in Figure \ref{Fig:model_comparision_SP500_5}.  
\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.65]{Figures/VaR_Plots_Nik25}
	\caption[SVR-GARCH-KDE and GARCH-SSTD for the Nikkei 225 at $\alpha = 0.025$]{VaR forecast model comparison for the Nikkei 225 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The upper panel shows VaR forecasts and violations for the SVR-GARCH-KDE hybrid and the lower panel for the GARCH-SSTD model.}
	\label{Fig:model_comparision_SP500_5}	
\end{figure}

\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.05}$} The best performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is rank two for the Nikkei 225. Here, it is only beaten by the EGARCH-SSTD model. For the other indices the SVR-GARCH-KDE hybrid ranks on place five. This is caused by having relatively low $p$-values for the ID test. In terms of UC, the SVR-GARCH-KDE hybrid is the second and third best model for the S\&P 500 and Nikkei 225, respectively. In comparison to the results for $\alpha \in \{0.005, 0.01\}$, the models with a normal distribution are not the worst for $\alpha \in \{0.025, 0.05\}$. However, using the skewed $t$ distribution leads also for $\alpha \in \{0.025, 0.05\}$ to the best rankings.  \\

\noindent Summarizing the results observed across all indices and quantiles, we conclude that the SVR-GARCH-KDE hybrid displays an average performance. Unlike the benchmarks, the SVR-GARCH-KDE hybrid tends to overestimate market risk. This might come from the choice of time interval for SVR parameter tuning. In particular, the tuning period covers the financial crisis of 2008 where market risk was extremely high. However, the SVR-GARCH-KDE hybrid usually outperforms benchmark models coupled with a normal distribution. This can be seen in Table \ref{Tab:mean_ranks} where the mean ranks per index and quantile are presented for each model. Moreover, there is no setting where the models using a normal distribution perform best. This provides further evidence that using the normal distribution to measure market risk is inappropriate. However, models with a skewed $t$ distribution show in many cases the best performance. For instance, the TGARCH model coupled with the skewed $t$ distribution is always among the top three. This confirms the results of previous research related to return distribution being skewed skewed.   
%Table has been moved to appendix

\begin{table}[ht]
	\centering
	\begin{tabular}{l|c}
		\hline
		 \textbf{Model} & \textbf{Mean Rank} \\ 
		 \hline
		\hline
		 TGARCH-SSTD & 2.1 \\ 
		 GARCH-SSTD & 2.4 \\ 
		 EGARCH-SSTD & 4.8 \\ 
		 TGARCH-STD & 4.8 \\ 
		 SVR-GARCH-KDE & 4.9 \\ 
		 GARCH-STD & 5.7 \\ 
		 TGARCH-NORM & 6.3 \\ 
		 GARCH-NORM & 6.6 \\ 
		 EGARCH-STD & 7.8 \\ 
		 EGARCH-NORM & 8.7 \\ 
		\hline
		\hline
	\end{tabular}
	\caption[Model comparison via mean ranks]{The models are presented with their mean rank. The mean rank was computed per index and quantile using the ties method \textit{min} in the \textit{frankv} function of the R package  data.table. The lower the mean rank, the better the model.}
	\label{Tab:mean_ranks}
\end{table}

%\clearpage
\newgeometry{left=6cm, right=1cm, top=3.5cm,bottom=1cm}
%\vspace*{-1cm}
\input{Tables/Results_Tunig_Results_Case_1.tex}

\input{Tables/Results_Case1_05.tex}
%\clearpage

%\vspace{-1cm}
\input{Tables/Results_Case1_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Results_Case1_5.tex}
%\clearpage
\restoregeometry

\clearpage

==> source code Version for upload/Sections/emp_study_short_2017Nov23.tex <==
\section{Empirical Study}\label{Sec:emp_study}

\subsection{General Setting}

The SVR-GARCH-KDE hybrid is tested using stock indices to evaluate the performance for different regions. We consider three indices, namely the Euro STOXX 50, S\&P 500 and Nikkei 225 which represent the Euro zone, the USA and Japan, respectively. The analysis is based on the log-returns of the adjusted index closing prices $P_t$:

\begin{equation}
r_t = \log(P_t) - \log(P_{t-1}).
\end{equation}

\noindent The descriptive statistics of the analyzed indices are given in Table \ref{Tab:desc_stats}.

\input{Tables/Descriptive_Statistics_Adjusted.tex}
\color{red}
We forecast VaR for the quantiles $\alpha \in \{0.01, 0.025, 0.05\}$, considering forecast horizons of one and ten trading days. Estimating VaR for a horizon of ten trading days is especially important regarding the applicability of a VaR model. Besides forecasting VaR for a confidence level of 99\%, which is equivalent to $\alpha = 0.01$ in our setting, a ten days forecast horizon is required in the regulations of the Basel Committee on Banking Supervision. 
\color{black}
In empirical applications, the quality of SVR depends on the kernel and parameter values which need to be set manually. The prevailing approach to determine parameter settings is grid search \citep[e.g.,][]{Lessmann.2017}, which we also apply in this study. For the density estimation via KDE, the Gaussian kernel function in combination with Silverman's rule of thumb are used to reduce computational cost. The Gaussian kernel function in KDE is equivalent to the standard normal distribution:

\begin{equation}
K(u) = \dfrac{1}{2\pi} e^{-\frac{u^2}{2}}.
\label{Eq:kde_gauss}
\end{equation}

\cite{Silverman.1986} showed that when (\ref{Eq:kde_gauss}) is used, robust density estimates can be obtained with the following estimator for the bandwidth $h$:

\begin{equation}
h_{rot} = 0.9 \min\{ \widehat{\sigma}_e, \widehat{\sigma}_{iqr} \} n^{-1/5}.
\label{Eq:kde_silverman}
\end{equation}

In \ref{Eq:kde_silverman} $\widehat{\sigma}_e$ denotes the empirical standard deviation and $\widehat{\sigma}_{iqr}$ is an estimate of the standard deviation that is based on the interquartile range $R$:

\begin{equation}
\widehat{\sigma}_{iqr} = \dfrac{R}{1.34}.
\label{Eq:kde_iqr_sd}
\end{equation}

The rule-of-thumb estimator $h_{rot}$ is computationally inexpensive whereas other proposed approaches to bandwidth estimation are more expensive since they are usually based on cross validation \citep{Hardle.2004}. Moreover, the importance of the kernel choice regarding the performance of KDE is limited. For instance, \cite{Hardle.2004} conclude that the kernel choice has almost no practical relevance after deriving the asymptotic mean integrated squared error for different kernel choices.

The evaluation of the models is based on \cite{Christoffersen.1998} who proposes a likelihood ratio (LR) test framework, which assesses the unconditional and conditional coverage as well as the independence of VaR exceedances. Moreover, \cite{Christoffersen.1998} shows that the test statistic for conditional coverage can be derived as the sum of the test statistics of the test for unconditional coverage and independence of VaR exceedances. Hence, it is possible to test whether the performance of a VaR model in terms of conditional coverage is determined by its ability to achieve correct unconditional coverage or adjust for changing volatility. This is useful in situations where the model has relatively bad conditional coverage but only one of the test statistics for unconditional coverage or independence is small. The hypotheses for the three tests are shown in Table \ref{Tab:hypotheses_cov} where $\alpha$ is the target quantile and $\mathcal{F}_{t-1}$ the information set available at $t-1$. $V_t$ is a series of VaR violations with $V_t = \mathbb{I}(r_t < -VaR_t^{\alpha})$ where $\mathbb{I}(x < c)$ denotes the indicator function:
	\begin{equation}
	\mathbb{I}(x < c) = \begin{cases}
	1 \text{ \ if \ } x < c \\
	0 \text{ \ if \ } x \ge c. \\
	\end{cases} 
	\end{equation}
For the test of independence of violations $V_t$ is assumed to be a binary first-order Markov chain. The corresponding transition probability matrix of $V_t$ is
	
	\begin{equation}
	\Pi_1 = \begin{bmatrix}
	1 - \pi_{01} & \pi_{01} \\
	1 - \pi_{11} & \pi_{11} 
	\end{bmatrix}
	\end{equation}
	
\noindent where 
	
	\begin{equation}
	\pi_{ij} = \mathbb{P}(V_t = j | V_{t-1} = i).
	\end{equation}
	

\begin{table}[ht]
	\centering
	\begin{tabular}{l|l|l}
		\hline
		\textbf{Test} & \boldmath{$\textbf{H}_0$} & \boldmath{$\textbf{H}_1$} \\ 
		\hline
		\hline
		Unconditional Coverage & $\mathbb{E}[V_t] = \alpha$ & $\mathbb{E}[V_t] \ne \alpha$  \\ 
		\hline
		Independence of Violations & $\pi_{01} = \pi_{11}$ & $\pi_{01} \ne \pi_{11}$ \\ 
		\hline
		Conditional Coverage & $\mathbb{E}[V_t| \mathcal{F}_{t-1}] = \alpha$ & $\mathbb{E}[V_t| \mathcal{F}_{t-1}] \ne \alpha$  \\ 

		\hline
		\hline
	\end{tabular}
	\caption{Hypotheses for evaluating the appropriateness of VaR forecasts with the testing framework introduced by \cite{Christoffersen.1998}.
	\label{Tab:hypotheses_cov}} 
\end{table}


 As criterion for selecting a model from grid search and evaluate the performance of the SVR-GARCH-KDE hybrid with respect to benchmark models, the $p$-value of the test for conditional coverage is used. Since the null hypothesis corresponds to correct conditional coverage which is the desired property, the one with the highest $p$-value is considered to be the best. 

\color{red} 
By using the framework of \cite{Christoffersen.1998} to evaluate and select models, the main focus is put on the statistical properties and VaR violations of the considered models. In order to measure the performance from the perspective of a loss function that also takes into account the magnitude of violations, the quadratic and asymmetric loss function that was introduced in one of the seminal papers for evaluating VaR models by \cite{Lopez.1998} will be used: 

\begin{equation}
L(r_t, VaR_t^{\alpha}) = \begin{cases}
1 + (r_t - VaR_t^{\alpha})^2  &\text{ \ if \ } r_t < VaR_t^{\alpha}  \\
0 &\text{ \ if \ } r_t \ge VaR_t^{\alpha}. \\
\end{cases} 
\end{equation}

\noindent The model losses will be evaluated by employing the superior predictive ability test (SPA) framework proposed by \cite{Hansen.2005}. Following the notation of \cite{Hansen.2005}, for a finite set of decision rules $[\delta_{k, t-h}, k = 0, 1, \dots, m]$ made $h$ periods in advance with respect to a random variable $\xi_t$, the relative performance corresponding to the benchmark $\delta_{0, t-h}$ is measured as

\begin{equation}
d_{k,t} = L(\xi_t, \delta_{0, t-h}) - L(\xi_t, \delta_{k, t-h}).
\end{equation}

\noindent Based on the assumption that the alternatives are superior if and only if  $\mathbb{E}[d_{k,t}] > 0$, \cite{Hansen.2005} formulates the hypothesis of interest for $ \boldsymbol{d_t} = (d_{1,t}, \dots, d_{m,t})^\top $ as

\begin{equation}
	 \text{H}_0: \mathbb{E}[\boldsymbol{d_t}] \le \boldmath{0}.
\end{equation}

\noindent A high $p$-value indicates that none of the alternatives is superior to the benchmark. For further information regarding the SPA test we refer to \cite{Hansen.2005}. As for the LR test of \cite{Christoffersen.1998}, the SPA test will be performed for every model. This is done by using every considered model once as benchmark in terms of \cite{Hansen.2005} and comparing it to all other models. Note that due to performing multiple statistical tests the $p$-values should be interpreted rather as an indication of model performance than in the context of a fixed significance level. 

\color{black}

We perform all analyses using the statistical software R. The data has been downloaded from Yahoo Finance using the quantmod package. For SVR, we use the package e1071, which is the R implementation of the LIBSVM library of \cite{Chang.2011}. To reduce computational time, we employ the doParallel package for parallelization of computations. The benchmark methods introduced below are implemented by using the rugarch package. All codes are available on \url{www.quantlet.de}. For details we refer to \cite{Borke.2018} and \cite{Borke.2017}.


\subsection{Benchmark Methods}

To test the SVR-GARCH-KDE hybrid, we compare its performance to the standard GARCH model and two of its variations. In particular, \cite{Franke.2011} state that the most important variations are the EGARCH and TGARCH model. Hence, they serve as benchmarks in the empirical comparison. The EGARCH and TGARCH models are introduced by \cite{Nelson.1991} and \cite{Zakoian.1994}, respectively. In contrast to standard GARCH models, both can account for asymmetric behavior with respect to past positive or negative returns. The two main differences between EGARCH and TGARCH models are that the former has a multiplicative and the latter an additive model structure. Moreover, TGARCH models allow for different coefficients depending on the lags whereas EGARCH models capture the asymmetric behavior for all lags with one coefficient. The GARCH-type models that \cite{Kuester.2005} analyze are coupled with different error distributions, i.e. the normal distribution, $t$-distribution and skewed $t$-distribution. We adopt this approach, which implies that we compare the SVR-GARCH-KDE hybrid to nine benchmarks.  

%\subsection{Popular Modifications of GARCH Models}
%
%\cite{Franke.2011} state that empirical studies found asymmetric reactions of the volatility depending on the sign of the return. In general, negative returns cause higher volatility than positive. To account for these empirical findings several variations of the standard GARCH model in (\ref{Eq:garch_original}) were proposed. Two crucial models are the exponential GARCH (EGARCH) and threshold GARCH (TGARCH) model which are presented below \cite[p. 308]{Franke.2011}.

%\subsubsection{Exponential GARCH Model}
%
%\cite{Nelson.1991} defines the EGARCH model as as follows, with $\omega_t$ and $\lambda_i$ denoting deterministic coefficients: 
%
%\begin{equation}
%\log(\sigma^2_t)  = \omega_t + \sum_{i = 1}^{\infty} \lambda_i m(z_{t-i}), \quad z_t \sim (0, 1) \ \text{i.i.d.}, \quad \lambda_1 = 1,
%\label{Eq:egarch_def}
%\end{equation}
%
%\noindent where
%
%\begin{equation}
%m(z_t) = \rho z_t + \gamma(|z_t| - \mathbb{E}[|z_t|]).
%\label{Eq:egarch_def_asyfct}
%\end{equation}
%
%\noindent Parameters $\rho$ and $\gamma$ are weights that need to be estimated. From $z_t \sim (0, 1) \ \text{i.i.d.}$ follows that $m(z_t)$ is i.i.d. with zero mean. There are some notable differences between the GARCH and EGARCH model. In equation (\ref{Eq:egarch_def}) $\sigma_t^2$ depends multiplicatively on past disturbances. This is in contrast to the standard GARCH model that depends additively on the mean model disturbances. Further, the asymmetric behavior of volatility is taken into account by $m(z_t)$ in (\ref{Eq:egarch_def}). Another difference is that there are no restrictions on the parameters in (\ref{Eq:egarch_def}) and (\ref{Eq:egarch_def_asyfct}).
%
%
%\subsubsection{Threshold GARCH Model}
%
%The TGARCH model is introduced by \cite{Zakoian.1994}. In TGARCH, asymmetries in the volatility are taken into account by modeling them as function of positive and negative disturbances. In contrast to the GARCH and EGARCH approach, \cite{Zakoian.1994} models the standard deviation rather than the variance. This is based on the work of \cite{Davidian.1987}, who find using absolute rather than squared disturbances to result in more efficient variance estimates. % \citep[p. 2]{Zakoian.1994}.
%Formally, with $u_t^+ = \max(u_t, 0)$ and $u_t^- = \min(u_t, 0)$ the TGARCH($p$,$q$) model is defined as:
%
%\begin{align}
%u_t &= \sigma_t z_t, \quad z_t \sim (0, 1) \ \text{i.i.d.},\\
%\sigma_t &= \omega + \sum_{i = 1}^{q} \delta_i^+ u_{t-i}^+ + \sum_{i = 1}^{q} \delta_i^- u_{t-i}^- + \sum_{j = 1}^{p} \theta_j \sigma_{t-i}.
%\label{Eq:tgarch_def}
%\end{align}
%
%\noindent \cite{Zakoian.1994} points out differences to the EGARCH model. First, the TGARCH model is additive whereas the EGARCH model is multiplicative due to modeling the logarithm of $\sigma^2_t$. Moreover, for EGARCH models, asymmetry is captured by the same structure for all lags since the coefficients in (\ref{Eq:egarch_def_asyfct}) are constant. In contrast, TGARCH models allow for different coefficients depending on the lag. 

\subsection{Results}
%\subsection{Analysis for $\boldsymbol{\mu_t = 0}$ and GARCH(1,1)}

\subsubsection{Model Setting and Tuning}

We assume the mean process of $r_t$ in (\ref{Eq:svr_mean_estimate}) is zero. Moreover, we assume the variance process to have one AR and one MA part. These assumptions are imposed on both the SVR-GARCH-KDE hybrid and the benchmark models. We then forecast VaR  for every index trading day from 2011-07-01 until 2016-06-30. The data is scaled to zero mean and unit variance in the SVR step; as suggested in the documentation of the e1071 package. 

The tuning of the hyperparameters is done in a moving window approach using 251 return observations, which corresponds to approximately one trading year. The hyperparameters are tuned for every combination of index and quantile separately. For a given set of hyperparameters the model is trained based on the returns of the last trading year to predict the next day's VaR. Then, the window is shifted by one trading day. The tuning period reaches from 2006-07-01 until 2011-06-30, where 2006-07-01 marks the date of the first VaR prediction. The considered parameter values in the grid for SVR are

\begin{itemize}
	\item $C \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$
	\item $\psi \in \{0, 0.1, \dots, 0.9 \}$  where $\epsilon = Q_{u^2_{scale}}(\psi)$
	\item $\gamma \in \{10^{-4}, 10^{-3}, \dots, 10^4 \}$.
\end{itemize}    
 
Note that the second point indicates that tuning is not done over fixed values of $\epsilon$. Instead, in every step of the estimation, $\epsilon$ is determined based on the $\psi$-quantile of the squared scaled disturbances of the mean model. This corresponds to the squared scaled returns because we assume zero mean of $r_t$. The motivation behind this is the tendency of returns to form volatility clusters. Hence, a fixed $\epsilon$ can lead to good results in one volatility regime but might have a poor performance after a regime change. For instance, in the case of a financial crisis, the right tail of the distribution of past volatilities gets thicker. Hence, an $\epsilon$ that depends on the quantile of the distribution will increase such that large volatilities have automatically a higher influence on the estimated parameters from the SVR optimization. By using squared values it is ensured that only positive values are obtained for $\epsilon$. However, notice that the distribution of the scaled squared disturbances, which are used in the SVR training, is shifted to the left of the distribution of the squared scaled disturbances. Hence, it is possible that for high values of $\psi$ no observations are outside the $\epsilon$-tube such that the model cannot be estimated.    

The parameter settings that resulted in the best models for the SVR-GARCH-KDE hybrid during the tuning period are shown in Table \ref{Tab:tuning_case1}.  
It can be seen that especially for $\psi$ only a certain range appears among the best models. Moreover, the optimal $\psi$ tends to be higher for lower quantiles. Based on the obtained parameters, VaR forecasts are produced from 2011-07-01 until 2016-06-30. 
%\vspace{-1cm}
\input{Tables/Results_Tunig_Results_Case_1_Only_1to5.tex}
%\clearpage

\subsubsection{Model Comparison}

\noindent The results are presented for each quantile separately at the end of the section. In the Tables \ref{Tab:case1_1}, \ref{Tab:case1_2.5} and \ref{Tab:case1_5} are the results for the one-day-ahead forecast. The results for the ten-days-ahead forecasts can be found in the Tables \ref{Tab:case1_10days_1}, \ref{Tab:case1_10days_2.5} and \ref{Tab:case1_10days_5}. To clearly identify the best performing models, every table is sorted in descending order for every index according to the $p$-value of the conditional coverage test. The $p$-value of the conditional coverage test is used for sorting to focus rather on statistical properties than pure losses. The abbreviations NORM, STD and SSTD indicate the normal, $t$- and skewed $t$-distribution, respectively. Additionally, the column headers UC, ID, CC and SPA refer to the corresponding $p$-value of the test for unconditional coverage, independence of violations, conditional coverage and superior predictive ability.  

%\paragraph{Model Evaluation for $\boldsymbol{\alpha = 0.005}$}
% For the Euro STOXX 50, the SVR-GARCH-KDE hybrid has together with the TGARCH-STD and TGARCH-SSTD model the best results according to their p-values of the LR test for conditional coverage. However, all models have low CC values in comparison to the other time series. This comes from many violations which lead to low values in the LR test for UC. Despite having the most independent violations for the Nikkei 225, there are five models being better than the SVR-GARCH-KDE hybrid according to the CC value. This is mainly caused due to overestimating the market risk; as shown by the violations. In practice, risk overestimation is more desirable than underestimation. In particular, overestimation may lead to some potential profits not being  realized, whereas risk underestimation can lead to bankruptcy in the short term. The SVR-GARCH-KDE hybrid is the second best model in terms of unconditional coverage for the S\&P 500 but tends to form violation clusters. This can be concluded from the $p$-value in the ID column. As a result, only the GARCH-NORM and EGARCH-NORM model perform worse in terms of CC. 

\paragraph{One-Step-Ahead Forecast Model Evaluation for $\alpha = 0.01$} The SVR-GARCH-KDE hybrid is the best model for the Euro STOXX 50 for $\alpha = 0.01$. A visualization of its performance is given in Figure~\ref{Fig:model_comparision_estoxx_1}. Here, the SVR-GARCH-KDE hybrid estimates in general higher values for VaR than the other models and exhibits more variability. For the S\&P 500 and Nikkei 225 the SVR-GARCH-KDE hybrid outperforms all models that are coupled with a normal distribution. However, all models using a skewed $t$-distribution perform better. Especially for the Nikkei 225 this is caused by having low unconditional coverage due to risk overestimation. However, since risk overestimation causes less losses the SPA test $p$-value is highest. In general, the models coupled with a normal distribution perform poorly for all indices. This comes as no surprise since the distribution of asset returns is usually leptokurtic. 


\paragraph{One-Step-Ahead Forecast Model Evaluation for $\alpha = 0.025$} The performance of the SVR-GARCH-KDE hybrid at the 2.5\% level is not as good as for $\alpha = 0.01$ for the Euro STOXX 50. We observe the lowest $p$-value in the test for independence of violations but the third best regarding the test for unconditional coverage. Interestingly, although the TGARCH and EGARCH model account for asymmetries in volatility, the former is the best and the latter the worst variance model. A relatively high risk overestimation for the S\&P 500 and Nikkei 225 causes the SVR-GARCH-KDE hybrid to be on the sixth and ninth rank, respectively. As seen for $\alpha = 0.01$ this leads, however, to high $p$-values in the SPA test due to lower losses. The performance for the S\&P 500 can be seen in Figure~\ref{Fig:model_comparision_SP500_25}.

\paragraph{One-Step-Ahead Forecast Model Evaluation for $\alpha = 0.05$} The best performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is rank two for the Nikkei 225. Here, it is only beaten by the EGARCH-SSTD model. A visualization is given in Figure~\ref{Fig:model_comparision_nikkei_5}. For the other indices the SVR-GARCH-KDE hybrid ranks on place five. This is caused by having relatively low $p$-values for the ID test. In terms of UC, the SVR-GARCH-KDE hybrid is the second and third best model for the S\&P 500 and Nikkei 225, respectively. In comparison to the results for $\alpha = 0.01$, the models with a normal distribution show a better performance for $\alpha \in \{0.025, 0.05\}$. However, using the skewed $t$-distribution leads also for $\alpha \in \{0.025, 0.05\}$ to the best rankings.  

\color{red}
\paragraph{Ten-Steps-Ahead Forecast Model Evaluation for $\alpha = 0.01$} As for the one-step-ahead forecasts, the SVR-GARCH-KDE hybrid is also the best model for the Euro STOXX 50. For the S\&P 500 and Nikkei 225 the SVR-GARCH-KDE hybrid is the second and third best model, respectively. For all indices, it is the only model not underestimating the risk. Especially the EGARCH models perform poorly. A visualization is given in Figure~\ref{Fig:model_comparision_nikkei_1_10days}. In contrast to the one-step-ahead forecasts, the models using a normal distribution are not shown but the EGARCH models due to their bad performance for ten-days-ahead forecasts. With respect to the SPA test, the SVR-GARCH-KDE hybrid causes less severe losses than any other model for all levels of the ten-steps-ahead forecast horizon.

\paragraph{Ten-Steps-Ahead Forecast Model Evaluation for $\alpha = 0.025$} Overall, the SVR-GARCH-KDE hybrid performs worse at the 2.5\% than for the 1\% level. In case of the the S\&P 500 and Nikkei 225 this is mainly driven by overestimating the risk leading to low $p$-values in the UC test. In contrast, even though the SVR-GARCH-KDE hybrid has the highest $p$-value in the UC test for the EURO STOXX 50, it is relatively low for the ID test. An exemplary visualization is given for the EURO STOXX 50 in Figure~\ref{Fig:model_comparision_eurostoxx_25_10days}.

\paragraph{Ten-Steps-Ahead Forecast Model Evaluation for $\alpha = 0.05$} The performance of the SVR-GARCH-KDE hybrid for $\alpha= 0.05$ is mixed. While it is by far the best model for the EURO STOXX 50, it achieves only rank seven and nine for the Nikkei 225 and S\&P 500, respectively. As for $\alpha = 0.025$ this is mainly driven by risk overestimation and low $p$-values for the UC test. Similar to the one-day-ahead forecasts, the models using a normal distribution perform better for $\alpha = 0.05$ than for the other quantiles. The TGARCH-NORM model is even the best for the S\&P 500. A visualization is shown in Figure~\ref{Fig:model_comparision_sap_5_10days}. 
\color{black}

\paragraph{Evaluation Summary} Summarizing the results observed across all indices, quantiles and the two forecast horizons, we conclude that the SVR-GARCH-KDE hybrid displays a competitive performance. This can be seen in Table \ref{Tab:mean_ranks} where the mean ranks per index and quantile are presented for each model with respect to the CC and SPA test as well as the two forecast horizons. The SVR-GARCH-KDE hybrid is overall and for the CC test $p$-values the third best model for both forecast horizons. Regarding the SPA test it has rank two for the one-day-ahead forecast horizon and is the best model for the ten-days-ahead forecast horizon. Benchmark models coupled with a normal distribution are usually outperformed by the SVR-GARCH-KDE hybrid. Consequently, the SVR-GARCH-KDE hybrid has a relatively high accuracy especially compared to models with a normal distribution. The importance of this result stems from the fact that GARCH models with a normal distribution can be seen as a popular standard approach for modeling VaR or volatility and are, therefore, a natural benchmark. Additionally, excepting the case of the ten-days-ahead S\&P 500 forecast for $\alpha = 0.05$ there is no setting where the models using a normal distribution perform best. This provides further evidence that using the normal distribution to measure market risk is inappropriate. However, models with a skewed $t$-distribution show in many cases the best performance. For instance, the TGARCH model coupled with the skewed $t$-distribution is with two exceptions always among the top three in terms of the CC test. This confirms the results of previous research showing usually skewed return distributions. Unlike the benchmarks, the SVR-GARCH-KDE hybrid tends to overestimate market risk. This might come from the choice of time interval for SVR parameter tuning. In particular, the tuning period covers the financial crisis of 2008 where market risk was extremely high. However, in the context of risk management, risk underestimation is more critical than risk overestimation because it can lead to bankruptcy in the short term. For instance, assume a hypothetical situation with the goal to forecast the 5\% VaR, where the SVR-GARCH-KDE hybrid and a benchmark model have the same $p$-value regarding the independence test. Additionally, assume the $p$-value of the benchmark in the test of conditional coverage is higher because it has an unconditional coverage of 5.5\% whereas that of the SVR-GARCH-KDE hybrid is 4\%. The 1\% overestimation of the SVR-GARCH-KDE hybrid works like a buffer for model risk since all estimation techniques exhibit statistical uncertainty. Hence, the use of the SVR-GARCH-KDE hybrid may be still more appealing than the use of benchmark models that tend to underestimate risk.    
   
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Table has been moved to appendix

\begin{table}[ht]
	\centering
	\begin{tabular}{l|c|c|c|c|c|c}
		\hline
		 \textbf{Model} & \textbf{Overall} & \textbf{CC 1 Day}  & \textbf{SPA 1 Day}  & \textbf{CC 10 Days} & \textbf{SPA 10 Days}  \\ 
		 \hline
 		\hline
TGARCH-SSTD & 2.3 & 2.2 & 1.4 & 2.3 & 3.2 \\ 
GARCH-SSTD & 2.6 & 2.3 & 2.6 & 2.7 & 2.7 \\ 
SVR-GARCH-KDE & 3.2 & 4.9 & 2.2 & 4.8 & 1.0 \\ 
GARCH-STD & 5.9 & 6.1 & 6.4 & 4.9 & 6.3 \\ 
TGARCH-NORM & 6.0 & 6.0 & 7.7 & 5.1 & 5.1 \\ 
GARCH-NORM & 6.6 & 6.1 & 6.8 & 6.3 & 7.3 \\ 
TGARCH-STD & 6.7 & 5.3 & 9.0 & 5.1 & 7.4 \\ 
EGARCH-SSTD & 6.9 & 5.0 & 5.3 & 9.4 & 7.9 \\ 
EGARCH-NORM & 8.6 & 8.7 & 7.3 & 9.3 & 9.0 \\ 
EGARCH-STD & 8.6 & 8.8 & 7.2 & 9.6 & 8.8 \\ 
		 \hline
		\hline
	\end{tabular}
	\caption[Model comparison via mean ranks]{The models are presented with their mean rank. The mean rank was computed per index and quantile using the ties method \textit{max} in the \textit{frankv} function of the R package data.table. The lower the mean rank, the better the model.}
	\label{Tab:mean_ranks}
\end{table}



%\clearpage

%\vspace*{-1cm}
%\input{Tables/Results_Tunig_Results_Case_1_Only_1to5.tex}

%\newgeometry{left=6cm, right=1cm, top=3.5cm,bottom=1cm}
%\input{Tables/Results_Case1_05.tex}
%\clearpage

%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_1Day_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_1Day_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_1Day_5.tex}
%\clearpage
%\restoregeometry

% Fuer 10-Days-Ahead
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_10Day_1.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_10Day_25.tex}
%\clearpage

%\clearpage
%\vspace{-1cm}
\input{Tables/Case_1/Results_Case1_10Day_5.tex}

%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plots
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1/EuroStoxx50_1VaR}
	\caption{VaR one-day-ahead forecast model comparison for the Euro Stoxx 50 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the models using a normal distribution.}
	\label{Fig:model_comparision_estoxx_1}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1/SaP500_25VaR}
	\caption{VaR one-day-ahead forecast model comparison for the S\&P 500 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the models using a normal distribution.}
	\label{Fig:model_comparision_SP500_25}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1/Nikkei225_5VaR}
	\caption{VaR one-day-ahead forecast model comparison for the Nikkei 225 at $\alpha = 0.05$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the models using a normal distribution.}
	\label{Fig:model_comparision_nikkei_5}	
\end{figure}

%% 10 Days %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1_10Days/Nikkei225_1VaR}
	\caption{VaR ten-days-ahead forecast model comparison for the Nikkei 225 at $\alpha = 0.01$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the EGARCH models.}
	\label{Fig:model_comparision_nikkei_1_10days}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1_10Days/EuroStoxx50_25VaR}
	\caption{VaR ten-days-ahead forecast model comparison for the Euro Stoxx 50 at $\alpha = 0.025$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the EGARCH models.}
	\label{Fig:model_comparision_eurostoxx_25_10days}	
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale = 0.7]{Figures/Plots_Reviewer1_10Days/SaP500_5VaR}
	\caption{VaR ten-days-ahead forecast model comparison for the S\&P 500 at $\alpha = 0.05$ in the period from July 1, 2011 to June 30, 2016. The SVR-GARCH-KDE hybrid is compared to models that are overall on average better and to the EGARCH models.}
	\label{Fig:model_comparision_sap_5_10days}	
\end{figure}

\clearpage


==> source code Version for upload/Sections/garch.tex <==
\subsection{Modeling Volatility Using GARCH Models}\label{Sec:garch}
%%%%Comment out
\iffalse
%Due to the non-stationarity of financial time series it is inadequate to model the original series with ARMA models. 
Figure~\ref{vola_clust} depicts the returns of the adjusted daily closing prices of the Standard and Poors 500 (S\&P 500) from 1 July 1996 to 30 June 2016. The time series is mean stationary but not stationary because the variance of returns of financial time series were found to be conditionally heteroscedastic causing volatility clustering. Hence, this section introduces the standard approach for modeling volatility: GARCH models. The focus of the section is to present the structure of GARCH models due to its importance for the proposed SVR-GARCH-KDE hybrid.

%\begin{figure}[h!]
%	\centering
%	\includegraphics[scale = 0.7]{Figures/Price_SP500_SecGARCH}
%	\caption[Adjusted daily closing prices of the S\&P 500]{Adjusted daily closing prices of the S\&P 500 from 1 July 1996 to 30 June 2016. Data Source: Yahoo Finance.}
%	\label{mean_trend}	
%\end{figure}

%\noindent The time series exhibits a trend, i.e. it is not mean stationary. However, the return series is usually mean stationary but not stationary. The variance of returns of financial time series were found to be conditionally heteroscedastic causing volatility clustering. This effect is illustrated in Figure~\ref{vola_clust}.

\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.7]{Figures/Returns_SP500_SecGARCH}
	\caption[Log-returns of the adjusted daily closing prices of the S\&P 500]{Log-returns of the adjusted daily closing prices of the S\&P 500 from 1 July 1996 to 30 June 2016. Data Source: Yahoo Finance.}	
	\label{vola_clust}
\end{figure}

%\noindent Especially during the financial crisis in 2008, volatility was relatively high. In contrast, in the years before the crisis it was relatively low. 
%\noindent Hence, this section introduces the standard approach for modeling volatility: GARCH models. The focus of the section is to present the structure of GARCH models due to its importance for the proposed SVR-GARCH-KDE hybrid.  \\
\fi
%%%%%%%End comment out
\noindent \cite{Bollerslev.1986} introduces GARCH models by generalizing the volatility modeling approach of \cite{Engle.1982}. In deriving the GARCH regression model \cite{Bollerslev.1986} starts by assuming conditional normality of the return process $r_t$:

\begin{equation}
r_t|\mathcal{F}_{t-1} \sim N(\beta^\top x_t, \sigma_t^2).
\label{Eq:arch_cond_norm}
\end{equation}

\noindent where $x_t$ is a vector of lagged endogenous as well as exogenous variables, $\beta$ an unknown parameter vector and $\mathcal{F}_{t-1}$ the information set available at $t-1$. Rewriting (\ref{Eq:arch_cond_norm}) as linear model with conditionally heteroscedastic and normally distributed disturbances gives:

\begin{equation}
r_t = \beta^\top x_t + u_t, \qquad u_t|\mathcal{F}_{t-1} \sim N(0, \sigma_t^2).
\label{Eq:arch_mean_mdl}
\end{equation}


\noindent Then, the GARCH($p$,$q$) representation of the variance $\sigma_t^2$ is
 
\begin{equation}
\sigma_t^2 = \omega + \sum_{i = 1}^{q} \delta_i u^2_{t-i} + \sum_{j = 1}^{p} \theta_j\sigma^2_{t-j}.
\label{Eq:garch_original}
\end{equation}

\noindent \cite{Bollerslev.1986} notes that (\ref{Eq:garch_original}) has an ARMA representation. To see this let $\nu_t = u_t^2 - \sigma_t^2$ and substitute $\sigma_t^2$ in (\ref{Eq:garch_original}) with $u_t^2 - \nu_t$ to obtain

\begin{equation}
u_t^2 - \nu_t = \omega + \sum_{i = 1}^{q} \delta_i u^2_{t-i} + \sum_{j = 1}^{p} \theta_j(u_{t-j}^2 - \nu_{t-j}).
\label{Eq:garch_arma1}
\end{equation}

\noindent Rearranging (\ref{Eq:garch_arma1}) yields an ARMA representation for $u_t^2$:

\begin{align}
u_t^2  &= \omega + \sum_{i = 1}^{q} \delta_i u^2_{t-i} + \sum_{j = 1}^{p} \theta_j(u_{t-j}^2 - \nu_{t-j}) + \nu_t  \\
&=\omega + \sum_{i = 1}^{\max(p,q)} (\delta_i + \theta_i) u_{t-i}^2 - \sum_{j = 1}^{p} \theta_j \nu_{t-j} + \nu_t. 
\label{Eq:garch_arma2}
\end{align}

\noindent Based on (\ref{Eq:garch_arma2}) nonlinear and nonparametric volatility models can be introduced. This can be seen by noting that the conditional expectation of $u_t^2$ is equal to $\sigma^2$. Consequently, the variance process can be modeled solely based on the observed values without making assumptions about the distributional form of the residuals or the structure of the variance process. Hence, the volatility model in the SVR-GARCH-KDE hybrid is motivated by the ARMA representation of $\sigma^2$. 


==> source code Version for upload/Sections/intro.tex <==
\clearpage


%\section{Introduction}\label{Sec:intro}

Events as the world wide stock market crashes in 1987 and 2008 as well as the outcomes of the 2016 referendum in the UK or the presidential election in the USA came unexpected for most people. Therefore, from the perspective of financial risk management the words of Emil Gumbel, who made important contributions to the field of extreme value statistics, should be marked: \textit{"Il est impossible que l`improbable n`arrive jamais." (It is impossible for the improbable to never occur.)} \cite[p. 200]{Gumbel.1958}. Since such events happen rarely, they occur as outliers in data series. However, they can have a big impact on the solvency of single institutions and the whole economy. For instance, strategical decisions that are based on models which underestimate existing market risks can result in large losses or even bankruptcy of the institution. If a system-relevant financial institution goes bankrupt, it can cause an economic crisis. Additionally, systematically overestimated market risk can prevent institutions from taking actions to generate profits. Thus, the use of appropriate models for measuring market risk results in a competitive advantage. \\

\noindent The importance of risk management for financial institutions and the economy drew researchers attention to the development of tools for handling risk. One of the most famous measures of uncertainty in financial markets is Value-at-Risk (VaR) which is e.g. described in detail by \cite{Alexander.2010} and \cite{Jorion.2009}. VaR is based on the quantiles of a portfolio's loss distribution. It can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable number. However, the use of VaR has been criticized. For instance, \cite{Artzner.1999} note that VaR is not subadditive and therefore no coherent risk measure. As a consequence, diversification can increase VaR. Despite this, regulatory frameworks for the banking and insurance industry as Basel III or Solvency II rely on VaR for the determining capital requirements of financial institutions. \\

\noindent One approach for estimating VaR is based on generalized autoregressive conditional heteroscedasticity (GARCH) models. For example, in an empirical study with more than 30 years of historical returns \cite{Kuester.2005} show that VaR forecasts which are based on standard GARCH models are relatively good compared to other methods. However, they have a linear and parametric structure. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation (MLE)  \citep{Bollerslev.1986}. This makes it necessary to make distributional assumptions. However, the distribution of financial returns were empirically shown to have fat tails and being skewed \citep{Bali.2008,Harvey.2000}. Therefore, assuming e.g. normality can lead to an underestimation of risk. In contrast, support vector regression (SVR) introduced by \cite{Vapnik.1995,Vapnik.1998} is a method originating in statistical learning theory and was derived based on minimizing the generalization error. SVR can be classified as a method belonging to the domain of machine learning (ML). Additionally, kernel density estimation (KDE) is a nonparametric method to estimate the density of a random variable \citep{Hardle.2004}. In this paper a data driven VaR forecasting framework that is based on SVR and KDE is introduced. The aim is to compare the proposed approach with similar parametric GARCH-type models to see whether performance gains can be achieved. \\

\noindent The remainder of the paper is structured as follows. In Section \ref{Sec:Lit_Rev} the literature where ML methods are used to forecast VaR are reviewed. Moreover, approaches that are used to establish prediction intervals but are also a possible framework for modeling VaR are presented as well. In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Consequently, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. Based on this, the proposed SVR-GARCH-KDE hybrid is introduced at the end of the section. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions on how to modify the proposed framework for performance improvements are provided in the last section. 



==> source code Version for upload/Sections/introSL.tex <==
\section{Introduction}\label{Sec:intro}
Events like the 2008 financial crisis or the outcome of the 2016 referendum in the UK came unexpected for many people. Yet, as these examples illustrate, unlikely events occur at times and they might have far reaching consequences. Risk management is the practice to analyze the macro-environment of an organization, identify possible adverse developments, and design suitable countermeasures.

%%%%%%%%%%%%%%%%%%%%%
%% Risk Management %%
%%       VAR       %%
%%%%%%%%%%%%%%%%%%%%%

For financial institutions and systemically important institutions in particular, a key risk management responsibility is to sustain solvency under adverse economic conditions \citep[e.g.,][]{Silva.2017, Kraus.2017}. One of the most popular measures of uncertainty in financial markets is VaR (e.g., \cite{Alexander.2010}). VaR is based on the quantiles of a portfolio's profit and loss ($P\&L$) distribution and can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable figure \citep[e.g.,][]{Chen.2012}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% VaR critique %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Regulatory frameworks for the banking and insurance industry such as Basel III or Solvency II also rely on VaR for determining capital requirements. Compared to expected shortfall, an alternative risk measure with some superior mathematical properties \citep[e.g.,][]{Kim.2016}, an advantage of VaR may be seen in the fact that its estimation is more robust due to putting less weight on tail events and large losses, which may deteriorate the quality of statistical estimation routines \citep{Sarykalin.2008}.  %Especially the latter property makes VaR the right choice for this paper, which focuses on developing estimates of risk exposure using data-driven forecasting methods.  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% VAR ESTIMATION and related work %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parametric only

Several approaches have been proposed to estimate VaR including parametric statistical models and data-driven machine learning algorithms such as neural networks (NN) and SVR. In a seminal study, \cite{Kuester.2005} review several statistical methods and compare these in a forecasting benchmark. Using more than 30 years of historical returns data, they find standard GARCH models to forecast VaR with the highest accuracy on average.

GARCH models are also employed by \cite{Chen.2012} to estimate VaR for four daily series of stock market indices. More specifically, \cite{Chen.2012} rely on an asymmetric Laplace distribution and model volatility using a GJR-GARCH model to introduce leverage effects. They then develop a time-varying model to allow for dynamic higher moments. These extensions allow for wider application of the model beyond forecasting. 

% Models with some ML element
Unlike the parametric approach of \cite{Chen.2012}, \cite{Franke.2006} estimate VaR for the German stock index through fitting the mean and volatility of the return series using NNs. More specifically, they model the mean and volatility as an autoregressive (AR) and autoregressive conditionally heteroscedastic (ARCH) process, respectively. To derive VaR and expected shortfall, \cite{Franke.2006} use the predicted mean and variance with the normal distribution. This model outperforms a standard GARCH model in terms of VaR exceedances and proofs capable of quickly adjusting volatility in case of shocks with only short impact. \cite{Dunis.2010} also  propose a NN-based approach towards forecasting VaR and expected shortfall. 

\cite{Khan.2011} develops a VaR-model that forecasts realized volatilities using a combination of a heterogeneous AR model and SVR. VaR is then computed based on the normal, $t$- and skewed $t$-distribution. Applying this model to 5- and 15-minutes return data, \cite{Khan.2011} is able to confirm the suitability of the SVR component.  \cite{Stankovic.2015} provide further evidence that SVR is a useful method for VaR forecasting. Likewise, \cite{Xu.2016} introduce a multi-period VaR model using SVR in a quantile regression framework and show this approach to outperform GARCH models. 

% Shortcomings of (partly) parametric models
The findings of \cite{Xu.2016} seem to disagree with prior results of \cite{Kuester.2005} where GARCH models predict VaR with highest average accuracy and more accurately than quantile regression approaches in particular. Implementations of the quantile regression using a data-driven SVR model might explain the results of \cite{Xu.2016}. More specifically, the linear and parametric structure of standard GARCH models might be a limiting factor in VaR forecasting. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation \citep{Bollerslev.1986}. This necessitates distributional assumptions, which might be problematic since the distribution of financial returns is skewed and exhibits fat tails \citep{Bali.2008,Harvey.2000}. 

% Key paper of Schaumburg
Noting the possible limitation of the parametric framework, \cite{Schaumburg.2012} combines extreme value theory with nonparametric VaR estimation to forecast return distributions of four financial stock indices. A parametric conditional autoregressive value at risk (CAViaR) model serves as benchmark. The benchmark and the proposed model both circumvent the estimation of the mean and variance of the $P\&L$ distribution through predicting a quantile directly. In this regard, the approach of \cite{Schaumburg.2012} can be characterized as a nonparametric CAViaR model. 

% Soft critic of Schaumburg and contribution
VaR forecasts based on CAViaR frameworks have also been considered in the benchmarking study of \cite{Kuester.2005}. In fact, the authors also introduce a novel CAViaR model in the paper and test it alongside various other VaR models. However, GARCH models and models relying on the $t$-distribution in particular emerge as most suitable for VaR modeling.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Motivating Method (including suggestions of Kiho)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In summary, parametric GARCH models are superior to parametric quantile regression approaches for modeling VaR. To achieve better results with quantile regression approaches, it is necessary to include nonparametric parts into the model. Additionally, data driven GARCH models where the mean and variance components are modeled nonlinearly and nonparametrically lead to better results than parametric GARCH models. However, one shortcoming of the so far proposed data driven GARCH models is the use of parametric residual distributions. Particularly with regard to skewness and kurtosis, this can lead to misspecified residual distributions, resulting in wrong VaR estimates. Therefore, a novel purely nonparametric VaR model that grounds on the GARCH framework is proposed here. We apply data driven approaches to all GARCH components, i.e. mean, variance and residual distribution. Using this approach, we can overcome the possible misspecification of the residual distribution as well as the misspecifications of mean and variance. More specifically, we estimate the mean and variance of the $P\&L$ distribution using SVR and employ KDE to model the density of the standardized residuals  \citep[e.g.,][]{Hardle.2004}. We then integrate these components to derive a VaR forecast. In other words, we propose to start from the most effective parametric modeling approach of \cite{Kuester.2005} and develop models that estimate its components in a purely data-driven manner. Although KDE is not a new  approach in VaR forecasting \citep[e.g.,][]{Haerdle.2016, Schaumburg.2012, Malec.2014}, the particular combination of data-driven VaR estimation using SVR and nonparametric density estimation, which we propose in this paper, has, to the best of our knowledge, not been considered in prior work. 

% Evaluation
We assess the performance of the proposed model in comparison to GARCH-type models with different error distributions also including skewed and fat-tailed distributions. Empirical experiments using data from three major financial indices, namely the Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500), suggest that the SVR-GARCH-KDE hybrid typically outperforms models that are coupled with a normal distribution and performs competitive to other benchmark models. %For example, SVR-GARCH-KDE performs best model for the Euro STOXX 50 for the 0.5\% and 1\% quantile. In contrast, only one benchmark model performs worse for the Nikkei 225 at the 2.5\% level. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Structure  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
The remainder of the paper is organized as follows. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Specifically, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. The proposed SVR-GARCH-KDE hybrid is then developed based on these building blocks. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions for future research are provided in the last section.

















==> source code Version for upload/Sections/intro_v003.tex <==
\section{Introduction}\label{Sec:intro}
Events like the 2008 financial crisis or the outcome of the 2016 referendum in the UK came unexpected for many people. Yet, as these examples illustrate, unlikely events occur at times and they might have far reaching consequences. Risk management is the practice to analyze the macro-environment of an organization, identify possible adverse developments, and design suitable countermeasures.

%%%%%%%%%%%%%%%%%%%%%
%% Risk Management %%
%%       VAR       %%
%%%%%%%%%%%%%%%%%%%%%

For financial institutions and systemically important institutions in particular, a key risk management responsibility is to sustain solvency under adverse economic conditions \citep[e.g.,][]{Silva.2017, Kraus.2017}. One of the most popular measures of uncertainty in financial markets is VaR (e.g., \cite{Alexander.2010}). VaR is based on the quantiles of a portfolio's profit and loss ($P\&L$) distribution and can be interpreted as an upper bound on the potential loss that will not be exceeded with a given level of confidence. Its use is appealing because it summarizes the downside risk of an institution in one easily interpretable figure \citep[e.g.,][]{Chen.2012}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% VaR critique %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Regulatory frameworks for the banking and insurance industry such as Basel III or Solvency II also rely on VaR for determining capital requirements. Compared to expected shortfall, an alternative risk measure with some superior mathematical properties \citep[e.g.,][]{Kim.2016}, an advantage of VaR may be seen in the fact that its estimation is more robust due to putting less weight on tail events and large losses, which may deteriorate the quality of statistical estimation routines \citep{Sarykalin.2008}.  %Especially the latter property makes VaR the right choice for this paper, which focuses on developing estimates of risk exposure using data-driven forecasting methods.  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% VAR ESTIMATION and related work %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parametric only

Several approaches have been proposed to estimate VaR including parametric statistical models and data-driven machine learning algorithms such as neural networks (NN) and SVR. In a seminal study, \cite{Kuester.2005} review several statistical methods and compare these in a forecasting benchmark. Using more than 30 years of historical returns data, they find standard GARCH models to forecast VaR with the highest accuracy on average.

GARCH models are also employed by \cite{Chen.2012} to estimate VaR for four daily series of stock market indices. More specifically, \cite{Chen.2012} rely on an asymmetric Laplace distribution and model volatility using a GJR-GARCH model to introduce leverage effects. They then develop a time-varying model to allow for dynamic higher moments. These extensions allow for wider application of the model beyond forecasting. 

% Models with some ML element
Unlike the parametric approach of \cite{Chen.2012}, \cite{Franke.2006} estimate VaR for the German stock index through fitting the mean and volatility of the return series using NNs. More specifically, they model the mean and volatility as an autoregressive (AR) and autoregressive conditionally heteroscedastic (ARCH) process, respectively. To derive VaR and expected shortfall, \cite{Franke.2006} use the predicted mean and variance with the normal distribution. This model outperforms a standard GARCH model in terms of VaR exceedances and proofs capable of quickly adjusting volatility in case of shocks with only short impact. \cite{Dunis.2010} also  propose a NN-based approach towards forecasting VaR and expected shortfall. 

\cite{Khan.2011} develops a VaR-model that forecasts realized volatilities using a combination of a heterogeneous AR model and SVR. VaR is then computed based on the normal, $t$- and skewed $t$-distribution. Applying this model to 5- and 15-minutes return data, \cite{Khan.2011} is able to confirm the suitability of the SVR component.  \cite{Stankovic.2015} provide further evidence that SVR is a useful method for VaR forecasting. Likewise, \cite{Xu.2016} introduce a multi-period VaR model using SVR in a quantile regression framework and show this approach to outperform GARCH models. 

% Shortcomings of (partly) parametric models
The findings of \cite{Xu.2016} seem to disagree with prior results of \cite{Kuester.2005} where GARCH models predict VaR with highest average accuracy and more accurately than quantile regression approaches in particular. Implementations of the quantile regression using a data-driven SVR model might explain the results of \cite{Xu.2016}. More specifically, the linear and parametric structure of standard GARCH models might be a limiting factor in VaR forecasting. Moreover, the parameters of GARCH-type models are usually estimated via maximum likelihood estimation \citep{Bollerslev.1986}. This necessitates distributional assumptions, which might be problematic since the distribution of financial returns is skewed and exhibits fat tails \citep{Bali.2008,Harvey.2000}. 

% Key paper of Schaumburg
Noting the possible limitation of the parametric framework, \cite{Schaumburg.2012} combines extreme value theory with nonparametric VaR estimation to forecast return distributions of four financial stock indices. A parametric conditional autoregressive value at risk (CAViaR) model serves as benchmark. The benchmark and the proposed model both circumvent the estimation of the mean and variance of the $P\&L$ distribution through predicting a quantile directly. In this regard, the approach of \cite{Schaumburg.2012} can be characterized as a nonparametric CAViaR model. 

% Soft critic of Schaumburg and contribution
VaR forecasts based on CAViaR frameworks have also been considered in the benchmarking study of \cite{Kuester.2005}. In fact, the authors also introduce a novel CAViaR model in the paper and test it alongside various other VaR models. However, GARCH models and models relying on the $t$-distribution in particular emerge as most suitable for VaR modeling.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Motivating Method (including suggestions of Kiho)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In summary, parametric GARCH models are superior to parametric quantile regression approaches for modeling VaR. To achieve better results with quantile regression approaches, it is necessary to include nonparametric parts into the model. Additionally, data driven GARCH models where the mean and variance components are modeled nonlinearly and nonparametrically lead to better results than parametric GARCH models. However, one shortcoming of the so far proposed data driven GARCH models is the use of parametric residual distributions. Particularly with regard to skewness and kurtosis, this can lead to misspecified residual distributions, resulting in wrong VaR estimates. Therefore, a novel purely nonparametric VaR model that grounds on the GARCH framework is proposed here. We apply data driven approaches to all GARCH components, i.e. mean, variance and residual distribution. Using this approach, we can overcome the possible misspecification of the residual distribution as well as the misspecifications of mean and variance. More specifically, we estimate the mean and variance of the $P\&L$ distribution using SVR and employ KDE to model the density of the standardized residuals  \citep[e.g.,][]{Hardle.2004}. We then integrate these components to derive a VaR forecast. In other words, we propose to start from the most effective parametric modeling approach of \cite{Kuester.2005} and develop models that estimate its components in a purely data-driven manner. In contrast to other so far proposed GARCH based approaches to forecast VaR \citep[e.g.,][]{Youssef.2015, Khosravi.2013, Aloui.2010, Huang.2009, Fan.2008, Chan.2007, Hartz.2006} no assumptions about process dependence structures or the distribution of residuals are made by combining SVR and KDE in a GARCH like fashion. Training the SVR-GARCH-KDE hybrid is, therefore, mainly computationally driven. 

The use of SVR is motivated by the existence of a large body of research showing the effectiveness of SVR in forecasting financial time series \citep[e.g.,][]{Chang.2016, Devi.2015, Tay.2001}. Additionally, \cite{Sheta.2015} compare the forecasting performance of SVR, ANN and traditional linear regression for the S\&P 500. They find that SVR solves the task most successfully. \cite{Kazem.2013} also provide evidence that SVR based models outperform ANNs in the context of financial forecasting. Moreover, \cite{Chen.2009} use a SVR approach for predicting stock market volatility and use a recurrent ANN as benchmark which is outperformed. The use of nonparametric density estimation is motivated by the fact that the existence of fat tails and skewness in the distribution of financial returns can be considered as an empirically proven fact \citep[e.g.,][]{Bali.2008, Harvey.2000}. Although KDE is not a new  approach in VaR forecasting \citep[e.g.,][]{Haerdle.2016, Schaumburg.2012, Malec.2014}, the particular combination of data-driven VaR estimation using SVR and nonparametric density estimation, which we propose in this paper, has, to the best of our knowledge, not been considered in prior work. 

% Evaluation
We assess the performance of the proposed model in comparison to GARCH-type models with different error distributions also including skewed and fat-tailed distributions. Empirical experiments using data from three major financial indices, namely the Euro~STOXX~50, Nikkei~225 and Standard \& Poor's 500 (S\&P 500), suggest that the SVR-GARCH-KDE hybrid typically outperforms models that are coupled with a normal distribution and performs competitive to other benchmark models. %For example, SVR-GARCH-KDE performs best model for the Euro STOXX 50 for the 0.5\% and 1\% quantile. In contrast, only one benchmark model performs worse for the Nikkei 225 at the 2.5\% level. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Structure  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
The remainder of the paper is organized as follows. 
In Section \ref{Sec:meths} VaR is defined and the methods underlying the proposed VaR modeling framework are presented. Specifically, the standard GARCH approach, nonparametric density estimation via KDE and SVR are introduced. The proposed SVR-GARCH-KDE hybrid is then developed based on these building blocks. After outlining the theoretical background, the SVR-GARCH-KDE hybrid is compared to other models on different datasets in Section \ref{Sec:emp_study}. Concluding remarks and suggestions for future research are provided in the last section.











==> source code Version for upload/Sections/kde.tex <==
\subsection{Nonparametric Density Estimation}\label{Sec:NDE}

%The motivation for Section \ref{Sec:garch} was the existence of volatility clusters in stock returns. %Moreover, the conditional expectation was found to often exhibit a dependence on past information, e.g. the last day's return. 
 The volatility of stock returns varies over time and a similar behavior has been observed for the third and fourth moment of the return distribution. For example, \cite{Bali.2008} show that VaR forecasts can be improved by using past estimates of skewness and kurtosis. Given the evidence for the leptokurtic nature of stock returns \citep{Franke.2011}, parametric distributional models might lack the flexibility to capture such distributional characteristics, which motivates the use of nonparametric methods such as KDE  \citep[e.g.,][]{Hardle.2004}.
 
%In addition with the found evidence for the leptokurtic nature of stock returns, %parametric distribution models often lack the flexibility to appropriately capture the distributional characteristics of stock returns. 
%These considerations make the use of nonparametric methods appealingbecause they can estimate distributions more flexible than parametric approaches. %One approach is the histogram. However, it has some drawbacks, e.g. histograms are not smooth even if the underlying density fube. This and other critiques can be avoided by using KDE which has more favorable properties than the histogram.
%The nonparametric method introduced here is called kernel density estimation (KDE). The derivations are based on \cite{Hardle.2004} and \cite{Silverman.1986}. An overview for other nonparametric density estimators can be found in \cite{Silverman.1986}. This subsubsection considers only the univariate case. For the derivationp[e.g.,][] of multivariate KDE see \cite{Hardle.2004} or \cite{Silverman.1986}. 

%\subsubsection{Kernel Density Estimation}

Let $X$ be a random variable with an absolutely continuous distribution function $F$. Further, denote the corresponding density function as $f$ and let $\{x_1, \dots, x_n\}$ be a sample of i.i.d. realizations of $X$. Then, the kernel density estimator $\hat{f}_h(x)$ of $f(x)$ is defined as   

%$F$ can be estimated by the empirical distribution function $F_n$:
%
%\begin{equation}
%	F_n(x) = \frac{1}{n} \sum_{i = 1}^{n} \mathbb{I}(x_i \le x).
%	\label{kde_naive_set}
%\end{equation}
%
%\noindent Based on this, \cite{Parzen.1962} starts its derivation of the density estimator for $f(x)$ by the following approach:
%
%\begin{equation}
%\hat{f}_h(x) = \dfrac{F_n(x + h) - F_n(x - h) }{2h}.
%\label{Eq:emp_pdf}
%\end{equation}

%Then, the density $f(x)$ of $X$ can written as
%
%\begin{equation}
%f(x) = \lim_{x \to 0} \dfrac{1}{2h} P[x-h < X \le x + h].
%\label{pdf_approx}
%\end{equation}
%\newline
%\noindent Here, $h$ is a bandwidth parameter with $h>0$. \cite{Hardle.2004} write the estimator in (\ref{Eq:emp_pdf}) as
%
%\begin{equation}
%\hat{f}_h(x) = \dfrac{1}{2nh} \# \{x_i \in [x-h, x+h)\},
%\label{kde_naive_set}
%\end{equation}
%\newline
%where $\#\{\cdot\}$ denotes the cardinality of a set. Equation (\ref{kde_naive_set}) can be rewritten as
%
%\begin{align}
%\hat{f}_h(x)  &= \dfrac{1}{2hn} \sum_{i = 1}^{n} I\{x_i \in [x-h, x+h)\} \\ 
% &= \dfrac{1}{2hn} \sum_{i = 1}^{n} I\{ x-h \le x_i < x+h \} \\
% &= \dfrac{1}{hn} \sum_{i = 1}^{n} \dfrac{1}{2} I\{ -1 \le \dfrac{x_i - x}{h} < 1 \}. \label{Eq:kde_simple}
%\end{align}
%\newline
%\noindent In the initial formulation of \cite{Rosenblatt.1956} or \cite{Parzen.1962} \cite, the terms in the sum are replaced by a weight function. However, they used intervals that are open or closed, respectively. Following the approach of using a weight function $w(\cdot)$ with a closed interval as in \cite{Parzen.1962} and substituting $u = (x_i - x)/h$, (\ref{Eq:kde_simple}) can be written as 
%\begin{align}
%\hat{f}_h(x) &= \dfrac{1}{hn} \sum_{i = 1}^{n} \dfrac{1}{2} I\{|u| \le 1 \} \label{Eq:kde_uniform} \\
%&= \dfrac{1}{hn} \sum_{i = 1}^{is c). a  
%\%end{align}
%\noindent In the KDE literature $w(\cdot)$ is called the uniform kernel. By using the uniform kernel the same weight is assigned to every observation in the considered interval. However, assigning a high weight to observations that are close and a low weight to those far from $x$ preserves more information about the real density $f(x)$. Consequently, other weighting functions taking this into account were introduced. These are the so-called kernel functions. Introducing a general kernel function $K(u)$ into (\ref{Eq:kde_uniform}) results in

\begin{equation}
\hat{f}_h(x) = \dfrac{1}{hn} \sum_{i = 1}^{n} K\left(\dfrac{x_i - x}{h}\right) 
\label{Eq:kde_definition} 
\end{equation}

\noindent where $h$ is a bandwidth parameter with $h>0$ and $K$ is a so-called kernel function. %There exist different kernel functions. Table \ref{Tab:kernel_functions} is a list of kernel functions that are presented in \cite{Hardle.2004}. 
Usually, a kernel function is assumed to be a symmetric density function, i.e.  %%Therefore, the general form of the kernel density estimate is obtained as 

%\begin{equation}
%\hat{f}_h(x) = \dfrac{1}{n} \sum_{i = 1}^{n} K_h(x - x_i)
%\label{Eq:kde_general}
%\end{equation}
%
%\noindent with
%
%\begin{equation}
%K_h(\cdot) = \dfrac{1}{h} K\left(\dfrac{\cdot}{h}\right). 
%\end{equation}

%\noindent There exist different kernel functions. Table \ref{Tab:kernel_functions} is a list of kernel functions that are presented in \cite{Hardle.2004}. Usually, a kernel function is assumed to be a symmetric density function, i.e.

\begin{equation}
	\int_{-\infty}^{\infty} K(u)du = 1 \quad \text{with} \ K(u) \ge 0
	\label{Eq:kernel_function_density}
\end{equation}

\noindent and

\begin{equation}
\int_{-\infty}^{\infty} uK(u)du = 0.
\end{equation}

\noindent Conveniently, (\ref{Eq:kernel_function_density}) implies that $\hat{f}_h(x)$ is also a density. Note that $\hat{f}_h(x)$ inherits all properties of $K$ regarding continuity and differentiability.

\iffalse
\begin{table}[H]
	\begin{center}
	\begin{tabular}{c|c}
		\hline \hline
		\textbf{Kernel} & \textbf{K(u)} \\
		\hline
		Uniform & $\frac{1}{2}I(|u| \le 1)$ \\
	    \hline
		Triangel & $(1 - |u|)I(|u| \le 1)$ \\
		\hline
		Epanechnikov & $\frac{3}{4}(1 - u^2)I(|u| \le 1)$ \\
		\hline
		Quartic/Biweight & $\frac{15}{16}(1 - u^2)^2I(|u| \le 1)$ \\
		\hline
		Triweight & $\frac{35}{32}(1 - u^2)^3I(|u| \le 1)$ \\
		\hline
		Gaussian & $\frac{1}{\sqrt{2 \pi}}\exp (-\frac{u^2}{2})$ \\
		\hline
		Cosine & $\frac{\pi}{4} \cos (\frac{\pi u}{2}) I(|u| \le 1)$ \\
		\hline \hline
	\end{tabular}
	\end{center}
	\caption[Kernel functions for kernel density estimation]{The table shows possible functions that can be used in the process of estimating the density of a random variable via KDE. Source: \cite{Hardle.2004}.}
	 \label{Tab:kernel_functions}	
\end{table}
\fi

%%%%%end

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\subsubsection{Bias-Variance-Trade-Off}
%
%Choosing $h$ is a central point when using KDE. Since (\ref{Eq:kde_general}) is a biased estimator of $f(x)$, a too high $h$ will result in a high bias. Decreasing $h$ will, however, result in a higher variance. In order to indicate these dependencies, bias, variance and mean squared error (MSE) will be derived in this subsubsection. Since the derivations use Taylor expansions with Landau symbols it is assumed that $n \to \infty$, $h \to 0$ and $nh \to \infty$. Note that by $\mathcal{O}(\cdot)$ and $o(\cdot)$ it is referred to the big-O and little-o-notation.
%
%\subsubsection{Bias} \label{Sec:kde_bias_subsubsection}
%
%The bias $\mathbb{B}$ of an estimator $\hat{\beta}$ for a parameter $\beta$ is defined as 
%
%\begin{equation}
%\mathbb{B}[\hat{\beta}] = \mathbb{E}[\hat{\beta}] - \beta.
%\label{Eq:bias_def}
%\end{equation}
%
%\noindent In the case where $f(x)$ is a density and $\hat{f}_h(x)$ an estimator for $f(x)$, equation (\ref{Eq:bias_def}) becomes
%
%\begin{equation}
%\mathbb{B}[\hat{f}_h(x)] = \mathbb{E}[\hat{f}_h(x)] - f(x). 
%\end{equation}
%
%\noindent Deriving $\mathbb{E}[\hat{f}_h(x)]$ yields
%
%\begin{align}
%\mathbb{E}[\hat{f}_h(x)] &= \mathbb{E}\left[\dfrac{1}{n} \sum_{i=1}^{n} K_h(x - x_i)\right]  \\ &=  \dfrac{1}{n} \sum_{i=1}^{n} \mathbb{E}[K_h(x - x_i)] \\ 
%& =  \mathbb{E}[K_h(x - X)] \label{Eq:bias_kde_iid} \\
%& =  \int \dfrac{1}{h} K\left(\dfrac{x - z}{h}\right)f(z)dz.
%\end{align}
%
%\noindent Note that in (\ref{Eq:bias_kde_iid}) $x_i$ can be replaced by $X$ due to the i.i.d. assumption. Substituting $u = (z - x)/h$, exploiting that kernels are symmetric, i.e. $K(u) = K(-u)$, and approximating $f(z)$ around $x$ with a second-order Taylor expansion gives
%
%\begin{align}
%\mathbb{E}[\hat{f}_h(x)] &= \int \dfrac{1}{h} K\left(\dfrac{x - z}{h}\right)f(z)dz  \\
%&= \int K(u) \left(f(x) + uhf'(x) + \dfrac{u^2 h^2}{2} f''(x) + o(h^2)  \right)du\\
%&=  f(x) \underbrace{\int K(u)du}_\text{=1} + hf'(x)  \underbrace{\int K(u)udu}_\text{= 0} \\ &\phantom{{}=1} + \dfrac{h^2}{2} f''(x) \underbrace{\int K(u)u^2du}_\text{=:$\mu_2(K)$} + o(h^2) \notag \\
%&=  f(x)  + \dfrac{h^2}{2} f''(x)\mu_2(K) + o(h^2).  
%\end{align}
% 
%\noindent Consequently, the kernel density estimator is a biased estimator of $f(x)$:
%
%  \begin{equation}
%  \mathbb{B}[\hat{f}_h(x)] = \dfrac{h^2}{2} f''(x)\mu_2(K) + o(h^2).
%  \label{kde_bias}
%  \end{equation}
%  
%\noindent Equation (\ref{kde_bias}) implies that the bias vanishes as $h \to 0$. However, simply choosing a very small $h$ does not guarantee an appropriate estimate as will be shown in the next subsubsection. 
%
%\subsubsection{Variance}
%
%As in the derivation for the bias, the kernel density estimator is plugged into the variance formula and the i.i.d. assumption is exploited. 
%
%\begin{align}
%\mathbb{V}[\hat{f}_h(x)] &= \mathbb{V}\left[\dfrac{1}{n} \sum_{i=1}^{n} K_h(x - x_i)\right]  \\
%&=  \dfrac{n}{n^2 h^2} \mathbb{V}\left[K\left(\dfrac{x - X}{h}\right)\right] \\ 
%& =  \dfrac{1}{n h^2} \mathbb{E}\left[K\left(\dfrac{x - X}{h}\right)^2\right] -  \dfrac{1}{n} \mathbb{E}\left[\dfrac{1}{h} K\left(\dfrac{x - X}{h}\right)\right]^2. \label{Eq:kde_var_one}
%\end{align}
%\newline
%\noindent The result of the second term was already derived in Section \ref{Sec:kde_bias_subsubsection} because it follows from (\ref{Eq:bias_kde_iid})
%
%\begin{equation}
%\dfrac{1}{n} \mathbb{E}\left[\dfrac{1}{h} K\left(\dfrac{x - X}{h}\right)\right]^2 = \dfrac{1}{n}\left[f(x) + \mathbb{B}[\hat{f}_h(x)] \right]^2.
%\label{Eq:density_plus_bias}
%\end{equation}
%\newline
%\noindent Hence, the following steps consider the derivation of the first term in (\ref{Eq:kde_var_one}). In the first step a substitution as in the bias derivation is used. This is followed by a first order Taylor approximation of $f$ around $x$:
%
%\begin{align}
% \dfrac{1}{n h^2} \mathbb{E}\left[K\left(\dfrac{x - X}{h}\right)^2\right] &= \dfrac{1}{n} \int \dfrac{1}{h^2} K\left(\dfrac{x-z}{h}\right)^2 f(z) dz \\
%&= \dfrac{1}{n} \int \dfrac{1}{h} K\left(u \right)^2 f(x+hu) du \\
%&= \dfrac{1}{nh} \int K\left(u \right)^2\{f(x) + o(h)\} du. \label{Eq:var_taylor}
%\end{align}
%
%\noindent By noting that (\ref{Eq:density_plus_bias})  is $\mathcal{O}(n^{-1})$ and using $\int K(u)^2 du = ||K||_2^2 $ in (\ref{Eq:var_taylor}) the variance is 
%
%\begin{align}
%\mathbb{V}[\hat{f}_h(x)] &= \dfrac{1}{nh} ||K||_2^2 \{ f(x) + o(h) \} + \mathcal{O}(n^{-1}) \\
%&= \dfrac{1}{nh} ||K||_2^2 f(x) + o \left( \dfrac{1}{nh} \right).
%\label{Eq:kde_variance}
%\end{align}
%
%\noindent From (\ref{Eq:kde_variance}) can be inferred that the variance decreases with increasing $h$. Approximating $f(x)$ with large values of $h$ results in an estimator with low variability for different $x$. The variance gets also lower for higher $n$. Moreover, (\ref{Eq:kde_variance}) increases in the squared norm of the kernel $K$ as well. As \cite{Hardle.2004} indicate, due to the dependence on $||K||_2^2$ smooth and flat kernels can result in estimates with lower variance. %For instance, the uniform kernel assigns the same weight to observations in different samples from one random variable.              
%
%\subsubsection{Mean Squared Error}
%
%The derived bias in (\ref{kde_bias}) and variance in (\ref{Eq:kde_variance}) indicate the existence of a trade-off between bias and variance. For instance, choosing a small $h$ implies a small bias but a high variance. Considering the MSE is useful for balancing out this trade-off because the MSE can be written as sum of variance and squared bias:
%
%\begin{equation}
%\text{MSE}[\hat{f}_h(x)] = \mathbb{V}[\hat{f}_h(x)] + \mathbb{B}[\hat{f}_h(x)]^2.
%\label{Eq:mse_def}
%\end{equation}
%
%\noindent Plugging the results for bias and variance into (\ref{Eq:mse_def}) gives
%
%\begin{align}
%\text{MSE}[\hat{f}_h(x)] &= \dfrac{1}{nh} ||K||_2^2 f(x) + o \left( \dfrac{1}{nh} \right) + \left\{\dfrac{h^2}{2} f''(x)\mu_2(K) + o(h^2)\right\}^2\\
%&= \dfrac{1}{nh} ||K||_2^2 f(x) + \dfrac{h^4}{4} f''(x)^2\mu_2(K)^2 + o(h^4) + o \left( \dfrac{1}{nh} \right). \label{Eq:kde_mse}
%\end{align}
%\newline
%\noindent Moreover, the MSE can be used to infer consistency of an estimator. A main result in the asymptotic theory of statistics is that convergence in mean square implies convergence in probability, i.e. consistency. For $h \to 0$ and $nh \to \infty$ equation (\ref{Eq:kde_mse}) converges to zero. Therefore, the kernel density estimator is consistent. 
%\newline
%\newline
%\noindent Although the MSE is useful in proving consistency and understanding the bias-variance-trade-off in KDE, it is not advisable to derive the optimal bandwidth $h_{opt}$ with it. The MSE is a local measure of the estimation accuracy. Meaning that $h_{opt}$ would be a function of $x$. Therefore, the next subsubsection derives the mean integrated squared error (MISE) and the asymptotic MISE (AMISE) instead. In contrast to the MSE, the MISE and AMISE are global accuracy measures.  
%
%\subsubsection{Asymptotic Mean Integrated Squared Error}
%
%In order to derive $h_{opt}$ the MISE will be derived. This is done by integrating the MSE over $x$:
%
%\begin{align}
%\text{MISE}(\hat{f}_h) &= \int \text{MSE}[\hat{f_h}(x)]dx \\
%&=  \int\left\{\dfrac{1}{nh} ||K||_2^2 f(x) + \dfrac{h^4}{4} f''(x)^2\mu_2(K)^2 + o(h^4) + o \left( \dfrac{1}{nh} \right)\right\}dx \\
%&=  \dfrac{1}{nh} ||K||_2^2 \underbrace{\int f(x)dx}_\text{= 1} + \dfrac{h^4}{4}\mu_2(K)^2 \underbrace{\int f''(x)^2 dx}_\text{$||f''||^2_2$} + o(h^4) + o \left( \dfrac{1}{nh} \right) \\
%&= \dfrac{1}{nh} ||K||_2^2  + \dfrac{h^4}{4} \mu_2(K)^2 ||f''||^2_2 + o(h^4) + o \left( \dfrac{1}{nh} \right). \label{Eq:kde_mise}
%\end{align}
%
%\noindent The AMISE of the kernel density estimator is obtained by neglecting terms of higher order in (\ref{Eq:kde_mise}):
%
%\begin{equation}
%\text{AMISE}[\hat{f}_h] = \dfrac{1}{nh} ||K||_2^2  + \dfrac{h^4}{4} \mu_2(K)^2 ||f''||^2_2.
%\label{Eq:kde_amise}
%\end{equation}
%
%\noindent Based on (\ref{Eq:kde_amise}) $h_{opt}$ can be derived. This is done in the next subsubsection.

%\subsubsection{Optimal Bandwidth}
%
%After deriving the AMISE of the KDE, $h_{opt}$ can be derived by differentiating $(\ref{Eq:kde_amise})$. It will be shown that $h_{opt}$ depends on $||f''||^2_2$ which is unknown. Hence, two methods for determining $h_{opt}$ that follow different approaches are derived in this subsubsection. The first aims to minimize AMISE by referencing to a standard distribution. It is characterized by its computational simplicity. In contrast, the second approach is based on CV and minimizing a different criterion. \cite{Hardle.2004} classify the CV based bandwidth selector as one of the most popular. Other bandwidth selectors are shortly explained at the end of the subsubsection. 
%
%
%\subsubsection{Deriving the Optimal Bandwidth}
%
%The first derivative of (\ref{Eq:kde_amise}) is
%
%\begin{align}
%\frac{\partial \text{AMISE}(h)}{\partial h} &= \frac{\partial}{\partial h} \left \{ \dfrac{1}{nh} ||K||_2^2  + \dfrac{h^4}{4} \mu_2(K)^2 ||f''||^2_2 \right \} \\
%&= -\dfrac{1}{nh^{2}} ||K||_2^2  + h^3\mu_2(K)^2 ||f''||^2_2.
%\end{align}
%
%\noindent Then, the optimal bandwidth $h_{opt}$ can be derived as
%
%\begin{align}
% -\dfrac{1}{nh_{opt}^{2}} ||K||_2^2  + h_{opt}^3\mu_2(K)^2 ||f''||^2_2 &= 0 \\
%h_{opt}^3\mu_2(K)^2 ||f''||^2_2 &= \dfrac{1}{nh_{opt}^{2}} ||K||_2^2  \\
%h_{opt} &= \left(\dfrac{||K||_2^2 }{n\mu_2(K)^2 ||f''||^2_2} \right)^{1/5}. \label{Eq:kde_hopt}
%\end{align}
%\newline
%\noindent Due to the dependence of $h_{opt}$ on $||f''||^2_2$, equation (\ref{Eq:kde_hopt}) cannot be used directly to find an appropriate bandwidth. However, the result can be used to infer rule-of-thumb bandwidths by making an assumption for $f$. 
%
%\subsubsection{Bandwidth Selection by Reference Distribution} \label{Sec:kde_hopt_ref}
%
%\cite{Silverman.1986} sees referencing to a standard distribution as an easy and natural way to find $h_{opt}$. For instance, by referencing to the normal distribution it holds that
%
%\begin{align}
%%||f||_2^2 &= \sigma^{-5}\int \psi''(x)dx \\
%%&= \sigma^{-5} \dfrac{3}{8 \sqrt{\pi}}.
%||f||_2^2 = \sigma^{-5} \dfrac{3}{8 \sqrt{\pi}}. \label{Eq:f_curve_normal}
%\end{align}
%
%\noindent Then, by estimating $\sigma$ from the sample it can be plugged into (\ref{Eq:f_curve_normal}). However, this approach contradicts the nonparametric philosophy of not making distributional assumptions. \cite{Hardle.2004} justify its use because it is an explicit formula and a convenient way to compute an estimate of $h_{opt}$. Furthermore, its use is recommended in situations where the distribution of $X$ is similar to the normal distribution. \cite{Hardle.2004} state the following characteristics for similarity: unimodality, approximate symmetry and not too fat tails. If these conditions are fulfilled it is reasonable to choose the Gaussian kernel from Table~\ref{Tab:kernel_functions}. Consequently, with a Gaussian kernel the rule-of-thumb estimator $h_{rot}$ based on (\ref{Eq:kde_hopt}) becomes
%
%\begin{align}
%h_{rot} &= \left(\dfrac{||K||_2^2 }{n\mu_2(K)^2 ||f''||^2_2} \right)^{1/5} \\
%&= \left( \dfrac{4 \sigma^5}{3n} \right)^{1/5} \\
%&\approx 1.06\sigma n^{-1/5}.
%\label{Eq:hopt_kde_gauss}
%\end{align}
%
%\noindent In (\ref{Eq:hopt_kde_gauss}) $\sigma$ can be estimated by the empirical standard deviation $\widehat{\sigma}_{\text{\tiny E}}$. \cite{Silverman.1986} found that using $\widehat{\sigma}_{\text{\tiny E}}$ in (\ref{Eq:hopt_kde_gauss}) can give reasonable estimates if $f$ is multimodal. However, for fat-tailed and skewed densities it is suggested to use a more robust estimator for $\sigma$. The proposed robust estimator is based on the interquartile range (IQR) of the normal distribution. Assume that for the random variable underlying the sample holds that $X \sim N(\mu, \sigma^2)$ and let $Z \sim N(0, 1)$. Further, define $Q(0.25)_{X}$ and $Q(0.75)_{X}$ as well as $Q(0.25)_{Z}$ and $Q(0.75)_{Z}$ as the first and third quartile of $X$ and $Z$, respectively. Then, the IQR of $X$, which is denoted as $R$, can be approximated as follows:
%
%\begin{align}
%R &= Q(0.75)_{X} - Q(0.25)_{X} \\
%%&= (\mu + \sigma Q(0.75)_{X}) - (\mu + \sigma Q(0.25)_{X}) \\
%&= (\mu + \sigma Q(0.75)_{Z}) - (\mu + \sigma Q(0.25)_{Z}) \\ 
%&=  2 \sigma Q(0.75)_{Z} \\
%&\approx  1.34\sigma.  \label{Eq:interquartil_distance}
%\end{align}
%
%\noindent An implication of (\ref{Eq:interquartil_distance}) is that
%
%\begin{align}
%\widehat{\sigma}_{\text{\tiny IQR}} = \dfrac{R}{1.34}  
%\end{align}
%
%\noindent can be used as an estimator for $\sigma$. Then, the corresponding optimal bandwidth for the Gaussian kernel is obtained as
%
%\begin{align}
%\widehat{h}_{\text{\tiny IQR}}& = \dfrac{1.06}{1.34} R n^{-1/5}  \\
%&\approx 0.79Rn^{-1/5}.
%\label{Eq:hopt_iqr_1}
%\end{align} 
%
%\noindent \cite{Silverman.1986} showed in simulations that by using (\ref{Eq:hopt_kde_gauss}) as bandwidth also multimodal densities can be approximated, even though it tends to oversmooth. Moreover, it was shown that by using (\ref{Eq:hopt_iqr_1}) as bandwidth better results are obtained for skewed and fat-tailed distribution. However, the studies revealed also that (\ref{Eq:hopt_iqr_1}) yields worse results than (\ref{Eq:hopt_kde_gauss}) in situations where $f$ is multimodal. To combine the abilities of both bandwidth estimators \cite{Silverman.1986} defines the adaptive estimator $\widehat{\sigma}_A$:
%
%\begin{equation}
%\widehat{\sigma}_{\text{\tiny A}} = \min\{\widehat{\sigma}_{\text{\tiny E}}, \widehat{\sigma}_{\text{\tiny IQR}} \}.
%\end{equation}
%
%\noindent Furthermore, it is suggested to reduce the scaling factor from $1.06$ to $0.9$. Then, one obtains the following bandwidth estimator: 
%
%\begin{equation}
%\widehat{h}_{\text{\tiny A}} = 0.9\widehat{\sigma}_{\text{\tiny A}}n^{-1/5}. \label{Eq:hopt_adaptive_rot}
%\end{equation}
%
%\noindent According to \cite{Silverman.1986}, by using $\widehat{h}_{\text{\tiny A}}$ bimodal and skewed densities can be modeled appropriately. Therefore, $\widehat{h}_{\text{\tiny A}}$ is supposed to deliver reasonable results for many different densities. Consequently, in the rest of this thesis the bandwidth estimator in (\ref{Eq:hopt_adaptive_rot}) is referred to as Silverman's rule of thumb.
%
%\subsubsection{Least Squares Cross Validation} 
%
%A more flexible method than the rule-of-thumb estimator in the last subsubsection is least squares CV (LSCV). No distributional assumption about $X$ has to be made. Therefore, LSCV as a method to select $h_{opt}$ is in accordance with the nonparametric philosophy. LSCV uses the integrated squared error (ISE) as error measure:
%
%\begin{equation}
%\text{ISE}[\hat{f}_h] = \int \left(\hat{f_h}(x) - f(x) \right)^2 dx.
%\label{Eq:def_ise_kde}
%\end{equation}
%
%\noindent Then, the optimal bandwidth is found by minimizing the ISE of $\hat{f_h}$
%
%\begin{equation}
%h_\text{\tiny CV} =  \underset{h > 0}{\mathrm{argmin}} \ \text{ISE}[\hat{f}_h]. 
%\label{Eq:min_ise_kde}
%\end{equation}
%
%\noindent Rewriting (\ref{Eq:def_ise_kde}) results in 
%
%\begin{equation}
%\text{ISE}[\hat{f}_h] = \int \hat{f_h}(x)^2 dx -2\int \hat{f_h}(x)f(x)dx + \int f(x)^2 dx.
%\label{Eq:ise_kde_re}
%\end{equation}
%
%\noindent Since (\ref{Eq:min_ise_kde}) is minimized over $h$ and the last term in (\ref{Eq:ise_kde_re}) does not depend on $h$ it can be neglected. The second term of (\ref{Eq:ise_kde_re}) is the expected value of $\hat{f_h}(x)$. It can be derived based on another independent observation coming from $X$. \cite{Hardle.1991} suggests to estimate $\mathbb{E}[\hat{f_h}(X)]$ with the so-called leave-one-out estimator:
%
%\begin{equation}
%\mathbb{E}[\hat{f}_h(X)] = \dfrac{1}{n}\sum_{i = 1}^{n} \hat{f}_{h,i}(X_i)
%\label{Eq:exp_kde_cv}
%\end{equation}
%
%\noindent where
%
%\begin{equation}
%\hat{f}_{h,i}(X) = \dfrac{1}{(n-1)h} \sum_{\substack{j=1 \\ j\neq i}}^{n} K\left(\dfrac{X - X_j}{h}\right).
%\label{Eq: kde_loue}
%\end{equation}
%
%\noindent For estimating the first term of (\ref{Eq:ise_kde_re})  directly from the data, denote $K*K(X)$ as convolution of $K$ and obtain:
%
%\begin{equation}
%\int \hat{f_h^2} dx = \dfrac{1}{n^2 h} \sum_{i=1}^{n} \sum_{j=1}^{n} K*K\left( \dfrac{X_j - X_i}{h} \right).
%\label{Eq:kde_sq_conv}
%\end{equation}
% 
%\noindent Plugging (\ref{Eq:exp_kde_cv}), (\ref{Eq: kde_loue}) and (\ref{Eq:kde_sq_conv}) into (\ref{Eq:ise_kde_re}) gives the CV criterion
%
%\begin{equation}
%\text{CV}(h) = \dfrac{1}{n^2 h} \sum_{i=1}^{n} \sum_{j=1}^{n} K*K\left( \dfrac{X_j - X_i}{h} \right) - \dfrac{2}{(n-1)nh} \sum_{i = 1}^n \sum_{\substack{j=1 \\ j\neq i}}^{n} K\left(\dfrac{X_i - X_j}{h}\right).
%\end{equation}
%
%\noindent Therefore, the optimal bandwidth with respect to LSCV $h_{\text{\tiny CV}}$ is obtained as
%
%\begin{equation}
%h_{\text{\tiny CV}} =  \underset{h > 0}{\mathrm{argmin}} \ \text{CV}(h). 
%\label{Eq:min_cv_kde}
% \end{equation}
%
%\noindent With (\ref{Eq:min_cv_kde}) the bandwidth can be determined without any distributional assumption. Unlike the rule-of-thumb method in the last subsubsection, the LSCV bandwidth also adapts to the smoothness of $f(x)$. Moreover, \cite{Stone.1984} proved that if $f$ is bounded, $h_\text{\tiny CV}$ is asymptotically optimal in the sense that $\text{ISE}[h_\text{\tiny CV}]$ converges almost surely (a.s.) to $\underset{h > 0}{\min}\ \text{ISE}[h]$:
%\begin{equation}
%\dfrac{\text{ISE}[h_\text{\tiny CV}]}{\underset{h > 0}{\min} \ \text{ISE}[h]} \xrightarrow{a.s.} 1.
%\end{equation}
%\newline
%\noindent A disadvantage of the LSCV estimator is its computational complexity. \cite{Hardle.1991} notes that the number of computational steps to solve (\ref{Eq:min_cv_kde}) is of order $\mathcal{O}(mn^2)$ for $m$ denoting the number of candidate bandwidths. Thus, the number of computational steps increases quadratically in $n$.
%
%
%\subsubsection{Other Bandwidth Estimators}
%
%Another approach that \cite{Hardle.2004} refer to as one of the most popular are refined plug-in-methods. They are similar to the first presented method. However, instead of referencing to a distribution, $\|f\|_2^2$ is estimated nonparametrically as well. Despite relying on bandwidth selectors introduced in Section \ref{Sec:kde_hopt_ref} for estimating $\|f\|_2^2$, refined plug-in-methods deliver good estimates in simulations. \\
%
%\noindent Two other methods presented by \cite{Silverman.1986} are likelihood CV and the test graph method. Likelihood CV is based on computing $\log\left(\widehat{f}_h(x)\right)$ for all observations as leave-one-out estimate. Then, $h_{opt}$ corresponds to the value that maximizes the CV based likelihood criterion. However, likelihood CV is sensitive to outliers and results in inconsistent estimates for most standard densities. Thus, it is suggested to use LSCV to reduce the range for $h$ before likelihood CV is applied. The test graph method is constructed such that estimates are uniformly close to the true density. In doing so, $h_{opt}$ minimizes the maximum estimation error. However, due to the involved subjectivity it is suggested to use the test graph method as check for other estimators and not as single selection method. \\
%
%\noindent Another possible choice is the biased CV estimator proposed by \cite{Hall.1991}. It converges asymptotically with a rate of $\sqrt{n}$ to $h_{opt}$. However, studies showed its inferiority to other methods for small samples. Consequently, for most bandwidth selectors exist advantages and disadvantages and none of them has advantages only. As a result, \cite{Hardle.2004} draws the conclusion that there is no best method. Hence, estimates based on different methods should be compared to select the best one. %The final solution depends, therefore, still on a certain degree of subjectivity. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Choosing the Kernel Function}

%\subsubsection{The Asymptotically Optimal Kernel Function}
%
%Kernel functions can be compared based on their asymptotic approximation quality  by decomposing the AMISE. First, rewrite the optimal bandwidth that was derived by differentiating the AMISE in (\ref{Eq:kde_hopt}):
%
%\begin{align}
%h_{opt}^K &= \left(\dfrac{||K||_2^2 }{n\mu_2(K)^2 ||f''||^2_2} \right)^{1/5} \\
%&=  \underbrace{\left(\dfrac{||K||_2^2 }{\mu_2(K)^2} \right)^{1/5}}_\text{$=:\upsilon_K$} \underbrace{\left(\dfrac{1}{n||f''||^2_2} \right)^{1/5}}_\text{$=:\gamma_{f,n}$} \\
%&= \upsilon_K \gamma_{f,n}. \label{Eq:kde_hopt_re}
%\end{align}
%
%\noindent The first part of (\ref{Eq:kde_hopt_re}), $\upsilon_K$, depends on $K$ whereas the second part, $\gamma_{f,n}$, is independent of $K$. In the next step (\ref{Eq:kde_hopt_re}) is plugged into (\ref{Eq:kde_amise}) in order to decompose the AMISE into one part depending on $K$ and one not depending on $K$. This yields 
%
%\begin{align}
%\text{AMISE}[\hat{f}_{h_{opt}^K}] &= \dfrac{1}{nh_{opt}^K} ||K||_2^2  + \dfrac{(h_{opt}^K)^4}{4} \mu_2(K)^2 ||f''||^2_2 \\
%&= \dfrac{1}{n\upsilon_k \gamma_{f,n}} ||K||_2^2  + \dfrac{(\upsilon_k \gamma_{f,n})^4}{4} \mu_2(K)^2 ||f''||^2_2 \\
%&= \dfrac{1}{n\gamma_{f,n}} \dfrac{||K||_2^2  }{\upsilon_k}+ \dfrac{ \gamma_{f,n}^4}{4} ||f''||^2_2 \upsilon_k^4\mu_2(K)^2. \label{Eq:kde_amise_decom_p1}
%\end{align} 
%
%\noindent With 
%
%\begin{equation}
%\upsilon_K = \left(\dfrac{||K||_2^2 }{\mu_2(K)^2} \right)^{1/5}
%\end{equation}
%
%\noindent equation (\ref{Eq:kde_amise_decom_p1}) becomes 
%
%\begin{align}
%\text{AMISE}[\hat{f}_{h_{opt}^K}] &= \dfrac{1}{n\gamma_{f,n}} ||K||_2^{8/5}\mu_2(K)^{2/5}  + \dfrac{ \gamma_{f,n}^4}{4} ||f''||^2_2 ||K||_2^{8/5}\mu_2(K)^{2/5}  \\
%&= \left( \dfrac{1}{n\gamma_{f,n}} + \dfrac{\gamma_{f,n}^4}{4} ||f''||^2_2 \right) \underbrace{\left(||K||_2^8 \mu_2(K)^2 \right)^{\frac{1}{5}}}_\text{$=:T(K)$} \\
%&= \left( \dfrac{1}{n\gamma_{f,n}} + \dfrac{\gamma_{f,n}^4}{4} ||f''||^2_2 \right) T(K). \label{Eq:kde_amise_decom_p2}
%\end{align}
%
%\noindent $T(K)$ denotes the AMISE part depending on $K$ in (\ref{Eq:kde_amise_decom_p2}). Hence, the optimal kernel can be found by minimizing $T(K)$. The Epanechnikov kernel $K_{Epa}$ is derived by \cite{Epanechnikov.1969}. It can be shown that $K_{Epa}$ minimizes $T(K)$ if only nonnegative kernels with compact support are considered. The efficiency of different kernel functions is presented in Table \ref{Tab:kernel_efficency}. Moreover, the relative deviation of these kernels to $K_{Epa}$ is presented. \citet[p. 61]{Hardle.2004} suggest that from a practical point of view \textit{"the choice of the kernel function is almost irrelevant for the efficiency of the estimate"}. This conclusion is based on the small relative deviations of the other kernel functions from $T(K_{Epa})$. However, it can be argued that even though the deviations are small, $K_{Epa}$ is the most efficient kernel function and should therefore be favored over the others.
%
%\begin{table}[H]
%	\begin{center}
%		\begin{tabular}{c|c|c}
%			\hline \hline
%			\textbf{Kernel} & $\mathbf{T(K)}$ &  $\mathbf{T(K)/T(K_{Epa})}$ \\
%			\hline
%			Uniform & 0.3701  & 1.0602 \\ 
%			\hline
%			Triangel & 0.3531  & 1.0114  \\ 
%			\hline
%			Epanechnikov & 0.3491 & 1.0000  \\ 
%			\hline
%			Quartic/Biweight & 0.3507  & 1.0049 \\ 
%			\hline
%			Triweight & 0.3699 & 1.0595  \\
%			\hline
%			Gaussian & 0.3633 & 1.0408 \\
%			\hline
%			Cosine & 0.3494 & 1.0004  \\
%			\hline \hline
%		\end{tabular}
%	\end{center}
%	\caption[Kernel efficiency in kernel density estimation]{Efficiency of different kernel functions compared to the most efficient kernel, i.e. the Epanechnikov kernel. Source: \cite{Hardle.2004}.}
%	\label{Tab:kernel_efficency}	
%\end{table}

%\subsubsection{Asymptotic Normality of a Kernel Density Estimate}
%
%\cite{Parzen.1962} proved that the kernel density estimator is asymptotically normally distributed. By assuming $nh \to \infty$ and $h^2 \sqrt{nh} \to 0$ as in \cite{Pagan.1999} one obtains
%
%\begin{equation}
%\sqrt{hn} \left( \hat{f_h}(x) - f(x) \right) \xrightarrow{d}  N \left(0, f(x) ||K||_2^2 \right). 
%\end{equation}
%
%\noindent Let $\alpha \in [0,1]$ and $z_{\alpha} = \Phi^{-1}(\alpha)$ where $\Phi$ denotes the cumulative distribution function of the standard normal distribution. Then, the confidence interval ($CI^{\alpha}$) capturing $\alpha$100\% around $f(x)$ is 
%
%\begin{align}
%\left[f(x) -  z_{1 - \frac{\alpha}{2}} \left(\dfrac{||K||_2^2 f(x)}{nh}\right)^{1/2}, \ f(x) +  z_{1 - \frac{\alpha}{2}} \left(\dfrac{||K||_2^2 f(x)}{nh}\right)^{1/2} \right].
%\end{align}
%
%\noindent Since $f(x)$ is unknown, it is replaced by the KDE $\hat{f_h}(x)$
%
%\begin{align}
%\left[\hat{f_h}(x) -  z_{1 - \frac{\alpha}{2}} \left(\dfrac{||K||_2^2  \hat{f_h}(x)}{nh}\right)^{1/2}, \ \hat{f_h}(x) +  z_{1 - \frac{\alpha}{2}}  \left(\dfrac{||K||_2^2 \hat{f_h}(x)}{nh}\right)^{1/2} \right].
%\label{Eq:kde_conf_int}
%\end{align}
%
%\noindent CIs provide an uncertainty measure for $f(x)$. However, if the use of KDE is motivated by finding an appropriate parametric approximation for the observed data, an uncertainty measure for $f$ as a whole should be used. Confidence bands are the appropriate statistical tool in such situations. However, this goes beyond this work and it is instead referred to \cite{Hardle.2004} where an approach for determining confidence bands is presented. 

%\subsubsection{KDE Based Quantile Estimator}

The KDE based quantile estimator to forecast VaR can be derived as follows. First, the  estimator for $F(x)$ that is based on KDE needs to be derived. Denote $\widehat{F}_h(x)$ as the KDE based estimate of $F(x)$. Then, $\widehat{F}_h(x)$ can be derived as follows:

\begin{align}
\widehat{F}_h(x) &= \int_{-\infty}^{x} \hat{f}_h(z)dz \\
&= \int_{-\infty}^{x} \dfrac{1}{nh} \sum_{i = 1}^{n} K\left(\dfrac{z - x_i}{h}\right)dz \\
&= \dfrac{1}{nh} \sum_{i = 1}^{n} \int_{-\infty}^{x}  K\left(\dfrac{z - x_i}{h}\right)dz.
\end{align} 

\noindent Since the given kernel function $K$ is a density, let $\Gamma$ denote the corresponding CDF. Moreover, using the substitution $u = (z - x_i)/h$ one obtains

\begin{align}
\widehat{F}_h(x) &= \dfrac{1}{n} \sum_{i = 1}^{n} \int_{-\infty}^{\frac{x - x_i}{h}}  K\left(u\right)du \\ 
 &= \dfrac{1}{n} \sum_{i = 1}^{n} \Gamma \left( \dfrac{x - x_i}{h} \right).
 \label{Eq:kde_cdf_est}
\end{align} 

\noindent Thus, $\widehat{F}_h(x)$ is the mean of the CDF corresponding to $K$ evaluated at $(x-x_i)/h$ for $i = 1, \dots, n$. Then, for $\alpha  \in (0,1)$ the KDE based quantile function $\widehat{Q}_h$ is obtained as

\begin{equation}
	\widehat{Q}_h(\alpha) = \widehat{F}_h^{-1}(x).
\end{equation}

%\noindent However, it is not possible to obtain a closed form solution for every kernel function. For instance, in case the Gaussian kernel function is used, $\Gamma$ cannot be stated explicitly. Therefore, for the Gaussian kernel function, $\widehat{Q}_h(\alpha)$ is computed by numerically solving  
%
%\begin{equation}
%\widehat{Q}_h(\alpha) = \underset{x \in \mathbb{R}}{\mathrm{argmin}} \left| \dfrac{1}{n} \sum_{i = 1}^{n} \Phi \left( \dfrac{x - x_i}{h} \right) - \alpha \right|
%\label{Eq:kde_quantile_numerical}
%\end{equation}
%
%\noindent where $\Phi$ denotes the CDF of the standard normal distribution. Here, solving (\ref{Eq:kde_quantile_numerical}) corresponds to finding its root. Note, that this can be done with a reasonable speed because there exists an R function to compute $\Phi(u)$. 


==> source code Version for upload/Sections/lit_review.tex <==
\section{Literature Review}\label{Sec:Lit_Rev}

\cite{Kuester.2005} compare the performance of several classical statistical approaches for estimating VaR. Moreover, a comprehensive overview over existing statistical methods is given. Four categories are suggested to describe existing methods for VaR estimation. These categories are historical simulation, fully parametric models, extreme value theory and quantile regression. In the empirical study VaR models belonging to the location scale class are superior over other approaches. In the domain of ML the literature for quantile estimation focuses mainly on neural networks (NN) and SVR. For instance, the derivation of a general approach without an explicit target application can be found in \cite{White.1992}. He used single hidden layer feedforward NNs to derive a way for nonparametric conditional quantile estimation and proved its consistency. However, the ML VaR literature is not as broad as in classical statistics. 
Hence, this section also reviews literature where methods for the construction of prediction intervals (PI) were introduced that could be used in the estimation of VaR. Consequently, the reviewed literature is divided in three paragraphs: Prediction Intervals, Value-at-Risk and Data Driven Value-at-Risk. Here, the first two review the existing literature, whereas the last motivates the method proposed in this paper. 

\paragraph{Prediction Intervals} General approaches are developed by \cite{Hwang.1997} who derive asymptotically valid PIs and \cite{Veaux.1998} who propose a method to estimate PIs for NNs with nonlinear regression. \cite{LinWeng.2004} use SVR to generate out-of-sample residuals via cross validation (CV) and fit those to a Laplace or normal distribution for generating PIs. The results are compared to Bayesian SVR and historical simulation. Despite the mixed results they stress the competitiveness of their method especially due to its simplicity. Pointwise and simultaneous confidence intervals as well as PIs with bias correction for least-squares-SVR are derived by \cite{Brabanter.2011}.  %based on Sidak corrections and upcrossing allowing for heteroscedasticiy and modifying it because of its convervativity% - > 
%However, in comparison to bootstrapping, their method is not superior in simulations. \cite{Khosravi.2013} introduce a framework for constructing PIs of electricity prices. They employ a resampling scheme based on a moving bootstrap approach for data blocks rather than single observations to account for possible correlations. Then, NNs are trained on the bootstrapped data sets to forecast the mean of the time series as center of the prediction interval. The variance is estimated based on a GARCH model but not in the framework of MLE. Instead, they use a cost function directly related to the PI quality that can be minimized with gradient-free algorithms. The resulting mean and variance are then used in a normal distribution to get the PIs. They find that their method has a computational advantage over traditional methods. Moreover, the PIs of their approach are more informative. \cite{Lins.2015} propose a method for confidence intervals and PIs by combining bootstrapping and SVR to bagged SVR in the context of component degradation prediction in the offshore oil industry. They show that their method works in the proposed application.

\paragraph{Value-at-Risk} \cite{Franke.2006} estimate VaR for the German stock index (DAX) by fitting the mean and volatility of the return series with NNs. The mean is modeled autoregressively and the volatility is assumed to follow an autoregressive conditionally heteroscedastic (ARCH) process. Moreover, they include external regressors in both models. The predicted mean and variance are used with the normal distribution to derive the VaR and expected shortfall. As benchmark serves a standard GARCH model based on assuming normality of innovations. In terms of VaR exceedances their model is superior. Moreover, they note its ability to quickly adjust the volatility in case of shocks with only short impact. Another approach directly related to VaR is proposed by \cite{Dunis.2010} which use higher order NNs to forecast VaR. A hybrid model using higher order NNs for variance forecasting and RiskMetrics is shown to outperform other hybrid models empirically. They note also the relatively bad results of the unconditional POT method for quantile estimation. This is, however, not an appropriate comparison when benchmarked to conditional models as was e.g. shown by \cite{Kuester.2005}. \cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test. 
%A multiperiod VaR model was introduced by \cite{Xu.2016}. They use an exponentially weighted support vector quantile regression. In the corresponding empirical study, their approach outperforms other methods that are based on GARCH models, filtered historical simulation and quantile regression. Evaluation was done with different measures as e.g. mean absolute error and p-values of prediction tests.

\paragraph{Data Driven Value-at-Risk} Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. By considering the different model types presented in study of \cite{Kuester.2005}, they can be classified as quantile regression models. In the empirical study of  the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and peaks-over-threshold had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. Most of the proposed methods in the ML literature for estimating VaR or PIs are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this paper. Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions.



==> source code Version for upload/Sections/methods.tex <==
\section{Methodology} \label{Sec:meths}

\input{Sections/value_at_risk.tex}
\input{Sections/garch.tex}
\input{Sections/kde.tex}
\input{Sections/svrSL.tex}
\input{Sections/svrgarchkde.tex}



==> source code Version for upload/Sections/svr.tex <==
%\section{Support Vector Regression}\label{Sec:SVR}

%This section introduces regression based on support vector machines (SVM). Initially, the SVM algorithm was derived for classification. However, in this thesis the methodological focus lies on regression with SVMs. Hence, the SVM algorithm for classification is not covered. Instead, it is referred to \cite{Burges.1998} where a comprehensive and exemplified introduction of SVMs for classification is given. Generally, SVMs are embedded in the framework of statistical learning theory. Consequently, its fundamentals will be introduced in the following section that is based on \cite{Vapnik.1995,Vapnik.1998}. The second part of this section is concerned with SVR. 

%\subsection{Fundamentals of Statistical Learning Theory}
%\label{Sec:SVR_SLT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{The General Model}
%
%In \cite{Vapnik.1995} the framework for learning from data consists of three parts: a generator (G), supervisor (S) and learning machine (LM). G generates random input vectors $x \in \mathbb{R}^p$ that are i.i.d. with an unknown distribution function $F(x)$. Outputs $y$ which correspond to the input vectors $x$ are returned by S according to an unknown and fixed conditional distribution function $F(y|x)$. Although S is unknown, its existence is assumed. Additionally, S is also assumed to not change. Hence, the so-called training set with i.i.d. observations is obtained from G and S:
%\begin{equation}
%\{(y_i, x_i) | i = 1, \dots, n; \ n \in \mathbb{N}\}.
%\end{equation}  
%\noindent Then, the LM is concerned with finding a function to approximate the output of S based on the training set. Formally, for a parameter set $\Theta$, the LM learns the dependence between $x$ and $y$ by implementing a set of functions $g(x, \theta)$ with $\theta \in \Theta$. Consequently, the problem of how to determine $\theta \in \Theta$ for obtaining the best approximation of the supervisor's response needs to be solved. Solving this problem is the so-called learning process which can be described as follows: \textit{"The learning process is a process of choosing an appropriate function from a given set of functions."} \cite[p. 21]{Vapnik.1998}.
%
%%For a parameter set $\Theta$, the dependence between $x$ and $y$ is learned by a LM that implements a set of functions $g(x, \theta)$ with $\theta \in \Theta$. The function $g$ is determined by an i.i.d. training set $\{(y_i, x_i) | i = 1, \dots, l \in \mathbb{N}\}$ with the joint distribution $F(x,y) = F(x)F(y|x)$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Minimizing the Risk Functional}
%
%The LM is used to approximate the values $y$ returned by S. However, to find an appropriate approximation it is necessary to measure the discrepancy between $y$ and $g(x, \theta)$. In the terminology of \cite{Vapnik.1995, Vapnik.1998} this discrepancy is called loss. Hence, the so-called loss function $L(y, g(x, \theta))$ is introduced. Based on this, the risk functional $\mathcal{R}(\theta)$ which measures the expected loss and, therefore, the approximation's quality is defined as 
%
%\begin{equation}
%\mathcal{R}(\theta) = \int L(y, g(x, \theta)) dF(x,y).
%\label{Eq:risk_fct}
%\end{equation}
%
%\noindent Consequently, the optimal parameter $\theta_0 \in \Theta$ minimizes (\ref{Eq:risk_fct}):
%\begin{equation}
%\theta_{0} = \underset{\theta \in  \Theta}{\mathrm{argmin}} \ \mathcal{R}(\theta).
%\end{equation} 
%
%%Let $G = \{g(z) | z \in Z \subset \mathbb{R}^n \}$ be the set of admissible functions and $R(g(z))$ the function to measure the quality of the approximation. By constructing $R(g(z))$ so that its minimum corresponds the approximation with the highest quality, the optimal approximation $g(z)^* \in G$ is
%%\begin{equation}
%%g(x, \theta_{opt}) = \underset{g(x, \theta) \in \ G}{\mathrm{argmin}} \ R(g(x, \theta)).
%%\end{equation} 
%%
%%\noindent \cite{Vapnik.1995} defines $R(g(z))$ as the mathematical expectation: 
%%
%%\begin{equation}
%%R(\theta) = \int L(y, g(x, \theta)) dF((x,y)).
%%\label{risk_fct}
%%\end{equation}
%%
%%$R(\theta)$ is the so-called risk functional which is minimized by the function $g(x, \theta)$ that fits the training data best.
%
%\noindent Now, the problem arises of how to minimize (\ref{Eq:risk_fct}) with unknown $F(x,y)$. The only available information is contained in the training set. Thus, an approach based on the empirical data needs to be derived.
%%Direct minimization requires to find $g(x, \theta)$ whereas minimization with empirical data requires to state a construction criterion to choose the function. This follows from the unknownness of $F(x,y)$ whereby (\ref{Eq:risk_fct}) cannot be used as a selection criterion.   
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Empirical Risk Minimization Inductive Principle}
%     
%Since the joint distribution $F(x, y)$ is unknown, minimizing the risk functional in practice cannot be done analytically but relies on empirical data. For introducing a corresponding inductive principle, \cite{Vapnik.1995,Vapnik.1998} considers the general case of an i.i.d. sample $\{z_1, \dots, z_n\}$ coming from a random variable $Z$ with unknown probability measure $F(z)$. Further, a set of functions $P(z, \theta)$, $\theta \in \Theta$, is considered such that (\ref{Eq:risk_fct}) can be generalized to
%
%\begin{equation}
%\mathcal{R}(\theta) = \int P(z, \theta) dF(z).
%\label{Eq:risk_fct_general}
%\end{equation}
%  
%\noindent In terms of (\ref{Eq:risk_fct}), $P(z, \theta)$ represents the loss function and $z$ some values $(y,x)$. Then, instead of minimizing $\mathcal{R}(\theta)$ the corresponding explicitly defined empirical risk functional can be minimized: 
%
%\begin{equation}
%\mathcal{R}_{emp}(\theta) = \frac{1}{n}\sum_{i = 1}^{n} P(z_i, \theta).
%\end{equation}
%
%\noindent In addition to defining the empirical risk functional, denote $\theta_0$ and $\theta_{train}$ as the parameter vectors minimizing $\mathcal{R}(\theta)$ and $\mathcal{R}_{emp}(\theta)$, respectively. Then, minimizing $\mathcal{R}_{emp}(\theta)$ corresponds to approximating $P(z, \theta_0)$ with $P(z, \theta_{train})$. In summary, the core of the Empirical Risk Minimization (ERM) inductive principle is replacing $\mathcal{R}(\theta)$ with $\mathcal{R}_{emp}(\theta)$ and approximating $P(z, \theta_0)$ with $P(z, \theta_{train})$. \\
%
%\noindent The ERM principle is a central point in statistical learning theory because appropriate conditions must be found in order to approximate $P(z, \theta_0)$ closely. Moreover, \cite{Vapnik.1998} shows that classical methods as least squares regression and maximum likelihood based density estimation are covered by the ERM inductive principle. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Structural Risk Minimization Inductive Principle}
%
%The goal of the ERM inductive principle is to minimize the empirical risk. However, this is done without considering the complexity of the function that fits the training set best. Large sample sizes ensure that the ERM inductive principle is appropriate for minimizing risk. This is due to the fact that the empirical risk will be close to the actual risk. Hence, low empirical risk will be observed if the actual risk is low as well. However, in case of a small sample size overfitting might occur, i.e. the empirical risk is low even though the actual risk is not. Complex functions are able to perfectly fit the training data. However, while the empirical risk is minimized, their generalization ability can be bad in out-of-sample predictions. The Structural Risk Minimization (SRM) inductive principle is a way to overcome the above mentioned problems. The core of the SRM inductive principle is an error bound on the actual risk. This bound depends on the empirical risk and the complexity of the function.   \\ 
%
%
%%\cite{Vapnik.1995,Vapnik.1998} concludes this from a bound he derived for the actual risk functional (\ref{Eq:risk_fct}). This bound is the sum of the empirical risk and a confidence interval which depends on the so-called capacity of a function. \\
%
%\noindent For deriving the SRM inductive principle it is necessary to show how the complexity of a function can be measured. In doing so, the terminology of \cite{Vapnik.1995,Vapnik.1998} is used where capacity is used as synonym for complexity. Capacity in the considered bound is measured as Vapnik-Chervonenkis (VC) dimension $h$. Intuitively, in case of a classification problem, the VC dimension measures how many vectors can be classified correctly. For instance, \cite{Vapnik.1995} demonstrates that for a set of linear indicator functions with $p$ attributes the VC dimension is $h = p + 1$. The intuition behind this result is that at most $p + 1$ data points can be classified correctly. Figure~\ref{vc_dim_example} depicts the case of three random vectors coming from $\mathbb{R}^2$. Here, $p = 2$ and the VC dimension is consequently $h = 3$. Hence, all possible label assignments ($2^3 = 8$) of the three vectors can be perfectly classified. However, this does not hold for four vectors as is indicated in Figure~\ref{Fig:vc_dim_example}. Assume the labels of $z_2$ and $z_4$ are equal and different from $z_1$ and $z_3$. Then, there is no line that can separate $z_2$ and $z_4$ from $z_1$ and $z_3$. Thus, no perfect classification is possible using linear decision functions. \\
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale = 0.39]{Figures/vc_dim_burges}
%	\caption[VC dimension for three points in $\mathbb{R}^2$]{Shattering three points in $\mathbb{R}^2$ in case of linear indicator functions. The color of the point indicates the class. A perfect classifier can be found for all eight possible label assignments. Source: \cite{Burges.1998}.}
%	\label{vc_dim_example}
%\end{figure}
%  \begin{figure}[H]
% 	\centering
% 	\includegraphics[scale = 0.39]{Figures/vc_dim_vapnik}
% 	\caption[VC dimension for four points in $\mathbb{R}^2$]{Separating four points in $\mathbb{R}^2$ is not possible for all possible labels with linear decision functions. Source: \cite{Vapnik.1995}.}
% 	\label{Fig:vc_dim_example}
% \end{figure}
% 
%% \clearpage
% 
% \noindent To formally introduce the VC dimension consider the following definitions for indicator and real functions taken from \citet[p. 76-77]{Vapnik.1995}. 
%
%% In contrast, small sample sizes correspond usually to a small $l/h$. Consequently, low empirical risk does not necessarily imply low actual risk. Such cases can be accommodated by indtroducing the  \textit{Structural Risk Minimization} (SRM) inductive principle. The SRM inductive principle accounts in minimizing the risk functional for the empirical risk and the confidence interval. 
%%
%%Define S as a set of functions that consists of nested subsets of functions $S_k = \{P(z, \theta \in \Theta_k)\}$ with $S_1 \subset S_2 \subset \dots \subset S_n \dots$. The structure of $S$ is an \textit{admissible structure} if it has the properties stated in \cite[p.~90-91]{Vapnik.1995}. The ERM inductive principle was characterized by choosing the function $P(z, \theta_{train}$) which minimizes the empirical risk. In contrast, the SRM inductive principle takes the training error and complexity of $P(z, \theta_{train}$) into account. This is done by choosing the function from the subset $S_n$ where the empirical risk and error bound on the actual risk is minimized. 
%%
%%The error bounds were derived by CORTES AND VAPNIK and depend on the empirical risk and a confidence interval $\Psi$. $\Psi$ grows monotonically with the complexity $h_k$ of $S_k$. VAPNIK introduced the term \textit{capacity} to describe the complexity of a function. The so-called Vapnik-Chervonenkis (VC) dimension $h$ is a measure for the capacity of a function class. In \cite{Vapnik.1995}, the VC dimension for a set indicator and real functions is defined as follows.  
%\newtheorem{mydef}{Definition}
%\begin{mydef}
%	\textbf{The VC dimension of a set of indicator functions} 
%	
%	The VC dimension of a set of indicator functions $P(z, \theta)$, $\theta \in \Theta$, is the maximum number $h$ of vectors $z_1, \dots, z_n$ that can be separated into two classes in all $2^h$ possible ways using functions of the set (i.e., the maximum number of vectors that can be shattered by the set of functions). If for any $n$ there exists a set of $n$ vectors which can be shattered by the set $P(z, \theta)$, $\theta \in \Theta$, then the VC dimension is equal to infinity.
%
%\end{mydef}
%
%\begin{mydef}
%		
%	\textbf{The VC dimension of a set of real functions}
%	
%	Let $A \le P(z, \theta) \le B$, $\theta \in \Theta$, be a set of real functions bounded by constants $A$ and $B$ ($A$ can be $-\infty$ and $B$ can be $\infty$). Let us consider along with the set of real functions $P(z, \theta)$, $\theta \in \Theta$, the set of indicators
%	
%	\begin{equation}
%	\mathscr{I}(z, \theta, \beta) = \mathbb{I}(P(z,\theta)- \beta), \ \theta \in \Theta, \ \beta \in (A,B),
%	\end{equation}
%	
%	\noindent where $\mathbb{I}(z)$ is the step function
%	
%	\begin{equation}
%	\mathbb{I}(z) = \begin{cases}
%	0 \text{ \ if \ } z < 0 \\
%	1 \text{ \ if \ } z \ge 0. \\
%	\end{cases}
%	\end{equation}
%		
%	\noindent The VC dimension of a set of real functions $P(z,\theta)$, $\theta \in \Theta$, is defined to be the VC dimension of the set of corresponding indicators with parameters $\theta \in \Theta$ and $\beta \in (A,B)$.
%	
%\end{mydef}
%
%\noindent One should note that the VC dimension of a set of functions is not equal to the number of free parameters in the functions. \citet[p. 65]{Vapnik.1995} states that \textit{"constructive distribution-independent bounds"} can be obtained by using the VC dimension $h$ as a capacity measure for a set of functions. \\
%
%\noindent To obtain bounds for the actual risk let $S = \{P(z, \theta)| \ \theta \in \Theta\}$ be a set of functions with a structure such that $S$ consists of nested subsets of functions $S_m = \{P(z, \theta| \ \theta \in \Theta_m)\}$. \citet[p.~90-91]{Vapnik.1995} states conditions under which $S$ has an admissible structure. Consequently, in the following is assumed that $S$ fulfills these conditions. Then, a learning machine's generalization ability can be controlled by the corresponding risk bounds. In general, the bound on the actual risk for functions in $S_m$ is with probability $(1-\eta)$
%
%\begin{equation}
%\mathcal{R}(\theta_{train}^m) \le \mathcal{R}_{emp}(\theta_{train}^m) + B_m E_m(n) \left(1 + \sqrt{1 + \dfrac{4 \mathcal{R}_{emp}(\theta_{train}^m)}{B_m E_m(n)}} \right)
%\label{Eq:guaranteed_risk}
%\end{equation}
%
%\noindent with 
%
%\begin{equation}
%E_m(n) = \dfrac{4 h_m \left( \log \dfrac{2n}{h_m} + 1\right) - \log \dfrac{\eta}{4}}{n},
%\end{equation}
%
%\noindent where $h_m$ is the VC dimension, $B_m $ the upper bound for the functions in $S_m$ with $B_m \ge 0 $ and 
%\begin{equation}
%\sup \dfrac{ \sqrt[v]{ \mathbb{E}[P^v(z,\theta)] } }{ \mathbb{E}[P(z,\theta)] }  \le \tau_m < \infty.
%\end{equation}
%
%\noindent  Moreover, $h_m$, $B_m$ and $\tau_m$ are non-decreasing series:
%\begin{align}
%&h_1 \le h_2 \le \dots \le h_m \le \dots \label{Eq:kappa_nond} \\
%&B_1 \le B_2 \le \dots \le B_m \le \dots \\
%&\tau_1 \le \tau_2 \le \dots \le \tau_m \le \dots .
%\end{align}
%
%\noindent The ERM inductive principle was characterized by choosing the function $P(z, \theta_{train}$) which minimizes the empirical risk. In contrast, the SRM inductive principle takes the training error and complexity of $P(z, \theta_{train})$ into account. This is done by choosing the set of functions $S_m$ that minimizes the bound of the actual risk on the right hand side of (\ref{Eq:guaranteed_risk}). The term that is added to the empirical risk in (\ref{Eq:guaranteed_risk}) is called confidence interval. The confidence interval measures the complexity of a set of functions relative to the number of training instances. Figure~\ref{Fig:srm_fig} demonstrates the motivation behind the SRM inductive principle. In balancing out the trade-off between function capacity and empirical risk minimization, an appropriate nested subset of functions $S^*$ in $S$ is obtained to control possible over- and underfitting. Moreover, one can see that the capacity gets lower the deeper a set $S_m$ is nested in $S$. This follows from (\ref{Eq:kappa_nond}). Consequently, $S_1$ contains the functions with the lowest capacity.    
%\begin{figure}[H]
%	\centering
%	\includegraphics[scale = 0.5]{Figures/SRM_Figure}
%	\caption[Illustration of the SRM inductive principle]{Illustration of the SRM inductive principle. The sum of empirical risk and confidence interval is equal to the bound on the actual risk. The SRM inductive principle aims at finding a compromise between empirical risk minimization and function capacity for a given training set. Source: \cite{Vapnik.1995}.}
%	\label{Fig:srm_fig}
%\end{figure}
%
%%\subsubsection{Minimizing the Guaranteed Risk}
%
%%\noindent Thus, constructing a learning machine on the basis of the SRM inductive principle requires minimizing the guaranteed risk. The second term of the right hand side of (\ref{Eq:guaranteed_risk}) can be rewritten as a function $\Psi$ depending on the ratio $l/h_k$. So, rewriting (\ref{Eq:guaranteed_risk}) results in 
%%
%%\begin{equation}
%%R(\theta_{train}^k) \le R_{emp}(\theta_{train}^k) + \Psi (\dfrac{l}{h_k}).
%%\label{guaranteed_risk_simple}
%%\end{equation}
%
%%\noindent Based on (\ref{guaranteed_risk_simple}) \cite{Vapnik.1995} suggests two ways for minimizing the guaranteed risk: 
%
%%\begin{enumerate}
%%
%%\item Fix $\Psi (l/h_k)$ by choosing an appropriate $S_k$ and minimize $R_{emp}(\theta_{train}^k)$.
%%
%%\item Fix $R_{emp}(\theta_{train}^k)$ and minimize $\Psi (l/h_k)$.
%%
%%\end{enumerate}
%%
%%\noindent Neural Networks are an example for the first and Support Vector machines for the second approach. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Classification with Support Vector Machines} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Support Vector Regression}
SVR can be understood as a learning method to solve nonlinear regression tasks  \cite[e.g.,][]{Smola.2004}. It shares some similarities with a three-layer feed-forward neural network and is able to approximate arbitrarily complex functions (i.e., universal approximator) \citep{Chen.2009}. 
%\cite{Chen.2009} describe SVMs as feedforward NNs with one input, single hidden and output layer where the regression function is obtained via quadratic programming. In the hidden layer, the information of the input layer is mapped into a high-dimensional space to capture nonlinearities. As a consequence, SVMs can learn any nonlinear relationship if the dimension of the hidden space is high enough. The algorithm for doing regression with SVMs is introduced in this section. If not indicated otherwise, the derivations are based on the work of \cite{Smola.2004}. 
To describe the SVR model, 
%\subsubsection{Support Vector Regression and Dual Optimization}

let $\{(y_i, x_i)| i = 1,\dots, n; \ n\in \mathbb{N}\}$ with $x_i \in \mathbb{R}^p$ and $y_i \in \mathbb{R}$ denote the training data set. Suppose $f$ is a linear function such that 

\begin{equation}
f(x) = \omega^T x + b
\label{Eq:svr_lin_base_mdl}
\end{equation}

\noindent where  $\omega \in \mathbb{R}^p$ and $b \in \mathbb{R}$. Then, SVR aims to find an approximation of $f$ that deviates at most by $\epsilon$ from the observed target $y$ while being as flat as possible (i.e., in the sense that weights in $\omega$ are small). This translates into the following convex optimization problem:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 \\
& \text{subject to} & & \begin{cases}
y_i - \omega^T x_i - b \le \epsilon  \\
\omega^T x_i + b - y_i \le \epsilon.
\end{cases} 
\end{aligned}
\label{svm_mean_eq}
\end{equation}
\newline

In view that (\ref{svm_mean_eq}) might lack a feasible solution, \cite{Vapnik.1995} introduces an $\epsilon$-insensitive loss function: 

\begin{equation}
L_{\epsilon}(y - f(x))  = \begin{cases}
0 \qquad \qquad \qquad  \text{if} \ |y - f(x)| \le \epsilon \\
|y - f(x)| - \epsilon \ \ \text{otherwise}.
\end{cases}
\label{Eq:svr_alt_loss_fct}
\end{equation}

\noindent To measure empirical loss (and thus model fit) using (\ref{Eq:svr_alt_loss_fct}) \cite{Vapnik.1995} reformulates (\ref{svm_mean_eq}) using slack variables $\zeta$ and $\zeta^{*}$ that capture losses above and below the $\epsilon$-tube around $f(x)$, respectively. Figure~\ref{loss_fct} depicts this approach. Only points outside the gray shaded $\epsilon$-tube contribute linearly to the loss function. \\ 

%\cite{Vapnik.1995} integrated this type of loss function by using slack variables $\zeta_i$ and $\zeta^{*}_{i}$ in the optimization problem.
%
%To account for possibly infeasible constrains, SVR is defined with respect to a so-called $\epsilon$-insensitive loss function. \cite{Vapnik.1995} integrated this type of loss function by using slack variables $\zeta_i$ and $\zeta^{*}_{i}$ in the optimization problem. Based on this, the $\epsilon$-insensitive loss function $|\zeta|_\epsilon $ can be defined as

%\begin{equation}
%|\zeta|_\epsilon =: \begin{cases} 
%0 \text{  if   } |\zeta| \le \epsilon  \\
%|\zeta| - \epsilon \text{    otherwise}
%\end{cases}
%\label{Eq:slack_loss}
%\end{equation}


%\noindent It can be interpreted as tolerance measure for absolute errors that are greater than $\epsilon$. Based on this, \cite{Vapnik.1995} integrated slack variables $\zeta_i$ and $\zeta^{*}_{i}$ in the optimization problem.

\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.4]{Figures/svm_loss_fct_correct}
	\caption[The $\epsilon$-insensitive loss function]{The $\epsilon$-insensitive loss function of the SVR algorithm. Slack variable $\zeta$ captures the loss above the $\epsilon$-tube. Points within the grey shaded area have no impact on the loss. In contrast, all other observations contribute linearly to the loss. Source: \cite{Smola.2004}.}
	\label{loss_fct}
\end{figure}


Integrating the slack variables $\zeta$ and $\zeta^*$ into (\ref{svm_mean_eq}), the task to estimate a SVR model is equivalent to solving:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 + C\sum_{i = 1}^{n}(\zeta_i + \zeta^{*}_i) \\
& \text{subject to} & &  \begin{cases}
y_i - \omega^T x_i - b \le \epsilon + \zeta_i \\
\omega^T x_i + b - y_i \le \epsilon + \zeta_i^{*} \\
\zeta_i, \zeta_i^{*} \ge 0.
\end{cases} 
\end{aligned}
\label{svr_opt_fct}
\end{equation}
\newline

where $C > 0$ is a regularization parameter to balance between model fit and complexity \citep[e.g.,][]{Hastie.2009}. Larger (smaller) values of $C$ put more (less) weight on maximizing model fit during SVR learning. 
 
To capture nonlinear relationships between covariates and the response variable, SVR maps the input data into a higher dimensional feature space. The linear regression is then constructed in the transformed space, which corresponds to a nonlinear regression in the input space. The transformation is feasible from a computational point of view because SVR calculates the mapping implicitly using a kernel function 
$k(x_i^T x)=\Theta(x^T) \Theta(x)$. To implement this approach, it is common practice to estimate a SVR model through solving the dual of (\ref{svr_opt_fct}), which is given as \citep[e.g.,][]{Smola.2004}:

\begin{equation}
\begin{aligned}
& \text{maximize} 
	-\dfrac{1}{2} \sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)x_i^T x_j 
	-\epsilon\sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n}y_i(\rho_i - \rho_i^*)
 \\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
	\rho_i, \rho_i^* \in [0, C].
	\end{cases}
\end{aligned}
\label{dual_lin_opt}
\end{equation}
\newline

The dual program (\ref{dual_lin_opt}) includes the input data only in the form of scalar products $x_i^T x_j$. Replacing the scalar product by means of a kernel function is thus straightforward and does not affect the solver. In this work, we employ the Gaussian radial basis function (RBF) kernel (\ref{rbf_kernel}) because it includes other kernels as special cases, posses numerical advantages compared to alternatives, and often performs well in practical applications \citep{Keerthi.2003}.  

\begin{equation}
\begin{aligned}
k(x_i^T x)= \exp \left(\dfrac{\| x - x_i \|}{2 \gamma^2} \right)
\end{aligned}
\label{rbf_kernel}
\end{equation}
\newline



%######### SL####################################################################

among covariats and between 
It is common practice to estimate a SVR model through solving the dual of (\ref{svr_opt_fct}). In addition to computational advantages, an important feature of the dual is that the input data appears only in the form of scalar products $x_i^T x_j$. Replacing the scalar product with kernel function, which calculates the scalar product in a nonlinearly transformed feature space of higher dimension directly in the input space, enables SVR to account for nonlinear relationships. 


That is, forming the Langrangian (\ref{svr_opt_fct}) of An important  \citep[e.g.,][]{Smola.2004}. 
 
\iffalse

\noindent Solving (\ref{svr_opt_fct}) is usually easier by using its dual formulation. % which is moreover the central point in the estimation of nonlinear functions by SVR.
 This can be done by setting up the corresponding Lagrange function. The reason behind this is that it can be shown that the Lagrange function has a saddle point at the solution of an optimization problem with inequalities as constraints.
Let $ \rho $, $ \rho^* $, $ \eta $ and $ \eta^*$ be Lagrange multipliers which are consequently non-negative. Then, for SVR the corresponding Lagrange function is

\begin{equation}
\begin{aligned}
L(\omega, C, \zeta, \zeta^*, \rho, \rho^*, \eta, \eta^*) = & \frac{1}{2}\|\omega\|^2 + C\sum_{i=1}^{n}(\zeta_i + \zeta_i^*) \\
& - \sum_{i=1}^{n}(\eta_i\zeta_i + \eta_i^*\zeta_i^*) \\
& - \sum_{i=1}^{n}\rho_i(\epsilon + \zeta_i - y_i + \omega^Tx_i + b) \\
& - \sum_{i=1}^{n}\rho_i^*(\epsilon + \zeta_i^* + y_i - \omega^Tx_i - b).
\end{aligned}
\label{Eq:lagrange_lin_svr}
\end{equation}
\newline
\noindent The solution of the optimization problem (\ref{svr_opt_fct}) is at the saddle point of (\ref{Eq:lagrange_lin_svr}). Hence, for the partial derivatives of (\ref{Eq:lagrange_lin_svr}) with respect to $\omega$, $b$, $\zeta_i$ and $\zeta_i^*$ holds the following:

\begin{align}
\frac{\partial L(\cdot)}{\partial b} &= \sum_{i = 1}^{n} (\rho_i^* - \rho_i) = 0
\label{sp_c1} \\
\frac{\partial L(\cdot)}{\partial \omega} &= \omega - \sum_{i = 1}^{n} (\rho_i - \rho_i^*)x_i = 0
\label{sp_c2} \\
\frac{\partial L(\cdot)}{\partial \zeta_i} &= C - \rho_i - \eta_i = 0
\label{sp_c3} \\
\frac{\partial L(\cdot)}{\partial \zeta_i^*} &= C - \rho_i^* - \eta_i^* = 0.
\label{sp_c4} 
\end{align}

\fi

\noindent By solving (\ref{svr_opt_fct})
%substituting (\ref{sp_c1}), (\ref{sp_c2}), (\ref{sp_c3}) and (\ref{sp_c4}) into (\ref{Eq:lagrange_lin_svr}) 
one obtains 

\begin{equation}
\begin{aligned}
& \text{maximize}  
-\frac{1}{2}\sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)x_i^T x_j -\epsilon \sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n} y_i (\rho_i - \rho_i^*) 
\\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
\rho_i, \rho_i^* \in [0, C].
\end{cases}
\end{aligned}
\label{dual_lin_opt}
\end{equation}


%\begin{equation}
%\begin{aligned}
%& \text{maximize} && \begin{cases}
%-\frac{1}{2}\sum_{i,j = 1}^{j}(\rho_j - \rho_j^*)x_i' x_j \\
%-\epsilon \sum_{i = 1}^{l}(\rho_i + \rho_i^*) + \sum_{i = 1}^{l} y_i (\rho_i - \rho_i^*) 
%\end{cases} \\
%& \text{subject to} && \begin{cases} \sum_{1}^{l} (\rho_i - \rho_i^*) = 0\\
%\rho_i, \rho_i^* \in [0, C]
%\end{cases}
%\end{aligned}
%\label{dual_lin_opt}
%\end{equation}

\noindent Due to the dual formulation of the optimization problem one can 
%rearrange (\ref{sp_c2}) to 
%%%%Multiple steps skipped
get a representation of the weight vector $\omega$:

\begin{equation}
\omega = \sum_{i = 1}^{n} (\rho_i - \rho_i^*)x_i.
\label{Eq:weight_lin_svr}
\end{equation}
\newline
Thus, $\omega$ is a linear combination of the observations $x_i$. So, the theoretical starting point in (\ref{Eq:svr_lin_base_mdl}) can be rewritten as the so called SV expansion:
\begin{equation}
f(x) = \sum_{i = 1}^{n}(\rho_i - \rho_i^*)x_i^T x + b.  
\label{sv_exp_lin}
\end{equation}
\newline
For those $x_i$ where $f(x_i)$ is within the $\epsilon$-tube it holds that  $\rho_i = \rho_i^* = 0$. Hence, $f(x)$ is determined by the observations outside the $\epsilon$-tube. These $x_i$ are the so-called SVs. Consequently, the complexity of $f(x)$ depends on the number of SVs rather than the dimension of the input space.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Deriving the Constant Term}
%
%After $\rho_i$ and $\rho_i^*$ are obtained, $b$ can be derived from the Karush-Kuhn-Tucker (KKT) conditions. Their central statement is that the product of constraints and dual variables is zero at the solution. Therefore, the KKT conditions corresponding to (\ref{dual_lin_opt}) are:
%
%\begin{equation}
%\begin{aligned}
%\rho_i(\epsilon + \zeta_i - y_i + \omega' x_i + b) & = 0 \\
%\rho_i^*(\epsilon + \zeta_i^* + y_i - \omega' x_i - b) & = 0 \\
%(C - \rho_i)\zeta_i & = 0 \\
%(C - \rho_i^*)\zeta_i^* & = 0.
%\end{aligned}
%\label{kkt}
%\end{equation}
%From (\ref{kkt}) follows that  
%\begin{equation}
%\begin{aligned}
%\epsilon - y_i + \omega'x_i+ b & \ge 0 \text{\quad and \quad} \zeta_i = 0  & \text{if \quad} \rho_i < C \\
%\epsilon - y_i + \omega'x_i + b & \le 0                                     & \text{if \quad} \rho_i > 0.
%\end{aligned}
%\label{kkt_conc}
%\end{equation}
%
%\noindent By doing the same derivation for $\rho^*$ as for $\rho$ in (\ref{kkt_conc}) the following bounds on $b$ can be obtained:  
%% 
%%\begin{equation}
%%\begin{aligned}
%%\max_i & \{-\epsilon + y_i -\omega'x_i | \rho_i < C \text{ or } \rho_i^* > 0 \} \le b  \\ \min_i & \{-\epsilon + y_i - \omega'x_i | \rho_i > 0 \text{ or } \rho_i^* < C\} \ge b.
%%\end{aligned}
%%\label{ineq_b}
%%\end{equation}
%
%\begin{align}
%b_\text{lower} := \max_i & \{-\epsilon + y_i -\omega'x_i | \rho_i < C \text{ or } \rho_i^* > 0 \} \le b  \\ b_\text{upper} := \min_i & \{-\epsilon + y_i - \omega'x_i | \rho_i > 0 \text{ or } \rho_i^* < C\} \ge b.
%\end{align}
%
%
%\noindent Since $\rho_i$ and $\rho_i^*$ cannot be simultaneously nonzero the bounds are tight if $\rho_i\in(0, C)$ or $\rho_i^*\in(0, C)$ such that $b = b_\text{lower} = b_\text{upper}$. However, due to the constraints of (\ref{dual_lin_opt}) there can be training instances where $\rho_i$ or $\rho_i^*$ is equal to $C$. However, according to \cite{Chen.2009}, such situations can be hardly found in reality.  
%
%   
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Capturing Nonlinearity with Kernels}

%One approach to capture potential nonlinearities of the training data is to map the space of the training data $X$ into a feature space $F$, i.e. $\Theta: X \rightarrow F$. 
One approach to capture potential nonlinearities is to use a mapping $\Theta$ to map the training data space into some feature space. In practice, this can be done by preprocessing the training data to obtain polynomial features. Depending on the dimension of the training data space and order of the polynomials, the number of features can increase rapidly. More formally, for $p$ being the dimension of the training data space and $d$ being the degree to which polynomial features for all attributes of the training data are computed, the number of features will be determined by the binomial coefficient $\binom{d + p - 1}{d}$. The exponential increase of the feature space size is visualized in Figure~\ref{feat_size}. Hence, \cite{Smola.2004} consider this approach to be not feasible. \\
%%%out
\iffalse
\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.6]{Figures/size_feat_space}
	\caption[Feature space dimension for polynomial mappings]{Number of features in dependence of the dimension of the input space, i.e. training data space, and the degree of the polynomial mappings. Source: Own illustration.}
	\label{feat_size}
\end{figure}
\fi

\noindent A more feasible approach is obtained by noting that the solution of (\ref{dual_lin_opt}) depends on the input variables in form of dot products, i.e. $x^T x$. Hence, the input vectors can be mapped into a higher dimensional space by considering different dot products. As a consequence, it is not necessary to know $\Theta$ explicitly but sufficient to know the result of $\Theta(x^T) \Theta(x)$. Thus, by introducing the so-called kernel function $k(x^T, x) = \Theta(x^T)\Theta(x)$, (\ref{dual_lin_opt}) can be reformulated as follows:

\begin{equation}
\begin{aligned}
& \text{maximize} 
	-\dfrac{1}{2} \sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)k(x_i^T, x_j) 
	-\epsilon\sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n}y_i(\rho_i - \rho_i^*)
 \\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
	\rho_i, \rho_i^* \in [0, C].
	\end{cases}
\end{aligned}
\label{dual_nonlin_opt}
\end{equation}
\newline
\noindent Due to reformulating (\ref{dual_lin_opt}), the representation of the weight vector in (\ref{Eq:weight_lin_svr}) and  the SV expansion in (\ref{sv_exp_lin}) become 

\begin{equation}
\begin{aligned}
\omega & = \sum_{i = 1}^{n} (\rho_i - \rho_i^*)\Theta(x_i)  \\
f(x)& = \sum_{i = 1}^{n}(\rho_i - \rho_i^*)k(x_i^T, x) + b. 
\end{aligned}
\label{sv_exp_nonlin}
\end{equation}
\newline
The formulas in (\ref{sv_exp_nonlin}) depict two differences between the linear and nonlinear case. First, the restated optimization problem does not result in the flattest function of the input space but feature space. Moreover, since only the result of $k(x_i^T x)$ is needed in the computation of $f(x)$, $\omega$ is no longer given explicitly. \\

\noindent The use of kernel functions in SVR makes it necessary to establish conditions that ensure their results correspond to the dot product in a feature space. These conditions are the so-called Mercer's conditions which can be found in \cite{Smola.2004}. Three examples of kernel functions that are given by \cite{Smola.2004} are: 

\begin{align*}
%\text{Linear:}& \qquad x_i^T x  \\
\text{Polynomial:}& \quad (x_i^T x + c)^p \qquad &\text{with}& \ c \ge 0 \ \text{and} \ p \in \mathbb{N} \\
\text{Radial Basis Function:}& \quad \exp \left(\dfrac{\| x - x_i \|}{2 \gamma^2} \right)\qquad &\text{with}& \ \gamma > 0 \\
\text{Hyperbolic Tangent:}& \quad \text{tanh}(c +  h x_i^T x ) \qquad &\text{with}& \ c \in \mathbb{R}  \ \text{and} \ h \ge 0. \\
%\text{B-Spline:}& \quad B_{2n+1} ( \|x_i^T - x\|)  \qquad &\text{with}& \ B_k(z) = \otimes_{i = 1}^{k} \mathbb{I}(z \in [-0.5, 0.5]).
\end{align*}
\noindent %Here, $\otimes$ is the convolution operator.
 A special case of the polynomial kernel is the linear case which was used to introduce SVR. It is obtained for $c = 0$ and $p = 1$. Moreover, the hyperbolic tangent kernel is not an admissible kernel in the sense that it fulfills Mercer's conditions. However, it was shown to perform well in practice. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{SVR in Terms of Risk Minimization} \label{Sec:svr_ito_risk}
%
%SVR is rooted in statistical learning theory. However, the derivation was not based on the framework of the SRM inductive principle. The connection can be shown by reformulating the optimization problem in terms of a risk functional. In doing so, similarities of SVR and other function approximation methods can be seen. For instance, with respect to other methods for function approximation \cite{Smola.2004} show how SVR can be related to MLE. Consider the following empirical risk functional which is formulated in terms of the $\epsilon$-insensitive loss function in equation (\ref{Eq:svr_alt_loss_fct}):
%
%\begin{equation}
%\mathcal{R}_{emp}(f) = \frac{1}{n} \sum_{i = 1}^{n} L_{\epsilon}(y_i - f(x_i)).
%\label{Eq:svr_emp_risk}
%\end{equation}

%\noindent In the next step, a term to control the capacity of $f$ needs to be introduced. In (\ref{svr_opt_fct}) this was done by including $\| \omega \|^2$ in the minimization problem. Hence, the objective function to be minimized in SVR can be stated as the following regularized risk functional: 
%
%\begin{equation}
%\mathcal{R}_{reg}(f) = \frac{1}{n} \sum_{i = 1}^{n} L_{\epsilon}(y_i - f(x_i)) + \frac{\lambda}{2} \| \omega \|^2.
%\label{Eq:svr_alternative_min_fct}
%\end{equation}
%
%\noindent The parameter $\lambda > 0$ is a so-called regularization constant. Then, minimizing (\ref{Eq:svr_alternative_min_fct}) with $\lambda = 1/(C n)$ results in the same parameter estimates as solving the minimization problem in (\ref{svr_opt_fct}). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Modifications of the SV Regression Scheme}
%
%Many modifications of the SVR approach have been suggested. \cite{Smola.2004} mention two popular examples, i.e. SVR using linear programming and an approach that automatically adjusts the $\epsilon$-tube. 
%\paragraph{SVR and Linear Programming} 
%
%\noindent In the linear programming approach the regularization term in (\ref{Eq:svr_alternative_min_fct}) is replaced. This results in the following regularized risk functional
%
%\begin{equation}
%\mathcal{R}_{reg}(f) = \mathcal{R}_{emp}(f) + \lambda \sum_{i= 1}^{n} |\rho_i|
%\label{risk_svr_linear_programm}
%\end{equation}
%
%\noindent where $\rho_i$ relates to the corresponding SV expansion of (\ref{risk_svr_linear_programm}): 
%
%\begin{equation}
%f(x) = \sum_{i = 1}^{n} \rho_i k(x_i, x) + b.
%\end{equation}
%
%
% \noindent In case of an $\epsilon$-insensitive loss function (\ref{risk_svr_linear_programm}) results in a linear programming problem. Hence, it leads also to a computational advantage. However, other loss functions will not necessarily have the same advantage. \cite{Smola.2004} show that using the dualization method to minimize (\ref{risk_svr_linear_programm}) does not decrease the computational effort. The direct minimization of (\ref{risk_svr_linear_programm}) with linear optimizers is, therefore, the appropriate approach here.
%
%\paragraph{SVR with Automatized Tube Adjustment}
%
%In standard SVR, the loss function is an $\epsilon$-insensitive loss function where $\epsilon$ needs to be set manually. Thus, additionally to balancing out the trade-off between capacity and empirical risk, regression with the SV method requires to choose an adequate loss function as well. An automated adjustment of $\epsilon$ can be achieved by adding it to the risk function in (\ref{Eq:svr_alternative_min_fct}). This leads to the following risk functional that is to be minimized:
%
%\begin{equation}
%\mathcal{R}_\gamma(f) = \mathcal{R}_{emp}(f) + \dfrac{\lambda}{2}\|\omega\|^2 + \gamma \epsilon.
%\label{risk_svr_nu_reg}
%\end{equation}
%\newline
%By setting the restriction $\gamma > 0$, $\epsilon$ will be minimized. Using (\ref{risk_svr_nu_reg}) as an objective function leads asymptotically to a predetermined number of SVs. Based on (\ref{risk_svr_nu_reg}), the constrained optimization problem becomes
%
%\begin{equation}
%\begin{aligned}
%& \text{minimize} & & \frac{1}{2} \|\omega\|^2 + C\left(\sum_{i = 1}^{n}(\zeta_i + \zeta^{*}_i) + n \gamma \epsilon \right)  \\
%& \text{subject to} & &  \begin{cases}
%y_i - \omega' x_i - b \le \epsilon + \zeta_i \\
%\omega'x_i + b - y_i \le \epsilon + \zeta_i^{*} \\
%\zeta_i, \zeta_i^{*} \ge 0.
%\end{cases} 
%\end{aligned}
%\label{nu_svr_opt_fct}
%\end{equation}
%\newline
%\noindent Here, the relationship between $C$, $n$ and $\lambda$ stated in Section \ref{Sec:svr_ito_risk} was used to state a optimization problem similar to (\ref{dual_nonlin_opt}). Assuming the same loss function as in (\ref{svr_opt_fct}), the dual formulation of (\ref{nu_svr_opt_fct}) is 
%
%\begin{equation}
%\begin{aligned}
%& \text{maximize} && 
%-\frac{1}{2}\sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)k(x_i,x_j) 
%+ \sum_{i = 1}^{n} y_i (\rho_i - \rho_i^*) 
% \\
%& \text{subject to} && \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
%\sum_{i = 1}^{n} (\rho_i - \rho_i^*) \le C \gamma n\\
%\rho_i, \rho_i^* \in [0, C].
%\end{cases}
%\end{aligned}
%\label{dual_nu_svr_opt}
%\end{equation}
%\newline
%\noindent \cite{Smola.2004} point out that (\ref{dual_nu_svr_opt}) is similar to the dual formulation of the standard SVR in (\ref{dual_lin_opt}) and (\ref{dual_nonlin_opt}). Equation (\ref{dual_nu_svr_opt}) has one more constraint but the objective function is homogeneous and, therefore, simpler. Moreover, they show how an optimal $\gamma$ can be determined.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{The SV Algorithm at a Glance}
%
%In the last sections the SV algorithm for doing regression was derived. Figure~\ref{svm_algo} summarizes how the SV algorithm creates a regression machine from input data. At first, a mapping $\Theta$ is applied to the data contained in the test vector and the SVs. After mapping both into the feature space, dot products are computed which is equal to evaluating a kernel $k$. As given by (\ref{sv_exp_nonlin}), the last step is to multiply the evaluated kernels with weights $\nu_i = (\rho_i - \rho_i^*)$ and add $b$.  \\
%
%\begin{figure}[h!]
%\centering
%\includegraphics[scale = 0.4]{Figures/svm_algo_correct}
%\caption[The SVR architecture]{A visualization of a SV based regression machine. Source: \cite{Smola.2004}.}
%\label{svm_algo}
%\end{figure}
%
%\noindent \cite{Smola.2004} note that regression with NNs is similar to the SV approach. However, they differ with respect to the input data. Due to the $\epsilon$-insensitive loss function, only a subset of the training data is used in the SV algorithm. In contrast, NNs use different loss functions that do not exclude observations. Hence, the function that is estimated by the SV algorithm does not depend on the observations that are not SVs. Despite this redundancy, it is not advisable to exclude these observations to reduce the memory needed to store it. For instance, \cite{Smola.2004} note that this can cause difficulties when handling high-dimensional or noisy data. 
%
%
%
% 
%
%



==> source code Version for upload/Sections/svrSL.tex <==
\subsection{Support Vector Regression} \label{Sec:meths_svr}
SVR can be understood as a learning method to solve nonlinear regression tasks  \cite[e.g.,][]{Smola.2004}. It shares some similarities with a three-layer feed-forward NN and is able to approximate arbitrarily complex functions \citep{Chen.2009}. However, NNs are based on minimizing the so-called empirical risk and tend to find only locally optimal solutions. In contrast, SVR minimizes the so-called structural risk to achieve better generalization and solves a convex optimization problem leading to a globally optimal solution.
To describe the SVR model, let $\{(y_i, x_i)| i = 1,\dots, n; \ n\in \mathbb{N}\}$ with $x_i \in \mathbb{R}^p$ and $y_i \in \mathbb{R}$ denote the training data set. Suppose $f$ is a linear function such that 

\begin{equation}
f(x) = \omega^\top x + b
\label{Eq:svr_lin_base_mdl}
\end{equation}

\noindent where  $\omega \in \mathbb{R}^p$ and $b \in \mathbb{R}$. Then, SVR aims to find an approximation of $f$ that deviates at most by $\epsilon$ from the observed target $y$ while being as flat as possible (i.e., in the sense that weights in $\omega$ are small). This translates into the following convex optimization problem:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 \\
& \text{subject to} & & \begin{cases}
y_i - \omega^\top x_i - b \le \epsilon  \\
\omega^\top x_i + b - y_i \le \epsilon.
\end{cases} 
\end{aligned}
\label{svm_mean_eq}
\end{equation}
\newline
In view that (\ref{svm_mean_eq}) might lack a feasible solution, \cite{Vapnik.1995} introduces an $\epsilon$-insensitive loss function: 

\begin{equation}
L_{\epsilon}\left\{y - f(x)\right\}  = \begin{cases}
0 \qquad \qquad \qquad  \text{if} \ |y - f(x)| \le \epsilon \\
|y - f(x)| - \epsilon \ \ \text{otherwise}.
\end{cases}
\label{Eq:svr_alt_loss_fct}
\end{equation}

To measure empirical loss (and thus model fit) using (\ref{Eq:svr_alt_loss_fct}) \cite{Vapnik.1995} reformulates (\ref{svm_mean_eq}) using slack variables $\zeta$ and $\zeta^{*}$ that capture losses above and below the $\epsilon$-tube around $f(x)$, respectively. Figure~\ref{loss_fct} depicts this approach. Only points outside the gray shaded $\epsilon$-tube contribute linearly to the loss function. \\ 

\begin{figure}[h!]
	\centering
	\includegraphics[scale = 0.4]{Figures/svm_loss_fct_correct}
	\caption[The $\epsilon$-insensitive loss function]{The $\epsilon$-insensitive loss function of the SVR algorithm. Slack variable $\zeta$ captures the loss above the $\epsilon$-tube. Points within the grey shaded area have no impact on the loss. In contrast, all other observations contribute linearly to the loss. Source: \cite{Smola.2004}.}
	\label{loss_fct}
\end{figure}


Integrating the slack variables $\zeta$ and $\zeta^*$ into (\ref{svm_mean_eq}), the task to estimate a SVR model is equivalent to solving:

\begin{equation}
\begin{aligned}
& \text{minimize} & & \frac{1}{2} \|\omega\|^2 + C\sum_{i = 1}^{n}(\zeta_i + \zeta^{*}_i) \\
& \text{subject to} & &  \begin{cases}
y_i - \omega^\top x_i - b \le \epsilon + \zeta_i \\
\omega^\top x_i + b - y_i \le \epsilon + \zeta_i^{*} \\
\zeta_i, \zeta_i^{*} \ge 0,
\end{cases} 
\end{aligned}
\label{svr_opt_fct}
\end{equation}
where $C > 0$ is a regularization parameter to balance between model fit and complexity \citep[e.g.,][]{Hastie.2009}. Larger (smaller) values of $C$ put more (less) weight on maximizing model fit during SVR learning. 
 
To capture nonlinear relationships between covariates and the response variable, SVR maps the input data into a higher dimensional feature space. The linear regression is then constructed in the transformed space, which corresponds to a nonlinear regression in the input space. The transformation is feasible from a computational point of view because SVR calculates the mapping by implicitly using a kernel function 
$k(x_i^\top x)=\phi^\top(x_i) \phi(x)$. To implement this approach, it is common practice to estimate a SVR model through solving the dual of (\ref{svr_opt_fct}), which is given as \citep[e.g.,][]{Smola.2004}:

\begin{equation}
\begin{aligned}
& \text{maximize} 
	-\dfrac{1}{2} \sum_{i,j = 1}^{n}(\rho_i - \rho_i^*)(\rho_j - \rho_j^*)x_i^\top x_j 
	-\epsilon\sum_{i = 1}^{n}(\rho_i + \rho_i^*) + \sum_{i = 1}^{n}y_i(\rho_i - \rho_i^*)
 \\
& \text{subject to}  \begin{cases} \sum_{i = 1}^{n} (\rho_i - \rho_i^*) = 0\\
	\rho_i, \rho_i^* \in [0, C].
	\end{cases}
\end{aligned}
\label{dual_lin_opt}
\end{equation}
\newline
The dual program (\ref{dual_lin_opt}) includes the input data only in the form of scalar products $x_i^\top x_j$. Replacing the scalar product by means of a kernel function is thus straightforward and does not affect the solver. In this work, we employ the Gaussian radial basis function (RBF) kernel (\ref{rbf_kernel}) which is defined as
\begin{equation}
\begin{aligned}
k(x_i^\top x)= \exp \left(-\dfrac{\| x - x_i \|^2}{2 \gamma^2} \right)
\end{aligned}
\label{rbf_kernel}
\end{equation}
where the meta-parameter $\gamma>0$ governs the width of the Gaussian function and needs to be set by the modeler. The RBF kernel is used because it includes other kernels as special cases, possesses numerical advantages compared to alternatives, and often performs well in practical applications. Moreover, the RBF kernel can capture nonlinear relations. Other kernels that are usually presented as potential choices are e.g. the linear, polynomial or sigmoid kernel \citep[e.g.,][]{Smola.2004,Hastie.2009}. \cite{Keerthi.2003} show that the linear kernel is a special case of the RBF kernel. Moreover, the polynomial kernel has more parameters than the RBF kernel that make the tuning process more costly. Another advantage of the RBF over the polynomial kernel is that the polynomial kernel can converge to infinity which can cause numerical instability. In contrast, the domain of the RBF kernel is always between 0 and 1. Moreover, \cite{Lin.2003} show that the sigmoid kernel behaves similar to the RBF kernel for certain parameters.

In order to construct the regression function (\ref{Eq:svr_lin_base_mdl}), the weight vector $\omega$ is represented as a linear combination of observations in the training set:

\begin{equation}
\omega = \sum_{i = 1}^{n} (\rho_i - \rho_i^*)x_i.
\label{Eq:weight_lin_svr}
\end{equation}
\newline

More specifically, for observations $x_i$ where $f(x_i)$ is within the $\epsilon$-tube holds that  $\rho_i = \rho_i^* = 0$. Consequently, $f(x)$ depends only on the observations outside the $\epsilon$-tube. These $x_i$ are called support vectors. Accordingly, (\ref{Eq:weight_lin_svr}) is also called the support vector expansion of $\omega$. Rewriting the regression function in terms of the support vector expansion gives the SVR forecasting model:

\begin{equation}
f(x) = \sum_{i = 1}^{n}(\rho_i - \rho_i^*)x_i^\top x + b.  
\label{sv_exp_lin}
\end{equation}
\newline

\noindent In the nonlinear case, the scalar product in (\ref{sv_exp_lin}) is once again replaced by a kernel function.

==> source code Version for upload/Sections/svrgarchkde.tex <==
\subsection{SVR-GARCH-KDE Hybrid}\label{Sec:SVRGARCHKDE}
In the following section, we introduce a nonlinear GARCH hybrid to forecast VaR based on a combination of SVR and KDE. Subsequently, we elaborate on the estimation of the corresponding forecasting model. 
%\subsubsection{Derivation of the SVR-GARCH-KDE Hybrid}

%In the following a nonparametric and nonlinear GARCH hybrid to forecast VaR based on a combination of SVR and KDE is introduced. In equation (\ref{Eq:garch_arma2}) it was shown that GARCH processes can be given an ARMA representation. 

%Recall the formulation for a return series $r_t$ where the mean equation is described by an AR(1) process and the variance equation by a GARCH(1,1) process:
%
%%\begin{align}
%%r_t &= c + \alpha r_{t-1} + \epsilon_t, \qquad \epsilon_t \sim N(0, \sigma_t^2) \\
%%\sigma_t^2 &= \omega + \beta \sigma_{t-1}^2 + \delta \epsilon_{t-1}^2. \label{Eq:GARCH_11}
%%\end{align}
%%
%%\noindent Since the conditional expectation of $\epsilon_t^2$ is $\sigma_t^2$, the conditional variance in GARCH models can be modeled via an ARMA process \citep{Chen.2009}. \cite{Poo.2003} derived the ARMA representation for the general GARCH($p$,$q$) case. For the GARCH(1,1) model in (\ref{Eq:GARCH_11}) let $\nu_t = \epsilon^2_t - \sigma^2_t$ and replace $\sigma^2_t$ with $\epsilon_t^2 - \nu_t$ to obtain 
%%
%%\begin{equation}
%%\epsilon_t^2 - \nu_t = \omega + \beta (\epsilon_{t-1}^2 - \nu_{t-1}) + \delta \epsilon_{t-1}^2.
%%\label{garch_re1}
%%\end{equation}
%%
%%\noindent Rewriting (\ref{garch_re1}) in the form of an ARMA(1,1) process for $\epsilon_t^2$ results in 
%%
%%\begin{equation}
%%	u_t^2  = \omega + \sum_{i = 1}^{\max(p,q)} (\beta_i + \delta_i) u_{t-i}^2 - \sum_{j = 1}^{q} \beta_j \nu_{t-j} + \nu_t , \quad \nu_t \sim WN(0,u_t)
%%%\epsilon_t^2  = \omega + (\beta + \delta) \epsilon_{t-1}^2 - \beta \nu_{t-1} + \nu_t.
%%\label{garch_re2}
%%\end{equation}

We assume the distribution of the return series $r_t$ to belong to the location-scale class, such that:

\begin{equation}
r_t = \mu_t + u_t = \mu_t + \sigma_t z_t, \qquad z_t \sim (0,1) \ \text{i.i.d.}
\label{Eq:hybrid_locs}
\end{equation}

%\noindent \cite{Engle.1982} and \cite{Bollerslev.1986} assumed a parametric mean model with linear structure. Based on this, they derived ARCH and GARCH processes that are also linear and parametric. In addition, the proposed estimation procedures rely on MLE and therefore distributional assumptions. To overcome the restrictions of a linear parametric structure with distributional assumptions, a nonparametric and nonlinear GARCH hybrid to forecast VaR based on a combination of SVR and KDE is introduced. \\  

\noindent Consider an ARMA structure for the mean model where the only assumption  about the error distribution is a zero mean and a finite variance. In addition, recall equation (\ref{Eq:garch_arma2}), which shows that GARCH processes can also be given an ARMA representation. This leads to the following mean and variance model:
\begin{align}
r_t &= c + \sum_{i = 1}^{s} \alpha_i r_{t-i} + \sum_{j = 1}^{d} \kappa_j u_{t-j} + u_t, \quad u_t \sim (0, \sigma_t^2) \\
u_t^2 &=\omega + \sum_{i = 1}^{\max(p,q)} (\delta_i + \beta_i) u_{t-i}^2 - \sum_{j = 1}^{p} \beta_j \nu_{t-j} + \nu_t.
\end{align}


\noindent Let $e = \max(p,q)$, $\mathbf{r}_{t,s} = (r_{t-1}, r_{t-2}, \dots, r_{t-s})$, $\mathbf{u}_{t,k} = (u_{t-1}, u_{t-2}, \dots, u_{t-k})$ and 
$\boldsymbol{\nu}_{t,p} = (\nu_{t-1}, \nu_{t-2}, \dots, \nu_{t-p})$. Then,  following \cite{Chen.2009}, we introduce the nonlinear and nonparametric functions $h$ and $g$ such that the conditional mean and variance models of $r_t$ are

\begin{align}
r_t &= h(\mathbf{r_{t,s}}, \mathbf{u_{t,d}}) + u_t \qquad u_t \sim (0, \sigma_t^2) \label{Eq:garch_mean_no_dis}\\
u_t^2 &= g(\mathbf{u_{t,e}}, \boldsymbol{\nu_{t,p}}) +  \nu_{t} \qquad \nu_t \sim WN(0,a_t^2)\label{Eq:garch_var_no_dis}
\end{align}

%\noindent 
%Section \ref{Sec:NDE} was motivated by research showing time varying structures for stock return distribution regarding the first four moments. In order to obtain more flexibility in the estimation of VaR $\epsilon_t$ is replaced with $\epsilon_t^* \sim (0,  \sigma_t^2)$ such that no distributional assumption about the error term are made. Assuming zero mean and finite variance . This results in 
%\begin{align}
%r_t &= f(r_{t-1}) + \epsilon_t^* \qquad \epsilon_t^* \sim (0, \sigma_t^2)  \label{Eq:garch_mean_no_dis}\\
%\epsilon_t^{*2} &= g(\epsilon_{t-1}^{*2}, \nu_{t-1}^*) +  \nu_{t}^* \qquad \nu_t^* \sim WN(0,u_t). \label{Eq:garch_var_no_dis}
%\end{align}

\noindent where $ WN(0,a_t^2)$ denotes white noise with expectation zero and variance $a_t^2$. We propose to estimate $h(\cdot)$ and $g(\cdot)$ using SVR. The estimates for $\mu_t$ and $\sigma_t$ in (\ref{Eq:hybrid_locs}) are then obtained as:

\begin{align}
\widehat{\mu}_t &= h(\mathbf{r_{t,s}}, \mathbf{u_{t,d}}) \label{Eq:svr_mean_estimate} \\
\widehat{\sigma}_t &= \sqrt{g(\mathbf{u_{t,e}}, \boldsymbol{\nu_{t,p}})}.
\end{align}

\noindent By defining the estimated residuals as $\widehat{u}_t = r_t - \widehat{\mu}_t$, estimates of $z_t$ are obtained as
\begin{equation}
\widehat{z}_t = \dfrac{\widehat{u}_t}{\widehat{\sigma}_t}.
\label{Eq:standardizes_residuals}
\end{equation}


% However, $\widehat{z}_t$ has not necessarily have zero mean and unit variance. Hence, the quantile estimation will be done using scaled standardized residuals $\widehat{z}_t^*$:
%%
%\begin{equation}
%\widehat{z}_t^* = \dfrac{\widehat{z}_t - \overline{\widehat{z}_t}}{\sqrt{\frac{1}{n-1}\sum_{i = 1}^{T}  (\widehat{z}_t - \overline{\widehat{z}_t})^2  }}
%\end{equation}
%
%\noindent where $\overline{\widehat{z}_t}$ denotes the empirical mean of $\widehat{z}_t$.  
\noindent Then, for $\widehat{Q}_{\widehat{z}}(\alpha)$ being the estimated quantile function of $z$, the VaR estimate for $r_t$ is:

\begin{equation}
\widehat{VaR}_t^\alpha = - \left\{ h(\mathbf{r_{t,s}}, \mathbf{u_{t,d}}) +\sqrt{g(\mathbf{u_{t,e}}, \boldsymbol{\nu_{t,p}})} \widehat{Q}_{\widehat{z}}(\alpha) \right\}.
\label{Eq:nonlin_var}
\end{equation}

\noindent whereby we estimate $\widehat{Q}_{\widehat{z}}(\alpha)$ using KDE.
%\noindent Then, in the SVR-GARCH-KDE hybrid approach, the estimation of $f(\cdot)$ and $g(\cdot)$ is done via SVR and $Q_{\widehat{z}_t}(\alpha)$ is obtained through KDE.
%\subsubsection{Estimating the SVR-GARCH-KDE Hybrid}

We now present a procedure to estimate VaR as in (\ref{Eq:nonlin_var}) and describe it in the context of producing one-day-ahead VaR forecasts. A step-by-step overview is given in Algorithm \ref{Algo:svr-garch-kde_algo}. Let $\{r_t\}_{t = 1}^T$ be the training set consisting of the daily returns from a portfolio where $r_T$ is the most recent observation. In the first step, we model the mean process (\ref{Eq:garch_mean_no_dis}). To do this, we estimate an AR($s$) model using SVR to obtain the estimated returns $\{\widehat{r}_t\}_{t = 1+s}^T$. The set of estimated residuals $\{\widehat{u}_t\}_{t = 1 + s}^T$ is derived as $\widehat{u}_t = r_t - \widehat{r}_t$. Then, a moving average (MA) part can be introduced to the model such that $r_t$ can be modeled as an ARMA($s$,$d$) process by running SVR and including $\widehat{u}_t$. The sets of estimated returns and residuals from the ARMA($s$,$d$) model are denoted as $\{\widehat{r}_t^*\}_{t = 1 + s + d}^T$ and $\{\widehat{u}_t^*\}_{t = 1 + s + d}^T$ , respectively.

 We also estimate the variance process in a two step approach and start by fitting the squared mean model residuals $\{\widehat{u}_t^{*2}\}_{t = 1 + s +d}^T$ in the way of an AR($e$) process with SVR. Based on this, fitted variances $\{\widehat{\sigma}_t^2\}_{t = 1 + s+d +e}^T$ are obtained. Then, an ARMA model for (\ref{Eq:garch_var_no_dis}) is obtained in the same way as for the mean process by using the estimated model residuals $\{\widehat{\nu}_t\}_{t = 1 + s + d + e}^T$ where $\widehat{\nu}_t = \widehat{u}_t^{*2} - \widehat{\sigma}_t^2$. Consequently, the final set of fitted variances is denoted as $\{\widehat{\sigma}_t^{*2}\}_{t = 1 + s +d+e+p}^T$. No assumptions are made about the starting values of the residuals. Hence, the final estimation of (\ref{Eq:garch_var_no_dis}) is done using data for $T-s-d-e-p$ time points. Since SVR is applied without introducing further restrictions, it is not ensured that $\widehat{\sigma}_t^2$ and $\widehat{\sigma}_t^{*2}$ are positive. Therefore, if the SVR estimate is $\widehat{\sigma}_t^{\left(*\right)2} \le 0$, it will be replaced by the last positive estimated variance. In case the first fitted variance is negative, it will be replaced by the first squared residual from the final mean model. 

The set of estimated standardized residuals $\{\widehat{z}_t\}_{t = 1 + s +d+e+p}^T$ can be computed by applying (\ref{Eq:standardizes_residuals}). However, $\widehat{z}_t$ does not necessarily have zero mean and unit variance. Hence, we perform the quantile estimation using scaled standardized residuals $\widehat{z}_t^*$:

\begin{equation}
\widehat{z}_t^* = \dfrac{\widehat{z}_t - \overline{\widehat{z}_t}}{\sqrt{\frac{1}{T-1}\sum_{i = 1}^{T}  (\widehat{z}_t - \overline{\widehat{z}_t})^2  }}
\end{equation}

\noindent where $\overline{\widehat{z}_t}$ denotes the empirical mean of $\widehat{z}_t$. The forecasted mean $\widehat{\mu}_{T+1}$ and standard deviation $\widehat{\sigma}_{T+1}$ are obtained from the mean and variance model. Finally, we use KDE to estimate the $\alpha$-quantile of $\{\widehat{z}^*_t\}_{t = 1 + s + d+e+p}^T$. Then, the one-day-ahead VaR forecast is: 

%-----------------------------------------------------------------\\
% is estimated by SVR such that the estimates $\widehat{r}_t$ and $\widehat{\epsilon}_t^* = r_t - \widehat{r}_t$ are obtained for $r_t$ and $\epsilon_t^*$, respectively. The variance process is estimated by a two step procedure. Since $\nu_{t-1}^*$ is not available the estimation of (\ref{Eq:garch_var_no_dis}) starts by fitting the series $\{\widehat{\epsilon}_t^*: t = 2, \dots, T\}$ in the way of an AR(1) process with SVR. Then, an ARMA model for (\ref{Eq:garch_var_no_dis}) is obtained by using the estimated model residuals $\{\widehat{\nu}_t^*: t = 3, \dots, T\}$. Note that no assumptions are made about the starting values of the residuals. Hence, the final estimation of (\ref{Eq:garch_var_no_dis}) is done by using data for $T-3$ time points. Denote ${\{\widehat{\sigma}_t^2: t = 3, \dots, T\}}$ as set of estimated variances. Since the SVR is done without introducing further restrictions it is not ensured that $\widehat{\sigma}_t^2 > 0$. Therefore, if the SVR estimate is $\widehat{\sigma}_t^2 \le 0$, it will be replaced by $\widehat{\sigma}_{t-1}^2$. In order to obtain the set of estimated standardized residuals $\widehat{z}_t$ divide $\widehat{\epsilon}_t$ by $\widehat{\sigma}_t$. Theoretically holds that $z_t \sim (0, 1)$. This is not ensured in practical applications. To ensure that (\ref{Eq:nonlin_var}) holds $\widehat{z}_t$ will be standardized to zero mean and unit variance. The one-day ahead VaR forecast is then obtained by

\begin{equation}
\widehat{VaR}_{T+1}^\alpha = -[ \widehat{\mu}_{T+1} + \widehat{\sigma}_{T+1} \widehat{Q}_{\widehat{z}^*} (\alpha)].
\label{Eq:var_est_svrkde}
\end{equation}

An important aspect to note is that SVR and KDE depend on hyperparameters which cannot be derived analytically but must be found computationally. Therefore, the above described estimation procedure describes the estimation process only for one fixed set of hyperparameters. The hyperparameters for SVR given a RBF kernel is used are $\epsilon$, $\gamma$ and $C$. Additionally, if the SVR kernel is not set beforehand, it can be seen as hyperparameter itself. In the context of KDE the bandwidth $h$ and the KDE specific kernel function $K$ are hyperparameters. Since the goal is to train an efficient model on a purely data driven basis it is advisable to derive the hyperparameters computationally. However, for some hyperparameters exist theoretical results that support fixing them beforehand. As stated in Section \ref{Sec:meths_svr} the RBF kernel is a reasonable choice in SVR. Moreover, for KDE the kernel choice has only a low practical relevance and there exist rule-of-thumb estimators for $h$ when a Gaussian kernel  is used which are computationally inexpensive \citep{Hardle.2004, Silverman.1986}. Hence, the most relevant aspect in hyperparameter tuning of the SVR-GARCH-KDE hybrid are $\epsilon$, $\gamma$ and $C$ for the SVR with a RBF kernel. It is important to note that the overall goal is to forecast VaR. Hence, the hyperparameters should be set with respect to the measure that is used to evaluate quantile forecasts. There exist different approaches as grid search, random search or more advanced optimization strategies that can be used to automate the process of hyperparameter optimization.

%
%\noindent where $F_{\widehat{z_t}}^{-1}$ is obtained based on the nonparametric density estimation with KDE for $\widehat{z_t}$. 

%\renewcommand{\thealgorithm}{}
%\begin{algorithm*}
%	\caption{SV-GRACH-KDE Algorithm for forecasting VaR}
%	\begin{algorithmic}[1]
%	\State Estimate an AR(1) model for $\{r_t: t = 1, \dots, T\}$ using SVR
%	\State Compute the model residuals from Step 1 $\{\widehat{\epsilon}_t: t = 1, \dots, T\}$
%	\State Estimate an AR(1) model for $\{\widehat{\epsilon}_t^2: t = 1, \dots, T\}$ using SVR
%	\State Compute the model residuals from Step 3 $\{\widehat{\nu}_t: t = 2, \dots, T\}$
%	\State Reestimate the model in Step 3 as ARMA(1,1) by introducing $\{\widehat{\nu}_t: t = 2, \dots, T\}$
%	\State Obtain the set of estimated variances $\{\widehat{\sigma}_t^2: t = 3, \dots, T\}$ from Step 5
%	\State Compute the standardized residuals $z_t = \widehat{\epsilon}_t / \widehat{\sigma}_t$ for $t = 3, \dots, T$
%	\State Normalize $\widehat{z}_t$ to zero mean and unit variance
%	\State Estimate the $\alpha$-quantile $F_{\widehat{z_t}}^{-1}(\alpha)$ with KDE
%	\State Obtain $\widehat{r}_{T+1}$ and $\widehat{\sigma}_{T+1}$ by using the models from Step 1 and 5
%	\State Compute the VaR forecast as $VaR_{T+1}^\alpha = \widehat{r}_{T+1} + \widehat{\sigma}_{T+1} F_{\widehat{z_t}}^{-1} (\alpha)$
%	\end{algorithmic}
%\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%Moved to appendix%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Choose whether to move algorithm to appendix
%\iffalse
\begin{algorithm}
	\caption{SVR-GRACH-KDE Estimation Algorithm for Forecasting VaR}
	\label{Algo:svr-garch-kde_algo}
	\begin{algorithmic}[1]
		
		\State AR($s$) model for $\{r_t\}_{t=1}^T$ using SVR
		\vspace{0.1cm}
		\State Get errors from Step 1 $\{\widehat{u}\}_{t=1+s}^T$
		\vspace{0.1cm}
		\State ARMA($s$,$d$) model for $\{r_t\}_{t=1+s}^T$ with results from Step 2 using SVR
		\vspace{0.1cm}
		\State Get errors from Step 3 $\{\widehat{u}^*\}_{t=1+s+d}^T$
		\vspace{0.1cm}
		\State AR($e$) model for $\{\widehat{u}_t^{*2}\}_{t=1+s+d}^T$ using SVR
		\vspace{0.1cm}
		\State Get errors from Step 5 $\{\widehat{\nu}_t\}_{t=1+s+d+e}^T$
		\vspace{0.1cm}
		\State ARMA($e$,$p$) model for $\{\widehat{u}_t^{*2}\}_{t=1+s+d+e}^T$  with results from Step 6 using SVR
		\vspace{0.1cm}
		\State Obtain volatility estimates $\{\widehat{\sigma}^*\}_{t=1+s+d+e+p}^T$ from Step 7
		\vspace{0.1cm}
		\State Get standardized residuals $\widehat{z}_t = \widehat{u}_t^* / \widehat{\sigma}_t$ for $t = 1+s+d+e+p, \dots, T$
		\vspace{0.1cm}
		\State Scale $\{\widehat{z_t}\}_{t=1+s+d+e+p}^T$ to zero mean and unit variance and obtain $\{\widehat{z}_t^*\}_{t=1+s+d+e+p}^T$
		\vspace{0.1cm}
		\State Estimate the $\alpha$-quantile $\widehat{Q}_{\widehat{z}^*}(\alpha)$ with KDE
		\vspace{0.1cm}
		\State Obtain $\widehat{r}_{T+1}$ and $\widehat{\sigma}_{T+1}$ by using the models from Step 3 and 7
		\vspace{0.1cm}
		\State VaR forecast: $\widehat{VaR}_{T+1}^\alpha = -[ \widehat{\mu}_{T+1} + \widehat{\sigma}_{T+1} \widehat{Q}_{\widehat{z}^*} (\alpha)]$
		
		
	\end{algorithmic}
\end{algorithm}
%\fi

After defining the SVR-GARCH-KDE hybrid the question arises how model complexity, predictive power and the computational time for making VaR forecasts are related. Regarding the time to compute predictions the KDE part is fixed beforehand. This is can be seen in Equation \ref{Eq:kde_definition} and Algorithm \ref{Algo:svr-garch-kde_algo}. In order to compute an estimate the sum needs to be evaluated making the computational complexity $O(n)$ where $n$ is number of observations. Regarding the SVR-GARCH-KDE hybrid the computational complexity of the KDE part is reduced depending on the order of the autoregressive and moving-average part of the mean and variance process to $O(n-s-d-e-p)$. With respect to SVR the complexity of making a prediction is $O(n_{SV} d)$, where $d$ is the dimension of the feature space and $n_{SV}$ the number of SVs. For the proposed application of forecasting the mean and variance of a financial time series the number of features is usually low. Therefore, the computational time for generating predictions is mainly driven by the sample size and negligible in this application.
	
Regarding the predictive performance, the regression function of the mean and variance process is determined by the SVs which implies that the higher the number of SVs, the higher the complexity. Using a SVR decision function with a high number of SVs can, therefore, lead to a mediocre out-of-sample performance. However, it is not possible to make an ex ante exact statement since the Vapnik-Chervonenkis dimension of the RBF kernel is infinite \citep{Burges.1998}. %Hence, the generalization error which is the bound for the actual risk is also infinite. 
Moreover, the goal of the SVR-GARCH-KDE hybrid is to forecast quantiles. Evaluating the performance ex ante does, therefore, depend on the measure that is used to evaluate forecasted quantiles rather than the statistical properties of KDE and potential error bounds of SVR. In Section \ref{Sec:emp_study} the framework of \cite{Christoffersen.1998} will be applied. For achieving a good performance it is necessary to tune the parameters of the SVR and KDE part appropriately with respect to the target measure. Consequently, in this study the focus is put on the out-of-sample performance to optimize the quality of predictions and the hyperparameter tuning is done with a separate training set.


==> source code Version for upload/Sections/titlepage.tex <==
\begin{center}

	
	\LARGE \text{Humboldt-Universit{\"a}t zu Berlin} 
	
\vspace{0.5cm}

	\begin{figure}[h]
		\centering
		\includegraphics{Figures/hulogo}
	\end{figure}

\vspace{-0.5cm}

    {\LARGE{\bf Data Driven Value-at-Risk Forecasting \\ \vspace{0.1cm} Using a SVR-GARCH-KDE Hybrid}} \vspace{0.5cm}

\vspace{0.5cm}
   
    {\large Master Thesis by: \\ \vspace{0.1cm} \LARGE Marius Lux (558415)}
               
    \vspace{0.2cm}

\large

\begin{align*}
\text{First Supervisor:}& \text{ Prof. Dr. Stefan Lessmann} \\
\text{Second Supervisor:}& \text{ Prof. Dr. Wolfgang K. H{\"a}rdle} \\
\end{align*}
\vspace{-1.5cm}
	
	\normalsize  School of Business and Economics \\
	Chair of Information Systems \\ Ladislaus von Bortkiewicz Chair of Statistics

 \vspace{0.8cm}
 
 \large
In partial fulfillment of the requirements \\ for the degree \\ {\bf Master of Science in Statistics} 

 \vspace{.8cm}
 
 \large Berlin, March 30, 2017

\end{center}


==> source code Version for upload/Sections/value_at_risk.tex <==
%\section{Value-at-Risk}\label{Sec:var}
%$\R$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Defining Value at Risk
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Defining Value-at-Risk}

%\cite{Jorion.2009} defines VaR as \textit{"the worst loss over a target horizon that will not be exceeded with a given level of confidence"}. Therefore, two parameters are essential for measuring VaR. First, the confidence level $ 1 - \alpha$ which corresponds to the probability that no loss larger than the VaR occurs in a given time horizon. Here, $\alpha$ is referred to as significance level. The second parameter is the time horizon $d$ which is usually measured in trading days. For instance, assume an investor who has a portfolio with a total value of $100.000\$$. He wants to know the next day's VaR for a confidence level of $95\%$. Further assume the next day's return is higher than $-2.5\%$ with a probability of $95\%$. Then, the portfolio's VaR for a confidence level of $95\%$ and time horizon of one trading day is $100.000\$ \cdot 0.025 = 2.500\$$. \newline

%\noindent In general, VaR can be derived from the portfolio's loss distribution. However, since today's portfolio value is usually known, it suffices to model the return distribution. Hence, by following \cite{Kuester.2005} for a formal description of VaR, let the portfolio returns be a random variable $X \in \mathbb{R}$ with cumulative distribution function $F$. Then, the VaR in $d$ trading days for a confidence level $1-\alpha$ is defined as

In general, VaR can be derived from the portfolio's $P\&L$ distribution. However, since today's portfolio value is usually known, it suffices to model the return distribution. For a formal description of VaR, let the portfolio returns $r_t$ in period $t$ have the cumulative distribution function (CDF) $F_t$. Then, the VaR in $d$ trading days for a confidence level $1-\alpha$ is defined as

\begin{equation}
VaR_{t+d}^\alpha = -F^{-1}_{t+d}(\alpha) = -\inf\{ x \in \mathbb{R}: F_{t+d}(x) \geq \alpha \} \quad \text{with} \quad \alpha \in (0,1) .
\end{equation}

\noindent In the rest of the paper, VaR refers to the negative $\alpha$-quantile of the next period's portfolio return distribution. %This is illustrated in Figure~\ref{var_illu}. 

%\noindent Hence, VaR is the negative $\alpha$-quantile of the next period's portfolio return distribution which is equivalent in saying that VaR indicates the next period's loss that will not be exceeded with a probability of 100(1-$\alpha$)$\%$. Figure~\ref{var_illu} illustrates the VaR concept. Estimating VaR requires the estimation of the loss distribution. However, the next period's loss is derived by multiplying today's portfolio value with the relative change of the portfolio in $h$ trading days. Today's portfolio value is usually known. Therefore, by assuming the portfolio value is known it suffices to estimate next period's distribution of relative portfolio changes. Then, VaR is derived by multiplying  today's portfolio value with the negative $\alpha$-quantile of the next period's portfolio return distribution. Therefore, in the rest of this thesis the use of the term VaR refers to the $\alpha$ quantile of the a portfolios return distribution.

%\begin{figure}[h]
%	\centering
%	\includegraphics{Figures/var-quantile-tails_TEST}
%	\caption{Illustration of VaR for a hypothetical portfolio return density function. Source: \cite{Alexander.2010}}
%	\label{var_illu}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% APPROACHES FOR ESTIMATING VAR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Approaches for Estimating VaR}
%
%The VaR forecasting model proposed in this thesis combines nonlinear function approximation via SVR and nonparametric density estimation by KDE. Since this work aims to compare machine learning methods as SVR in risk management, the proposed method will be compared to similar traditional statistical methods. However, already existing approaches to quantile regression in machine learning are described as well. So, the following two sections review methods to estimate quantiles that were proposed in the context of traditional statistics and machine learning, respectively. 

%\subsubsection{Approaches Related Related to Traditional Statistics}
\subsection{Estimating VaR Using Location-Scale Models} \label{Sec:var_est_approaches}

%\cite{Kuester.2005} compare the performance of several approaches for estimating VaR. Moreover, a comprehensive overview over existing statistical methods is given. Four categories are suggested to describe existing methods for VaR estimation. These categories are historical simulation, fully parametric models, extreme value theory and quantile regression. In this section, the above mentioned modeling approaches are introduced by closely following \cite{Kuester.2005}. 
%
%\paragraph{Historical Simulation} \cite{Kuester.2005} use the term historical simulation to refer to methods using empirical quantiles of historical return data. However, this approach has some drawbacks. First, returns are typically not independent and identically distributed (i.i.d.). Historical simulation does not account for this. Moreover, VaR predictions are bounded by the observed minimum of the return data. As a consequence, in moving window approaches the entering or dropping out of large extreme returns from the data set can cause jumps in VaR. Hence, modifications were proposed. For instance, the return data can be pre-filtered with location-scale models described in the next paragraph. Based on this, i.i.d. disturbances of the return series can be obtained. Then, the i.i.d. disturbances can be bootstrapped to overcome the shortcomings. \\

%\paragraph{Fully Parametric Models}

The proposed VaR modeling framework is based on the location-scale approach. Models of this class estimate the entire distribution of asset returns and derive VaR as a quantile of that distribution \citep[e.g.,][]{Kuester.2005}. Such approaches assume the return process is described as

\begin{equation}
	r_t = \mu_t + u_t = \mu_t + \sigma_t z_t, \qquad z_t \sim (0,1) \ \text{i.i.d.}
	\label{Eq:location_scale_model}
\end{equation}

In (\ref{Eq:location_scale_model}), $\mu_t$ is the location and $\sigma_t > 0$ the scale parameter. Given $r_t$ belongs to the location-scale family and $F_z$ is the CDF of $z$, we can compute VaR as
 
\begin{equation}
	VaR_{t}^{\alpha} = -\left\{\mu_t + \sigma_tF^{-1}_{z}(\alpha)\right\}.
	\label{Eq:location_scale_var}
\end{equation}

\noindent Autoregressive moving average (ARMA) processes and GARCH-type models are commonly used to estimate $\mu_t$ and $\sigma_t$ in (\ref{Eq:location_scale_model}).

%\newline
%\noindent Standard dynamic feedback models estimate the distribution of a stochastic process as discrete mixture of normal distributions. Moreover, volatility can be modeled using a GARCH model. Let $u_t$ be generated by a conditionally heteroscedastic mixture of normal distributions. Further, let $w \in (0,1)^n$, $\mu \in \mathbb{R}^n$ and $\sigma_t \in \mathbb{R}_{>0}$. Then, 
%\begin{equation}
%u_t|\mathcal{F}_{t-1} \sim MN(w, \mu, \sigma_t^2) ,
%\end{equation}
%where MN denotes a mixture of normal distributions with density function 
%\begin{equation}
%f_{MN}(x, w, \mu, \sigma_t^2) = \sum_{i = 1}^{n} w_i \varphi (x, \mu_i, \sigma_{it}^2).
%\end{equation}
%Here, $\varphi$ is the probability density function of the normal distribution with $\sum_{i = 1}^{n} w_i = 1$ and $\mathcal{F}_{t-1}$ being the information set available at $t-1$. \cite{Kuester.2005} note that also mixtures of other distributions can be used. For instance, in their study they use the generalized exponential distribution and refer to literature where the t distribution was considered. 

%Assuming an unconditional model in equivalent in setting $\mu_t = \mu$ and $\sigma_t = \sigma$. Conditionally homoscedastic models incorporate the possibility of a time-varying conditional mean. Autoregressive moving average (ARMA) processes are a possible modeling approach. However, return series of financial time series are subject to volatility clustering. Hence, applying conditionally heteroscedastic models with a time-varying location and scale parameter are the most promising ones for VaR predictions.

%\paragraph{Extreme Value Theory} Procedures for modeling the tails rather than the entire distribution are developed in extreme value theory. There are two main approaches: block maxima (BM) and peaks over threshold (POT) models. \\
%
%\noindent To introduce the BM model let $M_n = \max\{X_1, \dots, X_n\}$ with $X_t$, $t = 1, \dots, n$, being i.i.d. random variables. For $c_n > 0$, $d_n \in \mathbb{R}$ and $G$ being a non-degenerate distribution, it holds that 
%\begin{equation}
%	\dfrac{M_n - d_n}{c_n} \xrightarrow{d} G \qquad \text{for} \ n \rightarrow \infty,
%\end{equation}
%where $G$ is the generalized extreme value distribution. Hence, sample maxima have only one class of limiting distributions. Based on this, VaR can be derived. \\
%
%\noindent POT models estimate the excess distribution $F_{\tau}$ of a random variable $X$ based on values exceeding a threshold $\tau$. Formally, $F_{\tau}$ is defined as   
%\begin{equation}
%	F_{\tau}(x) = \mathbb{P}(X - \tau \le x | X > \tau), \qquad x \ge 0.
%	\label{Eq:pot_excess_dist}
%\end{equation}
%Under this setting, the limiting distribution of scaled excesses is the generalized Pareto distribution. 
%
%
%\paragraph{Quantile Regression} 
%The aforementioned methods are based on modeling either the entire distribution or its tail. In contrast, quantile regression aims at estimating the quantile directly without considering other parts of the distribution. Hence, the $\alpha$-quantile of a random variable is modeled directly in dependence of explanatory variables $x_t \in \mathbb{R}^p$:   
%\begin{equation}
%		VaR_t^{\alpha} = -h_{\alpha}(x_t, \beta_{\alpha}).
%\end{equation}
%Note that the function $h(\cdot, \cdot)$ and parameter vector $\beta$ are depending directly on $\alpha$.
%
%%\cite{Abberger.1997} Kernel based forecast compared to GARCH. Did not compare results based on tests for the appropriateness of distribution. However, he compared the difference and found asymmetries by comparing the first and third quartile forecast showing asymetries in the data that can not be captured by normal distribution. -> Massive deviation. 

%\subsubsection{Approaches Related to Machine Learning}
%\subsection{Related Literature}
%
%In the domain of ML the literature for quantile estimation focuses mainly on neural networks (NN) and SVR. For instance, the derivation of a general approach without an explicit target application can be found in \cite{White.1992}. He used single hidden layer feedforward NNs to derive a way for nonparametric conditional quantile estimation and proved its consistency. However, the ML VaR literature is not as broad as in classical statistics. 
%Hence, this section also reviews literature where methods for the construction of prediction intervals (PI) were introduced that could be used in the estimation of VaR. Consequently, the reviewed literature is divided in three paragraphs: Prediction Intervals, Value-at-Risk and Data Driven Value-at-Risk. Here, the first two review the existing literature, whereas the last motivates the method proposed in this thesis. 
%
%%Hence, the literature is reviewed explicitly and the section is divided in three paragraphs: prediction intervals (PI), VaR and Data Driven VaR. Whereas the first two review the existing literature, the last motivates the method proposed in this thesis. 
%
%\paragraph{Prediction Intervals} General approaches are developed by \cite{Hwang.1997} who derive asymptotically valid PIs and \cite{Veaux.1998} who propose a method to estimate PIs for NNs with nonlinear regression. \cite{LinWeng.2004} use SVR to generate out-of-sample residuals via cross validation (CV) and fit those to a Laplace or normal distribution for generating PIs. The results are compared to Bayesian SVR and historical simulation. Despite the mixed results they stress the competitiveness of their method especially due to its simplicity. Pointwise and simultaneous confidence intervals as well as PIs with bias correction for least-squares-SVR are derived by \cite{Brabanter.2011}.  %based on Sidak corrections and upcrossing allowing for heteroscedasticiy and modifying it because of its convervativity% - > 
%However, in comparison to bootstrapping, their method is not superior in simulations. \cite{Khosravi.2013} introduce a framework for constructing PIs of electricity prices. They employ a resampling scheme based on a moving bootstrap approach for data blocks rather than single observations to account for possible correlations. Then, NNs are trained on the bootstrapped data sets to forecast the mean of the time series as center of the prediction interval. The variance is estimated based on a GARCH model but not in the framework of MLE. Instead, they use a cost function directly related to the PI quality that can be minimized with gradient-free algorithms. The resulting mean and variance are then used in a normal distribution to get the PIs. They find that their method has a computational advantage over traditional methods. Moreover, the PIs of their approach are more informative. \cite{Lins.2015} propose a method for confidence intervals and PIs by combining bootstrapping and SVR to bagged SVR in the context of component degradation prediction in the offshore oil industry. They show that their method works in the proposed application.
%
%\paragraph{Value-at-Risk} \cite{Franke.2006} estimate VaR for the German stock index (DAX) by fitting the mean and volatility of the return series with NNs. The mean is modeled autoregressively and the volatility is assumed to follow an autoregressive conditionally heteroscedastic (ARCH) process. Moreover, they include external regressors in both models. The predicted mean and variance are used with the normal distribution to derive the VaR and expected shortfall. As benchmark serves a standard GARCH model based on assuming normality of innovations. In terms of VaR exceedances their model is superior. Moreover, they note its ability to quickly adjust the volatility in case of shocks with only short impact. Another approach directly related to VaR is proposed by \cite{Dunis.2010} which use higher order NNs to forecast VaR. A hybrid model using higher order NNs for variance forecasting and RiskMetrics is shown to outperform other hybrid models empirically. They note also the relatively bad results of the unconditional POT method for quantile estimation. This is, however, not an appropriate comparison when benchmarked to conditional models as was e.g. shown by \cite{Kuester.2005}. \cite{Khan.2011} propose a VaR-model where realized volatilities are forecasted in an ARCH like manner via a heterogeneous autoregressive (AR) model combined with SVR. VaR is then computed based on the normal, t and skewed t distribution. Their model is applied to 5- and 15-minutes return data and it is shown to be favorable over models not using SVR. \cite{Stankovic.2015} forecast VaR by a combination of volatility forecasting and historical simulation without describing their method in more detail. Their comparisons to VaR models based on Markov regime switching models and a multi-layer-perceptron found the SVR approach to be superior based on the Kupiec test. A multiperiod VaR model was introduced by \cite{Xu.2016}. They use an exponentially weighted support vector quantile regression. In the corresponding empirical study, their approach outperforms other methods that are based on GARCH models, filtered historical simulation and quantile regression. Evaluation was done with different measures as e.g. mean absolute error and p-values of prediction tests.
%  
%\paragraph{Data Driven Value-at-Risk} Two methods that do not rely on distributional assumptions for VaR estimation are proposed by \cite{Wu.2005}. These are based on SVR and NNs. By considering the model types in Section \ref{Sec:var_est_approaches}, they can be classified as quantile regression models. In the empirical study of  the paper, both models are superior in comparison to benchmarks as Monte Carlo simulations based on the normal, log-normal, logistic or extreme value distribution. However, in the broad study of \cite{Kuester.2005} hybrid location-scale models allowing for skewed and fat-tailed error distributions performed best. For instance, a combination of GARCH and POT had superior test statistics overall. In contrast, quantile regression based methods delivered relatively poor results. Most of the proposed methods in the ML literature for estimating VaR or PIs are location-scale models. However, only mean and variance are estimated. For the distribution of disturbances standard assumptions as normality are made. This contradicts the data driven nature of ML methods. In order to obtain a purely data driven location-scale VaR approach, a hybrid based on SVR and nonparametric density estimation is introduced in this thesis. Its performance will be evaluated with respect to GARCH-type models with different error distributions that include also skewed and fat-tailed distributions.
%

    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% EVALUATING VAR MODELS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%\subsection{Evaluating VaR-Models}
%
%\cite{Christoffersen.1998} proposes a framework for assessing interval forecasts and uses it for evaluating VaR models. This approach is also applied here. Let ${V_t = \mathbb{I}(r_t < -VaR_t^{\alpha})}$, with $t = 1, \dots, n$, be a series of VaR violations where $\mathbb{I}(x < c)$ denotes the indicator function:
%%Let $\{V_t\}_{t=1}^n$ be a series of VaR violations with $V_t = \mathbb{I}(r_t < -VaR_t^{\alpha})$ where $\mathbb{I}(x < c)$ denotes the indicator function: 
%\begin{equation}
%\mathbb{I}(x < c) = \begin{cases}
%1 \text{ \ if \ } x < c \\
%0 \text{ \ if \ } x \ge c. \\
%\end{cases} 
%\end{equation}
%
%\noindent Moreover, let $\mathcal{F}_{t-1}$ be the information set available at time ${t-1}$. Then, according to \cite{Christoffersen.1998} a VaR forecast model is efficient if
%
%\begin{equation}
%\mathbb{E}[V_t | \mathcal{F}_{t-1}] = \alpha.
%\label{Eq:chris_mdl_eff}
%\end{equation}
%
%\noindent \cite{Kuester.2005} note that (\ref{Eq:chris_mdl_eff}) implies that $V_t$ is uncorrelated with any function of a variable contained in $\mathcal{F}_{t-1}$. Additionally, under (\ref{Eq:chris_mdl_eff}) VaR models exhibit conditionally and unconditionally the correct number of violations. Consequently, they are optimal because no further improvement is possible. Moreover, \cite{Christoffersen.1998} proves that for $\{V_1, V_2, \dots, V_{t-1} \} \subseteq \mathcal{F}_{t-1}$ the following holds:
%
%\begin{equation}
%V_t | \mathcal{F}_{t-1} \sim Bern(\alpha) \quad \text{i.i.d.},
%\label{Eq:eval_cc_bern}
%\end{equation}
%
%\noindent which is considered as correct conditional coverage. Here, $Bern$ denotes the Bernoulli distribution. Based on this, \cite{Christoffersen.1998} derives a testing framework by combining three likelihood ratio (LR) tests to evaluate the correct unconditional coverage, independence of violations and correct conditional coverage of interval forecasts. The use of this approach is appealing because it allows to evaluate VaR models from different perspectives. 
%
%\subsubsection{Test for Correct Unconditional Coverage}
%
%The test for correct unconditional coverage is used to examine whether the relative number of VaR violations is appropriate for the chosen $\alpha$. By the law of iterated expectations it can be shown that (\ref{Eq:chris_mdl_eff}) implies correct unconditional coverage, i.e.
%
%\begin{equation}
%\mathbb{E}[V_t] = \alpha.
%\end{equation}
%
%\noindent To test for the correct number of violations, the following hypotheses are stated:
%
%\begin{equation}
%\text{H}_0: \mathbb{E}[V_t] = \alpha \qquad \text{vs.} \qquad \text{H}_1: \mathbb{E}[V_t] \ne \alpha.
%\end{equation}
%
%\noindent Since $V_t$ has a Bernoulli distribution under $\text{H}_0$, the corresponding likelihood is with $n$ denoting the sample size and $n_1$ being the number of VaR violations
%
%\begin{equation}
%	L(\alpha; V_1, V_2, \dots, V_{n}) = (1 - \alpha)^{n - n_1} \alpha^{n_1}. 
%	\label{Eq:ll_uc_h0}
%\end{equation} 
%
%\noindent The maximum likelihood estimate of $\alpha$ based on (\ref{Eq:ll_uc_h0}) is obtained as
%
%\begin{equation}
%\hat{\alpha} = \dfrac{n_1}{n}.
%\end{equation}
%
%\noindent Denote the log-likelihood function as $\mathcal{L}(\cdot) = \log L(\cdot)$. Then, by plugging $\hat{\alpha}$ into (\ref{Eq:ll_uc_h0}), the following result can be used to perform a LR test for correct unconditional coverage: 
%\begin{equation}
%\text{LR}_{\tiny\text{UC}} = 2\left[\mathcal{L}(\hat{\alpha}; V_1, V_2, \dots, V_n) - \mathcal{L}(\alpha; V_1, V_2, \dots, V_n) \right] \stackrel{\text{asy}}{\sim}  \mathcal{X}^2_1.
%\label{Eq:lr_uc}
%\end{equation} 
%
%\noindent Here, $\mathcal{X}^2_1$ denotes the $\mathcal{X}^2$ distribution with one degree of freedom. In (\ref{Eq:lr_uc}) only the number of violations is considered. However, it is not tested for the existence of violation clusters, i.e. dependence of the violations. As a consequence, a model can have optimal unconditional coverage even though it does not appropriately adjust for changed market risk. Testing for unconditional coverage is, therefore, not sufficient for appropriately evaluating the model. For instance, if the market risk increases and more violations occur, the model should adjust accordingly by forecasting higher VaR values. By taking this into account, \cite{Christoffersen.1998} introduces also a test for the independence of violations which is presented below. 
%
%%\noindent Here, $\hat{\alpha}$ is the maximum likelihood estimate of $\alpha$ which in case of a Bernoulli distribution is 
%
%%\begin{equation}
%%\hat{\alpha} = \dfrac{n_1}{n_0 + n_1}
%%\end{equation}
%%
%%\noindent where the denominator corresponds to the total number of observations and the numerator to number of exceedances. 
%
%\subsubsection{Test for Independence of Violations}
%
%%In the next step, \cite{Christoffersen.1998} introduces a framework for testing the independence of interval forecasts. \cite{Kuester.2005} notes that taking the independence of VaR forecasts into account is important for avoiding violation clusters. Testing for unconditional coverage is, therefore, not sufficient for appropriately evaluating the model.
%To test for independence of VaR violations assume $V_t$ is a binary first-order Markov chain. Define the transition probability matrix of $V_t$ as
% 
% \begin{equation}
% \Pi_1 = \begin{bmatrix}
% 1 - \pi_{01} & \pi_{01} \\
% 1 - \pi_{11} & \pi_{11} 
% \end{bmatrix}
% \end{equation}
% 
% \noindent where 
% 
% \begin{equation}
% \pi_{ij} = \mathbb{P}(V_t = j | V_{t-1} = i).
% \end{equation}
% 
% \noindent \cite{Christoffersen.1998} states the approximate likelihood function of $V_t$ as 
%
%\begin{equation}
%L(\Pi_1; V_1, \dots, V_n) = (1 - \pi_{01})^{n_{00}} \pi_{01}^{n_{01}} (1 - \pi_{11})^{n_{10}} \pi_{11}^{n_{11}}.
%\label{Eq:ll_indep}
%\end{equation}
%
%\noindent Here, $n_{ij}$ denotes the number of observations where state $i$ was followed by state $j$:
%
%\begin{equation}
%n_{ij} = \sum_{t = 2}^{n} \mathbb{I}(V_t = i| V_{t-1} = j).
%\end{equation}
%
%\noindent An estimate for $\Pi_1$ is obtained by conditioning (\ref{Eq:ll_indep}) on $V_1$ everywhere and maximizing the corresponding log-likelihood function. Then, the resulting maximum likelihood estimates are 
%
%\begin{equation}
%\hat{\pi}_{01} = \dfrac{n_{01}}{n_{00} + n_{01}} \qquad \text{and} \qquad \hat{\pi}_{11} = \dfrac{n_{11}}{n_{10} + n_{11}}.
%\label{Eq:ml_indep_tprob}
%\end{equation}
%
%\noindent Under the null hypothesis that the observed violations $V_t$ are independent, the transition probabilities $\pi_{01}$ and $\pi_{11}$ are equal such that the transition probability matrix becomes 
%
%\begin{equation}
%\Pi_2 = \begin{bmatrix}
%1 - \pi_{0} & \pi_{0} \\
%1 - \pi_{0} & \pi_{0} 
%\end{bmatrix}
%\end{equation}
%
%\noindent where $\pi_0 = \pi_{01} = \pi_{11}$. \noindent Hence, the hypotheses corresponding to the test of independent violations can be stated as follows: 
%
%\begin{equation}
%\text{H}_0: \pi_{01} = \pi_{11} \qquad \text{vs.} \qquad \text{H}_1: \pi_{01} \ne \pi_{11}.
%\end{equation}
%
%\noindent Consequently, the likelihood function corresponding to $\text{H}_0$ is  
%
%\begin{equation}
%L(\Pi_2; V_1, V_2, \dots, V_n) = (1 - \pi_{0})^{n_{00} + n_{10}} \pi_{0}^{n_{01} + n_{11}}
%\label{Eq:ll_indep_null}
%\end{equation}
%
%\noindent with the maximum likelihood estimate 
%
%\begin{equation}
%\hat{\pi}_{0} = \dfrac{n_{01} + n_{11}}{n_{00} + n_{10} + n_{01} + n_{11}}. %=  \dfrac{T_{01} + T_{11}}{T - 1}.
%\end{equation}
%
%
%\noindent \cite{HOEL.1954} derives the LR test statistic as a goodness of fit measure for Markov chains with unknown transition probabilities. Based on this work, \cite{Christoffersen.1998} concludes that the LR test statistic for independence has asymptotically a $\mathcal{X}^2$ distribution with one degree of freedom:
%
%\begin{equation}
%\text{LR}_{\text{ID}} = 2\left[\mathcal{L}\left(\widehat{\Pi}_1; V_1, V_2, \dots, V_n\right) - \mathcal{L}\left(\widehat{\Pi}_2; V_1, V_2, \dots, V_n \right) \right] \stackrel{\text{asy}}{\sim}  \mathcal{X}^2_1.
%\label{Eq:lr_ind}
%\end{equation} 
%
%\noindent Equation (\ref{Eq:lr_ind}) does not depend on the true coverage. Hence, it is limited to testing for independence. However, \cite{Christoffersen.1998} stresses the test's usefulness for assessing the dynamics of interval forecasts which is possible even though the true error distribution is unknown. \\
%
%\noindent \cite{Christoffersen.2004} notes that especially for low $\alpha$ or small samples it is likely that $n_{11} = 0$. Consequently, also $\hat{\pi}_{11}$ and (\ref{Eq:ll_indep}) will be zero. Since $\log(0)$ is not defined, (\ref{Eq:lr_ind}) cannot be computed. To overcome this limitation, \cite{Christoffersen.2004} suggests to use the following modification of (\ref{Eq:ll_indep}) if $n_{11} = 0$: 
%
% \begin{equation}
% L(\Pi_1; V_1, V_2, \dots, V_n) = (1 - \pi_{01})^{n_{00}} \pi_{01}^{n_{01}}.
% \label{Eq:modification_ll_ind}
% \end{equation}
%
%\noindent This modification is used in the empirical study in Section \ref{Sec:emp_study}.
%
%
%\subsubsection{Test for Correct Conditional Coverage}
%
%Ideally, a model for forecasting VaR combines the ability to capture temporarily changing market risk regimes and has correct coverage. Although (\ref{Eq:lr_ind}) accounts for the former, it does not for the latter. However, both abilities can be assessed by introducing a test for correct conditional coverage. By combining (\ref{Eq:lr_uc}) and (\ref{Eq:lr_ind}), \cite{Christoffersen.1998} derives the following likelihood ratio test statistic for correct conditional coverage:
%
%\begin{equation}
%\text{LR}_{\text{CC}} = 2\left[ \mathcal{L}(\hat{\Pi}_1; V_1, V_2, \dots, V_n) - \mathcal{L}(\alpha; V_1, V_2, \dots, V_n) \right] \stackrel{\text{asy}}{\sim}  \mathcal{X}^2_2.
%\label{Eq:LR_cc}
%\end{equation}
%
%\noindent Note that (\ref{Eq:LR_cc}) is asymptotically $\mathcal{X}^2$ distributed with two degrees of freedom. Moreover, \cite{Christoffersen.1998} points out that from conditioning on $V_1$ in (\ref{Eq:lr_uc}) it follows that $\hat{\alpha} = \hat{\pi}_0$. Then, by neglecting $V_1$, $\text{LR}_{\text{CC}}$ can be rewritten as
%
%\begin{equation}
%\text{LR}_{\text{CC}} = \text{LR}_{\text{UC}} + \text{LR}_{\text{ID}}.
%\label{Eq:LR_cc_re}
%\end{equation}
%
%\noindent Rewriting (\ref{Eq:LR_cc}) as (\ref{Eq:LR_cc_re}) makes it possible to evaluate whether the performance of a VaR model in terms of correct conditional coverage is determined by its ability to achieve correct coverage or adjust for changing volatility. This is useful in situations where $\text{LR}_{\text{CC}}$ is relatively small but only one of the test statistics, i.e. $\text{LR}_{\text{UC}}$ or $\text{LR}_{\text{ID}}$, is small. Then, it is easier to appropriately adjust the model.
%
%%\subsection{Other Risk Measures}
%


==> source code Version for upload/Tables/Case_1/Archiv/Results_Case1_10Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:13:17 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 1 & 1.03 & 90.58 & 30.09 & 29.88 & 13.8 \\ 
  SVR-KDE & S\&P500 & 1 & 0.95 & 86.85 & 25.94 & 25.59 & 58.2 \\ 
  GARCH-SSTD & S\&P500 & 1 & 1.19 & 50.57 & 3.91 & 3.14 & 9.2 \\ 
  TGARCH-STD & S\&P500 & 1 & 1.99 & 0.19 & 25.26 & 0.21 & 0.8 \\ 
  GARCH-STD & S\&P500 & 1 & 1.99 & 0.19 & 25.26 & 0.21 & 3.8 \\ 
  TGARCH-NORM & S\&P500 & 1 & 2.31 & 0.01 & 39.72 & 0.01 & 3 \\ 
  GARCH-NORM & S\&P500 & 1 & 2.54 & 0 & 51.83 & 0 & 2.6 \\ 
  EGARCH-STD & S\&P500 & 1 & 2.78 & 0 & 64.14 & 0 & 0 \\ 
  EGARCH-SSTD & S\&P500 & 1 & 2.7 & 0 & 4.5 & 0 & 0.6 \\ 
  EGARCH-NORM & S\&P500 & 1 & 3.26 & 0 & 14.87 & 0 & 0.6 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1 & 1.45 & 13.59 & 52.97 & 17.42 & 2.6 \\ 
  GARCH-SSTD & Nikkei225 & 1 & 1.45 & 13.59 & 52.97 & 17.42 & 2.8 \\ 
  SVR-KDE & Nikkei225 & 1 & 0.32 & 0.51 & 87.23 & 1.97 & 0 \\ 
  GARCH-STD & Nikkei225 & 1 & 1.85 & 0.7 & 19.57 & 0.51 & 1.2 \\ 
  TGARCH-STD & Nikkei225 & 1 & 1.93 & 0.34 & 22.56 & 0.31 & 2 \\ 
  GARCH-NORM & Nikkei225 & 1 & 2.01 & 0.16 & 25.77 & 0.18 & 2.2 \\ 
  TGARCH-NORM & Nikkei225 & 1 & 2.09 & 0.07 & 5.45 & 0.02 & 2.2 \\ 
  EGARCH-STD & Nikkei225 & 1 & 3.95 & 0 & 75.92 & 0 & 0.2 \\ 
  EGARCH-SSTD & Nikkei225 & 1 & 2.5 & 0 & 48.53 & 0 & 0.8 \\ 
  EGARCH-NORM & Nikkei225 & 1 & 2.58 & 0 & 15.65 & 0 & 1.4 \\ 
   \hline
\hline
SVR-KDE & EuroStoxx50 & 1 & 0.97 & 90.41 & 62.85 & 88.31 & 0 \\ 
  GARCH-SSTD & EuroStoxx50 & 1 & 2.01 & 0.16 & 25.77 & 0.18 & 9.6 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1 & 2.33 & 0.01 & 40.43 & 0.01 & 6.2 \\ 
  TGARCH-STD & EuroStoxx50 & 1 & 2.58 & 0 & 15.65 & 0 & 6.8 \\ 
  TGARCH-NORM & EuroStoxx50 & 1 & 2.66 & 0 & 18.07 & 0 & 5.8 \\ 
  GARCH-STD & EuroStoxx50 & 1 & 2.33 & 0.01 & 9.64 & 0 & 7.4 \\ 
  GARCH-NORM & EuroStoxx50 & 1 & 2.58 & 0 & 15.65 & 0 & 1.4 \\ 
  EGARCH-STD & EuroStoxx50 & 1 & 4.03 & 0 & 17.32 & 0 & 1.4 \\ 
  EGARCH-SSTD & EuroStoxx50 & 1 & 3.7 & 0 & 2.49 & 0 & 1.2 \\ 
  EGARCH-NORM & EuroStoxx50 & 1 & 3.3 & 0 & 44.47 & 0 & 0.6 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> source code Version for upload/Tables/Case_1/Archiv/Results_Case1_10Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:13:17 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 2.5 & 2.62 & 78.12 & 55.96 & 53.84 & 10.8 \\ 
  GARCH-SSTD & S\&P500 & 2.5 & 2.78 & 52.88 & 22.94 & 18.81 & 3.6 \\ 
  GARCH-STD & S\&P500 & 2.5 & 3.18 & 13.82 & 39.68 & 13.22 & 3.6 \\ 
  TGARCH-STD & S\&P500 & 2.5 & 3.42 & 4.8 & 51.32 & 7.27 & 0.8 \\ 
  GARCH-NORM & S\&P500 & 2.5 & 3.58 & 2.14 & 59.33 & 4.2 & 1 \\ 
  SVR-KDE & S\&P500 & 2.5 & 1.75 & 7.15 & 16.45 & 3.24 & 55.8 \\ 
  TGARCH-NORM & S\&P500 & 2.5 & 3.58 & 2.14 & 25.03 & 1.77 & 0.8 \\ 
  EGARCH-STD & S\&P500 & 2.5 & 4.37 & 0.01 & 30.25 & 0.02 & 0.2 \\ 
  EGARCH-SSTD & S\&P500 & 2.5 & 4.77 & 0 & 22.74 & 0 & 0 \\ 
  EGARCH-NORM & S\&P500 & 2.5 & 4.61 & 0 & 17.75 & 0 & 0 \\ 
   \hline
\hline
GARCH-STD & Nikkei225 & 2.5 & 2.74 & 59.74 & 60.95 & 53.02 & 0.6 \\ 
  GARCH-SSTD & Nikkei225 & 2.5 & 2.25 & 57.31 & 36.53 & 31.17 & 8.6 \\ 
  GARCH-NORM & Nikkei225 & 2.5 & 3.3 & 8.45 & 86.53 & 19.54 & 0 \\ 
  TGARCH-SSTD & Nikkei225 & 2.5 & 2.74 & 59.74 & 20.72 & 18.02 & 0 \\ 
  TGARCH-STD & Nikkei225 & 2.5 & 3.06 & 22.21 & 33.3 & 15.8 & 0 \\ 
  TGARCH-NORM & Nikkei225 & 2.5 & 3.46 & 3.99 & 52.4 & 6.35 & 0 \\ 
  EGARCH-SSTD & Nikkei225 & 2.5 & 4.03 & 0.15 & 43.03 & 0.28 & 0.2 \\ 
  EGARCH-NORM & Nikkei225 & 2.5 & 4.11 & 0.09 & 46.87 & 0.19 & 0 \\ 
  SVR-KDE & Nikkei225 & 2.5 & 1.29 & 0.26 & 5.17 & 0.06 & 7 \\ 
  EGARCH-STD & Nikkei225 & 2.5 & 5.31 & 0 & 96.4 & 0 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.5 & 3.22 & 11.91 & 40.62 & 12.06 & 49.2 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.5 & 3.3 & 8.45 & 44.47 & 10.04 & 49.8 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.5 & 3.38 & 5.87 & 48.4 & 8.11 & 8.2 \\ 
  GARCH-STD & EuroStoxx50 & 2.5 & 3.46 & 3.99 & 52.4 & 6.35 & 9.4 \\ 
  SVR-KDE & EuroStoxx50 & 2.5 & 3.06 & 22.21 & 9.73 & 4.61 & 61 \\ 
  TGARCH-STD & EuroStoxx50 & 2.5 & 3.46 & 3.99 & 20.23 & 2.45 & 12.2 \\ 
  GARCH-NORM & EuroStoxx50 & 2.5 & 3.78 & 0.7 & 68.4 & 1.8 & 0.2 \\ 
  EGARCH-STD & EuroStoxx50 & 2.5 & 5.88 & 0 & 43.78 & 0 & 0.4 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.5 & 4.91 & 0 & 3.67 & 0 & 0.4 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.5 & 4.83 & 0 & 23.77 & 0 & 0 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archiv/Results_Case1_10Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:13:17 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
TGARCH-NORM & S\&P500 & 5 & 5.09 & 88.72 & 34.98 & 34.63 & 1.2 \\ 
  TGARCH-STD & S\&P500 & 5 & 5.01 & 98.97 & 31.66 & 31.66 & 0 \\ 
  GARCH-SSTD & S\&P500 & 5 & 4.29 & 23.85 & 57.38 & 28.64 & 1.8 \\ 
  GARCH-STD & S\&P500 & 5 & 5.17 & 78.7 & 17.88 & 17.24 & 0.2 \\ 
  TGARCH-SSTD & S\&P500 & 5 & 4.21 & 18.86 & 24.22 & 10.2 & 5 \\ 
  GARCH-NORM & S\&P500 & 5 & 5.48 & 43.69 & 4.89 & 3.62 & 0.2 \\ 
  EGARCH-NORM & S\&P500 & 5 & 6.52 & 1.8 & 29.69 & 1.81 & 0 \\ 
  EGARCH-STD & S\&P500 & 5 & 6.6 & 1.3 & 32.87 & 1.5 & 0 \\ 
  SVR-KDE & S\&P500 & 5 & 3.34 & 0.41 & 17.11 & 0.28 & 5 \\ 
  EGARCH-SSTD & S\&P500 & 5 & 7.23 & 0.06 & 62.62 & 0.18 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 5 & 5.23 & 70.78 & 94.63 & 88.21 & 16 \\ 
  GARCH-SSTD & Nikkei225 & 5 & 4.99 & 98.96 & 87.41 & 87.4 & 20.4 \\ 
  TGARCH-STD & Nikkei225 & 5 & 5.31 & 61.51 & 72.91 & 64.25 & 8.8 \\ 
  TGARCH-NORM & Nikkei225 & 5 & 5.31 & 61.51 & 72.91 & 64.25 & 7 \\ 
  GARCH-NORM & Nikkei225 & 5 & 5.72 & 25.68 & 99.95 & 52.55 & 6.8 \\ 
  GARCH-STD & Nikkei225 & 5 & 5.72 & 25.68 & 89.19 & 46.89 & 6.4 \\ 
  SVR-KDE & Nikkei225 & 5 & 3.95 & 7.7 & 75.92 & 15.9 & 46.4 \\ 
  EGARCH-SSTD & Nikkei225 & 5 & 6.36 & 3.44 & 90.35 & 9.65 & 0.2 \\ 
  EGARCH-NORM & Nikkei225 & 5 & 6.12 & 7.99 & 31.6 & 6.82 & 2.2 \\ 
  EGARCH-STD & Nikkei225 & 5 & 7.97 & 0 & 91.62 & 0 & 0 \\ 
   \hline
\hline
SVR-KDE & EuroStoxx50 & 5 & 5.07 & 90.69 & 61.34 & 60.92 & 4 \\ 
  TGARCH-NORM & EuroStoxx50 & 5 & 6.12 & 7.99 & 6.55 & 1.41 & 3.8 \\ 
  TGARCH-SSTD & EuroStoxx50 & 5 & 6.12 & 7.99 & 2.43 & 0.53 & 3.6 \\ 
  TGARCH-STD & EuroStoxx50 & 5 & 6.36 & 3.44 & 4.28 & 0.46 & 0.4 \\ 
  GARCH-NORM & EuroStoxx50 & 5 & 6.36 & 3.44 & 4.28 & 0.46 & 1 \\ 
  GARCH-SSTD & EuroStoxx50 & 5 & 6.52 & 1.85 & 6.06 & 0.38 & 1.8 \\ 
  GARCH-STD & EuroStoxx50 & 5 & 6.76 & 0.67 & 9.76 & 0.25 & 0.4 \\ 
  EGARCH-STD & EuroStoxx50 & 5 & 9.1 & 0 & 1.03 & 0 & 0.2 \\ 
  EGARCH-SSTD & EuroStoxx50 & 5 & 7.41 & 0.03 & 0.13 & 0 & 0.2 \\ 
  EGARCH-NORM & EuroStoxx50 & 5 & 7.17 & 0.1 & 0.18 & 0 & 0.8 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archiv/Results_Case1_1Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:10:35 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
EGARCH-SSTD & S\&P500 & 1 & 1.11 & 69.27 & 57.46 & 79.01 & 6.2 \\ 
  TGARCH-SSTD & S\&P500 & 1 & 0.72 & 28.52 & 71.87 & 52.94 & 64.4 \\ 
  GARCH-SSTD & S\&P500 & 1 & 1.27 & 35.24 & 43.34 & 28.13 & 23.6 \\ 
  TGARCH-STD & S\&P500 & 1 & 1.43 & 14.91 & 46.97 & 27.2 & 0.8 \\ 
  SVR-KDE & S\&P500 & 1 & 0.79 & 44.83 & 18.28 & 13.71 & 28.8 \\ 
  GARCH-STD & S\&P500 & 1 & 1.67 & 2.95 & 65.77 & 6.15 & 14.4 \\ 
  EGARCH-STD & S\&P500 & 1 & 1.75 & 1.58 & 37.62 & 3.67 & 7.2 \\ 
  TGARCH-NORM & S\&P500 & 1 & 2.15 & 0.04 & 27.64 & 0.1 & 3.6 \\ 
  EGARCH-NORM & S\&P500 & 1 & 2.23 & 0.02 & 25.88 & 0.04 & 2 \\ 
  GARCH-NORM & S\&P500 & 1 & 2.38 & 0 & 94.85 & 0.01 & 0.8 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1 & 1.21 & 47.61 & 54.48 & 64.58 & 5 \\ 
  GARCH-SSTD & Nikkei225 & 1 & 1.21 & 47.61 & 54.48 & 64.58 & 4.2 \\ 
  EGARCH-SSTD & Nikkei225 & 1 & 1.37 & 21.61 & 49.21 & 36.76 & 6.8 \\ 
  GARCH-STD & Nikkei225 & 1 & 1.69 & 2.6 & 66.33 & 5.56 & 2.6 \\ 
  TGARCH-STD & Nikkei225 & 1 & 1.77 & 1.37 & 37.3 & 3.23 & 0.8 \\ 
  SVR-KDE & Nikkei225 & 1 & 0.24 & 0.13 & 90.41 & 0.55 & 0 \\ 
  EGARCH-STD & Nikkei225 & 1 & 2.09 & 0.07 & 29.17 & 0.19 & 1.4 \\ 
  GARCH-NORM & Nikkei225 & 1 & 2.17 & 0.03 & 88.16 & 0.14 & 0.8 \\ 
  TGARCH-NORM & Nikkei225 & 1 & 2.33 & 0.01 & 93.19 & 0.03 & 0.2 \\ 
  EGARCH-NORM & Nikkei225 & 1 & 2.42 & 0 & 95.21 & 0.01 & 0.2 \\ 
   \hline
\hline
SVR-KDE & EuroStoxx50 & 1 & 1.53 & 8.17 & 44.23 & 16.36 & 67 \\ 
  GARCH-SSTD & EuroStoxx50 & 1 & 1.69 & 2.6 & 39.54 & 5.84 & 74.6 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1 & 1.69 & 2.6 & 66.33 & 5.56 & 44.2 \\ 
  TGARCH-STD & EuroStoxx50 & 1 & 1.77 & 1.37 & 70.53 & 3.39 & 1.2 \\ 
  GARCH-STD & EuroStoxx50 & 1 & 1.85 & 0.7 & 35.15 & 1.7 & 1.2 \\ 
  TGARCH-NORM & EuroStoxx50 & 1 & 2.09 & 0.07 & 85.17 & 0.28 & 0.8 \\ 
  GARCH-NORM & EuroStoxx50 & 1 & 2.17 & 0.03 & 27.33 & 0.08 & 5.2 \\ 
  EGARCH-STD & EuroStoxx50 & 1 & 2.33 & 0.01 & 93.19 & 0.03 & 12.4 \\ 
  EGARCH-SSTD & EuroStoxx50 & 1 & 2.42 & 0 & 95.21 & 0.01 & 2.8 \\ 
  EGARCH-NORM & EuroStoxx50 & 1 & 2.5 & 0 & 96.87 & 0 & 3.8 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> source code Version for upload/Tables/Case_1/Archiv/Results_Case1_1Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:10:35 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 2.5 & 2.62 & 78.12 & 98.97 & 95.22 & 30.6 \\ 
  EGARCH-SSTD & S\&P500 & 2.5 & 3.02 & 25.18 & 98.94 & 51.31 & 0.6 \\ 
  TGARCH-SSTD & S\&P500 & 2.5 & 2.38 & 79.19 & 22.6 & 46.4 & 61.8 \\ 
  GARCH-STD & S\&P500 & 2.5 & 3.5 & 3.24 & 93.45 & 9.47 & 2.8 \\ 
  GARCH-NORM & S\&P500 & 2.5 & 3.82 & 0.55 & 99.2 & 2.1 & 1 \\ 
  SVR-KDE & S\&P500 & 2.5 & 1.43 & 0.83 & 52.45 & 1.62 & 34.2 \\ 
  TGARCH-STD & S\&P500 & 2.5 & 3.9 & 0.33 & 75.52 & 1.02 & 0.2 \\ 
  TGARCH-NORM & S\&P500 & 2.5 & 4.05 & 0.12 & 69.37 & 0.36 & 0.4 \\ 
  EGARCH-STD & S\&P500 & 2.5 & 4.37 & 0.01 & 96.11 & 0.06 & 0 \\ 
  EGARCH-NORM & S\&P500 & 2.5 & 4.53 & 0 & 92.48 & 0.02 & 0.2 \\ 
   \hline
\hline
GARCH-SSTD & Nikkei225 & 2.5 & 2.9 & 38.01 & 99.9 & 67.96 & 44.2 \\ 
  TGARCH-SSTD & Nikkei225 & 2.5 & 2.42 & 84.78 & 22.29 & 46.72 & 69.6 \\ 
  TGARCH-STD & Nikkei225 & 2.5 & 3.14 & 16.44 & 97.67 & 37.15 & 2 \\ 
  TGARCH-NORM & Nikkei225 & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 & 0.4 \\ 
  EGARCH-NORM & Nikkei225 & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 & 0.6 \\ 
  GARCH-NORM & Nikkei225 & 2.5 & 3.38 & 5.87 & 92.85 & 15.55 & 0.2 \\ 
  GARCH-STD & Nikkei225 & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 & 0 \\ 
  EGARCH-SSTD & Nikkei225 & 2.5 & 3.06 & 22.21 & 12.14 & 14.3 & 17.4 \\ 
  SVR-KDE & Nikkei225 & 2.5 & 1.69 & 5.26 & 14.27 & 2.18 & 59 \\ 
  EGARCH-STD & Nikkei225 & 2.5 & 3.86 & 0.43 & 99.42 & 1.68 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.5 & 2.98 & 29.36 & 72.9 & 42 & 71.8 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.5 & 3.22 & 11.91 & 83.46 & 24.78 & 0.2 \\ 
  TGARCH-STD & EuroStoxx50 & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 & 0 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.5 & 3.46 & 3.99 & 91.84 & 11.13 & 73.4 \\ 
  SVR-KDE & EuroStoxx50 & 2.5 & 3.14 & 16.44 & 11.43 & 4.35 & 34.2 \\ 
  GARCH-STD & EuroStoxx50 & 2.5 & 3.7 & 1.11 & 97.42 & 3.88 & 3.4 \\ 
  GARCH-NORM & EuroStoxx50 & 2.5 & 3.95 & 0.26 & 75.92 & 0.81 & 6 \\ 
  EGARCH-STD & EuroStoxx50 & 2.5 & 4.27 & 0.03 & 88.73 & 0.12 & 0.6 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.5 & 4.51 & 0 & 95.5 & 0.02 & 1.6 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.5 & 4.59 & 0 & 97.11 & 0.01 & 1 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archiv/Results_Case1_1Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Aug 21 18:10:35 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{SPA} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 5 & 5.01 & 98.97 & 89.07 & 89.06 & 62.8 \\ 
  GARCH-NORM & S\&P500 & 5 & 5.72 & 24.94 & 99.79 & 51.4 & 0.2 \\ 
  TGARCH-SSTD & S\&P500 & 5 & 5.41 & 51.47 & 60.38 & 48.83 & 62.6 \\ 
  GARCH-STD & S\&P500 & 5 & 5.8 & 20.21 & 99.23 & 43.99 & 2.8 \\ 
  SVR-KDE & S\&P500 & 5 & 4.37 & 29.68 & 30.25 & 17.55 & 26.4 \\ 
  EGARCH-SSTD & S\&P500 & 5 & 6.44 & 2.47 & 83.92 & 6.73 & 0.4 \\ 
  TGARCH-NORM & S\&P500 & 5 & 6.6 & 1.3 & 77.88 & 3.56 & 0.4 \\ 
  EGARCH-NORM & S\&P500 & 5 & 6.76 & 0.65 & 94.35 & 2.33 & 0.8 \\ 
  TGARCH-STD & S\&P500 & 5 & 6.76 & 0.65 & 71.36 & 1.77 & 0 \\ 
  EGARCH-STD & S\&P500 & 5 & 7 & 0.21 & 87.46 & 0.78 & 0.6 \\ 
   \hline
\hline
EGARCH-SSTD & Nikkei225 & 5 & 5.23 & 70.78 & 97.26 & 90.66 & 13 \\ 
  SVR-KDE & Nikkei225 & 5 & 4.59 & 50.1 & 97.11 & 77.43 & 35.2 \\ 
  TGARCH-SSTD & Nikkei225 & 5 & 4.67 & 58.95 & 89.41 & 77.3 & 72.8 \\ 
  GARCH-SSTD & Nikkei225 & 5 & 5.07 & 90.69 & 75.29 & 74.78 & 34 \\ 
  TGARCH-NORM & Nikkei225 & 5 & 5.23 & 70.78 & 68.85 & 64.18 & 0 \\ 
  TGARCH-STD & Nikkei225 & 5 & 5.56 & 37.71 & 89.62 & 60.67 & 0 \\ 
  GARCH-NORM & Nikkei225 & 5 & 5.88 & 16.68 & 78.41 & 30.16 & 4 \\ 
  EGARCH-NORM & Nikkei225 & 5 & 5.72 & 25.68 & 49.18 & 25.85 & 0 \\ 
  GARCH-STD & Nikkei225 & 5 & 6.04 & 10.34 & 71.98 & 19.11 & 0 \\ 
  EGARCH-STD & Nikkei225 & 5 & 6.04 & 10.34 & 71.98 & 19.11 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 5 & 5.15 & 80.55 & 65.27 & 63.32 & 70.6 \\ 
  GARCH-SSTD & EuroStoxx50 & 5 & 5.96 & 13.21 & 95.83 & 30.84 & 56.8 \\ 
  GARCH-NORM & EuroStoxx50 & 5 & 5.96 & 13.21 & 95.83 & 30.84 & 47.2 \\ 
  TGARCH-NORM & EuroStoxx50 & 5 & 6.04 & 10.34 & 78.1 & 20.73 & 2.2 \\ 
  SVR-KDE & EuroStoxx50 & 5 & 5.48 & 44.9 & 26.86 & 20.17 & 29.6 \\ 
  EGARCH-SSTD & EuroStoxx50 & 5 & 6.12 & 7.99 & 68.65 & 14.82 & 1.2 \\ 
  TGARCH-STD & EuroStoxx50 & 5 & 6.2 & 6.11 & 59.29 & 10.26 & 0 \\ 
  EGARCH-NORM & EuroStoxx50 & 5 & 6.52 & 1.85 & 99.1 & 6.18 & 1.6 \\ 
  GARCH-STD & EuroStoxx50 & 5 & 6.6 & 1.33 & 96.58 & 4.52 & 3.8 \\ 
  EGARCH-STD & EuroStoxx50 & 5 & 6.84 & 0.46 & 69.51 & 1.27 & 0.8 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archive2/Results_Case1_10Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:36:26 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 1.03 & 11.78 & 90.58 & 30.09 & 29.88 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.95 & 94.01 & 86.85 & 25.94 & 25.59 \\ 
  GARCH-SSTD & S\&P500 & 1.19 & 10.38 & 50.57 & 3.91 & 3.14 \\ 
  TGARCH-STD & S\&P500 & 1.99 & 1.80 & 0.19 & 25.26 & 0.21 \\ 
  GARCH-STD & S\&P500 & 1.99 & 2.99 & 0.19 & 25.26 & 0.21 \\ 
  TGARCH-NORM & S\&P500 & 2.31 & 3.59 & 0.01 & 39.72 & 0.01 \\ 
  GARCH-NORM & S\&P500 & 2.54 & 3.39 & 0.00 & 51.83 & 0.00 \\ 
  EGARCH-STD & S\&P500 & 2.78 & 0.00 & 0.00 & 64.14 & 0.00 \\ 
  EGARCH-SSTD & S\&P500 & 2.70 & 0.80 & 0.00 & 4.50 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 3.26 & 0.60 & 0.00 & 14.87 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.45 & 3.19 & 13.59 & 52.97 & 17.42 \\ 
  GARCH-SSTD & Nikkei225 & 1.45 & 2.40 & 13.59 & 52.97 & 17.42 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.32 & 57.29 & 0.51 & 87.23 & 1.97 \\ 
  GARCH-STD & Nikkei225 & 1.85 & 0.80 & 0.70 & 19.57 & 0.51 \\ 
  TGARCH-STD & Nikkei225 & 1.93 & 1.80 & 0.34 & 22.56 & 0.31 \\ 
  GARCH-NORM & Nikkei225 & 2.01 & 1.80 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-NORM & Nikkei225 & 2.09 & 2.20 & 0.07 & 5.45 & 0.02 \\ 
  EGARCH-STD & Nikkei225 & 3.95 & 0.20 & 0.00 & 75.92 & 0.00 \\ 
  EGARCH-SSTD & Nikkei225 & 2.50 & 1.20 & 0.00 & 48.53 & 0.00 \\ 
  EGARCH-NORM & Nikkei225 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 0.97 & 64.07 & 90.41 & 62.85 & 88.31 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.01 & 8.78 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-SSTD & EuroStoxx50 & 2.33 & 5.99 & 0.01 & 40.43 & 0.01 \\ 
  TGARCH-STD & EuroStoxx50 & 2.58 & 4.99 & 0.00 & 15.65 & 0.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.66 & 4.79 & 0.00 & 18.07 & 0.00 \\ 
  GARCH-STD & EuroStoxx50 & 2.33 & 5.79 & 0.01 & 9.64 & 0.00 \\ 
  GARCH-NORM & EuroStoxx50 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
  EGARCH-STD & EuroStoxx50 & 4.03 & 1.40 & 0.00 & 17.32 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 3.70 & 1.80 & 0.00 & 2.49 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 3.30 & 0.20 & 0.00 & 44.47 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 10 days ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_1}
\end{table}


==> source code Version for upload/Tables/Case_1/Archive2/Results_Case1_10Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:36:26 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 2.62 & 13.57 & 78.12 & 55.96 & 53.84 \\ 
  GARCH-SSTD & S\&P500 & 2.78 & 6.99 & 52.88 & 22.94 & 18.81 \\ 
  GARCH-STD & S\&P500 & 3.18 & 3.39 & 13.82 & 39.68 & 13.22 \\ 
  TGARCH-STD & S\&P500 & 3.42 & 0.20 & 4.80 & 51.32 & 7.27 \\ 
  GARCH-NORM & S\&P500 & 3.58 & 2.79 & 2.14 & 59.33 & 4.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.75 & 95.21 & 7.15 & 16.45 & 3.24 \\ 
  TGARCH-NORM & S\&P500 & 3.58 & 0.40 & 2.14 & 25.03 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 30.25 & 0.02 \\ 
  EGARCH-SSTD & S\&P500 & 4.77 & 0.20 & 0.00 & 22.74 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 4.61 & 0.20 & 0.00 & 17.75 & 0.00 \\ 
   \hline
\hline
GARCH-STD & Nikkei225 & 2.74 & 0.20 & 59.74 & 60.95 & 53.02 \\ 
  GARCH-SSTD & Nikkei225 & 2.25 & 8.58 & 57.31 & 36.53 & 31.17 \\ 
  GARCH-NORM & Nikkei225 & 3.30 & 0.00 & 8.45 & 86.53 & 19.54 \\ 
  TGARCH-SSTD & Nikkei225 & 2.74 & 0.00 & 59.74 & 20.72 & 18.02 \\ 
  TGARCH-STD & Nikkei225 & 3.06 & 0.00 & 22.21 & 33.30 & 15.80 \\ 
  TGARCH-NORM & Nikkei225 & 3.46 & 0.00 & 3.99 & 52.40 & 6.35 \\ 
  EGARCH-SSTD & Nikkei225 & 4.03 & 0.40 & 0.15 & 43.03 & 0.28 \\ 
  EGARCH-NORM & Nikkei225 & 4.11 & 0.00 & 0.09 & 46.87 & 0.19 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.29 & 48.10 & 0.26 & 5.17 & 0.06 \\ 
  EGARCH-STD & Nikkei225 & 5.31 & 0.20 & 0.00 & 96.40 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 3.22 & 50.30 & 11.91 & 40.62 & 12.06 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.30 & 50.10 & 8.45 & 44.47 & 10.04 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.38 & 9.38 & 5.87 & 48.40 & 8.11 \\ 
  GARCH-STD & EuroStoxx50 & 3.46 & 8.78 & 3.99 & 52.40 & 6.35 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.06 & 85.03 & 22.21 & 9.73 & 4.61 \\ 
  TGARCH-STD & EuroStoxx50 & 3.46 & 13.77 & 3.99 & 20.23 & 2.45 \\ 
  GARCH-NORM & EuroStoxx50 & 3.78 & 0.20 & 0.70 & 68.40 & 1.80 \\ 
  EGARCH-STD & EuroStoxx50 & 5.88 & 0.40 & 0.00 & 43.78 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.91 & 0.20 & 0.00 & 3.67 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.83 & 0.00 & 0.00 & 23.77 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 10 days ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_2.5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archive2/Results_Case1_10Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:36:26 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-NORM & S\&P500 & 5.09 & 1.20 & 88.72 & 34.98 & 34.63 \\ 
  TGARCH-STD & S\&P500 & 5.01 & 0.00 & 98.97 & 31.66 & 31.66 \\ 
  GARCH-SSTD & S\&P500 & 4.29 & 2.20 & 23.85 & 57.38 & 28.64 \\ 
  GARCH-STD & S\&P500 & 5.17 & 0.00 & 78.70 & 17.88 & 17.24 \\ 
  TGARCH-SSTD & S\&P500 & 4.21 & 4.39 & 18.86 & 24.22 & 10.20 \\ 
  GARCH-NORM & S\&P500 & 5.48 & 0.00 & 43.69 & 4.89 & 3.62 \\ 
  EGARCH-NORM & S\&P500 & 6.52 & 0.00 & 1.80 & 29.69 & 1.81 \\ 
  EGARCH-STD & S\&P500 & 6.60 & 0.00 & 1.30 & 32.87 & 1.50 \\ 
  SVR-GARCH-KDE & S\&P500 & 3.34 & 56.89 & 0.41 & 17.11 & 0.28 \\ 
  EGARCH-SSTD & S\&P500 & 7.23 & 0.00 & 0.06 & 62.62 & 0.18 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 5.23 & 10.18 & 70.78 & 94.63 & 88.21 \\ 
  GARCH-SSTD & Nikkei225 & 4.99 & 21.16 & 98.96 & 87.41 & 87.40 \\ 
  TGARCH-STD & Nikkei225 & 5.31 & 8.18 & 61.51 & 72.91 & 64.25 \\ 
  TGARCH-NORM & Nikkei225 & 5.31 & 12.18 & 61.51 & 72.91 & 64.25 \\ 
  GARCH-NORM & Nikkei225 & 5.72 & 5.99 & 25.68 & 99.95 & 52.55 \\ 
  GARCH-STD & Nikkei225 & 5.72 & 8.18 & 25.68 & 89.19 & 46.89 \\ 
  SVR-GARCH-KDE & Nikkei225 & 3.95 & 88.82 & 7.70 & 75.92 & 15.90 \\ 
  EGARCH-SSTD & Nikkei225 & 6.36 & 0.60 & 3.44 & 90.35 & 9.65 \\ 
  EGARCH-NORM & Nikkei225 & 6.12 & 3.59 & 7.99 & 31.60 & 6.82 \\ 
  EGARCH-STD & Nikkei225 & 7.97 & 0.00 & 0.00 & 91.62 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 5.07 & 50.10 & 90.69 & 61.34 & 60.92 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.12 & 2.59 & 7.99 & 6.55 & 1.41 \\ 
  TGARCH-SSTD & EuroStoxx50 & 6.12 & 4.99 & 7.99 & 2.43 & 0.53 \\ 
  TGARCH-STD & EuroStoxx50 & 6.36 & 0.00 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-NORM & EuroStoxx50 & 6.36 & 2.20 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-SSTD & EuroStoxx50 & 6.52 & 2.99 & 1.85 & 6.06 & 0.38 \\ 
  GARCH-STD & EuroStoxx50 & 6.76 & 0.40 & 0.67 & 9.76 & 0.25 \\ 
  EGARCH-STD & EuroStoxx50 & 9.10 & 0.20 & 0.00 & 1.03 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 7.41 & 0.20 & 0.03 & 0.13 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 7.17 & 0.60 & 0.10 & 0.18 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 10 days ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archive2/Results_Case1_1Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:34:41 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
EGARCH-SSTD & S\&P500 & 1.11 & 4.99 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & S\&P500 & 0.72 & 92.22 & 28.52 & 71.87 & 52.94 \\ 
  GARCH-SSTD & S\&P500 & 1.27 & 20.76 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & S\&P500 & 1.43 & 0.20 & 14.91 & 46.97 & 27.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.79 & 29.34 & 44.83 & 18.28 & 13.71 \\ 
  GARCH-STD & S\&P500 & 1.67 & 16.17 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & S\&P500 & 1.75 & 5.79 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & S\&P500 & 2.15 & 3.39 & 0.04 & 27.64 & 0.10 \\ 
  EGARCH-NORM & S\&P500 & 2.23 & 2.40 & 0.02 & 25.88 & 0.04 \\ 
  GARCH-NORM & S\&P500 & 2.38 & 0.20 & 0.00 & 94.85 & 0.01 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.21 & 4.99 & 47.61 & 54.48 & 64.58 \\ 
  GARCH-SSTD & Nikkei225 & 1.21 & 2.79 & 47.61 & 54.48 & 64.58 \\ 
  EGARCH-SSTD & Nikkei225 & 1.37 & 4.19 & 21.61 & 49.21 & 36.76 \\ 
  GARCH-STD & Nikkei225 & 1.69 & 1.80 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & Nikkei225 & 1.77 & 1.00 & 1.37 & 37.30 & 3.23 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.24 & 59.48 & 0.13 & 90.41 & 0.55 \\ 
  EGARCH-STD & Nikkei225 & 2.09 & 0.80 & 0.07 & 29.17 & 0.19 \\ 
  GARCH-NORM & Nikkei225 & 2.17 & 0.40 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & Nikkei225 & 2.33 & 0.20 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & Nikkei225 & 2.42 & 0.20 & 0.00 & 95.21 & 0.01 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 1.53 & 76.25 & 8.17 & 44.23 & 16.36 \\ 
  GARCH-SSTD & EuroStoxx50 & 1.69 & 72.85 & 2.60 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1.69 & 43.51 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & EuroStoxx50 & 1.77 & 1.60 & 1.37 & 70.53 & 3.39 \\ 
  GARCH-STD & EuroStoxx50 & 1.85 & 1.80 & 0.70 & 35.15 & 1.70 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.09 & 0.20 & 0.07 & 85.17 & 0.28 \\ 
  GARCH-NORM & EuroStoxx50 & 2.17 & 6.19 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & EuroStoxx50 & 2.33 & 9.38 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.42 & 4.79 & 0.00 & 95.21 & 0.01 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.50 & 3.19 & 0.00 & 96.87 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 1 day ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> source code Version for upload/Tables/Case_1/Archive2/Results_Case1_1Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:34:41 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 2.62 & 34.33 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & S\&P500 & 3.02 & 1.40 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & S\&P500 & 2.38 & 80.44 & 79.19 & 22.60 & 46.40 \\ 
  GARCH-STD & S\&P500 & 3.50 & 0.80 & 3.24 & 93.45 & 9.47 \\ 
  GARCH-NORM & S\&P500 & 3.82 & 1.20 & 0.55 & 99.20 & 2.10 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.43 & 34.53 & 0.83 & 52.45 & 1.62 \\ 
  TGARCH-STD & S\&P500 & 3.90 & 0.00 & 0.33 & 75.52 & 1.02 \\ 
  TGARCH-NORM & S\&P500 & 4.05 & 1.60 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & S\&P500 & 4.53 & 0.20 & 0.00 & 92.48 & 0.02 \\ 
   \hline
\hline
GARCH-SSTD & Nikkei225 & 2.90 & 43.91 & 38.01 & 99.90 & 67.96 \\ 
  TGARCH-SSTD & Nikkei225 & 2.42 & 71.66 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & Nikkei225 & 3.14 & 0.40 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & Nikkei225 & 3.22 & 1.60 & 11.91 & 96.33 & 28.60 \\ 
  EGARCH-NORM & Nikkei225 & 3.22 & 0.40 & 11.91 & 96.33 & 28.60 \\ 
  GARCH-NORM & Nikkei225 & 3.38 & 0.00 & 5.87 & 92.85 & 15.55 \\ 
  GARCH-STD & Nikkei225 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & Nikkei225 & 3.06 & 13.97 & 22.21 & 12.14 & 14.30 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.69 & 73.65 & 5.26 & 14.27 & 2.18 \\ 
  EGARCH-STD & Nikkei225 & 3.86 & 0.20 & 0.43 & 99.42 & 1.68 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.98 & 79.84 & 29.36 & 72.90 & 42.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.22 & 0.00 & 11.91 & 83.46 & 24.78 \\ 
  TGARCH-STD & EuroStoxx50 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.46 & 68.86 & 3.99 & 91.84 & 11.13 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.14 & 29.74 & 16.44 & 11.43 & 4.35 \\ 
  GARCH-STD & EuroStoxx50 & 3.70 & 5.19 & 1.11 & 97.42 & 3.88 \\ 
  GARCH-NORM & EuroStoxx50 & 3.95 & 5.59 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & EuroStoxx50 & 4.27 & 1.20 & 0.03 & 88.73 & 0.12 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.51 & 1.40 & 0.00 & 95.50 & 0.02 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.59 & 1.60 & 0.00 & 97.11 & 0.01 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 1 day ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> source code Version for upload/Tables/Case_1/Archive2/Results_Case1_1Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Sep 01 15:34:41 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 5.01 & 57.49 & 98.97 & 89.07 & 89.06 \\ 
  GARCH-NORM & S\&P500 & 5.72 & 0.00 & 24.94 & 99.79 & 51.40 \\ 
  TGARCH-SSTD & S\&P500 & 5.41 & 87.82 & 51.47 & 60.38 & 48.83 \\ 
  GARCH-STD & S\&P500 & 5.80 & 2.20 & 20.21 & 99.23 & 43.99 \\ 
  SVR-GARCH-KDE & S\&P500 & 4.37 & 24.95 & 29.68 & 30.25 & 17.55 \\ 
  EGARCH-SSTD & S\&P500 & 6.44 & 1.20 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & S\&P500 & 6.60 & 0.40 & 1.30 & 77.88 & 3.56 \\ 
  EGARCH-NORM & S\&P500 & 6.76 & 1.00 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & S\&P500 & 6.76 & 0.00 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 7.00 & 0.80 & 0.21 & 87.46 & 0.78 \\ 
   \hline
\hline
EGARCH-SSTD & Nikkei225 & 5.23 & 15.17 & 70.78 & 97.26 & 90.66 \\ 
  SVR-GARCH-KDE & Nikkei225 & 4.59 & 27.74 & 50.10 & 97.11 & 77.43 \\ 
  TGARCH-SSTD & Nikkei225 & 4.67 & 94.81 & 58.95 & 89.41 & 77.30 \\ 
  GARCH-SSTD & Nikkei225 & 5.07 & 34.93 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & Nikkei225 & 5.23 & 0.20 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & Nikkei225 & 5.56 & 0.20 & 37.71 & 89.62 & 60.67 \\ 
  GARCH-NORM & Nikkei225 & 5.88 & 4.99 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & Nikkei225 & 5.72 & 0.60 & 25.68 & 49.18 & 25.85 \\ 
  GARCH-STD & Nikkei225 & 6.04 & 0.00 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & Nikkei225 & 6.04 & 0.60 & 10.34 & 71.98 & 19.11 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 5.15 & 89.62 & 80.55 & 65.27 & 63.32 \\ 
  GARCH-SSTD & EuroStoxx50 & 5.96 & 57.29 & 13.21 & 95.83 & 30.84 \\ 
  GARCH-NORM & EuroStoxx50 & 5.96 & 48.90 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.04 & 2.59 & 10.34 & 78.10 & 20.73 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 5.48 & 33.53 & 44.90 & 26.86 & 20.17 \\ 
  EGARCH-SSTD & EuroStoxx50 & 6.12 & 1.40 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & EuroStoxx50 & 6.20 & 0.00 & 6.11 & 59.29 & 10.26 \\ 
  EGARCH-NORM & EuroStoxx50 & 6.52 & 1.80 & 1.85 & 99.10 & 6.18 \\ 
  GARCH-STD & EuroStoxx50 & 6.60 & 3.99 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & EuroStoxx50 & 6.84 & 0.80 & 0.46 & 69.51 & 1.27 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for 1 day ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> source code Version for upload/Tables/Case_1/Results_Case1_10Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:07:04 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 1.03 & 11.78 & 90.58 & 30.09 & 29.88 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.95 & 94.01 & 86.85 & 25.94 & 25.59 \\ 
  GARCH-SSTD & S\&P500 & 1.19 & 10.38 & 50.57 & 3.91 & 3.14 \\ 
  TGARCH-STD & S\&P500 & 1.99 & 1.80 & 0.19 & 25.26 & 0.21 \\ 
  GARCH-STD & S\&P500 & 1.99 & 2.99 & 0.19 & 25.26 & 0.21 \\ 
  TGARCH-NORM & S\&P500 & 2.31 & 3.59 & 0.01 & 39.72 & 0.01 \\ 
  GARCH-NORM & S\&P500 & 2.54 & 3.39 & 0.00 & 51.83 & 0.00 \\ 
  EGARCH-STD & S\&P500 & 2.78 & 0.00 & 0.00 & 64.14 & 0.00 \\ 
  EGARCH-SSTD & S\&P500 & 2.70 & 0.80 & 0.00 & 4.50 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 3.26 & 0.60 & 0.00 & 14.87 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.45 & 3.19 & 13.59 & 52.97 & 17.42 \\ 
  GARCH-SSTD & Nikkei225 & 1.45 & 2.40 & 13.59 & 52.97 & 17.42 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.32 & 57.29 & 0.51 & 87.23 & 1.97 \\ 
  GARCH-STD & Nikkei225 & 1.85 & 0.80 & 0.70 & 19.57 & 0.51 \\ 
  TGARCH-STD & Nikkei225 & 1.93 & 1.80 & 0.34 & 22.56 & 0.31 \\ 
  GARCH-NORM & Nikkei225 & 2.01 & 1.80 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-NORM & Nikkei225 & 2.09 & 2.20 & 0.07 & 5.45 & 0.02 \\ 
  EGARCH-STD & Nikkei225 & 3.95 & 0.20 & 0.00 & 75.92 & 0.00 \\ 
  EGARCH-SSTD & Nikkei225 & 2.50 & 1.20 & 0.00 & 48.53 & 0.00 \\ 
  EGARCH-NORM & Nikkei225 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 0.97 & 64.07 & 90.41 & 62.85 & 88.31 \\ 
  GARCH-SSTD & EuroStoxx50 & 2.01 & 8.78 & 0.16 & 25.77 & 0.18 \\ 
  TGARCH-SSTD & EuroStoxx50 & 2.33 & 5.99 & 0.01 & 40.43 & 0.01 \\ 
  TGARCH-STD & EuroStoxx50 & 2.58 & 4.99 & 0.00 & 15.65 & 0.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.66 & 4.79 & 0.00 & 18.07 & 0.00 \\ 
  GARCH-STD & EuroStoxx50 & 2.33 & 5.79 & 0.01 & 9.64 & 0.00 \\ 
  GARCH-NORM & EuroStoxx50 & 2.58 & 0.80 & 0.00 & 15.65 & 0.00 \\ 
  EGARCH-STD & EuroStoxx50 & 4.03 & 1.40 & 0.00 & 17.32 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 3.70 & 1.80 & 0.00 & 2.49 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 3.30 & 0.20 & 0.00 & 44.47 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for ten-days-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_1}
\end{table}


==> source code Version for upload/Tables/Case_1/Results_Case1_10Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:07:04 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-SSTD & S\&P500 & 2.62 & 13.57 & 78.12 & 55.96 & 53.84 \\ 
  GARCH-SSTD & S\&P500 & 2.78 & 6.99 & 52.88 & 22.94 & 18.81 \\ 
  GARCH-STD & S\&P500 & 3.18 & 3.39 & 13.82 & 39.68 & 13.22 \\ 
  TGARCH-STD & S\&P500 & 3.42 & 0.20 & 4.80 & 51.32 & 7.27 \\ 
  GARCH-NORM & S\&P500 & 3.58 & 2.79 & 2.14 & 59.33 & 4.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.75 & 95.21 & 7.15 & 16.45 & 3.24 \\ 
  TGARCH-NORM & S\&P500 & 3.58 & 0.40 & 2.14 & 25.03 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 30.25 & 0.02 \\ 
  EGARCH-SSTD & S\&P500 & 4.77 & 0.20 & 0.00 & 22.74 & 0.00 \\ 
  EGARCH-NORM & S\&P500 & 4.61 & 0.20 & 0.00 & 17.75 & 0.00 \\ 
   \hline
\hline
GARCH-STD & Nikkei225 & 2.74 & 0.20 & 59.74 & 60.95 & 53.02 \\ 
  GARCH-SSTD & Nikkei225 & 2.25 & 8.58 & 57.31 & 36.53 & 31.17 \\ 
  GARCH-NORM & Nikkei225 & 3.30 & 0.00 & 8.45 & 86.53 & 19.54 \\ 
  TGARCH-SSTD & Nikkei225 & 2.74 & 0.00 & 59.74 & 20.72 & 18.02 \\ 
  TGARCH-STD & Nikkei225 & 3.06 & 0.00 & 22.21 & 33.30 & 15.80 \\ 
  TGARCH-NORM & Nikkei225 & 3.46 & 0.00 & 3.99 & 52.40 & 6.35 \\ 
  EGARCH-SSTD & Nikkei225 & 4.03 & 0.40 & 0.15 & 43.03 & 0.28 \\ 
  EGARCH-NORM & Nikkei225 & 4.11 & 0.00 & 0.09 & 46.87 & 0.19 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.29 & 48.10 & 0.26 & 5.17 & 0.06 \\ 
  EGARCH-STD & Nikkei225 & 5.31 & 0.20 & 0.00 & 96.40 & 0.00 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 3.22 & 50.30 & 11.91 & 40.62 & 12.06 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.30 & 50.10 & 8.45 & 44.47 & 10.04 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.38 & 9.38 & 5.87 & 48.40 & 8.11 \\ 
  GARCH-STD & EuroStoxx50 & 3.46 & 8.78 & 3.99 & 52.40 & 6.35 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.06 & 85.03 & 22.21 & 9.73 & 4.61 \\ 
  TGARCH-STD & EuroStoxx50 & 3.46 & 13.77 & 3.99 & 20.23 & 2.45 \\ 
  GARCH-NORM & EuroStoxx50 & 3.78 & 0.20 & 0.70 & 68.40 & 1.80 \\ 
  EGARCH-STD & EuroStoxx50 & 5.88 & 0.40 & 0.00 & 43.78 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.91 & 0.20 & 0.00 & 3.67 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.83 & 0.00 & 0.00 & 23.77 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for ten-days-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_2.5}
\end{table}


==> source code Version for upload/Tables/Case_1/Results_Case1_10Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:07:04 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
TGARCH-NORM & S\&P500 & 5.09 & 1.20 & 88.72 & 34.98 & 34.63 \\ 
  TGARCH-STD & S\&P500 & 5.01 & 0.00 & 98.97 & 31.66 & 31.66 \\ 
  GARCH-SSTD & S\&P500 & 4.29 & 2.20 & 23.85 & 57.38 & 28.64 \\ 
  GARCH-STD & S\&P500 & 5.17 & 0.00 & 78.70 & 17.88 & 17.24 \\ 
  TGARCH-SSTD & S\&P500 & 4.21 & 4.39 & 18.86 & 24.22 & 10.20 \\ 
  GARCH-NORM & S\&P500 & 5.48 & 0.00 & 43.69 & 4.89 & 3.62 \\ 
  EGARCH-NORM & S\&P500 & 6.52 & 0.00 & 1.80 & 29.69 & 1.81 \\ 
  EGARCH-STD & S\&P500 & 6.60 & 0.00 & 1.30 & 32.87 & 1.50 \\ 
  SVR-GARCH-KDE & S\&P500 & 3.34 & 56.89 & 0.41 & 17.11 & 0.28 \\ 
  EGARCH-SSTD & S\&P500 & 7.23 & 0.00 & 0.06 & 62.62 & 0.18 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 5.23 & 10.18 & 70.78 & 94.63 & 88.21 \\ 
  GARCH-SSTD & Nikkei225 & 4.99 & 21.16 & 98.96 & 87.41 & 87.40 \\ 
  TGARCH-STD & Nikkei225 & 5.31 & 8.18 & 61.51 & 72.91 & 64.25 \\ 
  TGARCH-NORM & Nikkei225 & 5.31 & 12.18 & 61.51 & 72.91 & 64.25 \\ 
  GARCH-NORM & Nikkei225 & 5.72 & 5.99 & 25.68 & 99.95 & 52.55 \\ 
  GARCH-STD & Nikkei225 & 5.72 & 8.18 & 25.68 & 89.19 & 46.89 \\ 
  SVR-GARCH-KDE & Nikkei225 & 3.95 & 88.82 & 7.70 & 75.92 & 15.90 \\ 
  EGARCH-SSTD & Nikkei225 & 6.36 & 0.60 & 3.44 & 90.35 & 9.65 \\ 
  EGARCH-NORM & Nikkei225 & 6.12 & 3.59 & 7.99 & 31.60 & 6.82 \\ 
  EGARCH-STD & Nikkei225 & 7.97 & 0.00 & 0.00 & 91.62 & 0.00 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 5.07 & 50.10 & 90.69 & 61.34 & 60.92 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.12 & 2.59 & 7.99 & 6.55 & 1.41 \\ 
  TGARCH-SSTD & EuroStoxx50 & 6.12 & 4.99 & 7.99 & 2.43 & 0.53 \\ 
  TGARCH-STD & EuroStoxx50 & 6.36 & 0.00 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-NORM & EuroStoxx50 & 6.36 & 2.20 & 3.44 & 4.28 & 0.46 \\ 
  GARCH-SSTD & EuroStoxx50 & 6.52 & 2.99 & 1.85 & 6.06 & 0.38 \\ 
  GARCH-STD & EuroStoxx50 & 6.76 & 0.40 & 0.67 & 9.76 & 0.25 \\ 
  EGARCH-STD & EuroStoxx50 & 9.10 & 0.20 & 0.00 & 1.03 & 0.00 \\ 
  EGARCH-SSTD & EuroStoxx50 & 7.41 & 0.20 & 0.03 & 0.13 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 & 7.17 & 0.60 & 0.10 & 0.18 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for ten-days-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_10days_5}
\end{table}


==> source code Version for upload/Tables/Case_1/Results_Case1_1Day_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:04:49 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
EGARCH-SSTD & S\&P500 & 1.11 & 4.99 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & S\&P500 & 0.72 & 92.22 & 28.52 & 71.87 & 52.94 \\ 
  GARCH-SSTD & S\&P500 & 1.27 & 20.76 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & S\&P500 & 1.43 & 0.20 & 14.91 & 46.97 & 27.20 \\ 
  SVR-GARCH-KDE & S\&P500 & 0.79 & 29.34 & 44.83 & 18.28 & 13.71 \\ 
  GARCH-STD & S\&P500 & 1.67 & 16.17 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & S\&P500 & 1.75 & 5.79 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & S\&P500 & 2.15 & 3.39 & 0.04 & 27.64 & 0.10 \\ 
  EGARCH-NORM & S\&P500 & 2.23 & 2.40 & 0.02 & 25.88 & 0.04 \\ 
  GARCH-NORM & S\&P500 & 2.38 & 0.20 & 0.00 & 94.85 & 0.01 \\ 
   \hline
\hline
TGARCH-SSTD & Nikkei225 & 1.21 & 4.99 & 47.61 & 54.48 & 64.58 \\ 
  GARCH-SSTD & Nikkei225 & 1.21 & 2.79 & 47.61 & 54.48 & 64.58 \\ 
  EGARCH-SSTD & Nikkei225 & 1.37 & 4.19 & 21.61 & 49.21 & 36.76 \\ 
  GARCH-STD & Nikkei225 & 1.69 & 1.80 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & Nikkei225 & 1.77 & 1.00 & 1.37 & 37.30 & 3.23 \\ 
  SVR-GARCH-KDE & Nikkei225 & 0.24 & 59.48 & 0.13 & 90.41 & 0.55 \\ 
  EGARCH-STD & Nikkei225 & 2.09 & 0.80 & 0.07 & 29.17 & 0.19 \\ 
  GARCH-NORM & Nikkei225 & 2.17 & 0.40 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & Nikkei225 & 2.33 & 0.20 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & Nikkei225 & 2.42 & 0.20 & 0.00 & 95.21 & 0.01 \\ 
   \hline
\hline
SVR-GARCH-KDE & EuroStoxx50 & 1.53 & 76.25 & 8.17 & 44.23 & 16.36 \\ 
  GARCH-SSTD & EuroStoxx50 & 1.69 & 72.85 & 2.60 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & EuroStoxx50 & 1.69 & 43.51 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & EuroStoxx50 & 1.77 & 1.60 & 1.37 & 70.53 & 3.39 \\ 
  GARCH-STD & EuroStoxx50 & 1.85 & 1.80 & 0.70 & 35.15 & 1.70 \\ 
  TGARCH-NORM & EuroStoxx50 & 2.09 & 0.20 & 0.07 & 85.17 & 0.28 \\ 
  GARCH-NORM & EuroStoxx50 & 2.17 & 6.19 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & EuroStoxx50 & 2.33 & 9.38 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & EuroStoxx50 & 2.42 & 4.79 & 0.00 & 95.21 & 0.01 \\ 
  EGARCH-NORM & EuroStoxx50 & 2.50 & 3.19 & 0.00 & 96.87 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for one-day-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> source code Version for upload/Tables/Case_1/Results_Case1_1Day_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:04:49 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 2.62 & 34.33 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & S\&P500 & 3.02 & 1.40 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & S\&P500 & 2.38 & 80.44 & 79.19 & 22.60 & 46.40 \\ 
  GARCH-STD & S\&P500 & 3.50 & 0.80 & 3.24 & 93.45 & 9.47 \\ 
  GARCH-NORM & S\&P500 & 3.82 & 1.20 & 0.55 & 99.20 & 2.10 \\ 
  SVR-GARCH-KDE & S\&P500 & 1.43 & 34.53 & 0.83 & 52.45 & 1.62 \\ 
  TGARCH-STD & S\&P500 & 3.90 & 0.00 & 0.33 & 75.52 & 1.02 \\ 
  TGARCH-NORM & S\&P500 & 4.05 & 1.60 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & S\&P500 & 4.37 & 0.00 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & S\&P500 & 4.53 & 0.20 & 0.00 & 92.48 & 0.02 \\ 
   \hline
\hline
GARCH-SSTD & Nikkei225 & 2.90 & 43.91 & 38.01 & 99.90 & 67.96 \\ 
  TGARCH-SSTD & Nikkei225 & 2.42 & 71.66 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & Nikkei225 & 3.14 & 0.40 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & Nikkei225 & 3.22 & 1.60 & 11.91 & 96.33 & 28.60 \\ 
  EGARCH-NORM & Nikkei225 & 3.22 & 0.40 & 11.91 & 96.33 & 28.60 \\ 
  GARCH-NORM & Nikkei225 & 3.38 & 0.00 & 5.87 & 92.85 & 15.55 \\ 
  GARCH-STD & Nikkei225 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & Nikkei225 & 3.06 & 13.97 & 22.21 & 12.14 & 14.30 \\ 
  SVR-GARCH-KDE & Nikkei225 & 1.69 & 73.65 & 5.26 & 14.27 & 2.18 \\ 
  EGARCH-STD & Nikkei225 & 3.86 & 0.20 & 0.43 & 99.42 & 1.68 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 2.98 & 79.84 & 29.36 & 72.90 & 42.00 \\ 
  TGARCH-NORM & EuroStoxx50 & 3.22 & 0.00 & 11.91 & 83.46 & 24.78 \\ 
  TGARCH-STD & EuroStoxx50 & 3.38 & 0.00 & 5.87 & 89.33 & 14.96 \\ 
  GARCH-SSTD & EuroStoxx50 & 3.46 & 68.86 & 3.99 & 91.84 & 11.13 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 3.14 & 29.74 & 16.44 & 11.43 & 4.35 \\ 
  GARCH-STD & EuroStoxx50 & 3.70 & 5.19 & 1.11 & 97.42 & 3.88 \\ 
  GARCH-NORM & EuroStoxx50 & 3.95 & 5.59 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & EuroStoxx50 & 4.27 & 1.20 & 0.03 & 88.73 & 0.12 \\ 
  EGARCH-SSTD & EuroStoxx50 & 4.51 & 1.40 & 0.00 & 95.50 & 0.02 \\ 
  EGARCH-NORM & EuroStoxx50 & 4.59 & 1.60 & 0.00 & 97.11 & 0.01 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for one-day-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> source code Version for upload/Tables/Case_1/Results_Case1_1Day_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Tue Sep 03 09:04:49 2019
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
\textbf{Model} & \textbf{Index} & \textbf{Violations} & \textbf{SPA} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
GARCH-SSTD & S\&P500 & 5.01 & 57.49 & 98.97 & 89.07 & 89.06 \\ 
  GARCH-NORM & S\&P500 & 5.72 & 0.00 & 24.94 & 99.79 & 51.40 \\ 
  TGARCH-SSTD & S\&P500 & 5.41 & 87.82 & 51.47 & 60.38 & 48.83 \\ 
  GARCH-STD & S\&P500 & 5.80 & 2.20 & 20.21 & 99.23 & 43.99 \\ 
  SVR-GARCH-KDE & S\&P500 & 4.37 & 24.95 & 29.68 & 30.25 & 17.55 \\ 
  EGARCH-SSTD & S\&P500 & 6.44 & 1.20 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & S\&P500 & 6.60 & 0.40 & 1.30 & 77.88 & 3.56 \\ 
  EGARCH-NORM & S\&P500 & 6.76 & 1.00 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & S\&P500 & 6.76 & 0.00 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & S\&P500 & 7.00 & 0.80 & 0.21 & 87.46 & 0.78 \\ 
   \hline
\hline
EGARCH-SSTD & Nikkei225 & 5.23 & 15.17 & 70.78 & 97.26 & 90.66 \\ 
  SVR-GARCH-KDE & Nikkei225 & 4.59 & 27.74 & 50.10 & 97.11 & 77.43 \\ 
  TGARCH-SSTD & Nikkei225 & 4.67 & 94.81 & 58.95 & 89.41 & 77.30 \\ 
  GARCH-SSTD & Nikkei225 & 5.07 & 34.93 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & Nikkei225 & 5.23 & 0.20 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & Nikkei225 & 5.56 & 0.20 & 37.71 & 89.62 & 60.67 \\ 
  GARCH-NORM & Nikkei225 & 5.88 & 4.99 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & Nikkei225 & 5.72 & 0.60 & 25.68 & 49.18 & 25.85 \\ 
  GARCH-STD & Nikkei225 & 6.04 & 0.00 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & Nikkei225 & 6.04 & 0.60 & 10.34 & 71.98 & 19.11 \\ 
   \hline
\hline
TGARCH-SSTD & EuroStoxx50 & 5.15 & 89.62 & 80.55 & 65.27 & 63.32 \\ 
  GARCH-SSTD & EuroStoxx50 & 5.96 & 57.29 & 13.21 & 95.83 & 30.84 \\ 
  GARCH-NORM & EuroStoxx50 & 5.96 & 48.90 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & EuroStoxx50 & 6.04 & 2.59 & 10.34 & 78.10 & 20.73 \\ 
  SVR-GARCH-KDE & EuroStoxx50 & 5.48 & 33.53 & 44.90 & 26.86 & 20.17 \\ 
  EGARCH-SSTD & EuroStoxx50 & 6.12 & 1.40 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & EuroStoxx50 & 6.20 & 0.00 & 6.11 & 59.29 & 10.26 \\ 
  EGARCH-NORM & EuroStoxx50 & 6.52 & 1.80 & 1.85 & 99.10 & 6.18 \\ 
  GARCH-STD & EuroStoxx50 & 6.60 & 3.99 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & EuroStoxx50 & 6.84 & 0.80 & 0.46 & 69.51 & 1.27 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Results for one-day-ahead VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID, CC and SPA indicate the p-value of the corresponding test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID, CC and SPA are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> source code Version for upload/Tables/Case_1Results_Case1_EuroStoxx50.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Jan 28 15:27:23 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 0.79 & 17.22 & 18.28 & 7.2 \\ 
  TGARCH-STD & 0.5 & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  TGARCH-SSTD & 0.5 & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  SGARCH-STD & 0.5 & 1.21 & 0.28 & 54.48 & 0.95 \\ 
  EGARCH-STD & 0.5 & 1.29 & 0.1 & 43.8 & 0.2 \\ 
  SGARCH-SSTD & 0.5 & 1.37 & 0.04 & 49.21 & 0.13 \\ 
  TGARCH-NORM & 0.5 & 1.45 & 0.01 & 46.68 & 0.05 \\ 
  SGARCH-NORM & 0.5 & 1.53 & 0 & 44.23 & 0.01 \\ 
  EGARCH-SSTD & 0.5 & 1.61 & 0 & 61.98 & 0 \\ 
  EGARCH-NORM & 0.5 & 1.93 & 0 & 78.34 & 0 \\ 
   \hline
\hline
SGARCH-SSTD & 1 & 1.69 & 2.6 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & 1 & 1.69 & 2.6 & 66.33 & 5.56 \\ 
  TGARCH-STD & 1 & 1.77 & 1.37 & 70.53 & 3.39 \\ 
  SGARCH-STD & 1 & 1.85 & 0.7 & 35.15 & 1.7 \\ 
  SVM-KDE & 1 & 1.91 & 0.4 & 77.78 & 1.24 \\ 
  TGARCH-NORM & 1 & 2.09 & 0.07 & 85.17 & 0.28 \\ 
  SGARCH-NORM & 1 & 2.17 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & 1 & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & 1 & 2.42 & 0 & 95.21 & 0.01 \\ 
  EGARCH-NORM & 1 & 2.5 & 0 & 96.87 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & 2.5 & 2.98 & 29.36 & 72.9 & 42 \\ 
  TGARCH-NORM & 2.5 & 3.22 & 11.91 & 83.46 & 24.78 \\ 
  SVM-KDE & 2.5 & 3.1 & 18.85 & 36.01 & 15.17 \\ 
  TGARCH-STD & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  SGARCH-SSTD & 2.5 & 3.46 & 3.99 & 91.84 & 11.13 \\ 
  SGARCH-STD & 2.5 & 3.7 & 1.11 & 97.42 & 3.88 \\ 
  SGARCH-NORM & 2.5 & 3.95 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & 2.5 & 4.35 & 0.02 & 91.29 & 0.07 \\ 
  EGARCH-SSTD & 2.5 & 4.51 & 0 & 95.5 & 0.02 \\ 
  EGARCH-NORM & 2.5 & 4.59 & 0 & 97.11 & 0.01 \\ 
   \hline
\hline
TGARCH-SSTD & 5 & 5.15 & 80.55 & 65.27 & 63.32 \\ 
  SGARCH-SSTD & 5 & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  SGARCH-NORM & 5 & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & 5 & 6.04 & 10.34 & 78.1 & 20.73 \\ 
  EGARCH-SSTD & 5 & 6.12 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & 5 & 6.2 & 6.11 & 59.29 & 10.26 \\ 
  SVM-KDE & 5 & 4.69 & 61.03 & 7.46 & 6.56 \\ 
  EGARCH-NORM & 5 & 6.52 & 1.85 & 99.1 & 6.18 \\ 
  SGARCH-STD & 5 & 6.6 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & 5 & 6.84 & 0.46 & 69.51 & 1.27 \\ 
  \end{tabular}
\caption{Results for the VaR forecasts from 1 July 2011 to 30 June 2016 for EuroStoxx50.} 
\end{table}


==> source code Version for upload/Tables/Case_1Results_Case1_Nikkei225.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Jan 28 15:27:23 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
SGARCH-SSTD & 0.5 & 0.48 & 93.23 & 80.93 & 96.78 \\ 
  EGARCH-SSTD & 0.5 & 0.56 & 75.55 & 77.82 & 91.56 \\ 
  TGARCH-SSTD & 0.5 & 0.64 & 49.07 & 74.74 & 74.87 \\ 
  SVM-KDE & 0.5 & 0.24 & 15.09 & 90.41 & 35.39 \\ 
  TGARCH-STD & 0.5 & 0.81 & 16.15 & 68.7 & 34.6 \\ 
  SGARCH-STD & 0.5 & 0.81 & 16.15 & 68.7 & 34.6 \\ 
  EGARCH-STD & 0.5 & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  SGARCH-NORM & 0.5 & 1.45 & 0.01 & 52.97 & 0.03 \\ 
  TGARCH-NORM & 0.5 & 1.61 & 0 & 41.84 & 0 \\ 
  EGARCH-NORM & 0.5 & 1.61 & 0 & 41.84 & 0 \\ 
   \hline
\hline
TGARCH-SSTD & 1 & 1.21 & 47.61 & 54.48 & 64.58 \\ 
  SGARCH-SSTD & 1 & 1.21 & 47.61 & 54.48 & 64.58 \\ 
  SVM-KDE & 1 & 0.64 & 17.76 & 74.74 & 38.26 \\ 
  EGARCH-SSTD & 1 & 1.37 & 21.61 & 49.21 & 36.76 \\ 
  SGARCH-STD & 1 & 1.69 & 2.6 & 66.33 & 5.56 \\ 
  TGARCH-STD & 1 & 1.77 & 1.37 & 37.3 & 3.23 \\ 
  EGARCH-STD & 1 & 2.09 & 0.07 & 29.17 & 0.19 \\ 
  SGARCH-NORM & 1 & 2.17 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & 1 & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & 1 & 2.42 & 0 & 95.21 & 0.01 \\ 
   \hline
\hline
SGARCH-SSTD & 2.5 & 2.9 & 38.01 & 99.9 & 67.96 \\ 
  TGARCH-SSTD & 2.5 & 2.42 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & 2.5 & 3.14 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 \\ 
  EGARCH-NORM & 2.5 & 3.22 & 11.91 & 96.33 & 28.6 \\ 
  SGARCH-NORM & 2.5 & 3.38 & 5.87 & 92.85 & 15.55 \\ 
  SGARCH-STD & 2.5 & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & 2.5 & 3.06 & 22.21 & 12.14 & 14.3 \\ 
  SVM-KDE & 2.5 & 2.42 & 84.78 & 11.43 & 11.23 \\ 
  EGARCH-STD & 2.5 & 3.86 & 0.43 & 99.42 & 1.68 \\ 
   \hline
\hline
EGARCH-SSTD & 5 & 5.23 & 70.78 & 97.26 & 90.66 \\ 
  SVM-KDE & 5 & 5.23 & 70.78 & 94.63 & 88.21 \\ 
  TGARCH-SSTD & 5 & 4.67 & 58.95 & 89.41 & 77.3 \\ 
  SGARCH-SSTD & 5 & 5.07 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & 5 & 5.23 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & 5 & 5.56 & 37.71 & 89.62 & 60.67 \\ 
  SGARCH-NORM & 5 & 5.88 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & 5 & 5.72 & 25.68 & 49.18 & 25.85 \\ 
  SGARCH-STD & 5 & 6.04 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & 5 & 6.04 & 10.34 & 71.98 & 19.11 \\ 
  \end{tabular}
\caption{Results for the VaR forecasts from 1 July 2011 to 30 June 2016 for Nikkei225.} 
\end{table}


==> source code Version for upload/Tables/Case_1Results_Case1_SP500.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Jan 28 15:27:23 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
\hline
EGARCH-SSTD & 0.5 & 0.4 & 59.27 & 84.17 & 84.96 \\ 
  SVM-KDE & 0.5 & 0.63 & 53.09 & 75.03 & 78.11 \\ 
  TGARCH-SSTD & 0.5 & 0.32 & 32.65 & 87.31 & 61.01 \\ 
  SGARCH-SSTD & 0.5 & 0.72 & 30.91 & 71.87 & 55.87 \\ 
  TGARCH-STD & 0.5 & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  EGARCH-STD & 0.5 & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  TGARCH-NORM & 0.5 & 1.11 & 0.8 & 57.46 & 2.54 \\ 
  SGARCH-STD & 0.5 & 1.11 & 0.8 & 57.46 & 2.54 \\ 
  SGARCH-NORM & 0.5 & 1.67 & 0 & 65.77 & 0 \\ 
  EGARCH-NORM & 0.5 & 1.67 & 0 & 39.84 & 0 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.02 & 93.73 & 60.44 & 87.17 \\ 
  EGARCH-SSTD & 1 & 1.11 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & 1 & 0.72 & 28.52 & 71.87 & 52.94 \\ 
  SGARCH-SSTD & 1 & 1.27 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & 1 & 1.43 & 14.91 & 46.97 & 27.2 \\ 
  SGARCH-STD & 1 & 1.67 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & 1 & 1.75 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & 1 & 2.15 & 0.04 & 27.64 & 0.1 \\ 
  EGARCH-NORM & 1 & 2.23 & 0.02 & 25.88 & 0.04 \\ 
  SGARCH-NORM & 1 & 2.38 & 0 & 94.85 & 0.01 \\ 
   \hline
\hline
SGARCH-SSTD & 2.5 & 2.62 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & 2.5 & 3.02 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & 2.5 & 2.38 & 79.19 & 22.6 & 46.4 \\ 
  SGARCH-STD & 2.5 & 3.5 & 3.24 & 93.45 & 9.47 \\ 
  SGARCH-NORM & 2.5 & 3.82 & 0.55 & 99.2 & 2.1 \\ 
  TGARCH-STD & 2.5 & 3.9 & 0.33 & 75.52 & 1.02 \\ 
  SVM-KDE & 2.5 & 1.57 & 2.31 & 11.5 & 0.87 \\ 
  TGARCH-NORM & 2.5 & 4.05 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & 2.5 & 4.37 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & 2.5 & 4.53 & 0 & 92.48 & 0.02 \\ 
   \hline
\hline
SGARCH-SSTD & 5 & 5.01 & 98.97 & 89.07 & 89.06 \\ 
  SGARCH-NORM & 5 & 5.72 & 24.94 & 99.79 & 51.4 \\ 
  TGARCH-SSTD & 5 & 5.41 & 51.47 & 60.38 & 48.83 \\ 
  SGARCH-STD & 5 & 5.8 & 20.21 & 99.23 & 43.99 \\ 
  EGARCH-SSTD & 5 & 6.44 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & 5 & 6.6 & 1.3 & 77.88 & 3.56 \\ 
  EGARCH-NORM & 5 & 6.76 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & 5 & 6.76 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & 5 & 7 & 0.21 & 87.46 & 0.78 \\ 
  SVM-KDE & 5 & 4.72 & 64.02 & 0 & 0 \\ 
  \end{tabular}
\caption{Results for the VaR forecasts from 1 July 2011 to 30 June 2016 for Standard and Poors 500.} 
\end{table}


==> source code Version for upload/Tables/Descriptive_Statistics.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Feb 03 16:35:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
  \hline
  \hline
\textbf{Index} & \textbf{1st Quartile} & \textbf{Mean} & \textbf{Median} & \textbf{3rd Quartile} & \textbf{Variance} & \textbf{Skewness} & \textbf{Kurtosis} \\ 
  \hline
EuroStoxx50 & -0.74 & -0.01 & 0.01 & 0.78 & 2.39 & -0.06 & 5.15 \\ 
  S\&P500 & -0.46 & 0.02 & 0.07 & 0.59 & 1.74 & -0.33 & 9.94 \\ 
  Nikkei225 & -0.76 & 0.00 & 0.05 & 0.88 & 2.68 & -0.51 & 7.49 \\ 
   \hline
    \hline
\end{tabular}
\caption{Descriptive statistics for the log-returns of the analyzed
                      indices in the period from July 1, 2006 to June 30, 2016. Note that the log-returns were multiplied by 100
                      before computing the descriptive statistics.} 
\label{Tab:desc_stats}
\end{table}


==> source code Version for upload/Tables/Descriptive_Statistics_Adjusted.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Feb 03 16:35:24 2019
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c|c}
  \hline
  \hline
\textbf{Index} & \textbf{1st Quartile} & \textbf{Mean} & \textbf{Median} & \textbf{3rd Quartile} & \textbf{Variance} & \textbf{Skewness} & \textbf{Kurtosis} \\ 
  \hline
EuroStoxx50 & -0.74 & -0.01 & 0.01 & 0.78 & 2.39 & -0.06 & 5.15 \\ 
  S\&P500 & -0.46 & 0.02 & 0.07 & 0.59 & 1.74 & -0.33 & 9.94 \\ 
  Nikkei225 & -0.76 & 0.00 & 0.05 & 0.88 & 2.68 & -0.51 & 7.49 \\ 
   \hline
    \hline
\end{tabular}
\caption{Descriptive statistics for the log-returns of the analyzed
                      indices in the period from July 1, 2006 to June 30, 2016. Note that the log-returns were multiplied by 100
                      before computing the descriptive statistics.} 
\label{Tab:desc_stats}
\end{table}


==> source code Version for upload/Tables/Results_Case1_05.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
  \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
EGARCH-SSTD & S\&P500 %%& 0.5 
& 0.40 & 59.27 & 84.17 & 84.96 \\ 
  TGARCH-SSTD & S\&P500 %& 0.5 
  & 0.32 & 32.65 & 87.31 & 61.01 \\ 
  GARCH-SSTD & S\&P500 %& 0.5 
  & 0.72 & 30.91 & 71.87 & 55.87 \\ 
  TGARCH-STD & S\&P500 %& 0.5 
  & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  EGARCH-STD & S\&P500 %& 0.5 
  & 0.79 & 17.22 & 68.89 & 36.35 \\ 
  TGARCH-NORM & S\&P500 %& 0.5 
  & 1.11 & 0.80 & 57.46 & 2.54 \\ 
  GARCH-STD & S\&P500 %& 0.5 
  & 1.11 & 0.80 & 57.46 & 2.54 \\ 
  SVR-GARCH-KDE & S\&P500 %& 0.5 
  & 0.32 & 32.65 & 2.61 & 1.61 \\ 
  GARCH-NORM & S\&P500 %& 0.5 
  & 1.67 & 0.00 & 65.77 & 0.00 \\ 
  EGARCH-NORM & S\&P500 %& 0.5 
  & 1.67 & 0.00 & 39.84 & 0.00 \\ 
   \hline
GARCH-SSTD & Nikkei225 %& 0.5 
& 0.48 & 93.23 & 80.93 & 96.78 \\ 
  EGARCH-SSTD & Nikkei225 %& 0.5 %
  & 0.56 & 75.55 & 77.82 & 91.56 \\ 
  TGARCH-SSTD & Nikkei225 %& 0.5 
  & 0.64 & 49.07 & 74.74 & 74.87 \\ 
  TGARCH-STD & Nikkei225 %& 0.5 
  & 0.81 & 16.15 & 68.70 & 34.60 \\ 
  GARCH-STD & Nikkei225 %& 0.5 
  & 0.81 & 16.15 & 68.70 & 34.60 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 0.5 
  & 0.08 & 0.92 & 96.80 & 3.35 \\ 
  EGARCH-STD & Nikkei225 %& 0.5 
  & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  GARCH-NORM & Nikkei225 %& 0.5 
  & 1.45 & 0.01 & 52.97 & 0.03 \\ 
  TGARCH-NORM & Nikkei225 %& 0.5 
  & 1.61 & 0.00 & 41.84 & 0.00 \\ 
  EGARCH-NORM & Nikkei225 %& 0.5 
  & 1.61 & 0.00 & 41.84 & 0.00 \\ 
   \hline
TGARCH-STD & EuroStoxx50 %& 0.5 
& 1.13 & 0.72 & 57.21 & 2.29 \\ 
  TGARCH-SSTD & EuroStoxx50 %& 0.5 
  & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  SVR-GARCH-KDE & EuroStoxx50 %& 0.5 
  & 1.13 & 0.72 & 57.21 & 2.29 \\ 
  GARCH-STD & EuroStoxx50 %& 0.5 
  & 1.21 & 0.28 & 54.48 & 0.95 \\ 
  EGARCH-STD & EuroStoxx50 %& 0.5 
  & 1.29 & 0.10 & 43.80 & 0.20 \\ 
  GARCH-SSTD & EuroStoxx50 %& 0.5 
  & 1.37 & 0.04 & 49.21 & 0.13 \\ 
  TGARCH-NORM & EuroStoxx50 %& 0.5 
  & 1.45 & 0.01 & 46.68 & 0.05 \\ 
  GARCH-NORM & EuroStoxx50 %& 0.5 
  & 1.53 & 0.00 & 44.23 & 0.01 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 0.5 
  & 1.61 & 0.00 & 61.98 & 0.00 \\ 
  EGARCH-NORM & EuroStoxx50 %& 0.5 
  & 1.93 & 0.00 & 78.34 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.005$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.005$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_0.5}
\end{table}


==> source code Version for upload/Tables/Results_Case1_1.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
    \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
EGARCH-SSTD & S\&P500 %& 1 
& 1.11 & 69.27 & 57.46 & 79.01 \\ 
  TGARCH-SSTD & S\&P500 %& 1 
  & 0.72 & 28.52 & 71.87 & 52.94 \\ 
  GARCH-SSTD & S\&P500 %& 1 
  & 1.27 & 35.24 & 43.34 & 28.13 \\ 
  TGARCH-STD & S\&P500 %& 1 
  & 1.43 & 14.91 & 46.97 & 27.20 \\ 
  SVR-GARCH-KDE & S\&P500 %& 1 
  & 0.79 & 44.83 & 18.28 & 13.71 \\ 
  GARCH-STD & S\&P500 %& 1 
  & 1.67 & 2.95 & 65.77 & 6.15 \\ 
  EGARCH-STD & S\&P500 %& 1 
  & 1.75 & 1.58 & 37.62 & 3.67 \\ 
  TGARCH-NORM & S\&P500 %& 1 
  & 2.15 & 0.04 & 27.64 & 0.10 \\ 
  EGARCH-NORM & S\&P500 %& 1 
  & 2.23 & 0.02 & 25.88 & 0.04 \\ 
  GARCH-NORM & S\&P500 %& 1
  & 2.38 & 0.00 & 94.85 & 0.01 \\ 
   \hline
TGARCH-SSTD & Nikkei225 %& 1 
& 1.21 & 47.61 & 54.48 & 64.58 \\ 
  GARCH-SSTD & Nikkei225 %& 1 
  & 1.21 & 47.61 & 54.48 & 64.58 \\ 
  EGARCH-SSTD & Nikkei225 %& 1 
  & 1.37 & 21.61 & 49.21 & 36.76 \\ 
  GARCH-STD & Nikkei225 %& 1 
  & 1.69 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & Nikkei225 %& 1 
  & 1.77 & 1.37 & 37.30 & 3.23 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 1 
  & 0.24 & 0.13 & 90.41 & 0.55 \\ 
  EGARCH-STD & Nikkei225 %& 1 
  & 2.09 & 0.07 & 29.17 & 0.19 \\ 
  GARCH-NORM & Nikkei225 %& 1 
  & 2.17 & 0.03 & 88.16 & 0.14 \\ 
  TGARCH-NORM & Nikkei225 %& 1 
  & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-NORM & Nikkei225 %& 1 
  & 2.42 & 0.00 & 95.21 & 0.01 \\ 
   \hline
SVR-GARCH-KDE & EuroStoxx50 %& 1 
& 1.53 & 8.17 & 44.23 & 16.36 \\ 
  GARCH-SSTD & EuroStoxx50 %& 1 
  & 1.69 & 2.60 & 39.54 & 5.84 \\ 
  TGARCH-SSTD & EuroStoxx50 %& 1 
  & 1.69 & 2.60 & 66.33 & 5.56 \\ 
  TGARCH-STD & EuroStoxx50 %& 1 
  & 1.77 & 1.37 & 70.53 & 3.39 \\ 
  GARCH-STD & EuroStoxx50 %& 1 
  & 1.85 & 0.70 & 35.15 & 1.70 \\ 
  TGARCH-NORM & EuroStoxx50 %& 1 
  & 2.09 & 0.07 & 85.17 & 0.28 \\ 
  GARCH-NORM & EuroStoxx50 %& 1 
  & 2.17 & 0.03 & 27.33 & 0.08 \\ 
  EGARCH-STD & EuroStoxx50 %& 1 
  & 2.33 & 0.01 & 93.19 & 0.03 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 1 
  & 2.42 & 0.00 & 95.21 & 0.01 \\ 
  EGARCH-NORM & EuroStoxx50 %& 1 
  & 2.50 & 0.00 & 96.87 & 0.00 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.01$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.01$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_1}
\end{table}


==> source code Version for upload/Tables/Results_Case1_25.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
    \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
GARCH-SSTD & S\&P500 %& 2.5 
& 2.62 & 78.12 & 98.97 & 95.22 \\ 
  EGARCH-SSTD & S\&P500 %& 2.5 
  & 3.02 & 25.18 & 98.94 & 51.31 \\ 
  TGARCH-SSTD & S\&P500 %& 2.5 
  & 2.38 & 79.19 & 22.60 & 46.40 \\ 
  GARCH-STD & S\&P500 %& 2.5 
  & 3.50 & 3.24 & 93.45 & 9.47 \\ 
  GARCH-NORM & S\&P500 %& 2.5 
  & 3.82 & 0.55 & 99.2 & 2.10 \\ 
  SVR-GARCH-KDE & S\&P500 %& 2.5 
  & 1.43 & 0.83 & 52.45 & 1.62 \\ 
  TGARCH-STD & S\&P500 %& 2.5 
  & 3.90 & 0.33 & 75.52 & 1.02 \\ 
  TGARCH-NORM & S\&P500 %& 2.5 
  & 4.05 & 0.12 & 69.37 & 0.36 \\ 
  EGARCH-STD & S\&P500 %& 2.5 
  & 4.37 & 0.01 & 96.11 & 0.06 \\ 
  EGARCH-NORM & S\&P500 %& 2.5 
  & 4.53 & 0.00 & 92.48 & 0.02 \\ 
   \hline
GARCH-SSTD & Nikkei225 %& 2.5 
& 2.90 & 38.01 & 99.90 & 67.96 \\ 
  TGARCH-SSTD & Nikkei225 %& 2.5 
  & 2.42 & 84.78 & 22.29 & 46.72 \\ 
  TGARCH-STD & Nikkei225 %& 2.5 
  & 3.14 & 16.44 & 97.67 & 37.15 \\ 
  TGARCH-NORM & Nikkei225 %& 2.5 
  & 3.22 & 11.91 & 96.33 & 28.60 \\ 
  EGARCH-NORM & Nikkei225 %& 2.5 
  & 3.22 & 11.91 & 96.33 & 28.60 \\ 
  GARCH-NORM & Nikkei225 %& 2.5 
  & 3.38 & 5.87 & 92.85 & 15.55 \\ 
  GARCH-STD & Nikkei225 %& 2.5 
  & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  EGARCH-SSTD & Nikkei225 %& 2.5 
  & 3.06 & 22.21 & 12.14 & 14.30 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 2.5 
  & 1.69 & 5.26 & 14.27 & 2.18 \\ 
  EGARCH-STD & Nikkei225 %& 2.5 
  & 3.86 & 0.43 & 99.42 & 1.68 \\ 
   \hline
TGARCH-SSTD & EuroStoxx50 %& 2.5 
& 2.98 & 29.36 & 72.9 & 42.00 \\ 
  TGARCH-NORM & EuroStoxx50 %& 2.5 
  & 3.22 & 11.91 & 83.46 & 24.78 \\ 
  TGARCH-STD & EuroStoxx50 %& 2.5 
  & 3.38 & 5.87 & 89.33 & 14.96 \\ 
  GARCH-SSTD & EuroStoxx50 %& 2.5 
  & 3.46 & 3.99 & 91.84 & 11.13 \\ 
  SVR-GARCH-KDE & EuroStoxx50 %& 2.5 
  & 3.14 & 16.44 & 11.43 & 4.35 \\ 
  GARCH-STD & EuroStoxx50 %& 2.5 
  & 3.70 & 1.11 & 97.42 & 3.88 \\ 
  GARCH-NORM & EuroStoxx50 %& 2.5 
  & 3.95 & 0.26 & 75.92 & 0.81 \\ 
  EGARCH-STD & EuroStoxx50 %& 2.5 
  & 4.35 & 0.02 & 91.29 & 0.07 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 2.5 
  & 4.51 & 0.00 & 95.50 & 0.02 \\ 
  EGARCH-NORM & EuroStoxx50 %& 2.5 
  & 4.59 & 0.00 & 97.11 & 0.01 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.025$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.025$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_2.5}
\end{table}


==> source code Version for upload/Tables/Results_Case1_5.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sat Mar 25 14:11:57 2017
\begin{table}[ht]
\centering
\begingroup\fontsize{11pt}{12pt}\selectfont
\begin{tabular}{l|c|c|r|r|r|r}
  \hline
    \hline
\textbf{Model} & \textbf{Index} %& \textbf{Quantile} 
& \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
GARCH-SSTD & S\&P500 %%& 5
& 5.01 & 98.97 & 89.07 & 89.06 \\ 
  GARCH-NORM & S\&P500 %%& 5 
  & 5.72 & 24.94 & 99.79 & 51.40 \\ 
  TGARCH-SSTD & S\&P500 %& 5 
  & 5.41 & 51.47 & 60.38 & 48.83 \\ 
  GARCH-STD & S\&P500 %& 5 
  & 5.80 & 20.21 & 99.23 & 43.99 \\ 
  SVR-GARCH-KDE & S\&P500 %& 5 
  & 4.37 & 29.68 & 30.25 & 17.55 \\ 
  EGARCH-SSTD & S\&P500 %& 5 
  & 6.44 & 2.47 & 83.92 & 6.73 \\ 
  TGARCH-NORM & S\&P500 %& 5 
  & 6.60 & 1.30 & 77.88 & 3.56 \\ 
  EGARCH-NORM & S\&P500 %& 5 
  & 6.76 & 0.65 & 94.35 & 2.33 \\ 
  TGARCH-STD & S\&P500 %& 5 
  & 6.76 & 0.65 & 71.36 & 1.77 \\ 
  EGARCH-STD & S\&P500 %& 5 
  & 7.00 & 0.21 & 87.46 & 0.78 \\ 
   \hline
EGARCH-SSTD & Nikkei225 %& 5 
& 5.23 & 70.78 & 97.26 & 90.66 \\ 
  SVR-GARCH-KDE & Nikkei225 %& 5 
  & 4.59 & 50.1 & 97.11 & 77.43 \\ 
  TGARCH-SSTD & Nikkei225 %& 5 
  & 4.67 & 58.95 & 89.41 & 77.30 \\ 
  GARCH-SSTD & Nikkei225 %& 5 
  & 5.07 & 90.69 & 75.29 & 74.78 \\ 
  TGARCH-NORM & Nikkei225 %& 5 
  & 5.23 & 70.78 & 68.85 & 64.18 \\ 
  TGARCH-STD & Nikkei225 %& 5 
  & 5.56 & 37.71 & 89.62 & 60.67 \\ 
  GARCH-NORM & Nikkei225 %& 5 
  & 5.88 & 16.68 & 78.41 & 30.16 \\ 
  EGARCH-NORM & Nikkei225 %& 5 
  & 5.72 & 25.68 & 49.18 & 25.85 \\ 
  GARCH-STD & Nikkei225 %& 5 
  & 6.04 & 10.34 & 71.98 & 19.11 \\ 
  EGARCH-STD & Nikkei225 %& 5 
  & 6.04 & 10.34 & 71.98 & 19.11 \\ 
   \hline
TGARCH-SSTD & EuroStoxx50 %& 5 
& 5.15 & 80.55 & 65.27 & 63.32 \\ 
  GARCH-SSTD & EuroStoxx50 %& 5 
  & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  GARCH-NORM & EuroStoxx50 %& 5 
  & 5.96 & 13.21 & 95.83 & 30.84 \\ 
  TGARCH-NORM & EuroStoxx50 %& 5 
  & 6.04 & 10.34 & 78.10 & 20.73 \\ 
  SVR-GARCH-KDE & EuroStoxx50 %& 5 
  & 5.48 & 44.90 & 26.86 & 20.17 \\ 
  EGARCH-SSTD & EuroStoxx50 %& 5 
  & 6.12 & 7.99 & 68.65 & 14.82 \\ 
  TGARCH-STD & EuroStoxx50 %& 5 
  & 6.20 & 6.11 & 59.29 & 10.26 \\ 
  EGARCH-NORM & EuroStoxx50 %& 5 
  & 6.52 & 1.85 & 99.10 & 6.18 \\ 
  GARCH-STD & EuroStoxx50 %& 5 
  & 6.60 & 1.33 & 96.58 & 4.52 \\ 
  EGARCH-STD & EuroStoxx50 %& 5 
  & 6.84 & 0.46 & 69.51 & 1.27 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption[VaR forecast results for $\alpha = 0.05$]{Results for the VaR forecasts from July 1, 2011 to June 30, 2016 for $\alpha =  0.05$. UC, ID and CC indicate the p-value of the corresponding LR test. The results are in descending order with respect to CC for each index. All values in the columns Quantile, Violations, UC, ID and CC are given in percent.} 
\label{Tab:case1_5}
\end{table}


==> source code Version for upload/Tables/Results_EuroStoxx50.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Jan 16 13:55:04 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Exceedances} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{DUR} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 1.63 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 0.5 & 1.37 & 0 & 0 & 0 & 7.23 \\ 
  SGARCH-STD & 0.5 & 0.81 & 0.38 & NaN & NaN & 99.78 \\ 
  SGARCH-SSTD & 0.5 & 0.58 & 45.56 & NaN & NaN & 69.13 \\ 
  EGARCH-NORM & 0.5 & 1.61 & 0 & NaN & NaN & 53.96 \\ 
  EGARCH-STD & 0.5 & 0.97 & 0 & NaN & NaN & 83.03 \\ 
  EGARCH-SSTD & 0.5 & 0.71 & 4.22 & NaN & NaN & 45.85 \\ 
  TGARCH-NORM & 0.5 & 1.33 & 0 & 0 & 0 & 94.27 \\ 
  TGARCH-SSTD & 0.5 & 0.6 & 34.95 & NaN & NaN & 44.76 \\ 
  TGARCH-STD & 0.5 & 0.83 & 0.22 & NaN & NaN & 83.67 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.63 & 0 & 0 & 0.02 & 0 \\ 
  SGARCH-NORM & 1 & 2.42 & 0 & 0 & 0 & 32.76 \\ 
  SGARCH-STD & 1 & 1.55 & 0.03 & 0 & 0.05 & 53.39 \\ 
  SGARCH-SSTD & 1 & 1.31 & 3.44 & 0.22 & 2.02 & 44.87 \\ 
  EGARCH-NORM & 1 & 2.34 & 0 & 0 & 0 & 34.95 \\ 
  EGARCH-STD & 1 & 1.81 & 0 & 0 & 0 & 81.29 \\ 
  EGARCH-SSTD & 1 & 1.15 & 29.01 & 30.34 & 53.1 & 99.68 \\ 
  TGARCH-NORM & 1 & 2.14 & 0 & 0 & 0 & 99.92 \\ 
  TGARCH-SSTD & 1 & 0.99 & 96.04 & 81.53 & 81.63 & 58.64 \\ 
  TGARCH-STD & 1 & 1.65 & 0 & 0 & 0.01 & 27.39 \\ 
   \hline
\hline
SVM-KDE & 5 & 7.41 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 5 & 6.42 & 0 & 0 & 0 & 69.12 \\ 
  SGARCH-STD & 5 & 6.87 & 0 & 0 & 0 & 89.23 \\ 
  SGARCH-SSTD & 5 & 6.22 & 0.01 & 0 & 0.04 & 91.02 \\ 
  EGARCH-NORM & 5 & 6.38 & 0 & 0 & 0.01 & 31.65 \\ 
  EGARCH-STD & 5 & 6.75 & 0 & 0 & 0 & 43.89 \\ 
  EGARCH-SSTD & 5 & 5.66 & 3.51 & 1.05 & 9.65 & 35.1 \\ 
  TGARCH-NORM & 5 & 6.02 & 0.13 & 0 & 0.56 & 4.63 \\ 
  TGARCH-SSTD & 5 & 5.44 & 15.58 & 12.92 & 35.37 & 1.49 \\ 
  TGARCH-STD & 5 & 6.4 & 0 & 0 & 0.01 & 9.18 \\ 
   \hline
\hline
\end{tabular}
\caption{Results for the VaR forecasts from 1 July 1996 to 30 June 2016 for EuroStoxx50.} 
\end{table}


==> source code Version for upload/Tables/Results_Nikkei225.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Jan 16 13:55:04 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Exceedances} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{DUR} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 0.65 & 14.73 & 0.76 & 2.17 & 0 \\ 
  SGARCH-NORM & 0.5 & 1.36 & 0 & 0 & 0 & 82.6 \\ 
  SGARCH-STD & 0.5 & 0.91 & 0.02 & 0 & 0.08 & 21.74 \\ 
  SGARCH-SSTD & 0.5 & 0.79 & 0.73 & 0.05 & 1.69 & 81.34 \\ 
  EGARCH-NORM & 0.5 & 1.69 & 0 & 0 & 0 & 63.65 \\ 
  EGARCH-STD & 0.5 & 1.16 & 0 & 0 & 0 & 95.1 \\ 
  EGARCH-SSTD & 0.5 & 0.83 & 0.25 & NaN & NaN & 27.85 \\ 
  TGARCH-NORM & 0.5 & 1.44 & 0 & 0 & 0 & 89.71 \\ 
  TGARCH-SSTD & 0.5 & 0.73 & 3.05 & NaN & NaN & 41.02 \\ 
  TGARCH-STD & 0.5 & 0.97 & 0 & 0 & 0.01 & 84.41 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.56 & 0.02 & 0 & 0.09 & 0 \\ 
  SGARCH-NORM & 1 & 2.17 & 0 & 0 & 0 & 74.4 \\ 
  SGARCH-STD & 1 & 1.71 & 0 & 0 & 0 & 87.93 \\ 
  SGARCH-SSTD & 1 & 1.28 & 5.42 & 2.42 & 15.42 & 58.2 \\ 
  EGARCH-NORM & 1 & 2.38 & 0 & 0 & 0 & 65.63 \\ 
  EGARCH-STD & 1 & 2.03 & 0 & 0 & 0 & 59.8 \\ 
  EGARCH-SSTD & 1 & 1.6 & 0.01 & 0 & 0.04 & 78.46 \\ 
  TGARCH-NORM & 1 & 2.13 & 0 & 0 & 0 & 90.38 \\ 
  TGARCH-SSTD & 1 & 1.38 & 1.03 & 0.09 & 2.4 & 67.74 \\ 
  TGARCH-STD & 1 & 1.83 & 0 & 0 & 0 & 82.89 \\ 
   \hline
\hline
SVM-KDE & 5 & 6.78 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 5 & 6.72 & 0 & 0 & 0 & 61.05 \\ 
  SGARCH-STD & 5 & 7.15 & 0 & 0 & 0 & 44.01 \\ 
  SGARCH-SSTD & 5 & 6.38 & 0 & 0 & 0.01 & 58.28 \\ 
  EGARCH-NORM & 5 & 6.78 & 0 & 0 & 0 & 13.24 \\ 
  EGARCH-STD & 5 & 6.97 & 0 & 0 & 0 & 5.84 \\ 
  EGARCH-SSTD & 5 & 6.01 & 0.14 & 0 & 0.42 & 3.15 \\ 
  TGARCH-NORM & 5 & 6.34 & 0 & 0 & 0.01 & 0.86 \\ 
  TGARCH-SSTD & 5 & 5.81 & 0.96 & 0.12 & 3.35 & 5.09 \\ 
  TGARCH-STD & 5 & 6.58 & 0 & 0 & 0 & 1.75 \\ 
   \hline
\hline
\end{tabular}
\caption{Results for the VaR forecasts from 1 July 1996 to 30 June 2016 for Nikkei225.} 
\end{table}


==> source code Version for upload/Tables/Results_SP500.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Jan 16 13:55:04 2017
\begin{table}[ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c}
  \hline
\textbf{Model} & \textbf{Quantile} & \textbf{Exceedances} & \textbf{UC} & \textbf{ID} & \textbf{CC} & \textbf{DUR} \\ 
  \hline
\hline
SVM-KDE & 0.5 & 0.79 & 0.75 & 0.05 & 1.72 & 0 \\ 
  SGARCH-NORM & 0.5 & 1.24 & 0 & 0 & 0 & 55.51 \\ 
  SGARCH-STD & 0.5 & 0.73 & 3.1 & 0.53 & 5.38 & 87.95 \\ 
  SGARCH-SSTD & 0.5 & 0.49 & 93.48 & 28.46 & 28.56 & 29.03 \\ 
  EGARCH-NORM & 0.5 & 1.42 & 0 & 0 & 0 & 82.72 \\ 
  EGARCH-STD & 0.5 & 0.96 & 0 & 0 & 0.01 & 35.98 \\ 
  EGARCH-SSTD & 0.5 & 0.75 & 1.97 & 0.25 & 3.78 & 48.1 \\ 
  TGARCH-NORM & 0.5 & 1.36 & 0 & 0 & 0 & 95.12 \\ 
  TGARCH-SSTD & 0.5 & 0.63 & 20.78 & 8.98 & 19.85 & 17.05 \\ 
  TGARCH-STD & 0.5 & 0.91 & 0.02 & 0 & 0.09 & 22.12 \\ 
   \hline
\hline
SVM-KDE & 1 & 1.53 & 0.04 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 1 & 1.99 & 0 & 0 & 0 & 85.6 \\ 
  SGARCH-STD & 1 & 1.44 & 0.33 & 0.02 & 1.35 & 66.78 \\ 
  SGARCH-SSTD & 1 & 1.1 & 47.24 & 53.87 & 69.73 & 48.11 \\ 
  EGARCH-NORM & 1 & 1.99 & 0 & 0 & 0 & 82.16 \\ 
  EGARCH-STD & 1 & 1.63 & 0 & 0 & 0.01 & 66.5 \\ 
  EGARCH-SSTD & 1 & 1.24 & 9.79 & 6.27 & 24.69 & 70.94 \\ 
  TGARCH-NORM & 1 & 1.85 & 0 & 0 & 0 & 72.47 \\ 
  TGARCH-SSTD & 1 & 1.16 & 26.08 & 11.98 & 22.54 & 77.17 \\ 
  TGARCH-STD & 1 & 1.48 & 0.15 & 0 & 0.47 & 90.61 \\ 
   \hline
\hline
SVM-KDE & 5 & 7.44 & 0 & 0 & 0 & 0 \\ 
  SGARCH-NORM & 5 & 6.85 & 0 & 0 & 0 & 67.87 \\ 
  SGARCH-STD & 5 & 7.1 & 0 & 0 & 0 & 62.76 \\ 
  SGARCH-SSTD & 5 & 6.34 & 0 & 0 & 0.01 & 69.2 \\ 
  EGARCH-NORM & 5 & 6.89 & 0 & 0 & 0 & 8.24 \\ 
  EGARCH-STD & 5 & 7.02 & 0 & 0 & 0 & 12.46 \\ 
  EGARCH-SSTD & 5 & 6.2 & 0.02 & 0 & 0.07 & 26.53 \\ 
  TGARCH-NORM & 5 & 6.63 & 0 & 0 & 0 & 2.07 \\ 
  TGARCH-SSTD & 5 & 6.06 & 0.08 & 0 & 0.17 & 4.96 \\ 
  TGARCH-STD & 5 & 6.93 & 0 & 0 & 0 & 2.31 \\ 
   \hline
\hline
\end{tabular}
\caption{Results for the VaR forecasts from 1 July 1996 to 30 June 2016 for Standard and Poors 500.} 
\end{table}


==> source code Version for upload/Tables/Results_Tunig_Results_Case_1.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sat Jan 28 13:51:46 2017
%\begin{sidewaystable}

\begin{table}[h!t]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
  \hline
  \hline
\textbf{C} & $\boldsymbol{\psi}$ & $\boldsymbol{\gamma}$ & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
0.1 & 0.6 & 0.001 & EuroStoxx50 & 0.5 & 0.47 & 88.82 & 81.14 & 96.24 \\ 
  100 & 0.7 & 0.01 & EuroStoxx50 & 1 & 1.02 & 93.28 & 60.41 & 87.11 \\ 
  0.1 & 0.6 & 0.001 & EuroStoxx50 & 2.5 & 2.52 & 96.42 & 97.76 & 97.66 \\ 
  10000 & 0.6 & 10 & EuroStoxx50 & 5 & 4.96 & 94.86 & 99.71 & 99.50 \\ 
  \hline
1 & 0.7 & 0.001 & S\&P500 & 0.5 & 0.48 & 90.54 & 81.06 & 96.48 \\ 
  10 & 0.7 & 0.1 & S\&P500 & 1 & 0.95 & 86.62 & 63.08 & 87.84 \\ 
  10 & 0.7 & 0.01 & S\&P500 & 2.5 & 2.46 & 93.15 & 96.55 & 96.2 \\ 
  10 & 0.6 & 0.001 & S\&P500 & 5 & 5 & 99.48 & 99.57 & 99.57 \\ 
  \hline
10 & 0.8 & 0.01 & Nikkei225 & 0.5 & 0.41 & 63.92 & 83.95 & 87.77 \\ 
  100 & 0.8 & 0.01 & Nikkei225 & 1 & 0.82 & 50.63 & 68.48 & 73.85 \\ 
  100 & 0.7 & 0.01 & Nikkei225 & 2.5 & 2.7 & 66.43 & 57.80 & 52.61 \\ 
  100 & 0.7 & 0.10 & Nikkei225 & 5 & 4.49 & 40.84 & 94.38 & 67.06 \\ 
   \hline
\hline
\end{tabular}
\caption[Grid search results for SVR parameter tuning]{The best models in the tuning period according to the p-value of the test for conditional coverage.
                      UC, ID and CC indicate the p-value of the corresponding LR test. All values in the columns Quantile, Violations,
                      UC, ID and CC are given in percent.} 
\label{Tab:tuning_case1}
\end{table}
%\end{sidewaystable}

==> source code Version for upload/Tables/Results_Tunig_Results_Case_1_Only_1to5.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sat Jan 28 13:51:46 2017
%\begin{sidewaystable}

\begin{table}[h!t]
\centering
\begin{tabular}{c|c|c|c|c|c|r|r|r}
  \hline
  \hline
\textbf{C} & $\boldsymbol{\psi}$ & $\boldsymbol{\gamma}$ & \textbf{Index} & \textbf{Quantile} & \textbf{Violations} & \textbf{UC} & \textbf{ID} & \textbf{CC} \\ 
  \hline
  10 & 0.7 & 0.1 & S\&P500 & 1.0 & 0.95 & 86.62 & 63.08 & 87.84 \\ 
  10 & 0.7 & 0.01 & S\&P500 & 2.5 & 2.46 & 93.15 & 96.55 & 96.20 \\ 
  10 & 0.6 & 0.001 & S\&P500 & 5.0 & 5.00 & 99.48 & 99.57 & 99.57 \\ 
  \hline
  100 & 0.8 & 0.01 & Nikkei225 & 1.0 & 0.82 & 50.63 & 68.48 & 73.85 \\ 
  100 & 0.7 & 0.01 & Nikkei225 & 2.5 & 2.70 & 66.43 & 57.80 & 52.61 \\ 
  100 & 0.7 & 0.10 & Nikkei225 & 5.0 & 4.49 & 40.84 & 94.38 & 67.06 \\ 
      \hline
	100 & 0.7 & 0.01 & EuroStoxx50 & 1.0 & 1.02 & 93.28 & 60.41 & 87.11 \\ 
  0.1 & 0.6 & 0.001 & EuroStoxx50 & 2.5 & 2.52 & 96.42 & 97.76 & 97.66 \\ 
  10000 & 0.6 & 10 & EuroStoxx50 & 5.0 & 4.96 & 94.86 & 99.71 & 99.50 \\ 
   \hline
\hline
\end{tabular}
\caption[Grid search results for SVR parameter tuning]{The best models in the tuning period according to the p-value of the test for conditional coverage.
                      UC, ID and CC indicate the p-value of the corresponding LR test. All values in the columns Quantile, Violations,
                      UC, ID and CC are given in percent.} 
\label{Tab:tuning_case1}
\end{table}
%\end{sidewaystable}
